Symmetric Neural-Collapse Representations with Supervised Contrastive Loss: The Impact of ReLU and Batching

Supervised contrastive loss (SCL) is a competitive and often superior alternative to the cross-entropy loss for classification. While prior studies have demonstrated that both losses yield symmetric training representations under balanced data, this symmetry breaks under class imbalances. This paper presents an intriguing discovery: the introduction of a ReLU activation at the final layer effectively restores the symmetry in SCL-learned representations. We arrive at this finding analytically, by establishing that the global minimizers of an unconstrained features model with SCL loss and entry-wise non-negativity constraints form an orthogonal frame. Extensive experiments conducted across various datasets, architectures, and imbalance scenarios corroborate our finding. Importantly, our experiments reveal that the inclusion of the ReLU activation restores symmetry without compromising test accuracy. This constitutes the first geometry characterization of SCL under imbalances. Additionally, our analysis and experiments underscore the pivotal role of batch selection strategies in representation geometry. By proving necessary and sufficient conditions for mini-batch choices that ensure invariant symmetric representations, we introduce batch-binding as an efficient strategy that guarantees these conditions hold.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections_arxiv_v2/SMroadmap.tex <==

\section*{Roadmap to the Supplementary material}

%{\color{darkblue} 
The SM contains the following. In Section \ref{sec:SEL_mat_properties} we derive several useful properties of the simplex-encoded-label (\SEL)~matrix, which we then use  in Section \ref{sec:SELI_properties} to present  closed-form characterizations of the embeddings and classifiers geometries. Notably, these include explicit expressions for the norms and angles of both majority and minority classes, which we accompany with numerical illustrations shedding further light on the features of the proposed \emph{\ref{SELI}} geometry. Next, in Section \ref{sec:proofs_UF-SVM}, we use the derived properties of the \SEL~matrix to prove our main Theorem \ref{thm:SVM} and its corollaries. In Section \ref{sec:nuc_norm_SM} we derive several useful properties of the nuclear-norm penalized CE minimization, which we then use in Section \ref{sec:proofs_regularization} to prove the statements of Section \ref{Sec:reg}. Section \ref{sec:UFM} contains additional numerical results on the UFM, such as experiments with varying weight-decay and regularization choices. Additional experiments on real data (such as, isolated minority/majority geometry investigations, and classifiers/embeddings norm ratios), as well as further implementation details, are included in Section \ref{sec:real_exp_SM}. In Section \ref{sec:minority} we show how results relate to minority collapse providing additional theoretical justifications and novel perspectives to empirical observations reported by previous work. Finally, an elaborate discussion on additional related works is contained in Section \ref{sec:rel2}.
%}

==> sections_arxiv_v2/analysis.tex <==
\section{Analysis}

\begin{lemma}\label{lem:centering}
 Any global minimizer $(\hat\W,\hat\Hb)$ of \eqref{eq:svm_original} is such that $\sum_{c\in[k]}\hat\w_c=\zeros$.
\end{lemma}

\begin{proof}
For the sake of contradiction assume that $\bar\w:=\frac{1}{k}\sum_{c\in[k]}\hat\w_c\neq \zeros$, that is $\|\bar\w\|_2>0$. Consider the pair $({\Vb},\hat\Hb)$ where the columns of $\Vb$ are defined each such that $\vb_c=\hat\w_c-\bar\w$. Clearly, the new pair is feasible, since $(\hat\W,\hat\Hb)$ is feasible. But, 
$$
\sum_{c\in[k]}\|\vb_c\|^2 = \sum_{c\in[k]}\|\w_c\|^2 + k\|\bar\w\|^2 - \inp{\bar\w}{\sum_{c\in[k]}\w_c} =  \sum_{c\in[k]}\|\w_c\|^2 - k\|\bar\w\|^2 <\sum_{c\in[k]}\|\w_c\|^2,
$$
which contradicts optimality of $(\hat\W,\hat\Hb)$. Hence, it must be that $\bar\w=\zeros$.
\end{proof}


Consider first the minimization over $\Hb$ for any fixed $\W$:
\begin{align}
\Hb(\W):=\arg\min_{\Hb}~\frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
\end{align}
Note that this optimization is separable over the rows of $\Hb$ and each row of $\Hb(\W)$ is found by minimizing the following:
\begin{align}\label{eq:hi_sep}
\min_{\h}~\frac{1}{2}\|\h_i\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1\quad\forall c\neq y_i
\end{align}
The above optimization is strongly convex. Slater's conditions hold, thus KKT conditions are necessary and sufficient. Therefore the solution $\hat\h_i:=\h_i(\W)$ of the problem  above is unique and satisfies:
\begin{align}\label{eq:hi_KKT}
\hat\h_i = \A_{-{y_i}}^T\lab_i , \qquad \lab_i\geq \zeros,  \qquad \A_{y_i}\hat\h_i\geq \ones, \qquad \lab_i^T(\ones-\A_{-{y_i}}\hat\h_i)=0
\end{align}
for some optimal dual variable $\lab_i\in\R^{k-1}$. Also, from strong duality, the minimization in \eqref{eq:hi_sep} is equivalent to the following maximization
\begin{align}
\max_{\lab} ~-\frac{1}{2}\|\A_{y_i}^T\lab\|^2+\lab^T\ones \quad\quad\text{sub. to}\quad \lab \geq 0.
\end{align}

\begin{remark}
Note that {if $\A_{y_i}\A_{y_i}^T$ is invertible and $\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\geq \zeros$,} then the primal dual pair:
\begin{align}
 \hat\h_i=\A_{y_i}^T\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\qquad{\text{and}}\qquad\lab_i=\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones
\end{align}
 satisfies the KKT and is thus optimal. However, this might not be true for the optimal $\W$. Thus, we consider below the general case.
 \end{remark}
 
 In general, \eqref{eq:svm_original} reduces to the following min-max optimization
 \begin{align}\label{eq:cvx_onlyW}
\min_{\substack{\W\\
\A_{y_i}=\ones\w_{y_i}^T-\W_{-y_i}^T
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\|\W\|^2 -\frac{1}{2}\sum_{i\in[n]}\|\A_{y_i}^T\lab_i\|^2 + \sum_{i\in[n]}\lab_i^T\ones.
\end{align}
From Lemma \ref{lem:centering}, the optimization above does not change when we impose the additional constraint $\sum_c\w_c=\zeros$. Using this, note that $\w_c = -\W_{-c}\ones, \forall c\in[k]$. Therefore, 
\begin{align}
\A_c = \ones\w_c^T-\W_{-c}^T = -\ones\left(\W_{-c}\ones\right)^T-\W_{-c}^T = -\left(\Id+\ones\ones^T\right)\W_{-c}^T
\end{align}
Therefore,
$$
\A_c\A_c^T = \left(\Id+\ones\ones^T\right)\W_{-c}^T\W_{-c}\left(\Id+\ones\ones^T\right).
$$
Recalling the notation of the Gram matrix $\G$ and its submatrices $\G_{-c}, c$ and recognizing that $\G_{-c}=\W_{-c}^T\W_{-c}$, we can rewrite the optimization in \eqref{eq:cvx_onlyW} as follows
 \begin{align}\label{eq:cvx_onlyG}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{i\in[n]}\lab_i^T\left(\Id+\ones\ones^T\right)\G_{-y_i}\left(\Id+\ones\ones^T\right)\lab_i + \sum_{i\in[n]}\lab_i^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W \succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \sum_{c\in[k]}\w_c=\zeros \nn
\end{align}
By symmetry, for all $i: y_i=c$ it holds that $\la_i=\la_c$. Also, note that
$$
(\W^T\W\ones = \zeros ~~\text{ OR }~~ \ones^T\W^T\W = \zeros^T) \Leftrightarrow \W\ones=\zeros.
$$
 Using these, we can further reduce the above to the following
 \begin{align}\label{eq:cvx_onlyG_c}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_c\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\left(\Id+\ones\ones^T\right)\G_{-c}\left(\Id+\ones\ones^T\right)\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W\succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \G\ones=\zeros,~~ \ones^T\G=\zeros^T \nn
\end{align}
Finally, we can exploit the lemma below, to write the optimization only in terms of Gram matrices.
\begin{lemma}\label{lem:chol}
Consider arbitrary $\G\succeq\zeros_{k\times k}$ with $\G\ones=\zeros.$
%with $\rm{rank}(G)=r$. 
Assume $d\geq k-1$. Then, there exists $\W\in\R^{d\times k}$ such that $\G=\W^T\W$.
\end{lemma}
\begin{proof}
Recall that any positive semidefinite matrix $\G\succ\zeros_{k\times k}$ with $\rm{rank}(G)=r$ has a  Cholesky factorization $\G=\Lb\Lb^T$ with $\Lb\in\R^{k\times k}$ lower triangular with exactly $r$ positive diagonal elements and $k-r$ columns containing all zeros. Note since $\G\ones=\zeros$, $r\leq k-1$ in our case. Thus, $\Lb$ has at least one column containing all zeros. Remove that column and with some abuse of notation let $\Lb\in\R^{k\times (k-1)}$ be the remaining Cholesky factor. Then, for all $d\geq k-1$, we can choose $\W = \begin{bmatrix} \Lb^T \\ \zeros_{(d-(k-1))\times k} \end{bmatrix}$, which completes the proof.
 \end{proof}
 Indeed, using Lemma \eqref{lem:chol}, the optimziation in \eqref{eq:cvx_onlyG_c} is equivalent \footnote{Here, equivalence is in the following sense. If $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, then $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}. Also, if $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}, then $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, where here $\hat\W$ is such that $\hat\W^T\hat\W=\hat\G$ and its existence is guaranteed by Lemma \ref{lem:chol}.}
  to the following:
\begin{align}\label{eq:cvx_G}
&\min_{\substack{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}
}} ~\max_{\lab_c\geq \zeros }~~F(\G,\lab_c) :=\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\widetilde\J_c\G\widetilde\J_c^T\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones,
\end{align}
where we set $\widetilde\J_c:=\left(\Id_{k-1}+\ones\ones^T\right)\J_c.$

 
 We can write the inner maximization in \eqref{eq:cvx_G} using strong duality as follows
 \begin{align}
& \min_{\mub_c\geq \zeros}\max_{\lab_c}~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\tilde\J_c\G\tilde\J_c^T\lab_c + \sum_{c\in[k]}\lab_c^T\left(n_c\ones + \mub_c\right)\\
=&\min_{\mub_c\geq \zeros}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),
 \end{align}
 where we recall that $\G_{-c}:=\J_c\G\J_c^T.$
 
 \begin{propo}\label{eq:h_opt}
 	Let $(\hat\W,\hat\Hb)$ be any global minimizer of \eqref{eq:svm_original}. Then, the Gram matrix $\hat\G:=\hat\W^T\hat\W$ is a minimizers of the following convex SDP:
 \begin{align}\label{eq:SDP}
 &\min_{\G,\G_{-c},\mub_c}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right) 
 \\
 \nn
 &~~\text{sub. to}\quad \G\succeq \zeros_{k\times k},~~\G_{-c}=\J_c\G\J_c^T,~~\mub_c\geq\zeros_{k-1},~~\G\ones=(\ones^T\G)^T=\zeros.
 \end{align}
 Moreover, letting $\hat\mub_c, c\in[k]$ denote minimizers of the convex program above and defining $$\hat\lab_c = \frac{1}{n_c}\left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),$$
 it holds for all $i\in[n]$ that,
 $$
\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
 $$
 \end{propo}
 
 \begin{remark}
Solving \eqref{eq:SDP} in CVX gives $\hat\mub_c = 0, \forall c\in[k]$. Hence, $\lab_{c}>\zeros$, which would imply that all constraints are active. Unfortunately, we know that this is NOT true if we run GD. \red{Our conjecture (?) is that GD converges to a KKT point of \eqref{eq:SDP} that is NOT a global optimum.}
 \end{remark}
 
 \subsection{The Dual problem}

 \begin{propo}
 The dual of \eqref{eq:svm_original} is the following (convex) SDP:
 \begin{align}
& \max_{\lab_c\in\R^{k-1}, c\in[k]}~~\sum_{c\in[k]}n_c\lab_c^T\ones_{k-1}\\
& ~~~\text{sub. to}~~~~~ \lab_c \geq 0\nn\\
& \qquad\qquad\qquad \Pb_k\left(\Id_k - \sum_{c\in[k]}n_c\J_c^T\left(\Id_{k-1}+\ones\ones^T\right)\lab_c\lab_c^T\left(\Id_{k-1}+\ones\ones^T\right)\J_c\right)\Pb_k\succeq 0\nn
 \end{align}
 where we set $\Pb_k:=\Id_k-\frac{1}{k}\ones\ones.$ 
 \end{propo}

Remark: A fast way to see the above is from \eqref{eq:cvx_G}. The second constraint can be written in an SDP form using Schur complement.


\subsection{A direct tight convex relaxation}
The following program is a convex relaxation of \eqref{eq:svm_original} found by setting
\begin{align}\label{eq:X_rel}
\X_{2k \times 2k} = \begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix},
\end{align}
for $\bar\Hb_{d \times k}=[\bar\h_1, \ldots, \bar\h_k]$ the feature matrix. Here, we note in \eqref{eq:svm_original} that at the optimal $\h_i=\bar\h_{y_i}$ for all $i\in[n].$

\begin{align}\label{eq:cvx_X2}
&\min_{\X\in\R^{{2k \times 2k}}}~~\sum_{c\in[k]}\X[c,c] + \sum_{c\in[k]}n_c\X[k+c,k+c]\\
&~\text{sub.~to}~~~~\X[c,k+c]-\X[c',k+c]\geq 1,~c'\neq c, c\in[k] \\
&\qquad\qquad\quad\X\succeq 0_{2k\times 2k}
\end{align}

It is not hard to see that the relaxation is tight provided that $d\geq 2k$ \ct{(This is loose. The $\X$ matrix is not gonna be full rank at the optimal. For example, we can add without loss of generality the constraint that row-column sum of top $k\times k$ block is $0$)}. Indeed, for any $d\geq 2k$, we can decompose an optimal $\hat\X$ in factors $\hat\W$ and $\hat\Hb$ using Cholesky decomposition (see Lemma \ref{lem:chol}). It is easy to verify that these factors $\hat\W$ and $\hat\Hb$ are feasible in \eqref{eq:cvx_G}. Hence they are optimal.


 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%% December 6 -- optimize first over G, then over \la
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \subsection{Old}
%% Interestingly, the min-max problem in \eqref{eq:cvx_G} is convex-concave. {Also, it should be possible (check?) to show that the minimization can be equivalently performed in a bounded set.} Thus, by Sion's min-max theorem, we can flip the order of min-max. 
%%
%%For convenience, denote $\tilde\J_c:=\left(\Id+\ones\ones^T\right)\J_c$, $c\in[k].$ The objective can be written as 
%%$$
%%F(\G,\lab_c)= \frac{1}{2}\tr\left(\G \X \right) + \sum_{c\in[k]}n_c\lab_c^T\ones,
%%$$
%%where we defined
%%\begin{align}
%%\X := \Id - \sum_{c\in[k]} n_c \tilde\J_c^T\lab_c\lab_c^T\tilde\J_c.
%%\end{align}
%%
%%\begin{lemma}\label{lem:Gmin}
%%The following is true about the minimization over $G$:
%%\begin{align}
%%\min_{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}}\tr\left({\G\X}\right)=\begin{cases}
%%0 & \Pb^\perp_k\X\Pb^\perp_k\succeq \zeros \\
%%-\infty & \text{o.w.}
%%\end{cases}
%%\end{align}
%% \end{lemma}
%% Using Lemma \ref{lem:Gmin}, \eqref{eq:cvx_G} is reduces to the following maximization
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad \sum_{c\in[k]}n_c\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)^T\preceq \Pb^\perp_k
%% \end{align}
%% Using Schur-complement, we can write this as an SDP:
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad 
%% \begin{bmatrix} 
%%\Id_{k\times k}  & \sqrt{n_1}\tilde\J_1^T\lab_1 & \sqrt{n_2}\tilde\J_2^T\lab_2 & \cdots & \sqrt{n_k}\tilde\J_2^T\lab_2 \\
%% \sqrt{n_1}\lab_1^T\tilde\J_1  & 1 & 0 & \cdots & 0 \\  \sqrt{n_2}\lab_2^T\tilde\J_2  & 0 & 1 & \cdots & 0 \\  
%%\vdots & \vdots & \vdots & \cdots & \vdots \\
%%\\  \sqrt{n_k}\lab_k^T\tilde\J_1  & 0 & 0 & \cdots & 1  
%%  \end{bmatrix} \succeq \zeros_{2k \times 2k}
%% \end{align} 




%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\subsection{KKT conditions}
The Lagrangian of the convex problem of \eqref{eq:svm_original} is the following, for dual variables $\{\la_{i,c}\}, i\in[n], c\in[k], c\neq y_i$:
\begin{equation}
	\Ellc(\W, \Hb, \{\lambda_{i,c}\}) = \frac{1}{2}\sum_{c=1}^{K}\|\w_{c}\|^2+ \frac{1}{2}\sum_{i=1}^{N}\|\h_{i}\|^2 + \sum_{i\in[n]}\sum_{c'\neq y_i}\la_{i,c'}(1-\w_{y_i}^T\h_{i}+\w_{c'}^T\h_i)
\end{equation}
The KKT conditions are then as follows:
\begin{subequations}\label{eq:KKT}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}+\sum_{i:y_i\neq c}\la_{i,c}\h_i -\sum_{i:y_i=c}\Big(\sum_{c'\neq y_i} \la_{i,c'}\Big)\h_i = 0\\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{i\in[n]}\Big(\sum_{c'\neq y_i}\lambda_{i,c'}\Big)\w_{y_i}+\sum_{i\in[n]}\sum_{c'\neq y_i}\lambda_{i,c'}\w_{c'} = 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\lambda_{i,c} \geq 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \lambda_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}

The KKT conditions can be rewritten equivalently with respect to an augmented dual variable representation $\beta_{i,c}, i\in[n], c\in[k]$ as follows:
\begin{subequations}\label{eq:KKT_beta}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}-\sum_{i\in[n]}\beta_{i,c}\h_i  = 0 \,\Leftrightarrow\,  \W_{d\times k} = \Hb_{d\times n}\Bb^T_{n\times k} \\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{c\in[k]}\beta_{i,c}\w_c = 0\,\Leftrightarrow\,  \Hb_{d\times n} = \W_{d\times k}\Bb_{k\times n} \\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\beta_{i,c} \leq 0 \label{eq:beta_new}
	\\
	\forall i\in[n] \,&:\,\beta_{i,y_i} = -\sum_{c\neq y_i}\beta_{i,c}\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \beta_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}
To see that these are equivalent, set for all $i\in[n]$: $\beta_{i,c}=\begin{cases} \sum_{c'\neq c}\lambda_{i,c'} & c=y_i \\ -\lambda_{i,c} & c\neq y_i\end{cases}.$ Above, we have also defined an $k\times n$ matrix $\Bb$ with entries $[\Bb]_{c,i}=\beta_{i,c}.$ From constraint \eqref{eq:beta_new} it follows that $\Bb$ has column-sum equal to zero, i.e. $\Bb^T\ones_{k}=0.$ For instance this immediately yields $\W\ones_{k}=0$ (which we proved from first principles in Lemma \ref{lem:centering}).

Also, note that the first two conditions imply
\begin{align}
\Hb^T\W = \Hb^T\Hb \Bb^T \qquad\text{and}\qquad \W^T\Hb = \W^T\W\Bb.
\end{align}
Hence,
\begin{align}
\X_{(k+n)\times (k+n)}:=\begin{bmatrix}\W^T\W & \W^T\Hb \\ \Hb^T\W & \Hb^T\Hb\end{bmatrix}=\begin{bmatrix}\W^T\W & \zeros_{k\times n} \\ \zeros_{n\times k} &\Hb^T\Hb\end{bmatrix}
\underbrace{\begin{bmatrix}\Id_{k\times k} & \Bb_{k\times n} \\ \Bb^T_{n\times k} & \Id_{n\times n}\end{bmatrix}
}_{\widetilde{\Bb}}.
\end{align}
and
\begin{align}
\tr\Big(\widetilde{\Bb}^T\X \Big) = \tr\Big(\widetilde{\Bb}\cdot {\rm{bldiag}}(\W^T\W,\Hb^T\Hb) \cdot\widetilde{\Bb}\Big)
\end{align}




%A possibly interesting observation here is the following.
%\begin{lemma} Suppose $(\W,\Hb,\Bb)$ satisfy the KKT conditions \eqref{eq:KKT_beta}. If $\Bb$ is such that $\Id_{k\times k} \succeq \Bb\Bb^T$, then the matrix $\X=\begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix}$ is a solution to the SDP in \eqref{eq:cvx_X}.
%\end{lemma}




==> sections_arxiv_v2/convex_forms.tex <==
\subsection{Convex Equivalent form: Nuclear norm}\label{eq:svm_z_nuc}
\begin{align*}
	&\quad  \min_{\Z}~\|\Z\|_*
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\Z}~\left[\min_{\W,\Hb \ \text{s.t.} \ \W\Hb = \Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)\right]
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1
\end{align*}

%\subsection{Equality of margins/activeness of constraints:}
%\begin{center}
%	\begin{tabular}{||c ||c | c|| c | c ||} 
%		\hline
%		& BalERM-CE & BalSVM & ImbalERM-CE & ImbalSVM \\ [0.5ex] 
%		\hline\hline
%		$(\W,\Hb)$ & Equal & Active & Unequal & Active \\ 
%		\hline
%		$\Z$ & Equal & Active & Equal & Active \\ 
%		\hline
%		$\X$ &  &  &  &  \\ [1ex] 
%		\hline
%	\end{tabular}
%\end{center}


==> sections_arxiv_v2/discussion.tex <==
%In this section, we discuss a few key observations regarding our results and findings.

% \subsection{UFM vs \ref{eq:SCL_UFM_full}?}
% As discussed in Sec.~\ref{sec:theo_results}, the majority of previous works \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring} study the geometry of learned embeddings by investigating the proxy model, UFM. In case of SCL, as studied in e.g., \citet{graf2021dissecting}, the corresponding UFM is as follows,
% % 
% \begin{align}\label{eq:ufm_main}
%     \arg\min_{\Hb} \Lc_{\text{{full}}}
%     (\Hb)~~\text{{subj. to}}~~\|\h_i\|^2 = 1,\, \forall i\in[n].
%     \tag{$\text{UFM}$}
% \end{align}
% % 
% %Instead, in this paper, we study \ref{eq:SCL_UFM_full} which further constrains $\Hb$ to the non-negative orthant. 
% The works relying on the \ref{eq:ufm_main} as the proxy analysis model employ a common heuristic when called to compare the analysis outcome to the outcome of the experiments. This heuristic involves centering the  embeddings obtained from deep-net experiments around their global class mean before comparing them to the theoretical geometry (see Sec.~\ref{sec:centering}). The rationale behind this heuristic is that the experimentally observed features are non-negative as a result of the ReLU activations in the network. Instead, \ref{eq:SCL_UFM_full} explains the feature geometry learned by SCL without the need for a heuristic centering.

% In case of balanced data, \citet{graf2021dissecting} predicted, using \ref{eq:ufm_main}, that the geometry of the SCL-learned embeddings follow NC and the $k$ mean-embeddings form a simplex ETF (see Def.~\ref{def:etf}). The following lemma connects this result with our result obtained by studying \ref{eq:SCL_UFM_full}.
% \begin{lemma}\label{lem:OF2ETF_main}
% Suppose that a set of vectors $\{\vb_1,...,\vb_k\}$ form a $k$-OF in $\R^d$ with $d \geq k$, and their mean-centered counterparts are $\Bar{\vb}_c = \vb_c - \vb_G, \forall c \in [k]$, where $\vb_G = \frac{1}{k}\sum_{c\in[k]}\vb_c$.  Then, the centered embeddings $\{\Bar{\vb}_1,...,\Bar{\vb}_k\}$ form a simplex ETF spanning a $k-1$-dimensional subspace. 
% \end{lemma}
% In other words, a $k$-OF transforms to an ETF after \emph{centering}. This aligns our result with \cite[Thm. 2]{graf2021dissecting} when data is balanced. However, it is important to highlight the fact that the UFM analysis does not explain the centering trick, or describe that the (uncentered) embeddings form an OF. Specifically, transforming an ETF into a geometry with non-negative embeddings can be achieved in multiple ways; the uniqueness of where to relocate the center of the geometry is not guaranteed. This discrepancy is the reason behind the gap observed between the theoretical prediction and empirical observations depicted in \cite[Fig. 7]{graf2021dissecting} and Fig.~\ref{fig:intro}(a) (compare the red and green lines).

% Although in the balanced setup, the only difference between the \ref{eq:ufm_main} and \ref{eq:SCL_UFM_full} analysis lies in the centering trick, we argue that, in a general setup, this is not the only distinction. Specifically, by the following lemma, we show that the \ref{eq:ufm_main} solution is sensitive to the label distribution. This is against our empirical observation in Sec.~\ref{sec:Deepnet_SCLGeom_exp}, and our theoretical analysis with \ref{eq:SCL_UFM_full} in Sec.~\ref{sec:theo_results}.

% \begin{lemma}\label{lem:counterexample_main}
%     If classes in the training set are not balanced, % i.e., $\exists c,c'\in[k]$ such that $n_c\neq n_{c'}$, 
%     the global solution of \ref{eq:ufm_main} is not necessarily an ETF.  Thus, the solution of \ref{eq:SCL_UFM_full} (which according to Thm.~\ref{thm:scl_full} is an OF) is in general different to that of \ref{eq:ufm_main} even after centering is applied.
% \end{lemma}
% \begin{remark}
%      While \citet{zhu2022balanced} acknowledge that the global optima of the UFM do not conform to the ETF geometry in the presence of class imbalance, they do not provide a formal proof to support this claim. In this context, Lemma \ref{lem:counterexample_main} fulfills this purpose. \tina{omit the remark in the SM if remark moved to main}
% \end{remark}

% In Sec.~\ref{app:geometry}, we further elaborate on this discussion and provide the proof of the lemmas.

% \noindent\textbf{No heuristic \textit{centering} of embeddings.}~\new{In previous works that use the UFM to characterize the structure of learned features with balanced/imbalanced labels, a common heuristic is employed: centering the observed features obtained from deep-net experiments around their global class mean before comparing them to the theoretical geometry (see App.~\ref{sec:centering} for a definition). The rationale behind this heuristic is that the experimentally observed features are non-negative as a result of the ReLU activations in the network \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring}. Instead, \ref{eq:SCL_UFM_full} explains the feature geometry learned by SCL without the need for a heuristic centering. In this case, it is important to highlight that when the class-mean embeddings, which constitute a $k$-OF, are centered to have a zero global mean, the observed geometry transforms into an ETF, aligning with the prediction made by \cite[Thm. 2]{graf2021dissecting}. This transformation occurs because an OF geometry for the embeddings implies an ETF geometry for the centered embeddings. In App.~\ref{ref:OFvsETF} we discuss the straightforward relationship between OF and ETF.}

% \new{On the other hand, the reverse transformation is not necessarily valid as transforming an ETF into a geometry with non-negative embeddings can be achieved in multiple ways; the uniqueness of where to relocate the center of the geometry is not guaranteed. This discrepancy is the reason behind the gap observed between the theoretical prediction and empirical observations depicted in \cite[Fig. 7]{graf2021dissecting} and Figure \ref{fig:intro}(a) (compare the red and green lines).}




\subsection{Detailed comparison between UFM and UFM$_+$}\label{sec:UFMvsUFM+}
\input{./sections_v2/geometry2}

==> sections_arxiv_v2/exp_appex.tex <==
\subsection{Details on the main experimental setup}\label{sec:exp_details_SM}
In our deep-net experiments, we focus on two common network architectures, ResNet and DenseNet. Specifically, we use ResNet-18, ResNet-34 and DenseNet-40 with approximately $63$, $11$ million and $200$ thousand trainable parameters, respectively. For all models, we replace the last layer linear classifier with a normalization layer (normalizing such that $\| \h_i\|=1$ for $i \in [n]$) of feature dimension $d=512$. Specifically, following  \cite{graf2021dissecting}, we  directly optimize the normalized features that are then used for inference. (We note this is slightly different compared to \cite{khosla2020supervised}, where the authors train the output features of a projection head, then discard this projection head at inference time). We use this projection head when studying NCC test accuracy. In particular, we add a 2 layer non-linear MLP with with and without ReLU to report the test accuracies provided in Tab.~\ref{tab:cifar100_main}, Tab.~\ref{tab:relu_noRelu_all_test} and , Tab.~\ref{Tab:NCC_Bindings}. Following \cite{khosla2020supervised}, in addition to the NCC test accuracy on post-projection feature (final output), we evaluate the accuracies on the pre-projection features (without input to projector) as well. We remark that both ResNet and DenseNet architectures include ReLU activations before the final output, which enforces a non-negativity on the learned embeddings. Resnet-18 models with CIFAR10, MNIST have been trained for 350 epochs with a constant learning rate of $0.1$, no weight decay, batch size of $1024$, and SCL temperature parameter $\tau = 0.1$ (consistent with the choice of $\tau$ made in \cite{khosla2020supervised,graf2021dissecting}). For CIFAR100 and Tiny-ImageNet experiments, we train a ResNet-34 under a similar setup, for 500 epochs, (with batch binding in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}). For all experiments with other models or datasets, we provide experimental details in the following sections. All ResNet-18 and DenseNet models have been trained on a single Tesla V100 GPU machine and all ResNet-34 models were trained on a single machine with 2-4 Tesla V100 GPU, depending on experiment.

\subsection{Details on Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu} Heatmaps}\label{sec:exp_fig1_detail}
Since this particular experiment provides the most insight into the geometric behaviour of features, we have provided further explanation of the experimental setup and method. ResNet-18 models were trained for 350 epochs on MNIST using \textbf{CE}, \textbf{SCL} and \textbf{SCL + ReLU} under difference imbalance ratios. For SCL and SCL + ReLU we extract the features, calculate the class means and plot a heatmap of the gram matrices $G_{M}$. For CE, following previous work by \cite{papyan2018full, seli, zhu2021geometric} we center the class means by the global mean, ie $\overline{\mu_{c}} = \mu_{c} - \frac{1}{K} \sum_{i=1}^K \mu_{i}$ and then proceed to calculate $G_{M}$. In order to have a fair comparison, we normalize all gram matrices by dividing by the matrix maximum $\overline{G_{M}} = \frac{G_{M}}{\text{max}_{i,j} |G_{\mu}^{i,j}| }$. No projection layer was implemented for these results. The heatmaps were included to provide a clear visual, emphasizing the impact of ReLU on achieving symmetric geometry under imbalance. Each cell $[i,j]$ of the $G_{M}$ matrix represents the inner product $\mu_i^T \mu_j$, rather a normalized value representing the angle between the two class centers. In addition, as SCL includes a normalization layer, the diagonals $G_{M}[i,i]$ would be closer to zero as the features exhibit stronger neural collapse properties. 


% All ResNet models were trained for 350 epochs with a constant learning rate of $0.1$ and no weight decay. On the other hand, we observed slower convergence to OF geometry when training our DenseNet models on more complex datasets such as CIFAR10, and larger imbalance ratios $\RT$. To combat this, we increased the number of training epochs to 500 while annealing the learning rate by a factor of 0.1 on epoch 300, reduced to batch size to 128 to increase number of back-propagation iterations, and used binding examples to improve convergence speed. 

%\todo{Remove the following?}
%Given our focus on feature geometry, we did not perform any data augmentation to increase convergence speed.  \vala{mention this ? We did perform experiments with common-practice data augmentation techniques which showed general convergence towards OF, but more iterations for better convergence}.

% \vala{Do we need further specific detail for each ? }

% \noindent\textbf{Details for Fig.~\ref{fig:intro}} 

% \noindent\textbf{Details for Fig.~\ref{fig:GM matrices comparison}}


\subsection{Additional geometric analysis}

\begin{figure}[t]
% \centering
%\hspace*{-20pt}
\begin{subfigure}[b]{0.95\textwidth}
    \centering
    \begin{tikzpicture}
        \node at (0.0,0) 
        {\includegraphics[width=\textwidth]{Figs/NC1_Convergence_plots.pdf}};
        % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
        \node at (-4.7,2.6) [scale=0.9]{\textbf{MNIST}};
        \node at (-1.4,2.6) [scale=0.9]{\textbf{CIFAR10}};
        \node at (1.9,2.6) [scale=0.9]{\textbf{CIFAR100}};
        \node at (5.1,2.6) [scale=0.9]{\textbf{Tiny ImageNet}};
        \node at (-7.0,1.1)  [scale=0.9, rotate=90]{\textbf{Step}};
        \node at (-7.0,-0.9)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
        \node at (0.2,-2.3) [scale=0.9]{\textbf{Epoch}};
    \end{tikzpicture}
\end{subfigure}
\captionsetup{width=0.95\linewidth}
\caption
{Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for the corresponding experiments in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values are usually on the order of $10^{-2}$ suggesting strong convergence of embeddings to their class means.}
\label{fig:Deepnet_SCL_Geom_NC}
\end{figure}

     In addition to analyzing the convergence of the Gram-matrix of class-mean embeddings $\G_\M$ to the OF geometry (as provided in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}), we also keep track of Neural Collapse (Defn.~\ref{def:nc}) of individual embeddings and orthogonality of their class-means (Defn.~\ref{def:of}) separately. Furthermore, we qualitatively study the Gram matrices $\G_\M$ and $\G_\Hb$  and compare them to corresponding matrices for the CE loss under imbalances. 
     
     \subsubsection{Neural Collapse}~
     In order to quantify the collapse (NC) of embeddings, $\h_i, i \in [n]$, to their class-means,  we measure $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ \citep{NC}. Here, $\Sigma_B= \sum_{c\in [k]}(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})^\top$ is the between class covariance matrix, $\boldsymbol{\mu}_G = \frac{1}{k}\sum_{c\in[k]}\boldsymbol{\mu}_c$ is the  global mean, and $\Sigma_W  = \sum_{i\in [n]}(\h_i - \boldsymbol{\mu}_{y_i})(\h_i - \boldsymbol{\mu}_{y_i})^\top$ is the within class covariance matrix.

     For the experiments shown in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu} and Fig.~\ref{fig:loss_convergence} in the main body, the corresponding values of $\beta_\text{NC}$ can be found in Fig.~\ref{fig:Deepnet_SCL_Geom_NC} and Fig.~\ref{fig:loss NC and angle convergence SM}(b) respectively.

     
    % \begin{figure*}[h]
    %     % \centering
    %     \hspace*{-16pt}
    %     \begin{subfigure}[b]{\textwidth}
    %         \centering
    %         \begin{tikzpicture}
    %             \node at (0.0,0) 
    %             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
    %             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    %             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
    %             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
    %             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
    %             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
    %             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
    %             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
    %         \end{tikzpicture}
    %     \end{subfigure}
    %     % \vspace{-10}
    %     \caption
    %     {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values }
    %     \label{Fig:Deepnet_SCL_Geom_NC}
    %     % \vspace{-15}
    % \end{figure*}

% \begin{figure}[t]
% % \centering
% %\hspace*{-20pt}
% \begin{subfigure}[b]{0.95\textwidth}
%     \centering
%     \begin{tikzpicture}
%         \node at (0.0,0) 
%         {\includegraphics[width=\textwidth]{Figs/NC1_Convergence_plots.pdf}};
%         % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%         \node at (-4.7,2.6) [scale=0.9]{\textbf{MNIST}};
%         \node at (-1.4,2.6) [scale=0.9]{\textbf{CIFAR10}};
%         \node at (1.9,2.6) [scale=0.9]{\textbf{CIFAR100}};
%         \node at (5.1,2.6) [scale=0.9]{\textbf{Tiny ImageNet}};
%         \node at (-7.0,1.1)  [scale=0.9, rotate=90]{\textbf{Step}};
%         \node at (-7.0,-0.9)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%         \node at (0.2,-2.3) [scale=0.9]{\textbf{Epoch}};
%     \end{tikzpicture}
% \end{subfigure}
% \caption
% {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for the corresponding ResNet-18 experiments in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values are usually on the order of $10^{-3}$ suggesting strong convergence of embeddings to their class means.}
% \label{fig:Deepnet_SCL_Geom_NC}
% \end{figure}

    \subsubsection{Angular convergence}~
    Having confirmed convergence of embeddings to their respective class-means via NC ($\h_i \approx \mub_c $ for $i:y_i = c$), we can now compare the feature geometry to the OF geometry by calculating the average $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ between each pair of classes. Fig.~\ref{fig:Deepnet_SCL_Geom_angles} plots the average cosine similarity $\text{Ave}_{c\neq c'}\alpha_{\text{sim}}(c,c')$ between class means for the same experiment as that 
 of Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. The graphs indicate strong convergence to orthogonality between feature representations of different classes. Similarly, results for angular convergence corresponding to Fig.~\ref{fig:loss_convergence} are provided in Fig.~\ref{fig:loss NC and angle convergence SM}(c), indicating similar convergence to OF for the full-batch experiments.

    \begin{figure}[h]
    % \centering
    %\hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.85\textwidth]{Figs/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.4,2.35) [scale=0.9]{\textbf{MNIST}};
            \node at (-1.4,2.35) [scale=0.9]{\textbf{CIFAR10}};
            \node at (1.5,2.35) [scale=0.9]{\textbf{CIFAR100}};
            \node at (4.4,2.35) [scale=0.9]{\textbf{Tiny ImageNet}};
            \node at (-6.2,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $10^{-2}$, indicating strong orthogonality between class-mean embeddings.}
    \label{fig:Deepnet_SCL_Geom_angles}
\end{figure}

%     \begin{figure*}[h]
%     % \centering
%     \hspace*{-16pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/Angles_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
%             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
%         \end{tikzpicture}
%     \end{subfigure}
%     % \vspace{-10}
%     \caption
%     {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $1e-2$, indicating strong orthogonality between features from different classes assuming Neural Collapse property holds.}
%         \label{Fig:Deepnet_SCL_Geom_NC}
%     \label{Fig:Deepnet_SCL_Geom_GMu}
%     % \vspace{-15}
% \end{figure*}

     \subsubsection{Embedding heatmaps}~
     %\vala{This part could be rephrased to only include the $\Hb^T\Hb$ score, unless we want to include the case with normalizing CE.}
     As a qualitative measure, we have generated heatmaps  that visually represent the learned embedding geometries; see Figs.~\ref{fig:heatmap}, \ref{fig:GM matrices comparison_old}, \ref{fig:GH matrices}. Specifically, we generate heatmaps of the Gram-matrices $\G_\M = \M^\top\M$ and $\G_\Hb = \Hb^\top\Hb$. In Fig.~\ref{fig:heatmap} we train ResNet-18 with the full MNIST dataset. In Fig.~\ref{fig:GM matrices comparison_old} we run on a subset of the dataset ($n = 10000$ total examples) with a batch size of 1000. Specifically for Fig.~\ref{fig:GM matrices comparison_old}, when optimizing with CE loss we modify the network (ResNet-18) such that it has a normalization layer before the linear classifier head. We consider this additional setting to allow for a comparison where CE features are constrained to the unit sphere akin to our SCL experiments. Lastly, in Fig.~\ref{fig:GH matrices} we plot the learned features Gram-matrix $\G_\Hb$ for a ResNet-18 trained on CIFAR10 ($n = 10000$ total examples) with a batch size of $1000$.\footnote{In both Fig.~\ref{fig:GH matrices} and Fig.~\ref{fig:GM matrices comparison_old} no batch duplication is used as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}.} This heatmap qualitatively shows a more complete picture as we are plotting $\G_\Hb = \Hb^\top \Hb$ rather than $\G_\M$, thus simultaneously illustrating both Neural Collapse and convergence to the k-OF structure.  

\subsubsection{Experiments with MLPs}~
{In Fig.~\ref{fig:MLP convergence} we run experiments with a simple 6 layer multilayer perceptron (MLP) to further explore the impact of model complexity on geometric convergence. The MLP includes batch normalization and ReLU activation between each layer. Each layer has  512 hidden units. We train the model with a batch size of 1000 with random reshuffling at each epoch. Furthermore, we train under $R$-STEP imbalanced MNIST. No batch duplication was used. All other aspects of the implementation are as described in Sec.~\ref{sec:exp_details_SM}. As shown in Fig.~\ref{fig:MLP convergence} all metrics $\Delta_{\G_\M}$, $\beta_{\text{NC}}$, and $\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$ indicate strong convergence to the OF geometry, irrespective of imbalance ratio $R$.}


     
    \begin{figure*}[h]
        \centering
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{SCL}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
       % \vskip\baselineskip
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{CE}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GM]
        {$\G_\M$ Gram-matrices of mean-embeddings for various $R$-STEP imbalances at last epoch (350) of training with ResNet-18 on MNIST with $n = 10000$. To allow for fair comparison, the CE features are normalized before the classifier head akin to the SCL experiments.} 
        \label{fig:GM matrices comparison_old}
    \end{figure*}
  \begin{figure*}[h]
        \centering
        \hspace{-0.5in}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GH]
        {$\G_\Hb$ Gram-matrices of feature embeddings for various imbalances at last epoch (350) of training SCL with CIFAR10 and ResNet.} 
        \label{fig:GH matrices}
    \end{figure*}


\subsection{Optimization dynamics}

\subsubsection{Loss convergence}
     In order to compute the lower bounds shown in Fig.~\ref{fig:loss_convergence},  we use Thm.~\ref{thm:scl_full}, substituting $e^{-1}$ with $e^{-1/\tau}$ using $\tau = 0.1$ as employed in our experiments; this substitution is allowed thanks to  Remark \ref{rem:tau}. Furthermore, we compute the lower bounds and $\Lc(\Hb)$ on a per sample basis, thus we divide by $n = 1000$ which corresponds to the number of datapoints in our single batch. Lastly, as a method of maintaining numerical stability (as implemented in \cite{khosla2020supervised}) we apply a global scaling of the loss by a factor $\nicefrac{\tau}{\tau_b}$, where $\tau_b = 0.07$ is the base temperature \cite{khosla2020supervised}. The complete experiment, conducted over $2000$ epochs (with axes limited to $500$ epochs for clarity in Figure~\ref{fig:loss_convergence}), is available in Figure~\ref{fig:loss NC and angle convergence SM}.

      \begin{figure*}
        \centering
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/LossCompToLowerBound.pdf}};
                 \node at (0.1,-1.97) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(a) Loss}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/NC.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.2,-1.8) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(b) NC}};
               %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/PairWiseAngles_corrected_small.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.13,-1.9) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(c) Angles}};
                %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a $R$-STEP imbalanced subset of MNIST of size $n=1000$. \textbf{(a)} Loss converges to the lower bound (dashed lines) computed in Thm.~\ref{thm:scl_full}. 
        \textbf{(b)} Within-class feature variation becomes negligible (NC). \textbf{(c)} The average pairwise cosine similarity of class-means approaches zero. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:loss NC and angle convergence SM} 
    \end{figure*}

\subsubsection{Effect of $\tau$}~
%\vala{Maybe we should discuss this a bit}
\begin{remark}\label{rem:tau}
    The normalization of the embeddings in \ref{eq:SCL_UFM_full} corresponds to SCL with temperature $\tau=1$. More generally, the normalization becomes $\norm{\h_i}^2=1/\tau$. The conclusion of Thm.~\ref{thm:scl_full} is insensitive to the choice of $\tau$, thus stated above for $\tau=1$ without loss of generality. Although the value of $\tau$ does not affect the global optimizers of \ref{eq:SCL_UFM_full}, we have empirically observed that it impacts the speed of convergence during training.
\end{remark}

As described in Sec.~\ref{sec:Deepnet_SCLGeom_exp} and Sec.~\ref{sec:full_batch_theory} the optimality of the OF geometry for the \ref{eq:SCL_UFM_full} is invariant to the choice of the temperature parameter $\tau$. However, we have found that the speed of convergence to the OF geometry is dependent on the choice of $\tau$. Shown in Fig.~\ref{fig:effect of tau full batch} is a full batch SCL experiment on $n=1000$ samples of MNIST trained on ResNet-18 with $\tau = 0.1, 1, 10$. It is clear from Fig.~\ref{fig:effect of tau full batch} that: (a) the within-class feature variation converges significantly faster for smaller $\tau$; (b) the angles converge to k-OF faster and smoother for smaller $\tau$ as well (see Fig.~\ref{fig:effect of tau full batch} (b)). In all cases, values of $\beta_\text{NC}$ and  $\alpha_{\text{sim}}(c,c')$ continue to decrease, and we anticipate further convergence if the networks are trained for longer. These results qualitatively agree with the findings of  \cite{khosla2020supervised} which suggest that smaller $\tau$ improves training speed. 
\begin{figure*}[h]
        \centering
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/NC.pdf}};
                 \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(a) NC}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                 \node at (-3,0.0)  [scale=0.9, rotate=90]{$\beta_\text{NC}
                 $};
            \end{tikzpicture}
        \end{subfigure}
       %\hfill
       \hspace{0.5in}
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/PairWiseAngles_corrected.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(b) Angles}};
               \node at (-3.4,0.0)  [scale=0.9, rotate=90]{$\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a subset of MNIST of size $n=1000$ with different temperature parameters $\tau$. \textbf{(a)} Within-class feature variation (NC). \textbf{(b)} Average pairwise cosine similarity of class-means. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:effect of tau full batch} 
    \end{figure*}

\begin{figure*}
        \centering
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/MLP/GmComp.pdf}};
                 \node at (0.1,-2) [scale=0.7]{Epoch};
    			\node at (0.0,2.1) [scale=0.9]{\textbf{(a) $\Delta_{\G_\M}$}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/MLP/NC.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.2,-2) [scale=0.7]{Epoch};
    			\node at (0.0,2.1) [scale=0.9]{\textbf{(b)} $\beta_{\text{NC}}$};
               %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/MLP/PairWiseAngles_corrected.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.13,-2.05) [scale=0.7]{Epoch};
    			\node at (0.0,2.1) [scale=0.9]{\textbf{(c)} $\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$};
                %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Geometry convergence metrics \textbf{(a)} $\Delta_{\G_\M}$, \textbf{(b)} $\beta_{\text{NC}}$, and \textbf{(c)} $\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$  for a 6 layer multilayer perceptron (MLP) model with ReLU activations trained with SCL and MNIST under $R$-STEP imbalance.}
        \label{fig:MLP convergence} 
    \end{figure*}

\subsection{Complementary results and discussions on batch-binding}\label{app:comp_results}
In this section, we describe examples where batching methods and batch-binding help improve the convergence speed of embeddings geometries to OF. 

\subsubsection{How batch-binding ensures a unique OF geometry}~ %In Fig.~\ref{fig:Binding_Examples_Visuals}, we provide a simple illustration to how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}. We believe that there may exist other methods to ensure conditions required for unique OF geometry; however, adding the same $k$ examples to each batch is a straightforward solution to ensuring OF and is usually computationally inexpensive as batch sizes tend to be larger than number of classes $k$. \vala{Rephrase ?} 
Fig.~\ref{fig:Binding_Examples_Visuals} provides a simple illustration demonstrating how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}.
While there are alternative approaches to satisfy the graph conditions stated in Cor.~\ref{cor:batch} for ensuring a unique OF geometry, the method of adding the same $k$ examples to each batch is a straightforward technique that is often computationally efficient, considering that batch sizes typically exceed the number of classes $k$.

\begin{figure}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.65\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_1.pdf} }}%
    \newline
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.36\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_2.pdf} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=0.32\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_3.pdf} }}%
    \caption{A simple illustration to explain how adding binding examples to each batch satisfies the requirements of Cor.~\ref{cor:batch}, thus leads to unique OF geometry. \textbf{(a)} Gives a $3$ class (black, grey and white) classification  example with 3 batches. In addition to the data for each batch (included in red), the binding examples $1,2,3$ are added to each batch. \textbf{(b)} Gives the Batch Interaction Graph for the induced subgraph $G_1$ of the class (black) of example $1$
    %class $G_{1}$ 
    and illustrates how all batches are connected through examples $1$, satisfying the first condition of Cor.~\ref{cor:batch}. \textbf{(c)} Elaborates on how all three class  graphs $G_1,G_2,G_3$ are connected through the interactions of data points $1,2,3$, satisfying the second condition of Cor.~\ref{cor:batch}.}
    \label{fig:Binding_Examples_Visuals}%
\end{figure}



 \begin{figure}[ht]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,2.07) [scale=0.9]{\textbf{Step}};
            \node at (2.6,2.07) [scale=0.9]{\textbf{Long-tail}};
            \node at (-6.25,0.0)  [scale=0.9, rotate=90]{$\Delta_{\G_\M}$};
            \node at (0.2,-2.07) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a ResNet-18 model trained on CIFAR10 under STEP imbalance, with data augmentation. Results represent the average run results over 5 versions of the experiments with randomly chosen binding examples from each class. 
    }
    \label{Fig:error_bars_plotGM}
\end{figure}

\noindent\textbf{Geometry convergence for different batching schemes.}~ 
A comparison of OF convergence with three batch selection schemes was introduced in Sec.~\ref{sec:batching}. We considered three strategies: 1) \textbf{No batch-shuffling}, 2) \textbf{Batch-shuffling}, and 3) \textbf{No batch-shuffling + batch-binding}. We noted that optimization with batch-binding, even in absence of shuffling is very effective at guiding the solution to the unique OF geometry. 
% To verify the role of batch selection on the learned features, we train ResNet-18 on CIFAR-10 under three batching scenarios: 1) \textbf{No batch-shuffling}: a mini-batch set $\mathcal{B}$ that partitions the training examples once at initialization and is held constant across training epochs. 2) \textbf{Batch-shuffling}: the examples are divided into mini-batch partition, with a random reshuffle of the examples at \textit{every} epoch. 3) \textbf{No batch-shuffling + batch-binding}: we construct a fixed partition of examples into mini-batches. Further, to each mini-batch we append a fixed set of $k$ binding examples. This remains constant throughout the training. 

\begin{figure}[t]
    % \centering
    \hspace*{-16pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Batch_Exp/GMu_Convergence_plots_BindingBatches.pdf}};
            \node at (-3.5,2.7) [scale=0.9]{\textbf{No Batch Shuffling}};
            \node at (0.1,2.7) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (3.8,3.1) [scale=0.9]{\textbf{No Batch Shuffling}};
            \node at (3.7,2.7) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-0.8)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-2.7) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {{Convergence to the OF geometry for various batching schemes {including the analysis-inspired scheme ``No Batch Shuffling + Batch-Binding''}. See text for details. Experiments conducted with CIFAR-10 and ResNet-18.}}
    \vspace{-8pt}
    \label{Fig:Deepnet_SCL_Geom_NC_BindingBatch}
\end{figure}

Further, in Table~\ref{Tab:NCC_Bindings} in the appendix, we present experimental evidence in  suggesting that batch binding does not negatively effect the balanced test accuracy of \textit{Nearest Class Center} (NCC) classifier. This observation, paired with the impact of binding examples on OF convergence, motivates further analysis of the relationship between OF geometry and test accuracy.
% {In Sec.~\ref{app:exp_appex} we provide further examples of how batch-binding improves convergence to the OF geometry when training with more complex datasets (CIFAR100) or less powerful models (DenseNet).}}

% \ct{Add a sentence mentioning the additional experiments in the appendix: helps with densenet and helps with cifar100(?)}

% \todo{provide references to App}

% As a demonstration of the efficacy of our proposed scheme of binding examples, we note in Fig. \ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} (right) that the convergence to OF becomes substantially superior, as soon as the binding examples are introduced, without a need to shuffle the examples in every epoch. In particular, the convergence to OF geometry occurs even though the original batching did not lead to OF. These observations provide strong evidence supporting our analysis of batching predicting the behavior of SCL trained deepnets.}

% For a set of mini-batches, $\mathcal{B}$ we will append the binding examples to each batch, creating the set $\mathcal{B}'$. Now the modified mini-batches $\mathcal{B}'$ satisfy the conditions of Cor.~\ref{cor:batch}, guaranteeing OF geometry as the optimal feature configuration. Given the large batch sizes used to train deepnets with SC in practice (as described in \cite{khosla2020supervised}) and our experimental setup, this overhead of adding $k$ examples to each batch is negligible; however, there are more efficient ways to ensure connectivity of batches, specially for larger values of $k$. \newline


% Following this finding, we design an experiment by training a ResNet-18 model on CIFAR-10 with batch size of 128 under three batching scenarios. 1) \textbf{No batch-shuffling}: a mini-batch set $\mathcal{B}$ that partitions the training examples is drawn once at initialization and is held constant across training epochs. 2) \textbf{Batch-shuffling}: the examples are divided into mini-batch partition, with a random reshuffle of the examples at \textit{every} epoch. 3) \textbf{No batch-shuffling + binding examples}: follows the same construction as case one but adds the $k$ binding examples to each batch. \newline
% From Fig. \ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} we see that the fixed partition batching (Bottom) does not converge to OF, most noticeably with imbalance, which is consistent with the conditions identified by Thm.~\ref{thm:scl_mini}. While for the random reshuffling case (center) we observe better convergence, the convergence is not as straightforward and stable. This further supports our analysis as we hypothesize that random reshuffling allows for more interactions between datapoints and classes, improving the batch connectivity but does not provide any guarantees in a deterministic fashion. Finally the case including binding examples (top) has remarkably fast convergence to OF geometry, providing strong evidence to support our findings in Cor.~\ref{cor:batch}.

\begin{figure}[t]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots_compareBindings.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.8) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.3) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.8) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{CIFAR10}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{MNIST}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a DenseNet-40 model trained on CIFAR10 and MNIST under STEP imbalance with and without batch-binding. While the impact of batch-bindings is less noticeable when training on a simple dataset such as MNIST,  the convergence is significantly improved, particularly under imbalance, when training on a more complex dataset such as CIFAR10. %\vala{rewrite this ? add explanation in text} \ct{reads good !}
    }
    \vspace{-10pt}
    \label{Fig:DenseNet_BindingsComparison}
\end{figure}

% \vp
\noindent\textbf{Improving convergence for less powerful models.}~
When conducting our experiments, we noticed that DenseNet-40 converges slower compared to ResNet-18. A reason for this may be related to the very different complexities of the two models: ResNet-18 has substantially more trainable parameters compared to DenseNet-40. In an attempt to improve the convergence speed, we reduce the batch size for DenseNet experiments to $128$ to increase the number of SGD iterations. We also train DenseNet for $500$ epochs instead of $350$ while reducing the learning rate from $0.1$ to $0.01$ at epoch $300$. Yet, we observe that with much smaller batch sizes, the embedding geometry does not always converge to the OF geometry, especially when training with high imbalance ratios. Specifically when training with randomly reshuffled batches, there is a higher chance that the examples do not interact with each other even if trained for long, suggesting that the optimal solution for all batches is not necessarily OF. We hypothesize that this likelihood increases when using smaller batch sizes during training. In order to combat this effect, we ran the DenseNet experiments with the addition of binding examples to every batch. 
As shown in Fig.~\ref{Fig:DenseNet_BindingsComparison}, we find that adding such binding examples significantly improves the convergence to OF, particularly when training on more complex datasets (CIFAR10 compared to MNIST) and under more severe imbalances (STEP imbalance with $R= 50,100$). These results emphasize the impact of batch-binding and provide further evidence regarding our claims in Sec.~\ref{sec:mini_batch_theory}. While the convergence values of $\Delta_{\G_\M}$ are higher when compared to ResNet-18, we deem them reasonable  considering the difference in the number of parameters between the two architectures. Similar to ResNet-18, we provide geometric convergence results for DenseNet-40 on different datasets in Fig.~\ref{Fig:Deepnet_SCL_DenseNet_Geom} in the appendix.

\begin{figure}[t]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Cifar100/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.7) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.1) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.7) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of embeddings geometry to OF as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$ for ResNet-18 trained on imbalanced CIFAR100 with SCL and different batching schemes. %Models are trained with both random-shuffling and random-shuffling with batch-binding. 
    Adding binding examples helps with the convergence to the OF geometry, especially under STEP imbalance with larger imbalance ratios.}
    \label{Fig:Deepnet_SCL_CIFAR100_GMu}
    \vspace{-15pt}
\end{figure}


% \vp
% \noindent\textbf{Improving convergence for more complex datasets.}~
 In another experiment, we consider the convergence of ResNet-18 embeddings to the OF geometry when trained with CIFAR100. Models are trained for $500$ epochs with a constant learning rate of $0.1$ and a batch size of 1024. In Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}, we see that ResNet-18 easily converges to CIFAR10. However, without batch binding, in Fig.~\ref{Fig:Deepnet_SCL_CIFAR100_GMu} ResNet-18 struggles to convergence. With a large number of classes ($k = 100$ for CIFAR100), it becomes increasingly more likely for the randomly reshuffled batches to not allow sufficient interactions between examples. Particularly for large imbalance ratios (e.g., $R=100,50$), since the number of samples in each minority class could become as low as $5$-$10$, some batches might never encounter examples from minority classes. This is particularly noticeable for STEP-Imbalance and large imbalance ratios, where half of the classes are minorities. On the other hand, including the binding examples in each batch (right side) can improve the convergence of the feature geometry to OF.  

\subsubsection{Convergence in non-ReLU settings}
In addition to observing that batch-binding improves the convergence of SCL with ReLU to OF, we consider the setting without ReLU. In particular in Fig.~\ref{fig:binding_ETF} we compare the convergence of the Gram matrix of mean embeddings to the ETF geometry with and without batch-binding. We train a ResNet-18 model with CIFAR-10. We observe that with a reduced batch size of 128 the convergence can be significantly improved with binding-examples.
\begin{figure*}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=0.4\textwidth]{Figs/etfBindingConvergence/noReLU_ETF_Conv_batchSize128.pdf}};
            \end{tikzpicture}
        \caption{Geometry convergence of $\mathbf{G}_\mu = \mathbf{M}^\top\mathbf{M}$ to the ETF geometry with and without binding examples. A batch size of 128 is used, there is no ReLU on the output features.}
        \label{fig:binding_ETF} 
\end{figure*}
% \vp
% \noindent\textbf{What does batch-shuffling mean for convergence?}
\subsection{On the convergence of batch-shuffling to OF}\label{app:batch-shuffling}
{It can be readily observed  that a fixed mini-batch partition without shuffling (\emph{No batch-shuffling} in the experiments above) does not satisfy the conditions of  Cor.~\ref{cor:batch}. Consequently, OF is \emph{not} the unique minimizer geometry in such scenarios. This is clearly manifested by the inadequate convergence levels observed in our experiments, as depicted for example in Fig. \ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch}. In contrast, in our experiments, when the examples are randomly shuffled prior to partitioning into mini-batches at each epoch (which we call \emph{Batch Shuffling}), the convergence behavior to OF shows a significant improvement  compared to the case of \emph{No batch-shuffling}. The observed improvement can be attributed to the fact that shuffling enables interactions among examples across epochs. To elaborate on this notion, we present a formalization of batch shuffling below.}

%Recall that $n$ is the number of training examples. 

%To provide a clearer explanation, we first outline some notation for the batch-shuffling scheme. 
Let $\Sc$ denote the set of all permutations of $[n] = \{1,2,...,n\}$, where $n$ is the total number of training examples. Additionally, let $b$ %\ct{If you need $b\geq 2$ for Remark 3, just have here ``let $b\geq2$'' so that is not confusing later.} 
denote {a fixed} batch-size. For simplicity, assume $n$ is an integer multiple of $b$. At the beginning of each training epoch $t$, we sample a permutation $s_t=(i_1,i_2,....,i_n)$ uniformly from $\mathcal{S}$ \emph{with} replacement. We then define $\Pc(s_t) := \{\{i_1,...,i_b\},\{i_{b+1},...,i_{2b}\},...,\{i_{n-b+1},...,i_{n}\}\}$ as the collection of total $\frac{n}{b}$ mini-batches obtained by partitioning $s_t$. These are the mini-batches used at epoch $t$. Thus, SCL in this epoch can be written as follows:
\begin{align*}%\label{eq:scl_shuffled_s}
     \Lc_{s_t}(\Hb):=\sum_{B \in \Pc(s_t)}\sum_{i\in B} \Lc_B(\Hb;i), \quad \text{where } \Lc_B(\Hb;i):= \frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\big(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\big),
\end{align*}
and recall $n_{B,c} = |\{i:i\in B,y_i=c\}|$.
Consider also the loss over \emph{all} mini-batches obtained by partitioning each permutation of $\Sc$: %In other words, the loss is the following:
\begin{align}\label{eq:scl_all_permutations}
     \Lc_{\Sc}(\Hb):=\sum_{s \in \Sc}\sum_{B \in \Pc(s)}\sum_{i\in B}\Lc_B(\Hb;i),
\end{align}
Now, since $s_t$ is uniformly sampled from $S$, we have the following relation for the expected per-epoch loss to the total loss given in Eqn. \eqref{eq:scl_all_permutations}:  $\mathbb{E}_{s_t}\Lc_{s_t}(\Hb) = \nicefrac{1}{|\Sc|}\,\Lc_{\Sc}(\Hb)$. Therefore, training with batch-shuffling can be regarded as a stochastic version of minimizing the total loss in Eq. \eqref{eq:scl_all_permutations}. Regarding the latter, it can be checked (see Rem.~\ref{rem:big_shuffling} below) that it satisfies the conditions of Cor.~\ref{cor:batch}, thereby making OF its unique minimizer geometry. Taken together, these findings suggest that although the per-epoch loss $\Lc_{s_t}$ obtained through batch-shuffling does not satisfy the conditions of Cor. \ref{cor:batch} for any specific epoch $t$, it does satisfy them in expectation. In particular, this can be regarded as preliminary justification of the experimental observation of improved convergence \emph{with batch-shuffling} compared to \emph{No batch-shuffling} schemes. The latter schemes fail to satisfy Cor. \ref{cor:batch} under any circumstances, unless in the extreme case of a large batch size where $b=n$ and we recover $\Lc_{\text{full}}$. However, it is important to note that the aforementioned argument is a rough approximation, as it is not feasible to average over all $|\Sc|=n!$ permutations when optimization is typically performed over a limited number of epochs. This can explain why, despite exhibiting better convergence compared to the No batch-shuffling schemes, batch-shuffling schemes still demonstrate non-smooth and inconsistent convergence patterns in our experiments. This behavior becomes particularly evident when comparing the convergence levels of batch-shuffling to our \emph{batch-binding} scheme, which is specifically designed to satisfy the conditions of Cor. \ref{cor:batch} at \emph{each} epoch. 

\begin{remark}\label{rem:big_shuffling}
    To show that Eqn.~\eqref{eq:scl_all_permutations} satisfies Cor.~\ref{cor:batch}, we will show that the corresponding \emph{batch interaction graph} $G$ is a complete graph. This suffices, because the induced subgraphs $G_c$ from Def.~\ref{def:big} for a complete graph are connected graphs, and there exist multiple edges between $G_{c_1}$ and $G_{c_2}$ for $c_1,c_2\in [k]$. To show that $G$ is a complete graph, we argue as follows. Consider the set $\Bc$ of all mini-batches obtained by partitioning all $n!$ elements of $\Sc$. Fix $b \geq 2$, so that the mini-batches have at least two examples. We will consider a subset $\Bc_1\subseteq\Bc$ of mini-batches and show that the corresponding batch interaction graph for $\Bc_1$ is a complete graph, which would then imply the batch interaction graph of $\Bc$ is also a complete graph. Specifically, let $\Bc_1\subseteq\Bc$ denote the mini-batches comprising of the first $b$ indices in every permutation $s\in\Sc$. In other words, from a given $s = (i_1,i_2,...,i_n) \in \Sc$, we let $\Bc_1$ include the mini-batch $\{i_1,i_2,...,i_b\}$. Since $\Sc$ includes all permutations of $[n]$, $\Bc_1$ contains all $b$-length permutations of the elements of $[n]$, possibly with repetitions. Thus, the \emph{batch interaction graph} created by the mini-batches in $\Bc_1$ is a \emph{complete graph}. In the definition of the \emph{batch interaction graph}, since a repeated presence of a pair of examples does not alter the graph, the batch interaction graph for $\Bc$ is the same complete graph. Thus, $\Bc$ satisfies Cor.~\ref{cor:batch}.
\end{remark}

%Thus, we conjecture that batch-shuffled training has better convergence towards OF than \emph{fixed batch} schemes. On the other hand, as $\Sc = n!$ is much larger compared to the number of epochs (thereby the number of permutations sampled), the batch-shuffled optimization does not have a smooth convergence. Indeed, our experiments show that the convergence can be substantially improved by applying \emph{batch-binding}.

% Let then $\Pc(s_t)$ denote the set of $\frac{n}{b}$ mini-batches obtained as follows. Let $s_t = (i_1,i_2,....,i_n)$, an ordered sequence, such that $s_t \in \Sc$. Now, $\Pc(s_t) := \{\{i_1,...,i_b\},\{i_{b+1},...,i_{2b}\},...,\{i_{n-b+1},...,i_{n}\}\}$ is the set of mini-batches obtained by partitioning $s_t$. These are the mini-batches used in epoch $t$. SCL in this epoch can be written as follows:
% \begin{align}\label{eq:scl_shuffled_s}
%      \Lc_{s_t}(\Hb):=\sum_{B \in \Pc(s_t)}\sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\bigg(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\bigg),
% \end{align}
% where recall $n_{B,c} = |\{i:i\in B,y_i=c\}|$.
% Now, consider the loss over all mini-batches obtained by partitioning each member of $\Sc$. In other words, the loss is the following:
% \begin{align}\label{eq:scl_all_permutations}
%      \Lc_{\Sc}(\Hb):=\sum_{s \in \Sc}\sum_{B \in \Pc(s)}\sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\bigg(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\bigg),
% \end{align}
% Since $s_t$ is assumed to be uniformly sampled from $S$, the expectation over per-epoch loss $\mathbb{E}_{s_t}\Lc_{s_t}(\Hb) = |\Sc|\Lc_{\Sc}(\Hb)$.

%\new{Therefore, training with batch-shuffling can be viewed as a stochastic version of \eqref{eq:scl_all_permutations}. It can be checked that \eqref{eq:scl_all_permutations} satisfies Cor.~\ref{cor:batch} and has OF as the unique minimizer geometry. Thus, we conjecture that batch-shuffled training has better convergence towards OF than \emph{fixed batch} schemes. On the other hand, as $\Sc = n!$ is much larger compared to the number of epochs (thereby the number of permutations sampled), the batch-shuffled optimization does not have a smooth convergence. Indeed, our experiments show that the convergence can be substantially improved by applying \emph{batch-binding}.}







\subsection{ReLU does not compromise Accuracy}\label{sec:generalization}
Having discussed the symmetry-preserving value of ReLU activation in SCL training, we now turn towards the impact on generalization accuracy. While the exact relationship between the training feature geometry and generalization is an open question, it is conceivable that maintaining symmetry in features is beneficial to generalization \citep{behnia2023implicit, zhu2022balanced}. In fact, our experiments with class-imbalance reveal that ReLU improves the test accuracy significantly in a subset of the cases, while not deteriorating in others. There have been suggestions of loss function modifications in such a way that the feature geometry is symmetric in presence of class-imbalance, consequently also achieving improvements in generalization \cite{behnia2023implicit, zhu2022balanced}. Since the role of a projector block is of interest when training with SCL, we compare the experimental test accuracies both when the projector is retained (post-projection) as well as discarded (pre-projection) during inference \citep{khosla2020supervised,chen2020simple,zhu2022balanced}.

%\new{We consider the effect of ReLU in two representative settings, (i) linear layer projector (ii) two-layer MLP projector. The details on the projector structure are deferred to the SM.}

%\todo{only two tables from below to be retained in main body}


% \begin{table}[!ht]
% \fontsize{6pt}{15pt}\selectfont
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \cline{2-5}
%          \multicolumn{1}{c}{} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \hline
%         R & Step & LongTail & Step & LongTail \\ \hline
%           1 & \multicolumn{2}{|c}{72.17 +/- 0.23}  & \multicolumn{2}{|c|}{72.32 +/- 0.60} \\ \hline
%         10 & 56.58 +/- 0.50 & 57.10 +/- 1.04 & 58.16 +/- 0.76 & 57.88 +/- 1.05 \\ \hline
%         100 & 43.49+/- 0.30 & 37.19 +/- 2.50 & 43.80 +/- 0.25 & 39.71 +/- 0.09 \\ \hline
%     \end{tabular}
%     \caption{Test accuracy comparison for a ResNet-18 model trained using SCL on CIFAR100 both with an without ReLU after the MLP. As per \cite{khosla2020supervised} the pre-projection fetures is used for test accuracy comparison and use Nearest Class Center for classification. The results suggest that the addition of ReLU does not compromise the test accuracy. For more analysis, see \ref{sec:generalization} in SM.}
% \end{table}


\begin{table}[!ht]
\fontsize{6pt}{15pt}\selectfont
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \cline{3-10}
         \multicolumn{2}{c}{} & \multicolumn{4}{|c}{Pre-Projection}   & \multicolumn{4}{|c|}{Post-Projection}   \\  \cline{3-10}
         \multicolumn{2}{c}{} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c}{MLP + ReLU} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \cline{2-10}
        \multicolumn{1}{c|}{} & R & Step & LongTail & Step & LongTail & Step & LongTail & Step & LongTail \\ \cline{1-10}

         \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{CIFAR-10 }}} & 1 & \multicolumn{2}{|c}{91.88 $\pm$ 0.29}  & \multicolumn{2}{|c}{92.04 $\pm$ 0.10} & \multicolumn{2}{|c}{91.94 $\pm$ 0.04} & \multicolumn{2}{|c|}{91.79 $\pm$ 0.13} \\ \cline{2-10}
        & 10 & 83.70 $\pm$ 1.09 & 83.82 $\pm$ 0.70 & 83.41 $\pm$ 0.64 & 84.40 $\pm$ 0.79 & 82.35 $\pm$ 0.67 & 82.97 $\pm$ 0.83 & 80.81 $\pm$ 1.01 & 82.99 $\pm$ 1.03 \\ \cline{2-10}
        & 100 & 60.19 $\pm$ 1.75 & 68.75 $\pm$ 0.31 & 67.12 $\pm$ 1.04 & 68.57 $\pm$ 1.69  & 55.31 $\pm$ 1.98 & 63.67 $\pm$ 0.77 & 59.83 $\pm$ 1.75 & 62.65 $\pm$ 2.37 \\ \cline{1-10}

         \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{CIFAR-100 }}} & 1 & \multicolumn{2}{|c}{72.17 $\pm$ 0.23}  & \multicolumn{2}{|c}{72.32 $\pm$ 0.60} & \multicolumn{2}{|c}{72.30 $\pm$ 0.57} & \multicolumn{2}{|c|}{72.25 $\pm$ 0.35} \\ \cline{2-10}
        & 10 & 56.58 $\pm$ 0.50 & 57.10 $\pm$ 1.04 & 58.16 $\pm$ 0.76 & 57.88 $\pm$ 1.05 & 54.57 $\pm$ 0.49 & 56.27 $\pm$ 0.45 & 55.35 $\pm$ 0.33 & 57.08 $\pm$ 0.82 \\ \cline{2-10}
        & 100 & 43.49$\pm$ 0.30 & 37.19 $\pm$ 2.50 & 43.80 $\pm$ 0.25 & 39.71 $\pm$ 0.09  & 40.29 $\pm$ 0.33 & 35.29 $\pm$ 1.64 & 39.93 $\pm$ 0.33 & 37.21 $\pm$ 0.51 \\ \cline{1-10}
        
        \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Tiny ImageNet }}} & 1 & \multicolumn{2}{|c}{62.53 $\pm$ 1.23}  & \multicolumn{2}{|c}{62.26 $\pm$ 0.37} & \multicolumn{2}{|c}{62.71 $\pm$ 1.10} & \multicolumn{2}{|c|}{62.48 $\pm$ 0.40} \\ \cline{2-10}
        & 10 & 50.17 $\pm$ 1.44 & 50.8 $\pm$ 1.94 & 49.78 $\pm$ 0.67 & 49.81 $\pm$ 0.82 & 48.91 $\pm$ 1.6 & 50.23 $\pm$ 1.83 & 48.23 $\pm$ 0.53 & 48.76 $\pm$ 1.18 \\ \cline{2-10}
        & 100 & 39.13 $\pm$ 0.63 & 36.06 $\pm$ 0.89 & 40.02 $\pm$ 0.62 & 35.84 $\pm$ 1.33  & 37.41 $\pm$ 0.29 & 34.57 $\pm$ 0.95 & 37.19 $\pm$ 0.68 & 33.78 $\pm$ 1.34 \\ \cline{1-10}
    \end{tabular}
    \caption{Comparison of test accuracies for (i) CIFAR-10 (ii) CIFAR-100 (iii) Tiny ImageNet when ResNet-18 is trained with a 2-layer MLP projection head with and without ReLU on the output features. Comparisons in both Step and LT imbalance settings. Additionally a comparison of the performance using features before the projection head (pre-projection), and after the head (post-projection). }
    \label{tab:relu_noRelu_all_test}
\end{table}


% \begin{table}[!ht]
% \fontsize{8pt}{20pt}\selectfont
%     \centering
%     \begin{tabular}{|p{0.2cm}|l|l|l|l|l|}
%     \hline
%          & & \multicolumn{2}{|c|}{Pre-Projection}   & \multicolumn{2}{|c|}{Post-Projection}   \\  \hline 
%         & R & MLP & MLP + ReLU & MLP & MLP + ReLU  \\ \hline
%         \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ CIFAR-10 }}} & 1 & 62.53 +/- 1.23  & 62.26 +/- 0.37 & 62.71 +/- 1.10 & 62.48 +/- 0.40 \\ \cline{2-6}
%          & 10 & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \cline{2-6}
%          & 100 & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%          \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ CIFAR-100 }}} & 1 & 62.53 +/- 1.23  & 62.26 +/- 0.37 & 62.71 +/- 1.10 & 62.48 +/- 0.40 \\ \cline{2-6}
%          & 10 & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \cline{2-6}
%          & 100 & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%         \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{ Tiny  ImageNet }}} & 1 & 62.53 +/- 1.23  & 62.26 +/- 0.37 & 62.71 +/- 1.10 & 62.48 +/- 0.40 \\ \cline{2-6}
%          & 10 & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \cline{2-6}
%          & 100 & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%     \end{tabular}
%     \caption{\vala{New Tables} Post-projection, Tiny ImageNet}
% \end{table}



% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.91 +/- 0.23 \% & 91.79 +/- 0.21 \% & \textbf{91.88 +/- 0.29} \% & 91.86 +/- 0.32 \% \\ \hline
%         10 & 82.12 +/- 1.06 \% & 83.29 +/- 0.49 \% & \textbf{83.70 +/- 1.09} \% & 83.41 +/- 0.64 \% \\ \hline
%         100 & 61.25 +/- 0.64 \% & 62.98 +/- 0.68 \% & 60.19 +/- 1.75 \% & \textbf{67.12 +/- 1.04} \% \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR10-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.89 +/- 0.26 \% & 91.81 +/- 0.24 \% & 91.88 +/- 0.23 \% & \textbf{91.94 +/- 0.40} \% \\ \hline
%         10 & 81.11 +/- 1.24 \% & 81.02 +/- 0.60 \% & \textbf{82.35 +/- 0.67} \% & 80.81 +/- 1.01 \% \\ \hline
%         100 & 55.74 +/- 1.08 \% & 57.07 +/- 0.60 \% & 55.31 +/- 1.98 \% & \textbf{59.83 +/- 1.75} \% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR10-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.17 +/- 0.23 \% & \textbf{72.32 +/- 0.60\%} \\ \hline
%         10 & 56.58 +/- 0.50 \% & \textbf{58.16 +/- 0.76\%} \\ \hline
%         100 & 43.49 +/- 0.30\% & \textbf{43.80 +/- 0.25\%} \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR100-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & \textbf{72.30 +/- 0.57} \% & 72.25 +/- 0.35\% \\ \hline
%         10 & 54.57 +/- 0.49 \% & \textbf{55.35 +/- 0.33\%} \\ \hline
%         100 & \textbf{40.29 +/- 0.33\%} & 39.93 +/- 0.14\% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR100-STEP}
% \end{table}



% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.73 +/- 0.30\% & 91.96 +/- 0.26\% & \textbf{92.04 +/- 0.10\%} & 91.79 +/- 0.13\% \\ \hline
%         10 & 83.25 +/- 0.55\% & 84.02 +/- 0.68\% & 83.70 +/- 0.70\% & \textbf{84.40 +/- 0.79\%} \\ \hline
%         100 & 68.40 +/- 1.35\% & 67.88 +/- 1.21\% & \textbf{68.75 +/- 0.31\%} & 68.57 +/- 1.69\% \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR10-LT}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.73 +/- 0.29\% & 91.81 +/- 0.36\% & \textbf{92.04 +/- 0.13\%} & 91.91 +/- 0.17\% \\ \hline
%         10 & 82.55 +/- 0.64\% & 82.98 +/- 0.98\% & 82.97 +/- 0.83\% & \textbf{82.99 +/- 1.03\%} \\ \hline
%         100 & 63.64 +/- 0.99\% & 63.51 +/- 1.39\% & \textbf{63.67 +/- 0.77\%} & 62.65 +/- 2.37\% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR10-LT}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.25 +/- 0.33 \% & \textbf{72.30 +/- 0.19\%} \\ \hline
%         10 & 57.10 +/- 1.04 \% & \textbf{57.88 +/- 1.05\%} \\ \hline
%         100 & 37.19 +/- 2.50\% & \textbf{39.71 +/- 0.09\%} \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR100-LT}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.37 +/- 0.32 \% & \textbf{72.44 +/- 0.29\%} \\ \hline
%         10 & 56.27 +/- 0.45 \% & \textbf{57.08 +/- 0.82\%} \\ \hline
%         100 & 35.29 +/- 1.64\% & \textbf{37.21 +/- 0.51\%} \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR100-LT}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%          & \multicolumn{2}{|c|}{Pre-Projection}   & \multicolumn{2}{|c|}{Post-Projection}   \\  \hline 
%         R & MLP & MLP + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 62.53 +/- 1.23  & 62.26 +/- 0.37 & 62.71 +/- 1.10 & 62.48 +/- 0.40 \\ \hline
%         10 \text{ (Step) } & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \hline
%         10 \text{ (LT) } & 51.22 +/- 1.94 & 49.81 +/- 0.82 & 50.99 +/- 1.83 & 48.76 +/- 1.18 \\ \hline
%         100 \text{ (Step) } & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%         100 \text{ (LT) } & 36.06 +/- 0.89 & 35.84 +/- 1.33 & 34.57 +/- 0.95 & 33.78 +/- 1.34 \\ \hline
%     \end{tabular}
%     \caption{\vala{New Tables} Post-projection, Tiny ImageNet}
% \end{table}


Thus, as noted in Table \ref{tab:relu_noRelu_all_test} we make a remarkable observation that simply adding ReLU to the network can yield significant improvements in test accuracy in certain cases, while at least matching that of the case without ReLU in others. In light of this, our finding of the insensitivity of the embedding geometry in presence of ReLU serves a potential explanation. Our analysis therefore paves an important direction for future empirical investigations into the role of the activation functions in the projector network on generalization of SCL.





\subsubsection{Impact of batch-binding on generalization}
To study the effect of binding examples on generalization, we  consider the \textit{Nearest Class Center} (NCC) classifier. For this, each test example is assigned the label of the class center $\mub_c$ learned during training that is closest to it (in Euclidean distance). We consider a simple setup of training a ResNet-18 model on CIFAR10 under imbalances $R = 10,100$ both with and without the binding examples. Models are trained with a batch size of $128$ for $350$ epochs. We ran the experiments with a smaller batch size to increase the number of back-propagation steps as adding data augmentations slows down convergence to OF geometry . We start with a learning rate of $0.1$, which is reduced by a factor of 10 on epochs $250$ and $300$. Weight decay is set to $5\times10^{-4}$.
In addition, we apply data augmentation as it is common practice when considering generalization and test accuracy. In particular, rather than simply adding horizontally flipped images (as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}) we allow for generic augmentations that include simple horizontal or vertical flips and random cropping with a probability of $0.5$. %In order to help with the convergence speed, we implement the augmentation on the duplicate version of the batches which are added to each batch (previously, this duplicate batch simply included a horizontally flipped version of each data point). These augmentations include simple horizontal or vertical flips and random cropping with a probability of $0.5$.  
The NCC test accuracy was measured across $5$ versions of the experiment with the $k$ binding examples sampled randomly every time and $5$ versions without any batch-binding. The results for NCC balanced test accuracies are provided in Table~\ref{Tab:NCC_Bindings}. While making definitive conclusions regarding the impact of the embeddings geometries and binding examples on generalization requires further investigation, this preliminary investigation suggests that batch-binding does \emph{not} negatively impact NCC test accuracy.


Finally, Fig.~\ref{Fig:error_bars_plotGM} shows convergence of embeddings geometry to OF for the same experiments. As expected, the convergence is slightly slower in this case due to the inclusion of data augmentation (random crops and flips).

\begin{table}[ht]
  \caption{NCC test accuracy for Batch-Binding}
  \hspace*{-20pt}
  \label{Tab:NCC_Bindings}
  \centering
  \begin{tabular}{l|ll|ll}
  \toprule
    & \multicolumn{2}{c}{Step} & \multicolumn{2}{c}{Long-tail}\\ 
    \cmidrule(r){2-3} \cmidrule(r){4-5}
    Ratio \\ ($R$)      & Reshuffling  & Reshuffling & Reshuffling  & Reshuffling \\ & & + Batch-Binding &  & + Batch-Binding  \\ 
    \midrule
    $10$ & $83.31 \pm 0.65 \%$ &   $83.27 \pm 0.27 \%$  & $85.04 \pm 0.28 \%$  &  $85.03 \pm 0.57 \%$  \\
    $100$     & $64.07 \pm 1.79 \%$ & $64.18 \pm 1.25 \%$   &  $67.75 \pm 1.21 \%$ & $68.08 \pm 0.72 \%$\\
  \end{tabular}
\end{table}

\begin{figure*}[h]
    % \centering
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0.9) 
            {\includegraphics[width=0.8\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-3.4,3.4) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.2,3.4) [scale=0.9]{\textbf{MNIST}};
            \node at (3.7,3.4) [scale=0.9]{\textbf{FMNIST}};
            \node at (-5.8,2.0)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-5.8,-0.0)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-1.7) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{$\G_\M$ Convergence to OF}
    \end{subfigure}
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0.9) 
            {\includegraphics[width=0.8\textwidth]{Figs/DenseNet_Geometry/NC_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-3.4,3.4) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.2,3.4) [scale=0.9]{\textbf{MNIST}};
            \node at (3.7,3.4) [scale=0.9]{\textbf{FMNIST}};
            \node at (-5.8,2.0)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-5.8,-0.0)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-1.7) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Neural Collapse}
    \end{subfigure}
    % \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0.9) 
            {\includegraphics[width=0.8\textwidth]{Figs/DenseNet_Geometry/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-3.4,3.4) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.2,3.4) [scale=0.9]{\textbf{MNIST}};
            \node at (3.7,3.4) [scale=0.9]{\textbf{FMNIST}};
            \node at (-5.8,2.0)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-5.8,-0.0)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-1.7) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Angles between class-means}
    \end{subfigure}
    \caption
    {Geometric convergence of embeddings (as based on Def.~\ref{def:nc}, Def.~\ref{def:of}, and Def.~\ref{def:ncof}) of DenseNet-40 trained with batch-binding. We measure: \textbf{(a)} $\Delta_{\G_\M}$, \textbf{(b)} $\beta_{\text{NC}}$, and \textbf{(c)} $\text{Ave}_{c \neq c'} \alpha_{\text{sim}}(c,c')$ as defined in text.}
    \label{Fig:Deepnet_SCL_DenseNet_Geom}
\end{figure*}

% \pagebreak 

==> sections_arxiv_v2/exp_appex_old.tex <==
\subsection{Details on the main experimental setup}\label{sec:exp_details_SM}
In our deep-net experiments, we focus on two common network architectures, ResNet and DenseNet. Specifically, we use ResNet-18 and DenseNet-40 with approximately $11$ million and $200$ thousand trainable parameters, respectively. For both models, we replace the last layer linear classifier with a normalization layer (normalizing such that $\| \h_i\|=1$ for $i \in [n]$) of feature dimension $d=512$. Specifically, following  \cite{graf2021dissecting}, we  directly optimize the normalized features that are then used for inference. (We note this is slightly different compared to \cite{khosla2020supervised}, where the authors train the output features of a projection head, then discard this projection head at inference time). We remark that both ResNet and DenseNet architectures include ReLU activations before the final output, which enforces a non-negativity on the learned embeddings. Resnet-18 models with CIFAR10, MNIST and FashionMNIST have been trained for 350 epochs with a constant learning rate of $0.1$, no weight decay, batch size of $1024$, and SCL temperature parameter $\tau = 0.1$ (consistent with the choice of $\tau$ made in \cite{khosla2020supervised,graf2021dissecting}). For all experiments with other models or datasets, we provide experimental details in the following sections. All models, regardless of architecture or dataset, have been trained on a single Tesla V100 GPU machine. 

% All ResNet models were trained for 350 epochs with a constant learning rate of $0.1$ and no weight decay. On the other hand, we observed slower convergence to OF geometry when training our DenseNet models on more complex datasets such as CIFAR10, and larger imbalance ratios $\RT$. To combat this, we increased the number of training epochs to 500 while annealing the learning rate by a factor of 0.1 on epoch 300, reduced to batch size to 128 to increase number of back-propagation iterations, and used binding examples to improve convergence speed. 

%\todo{Remove the following?}
%Given our focus on feature geometry, we did not perform any data augmentation to increase convergence speed.  \vala{mention this ? We did perform experiments with common-practice data augmentation techniques which showed general convergence towards OF, but more iterations for better convergence}.

% \vala{Do we need further specific detail for each ? }

% \noindent\textbf{Details for Fig.~\ref{fig:intro}} 

% \noindent\textbf{Details for Fig.~\ref{fig:GM matrices comparison}}

\subsection{Additional geometric analysis}
     
     In addition to analyzing the convergence of the Gram-matrix of class-mean embeddings $\G_\M$ to the OF geometry (as provided in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}), we also keep track of Neural Collapse (Defn.~\ref{def:nc}) of individual embeddings and orthogonality of their class-means (Defn.~\ref{def:of}) separately. Furthermore, we qualitatively study the Gram matrices $\G_\M$ and $\G_\Hb$  and compare them to corresponding matrices for the CE loss under imbalances. 
     
     \noindent\textbf{Neural Collapse.}~
     In order to quantify the collapse (NC) of embeddings, $\h_i, i \in [n]$, to their class-means,  we measure $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ \cite{NC}. Here, $\Sigma_B= \sum_{c\in [k]}(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})^\top$ is the between class covariance matrix, $\boldsymbol{\mu}_G = \frac{1}{k}\sum_{c\in[k]}\boldsymbol{\mu}_c$ is the  global mean, and $\Sigma_W  = \sum_{i\in [n]}(\h_i - \boldsymbol{\mu}_{y_i})(\h_i - \boldsymbol{\mu}_{y_i})^\top$ is the within class covariance matrix.

     For the experiments shown in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu} and Fig.~\ref{fig:loss_convergence} in the main body, the corresponding values of $\beta_\text{NC}$ can be found in Fig.~\ref{fig:Deepnet_SCL_Geom_NC} and Fig.~\ref{fig:loss NC and angle convergence SM}(b) respectively.

     
    % \begin{figure*}[h]
    %     % \centering
    %     \hspace*{-16pt}
    %     \begin{subfigure}[b]{\textwidth}
    %         \centering
    %         \begin{tikzpicture}
    %             \node at (0.0,0) 
    %             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
    %             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    %             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
    %             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
    %             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
    %             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
    %             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
    %             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
    %         \end{tikzpicture}
    %     \end{subfigure}
    %     % \vspace{-10}
    %     \caption
    %     {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values }
    %     \label{Fig:Deepnet_SCL_Geom_NC}
    %     % \vspace{-15}
    % \end{figure*}

    \begin{figure}[t]
    % \centering
    %\hspace*{-20pt}
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.3) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.3) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.3) [scale=0.9]{\textbf{FMNIST}};
            \node at (-7.8,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-7.8,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.3) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for corresponding ResNet-18 training results from Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values are usually on the order of $10^{-3}$ suggesting strong convergence of embeddings to their class means.}
    \label{fig:Deepnet_SCL_Geom_NC}
\end{figure}

    \noindent\textbf{Angular convergence.}~
    Having confirmed convergence of embeddings to their respective class-means via NC ($\h_i \approx \mub_c $ for $i:y_i = c$), we can now compare the feature geometry to the OF geometry by calculating the average $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ between each pair of classes. Fig.~\ref{fig:Deepnet_SCL_Geom_angles} plots the average cosine similarity $\text{Ave}_{c\neq c'}\alpha_{\text{sim}}(c,c')$ between class means for the same experiment as that 
 of Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. The graphs indicate strong convergence to orthogonality between feature representations of different classes. Similarly, results for angular convergence corresponding to Fig.~\ref{fig:loss_convergence} are provided in Fig.~\ref{fig:loss NC and angle convergence SM}(c), indicating similar convergence to OF for the full-batch experiments.

    \begin{figure}[h]
    % \centering
    %\hspace*{-20pt}
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.975\textwidth]{Figs/Deepnet_Geometry_Exp/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.3) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.3) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.3) [scale=0.9]{\textbf{FMNIST}};
            \node at (-7.6,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-7.6,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.3) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $10^{-2}$, indicating strong orthogonality between class-mean embeddings.}
    \label{fig:Deepnet_SCL_Geom_angles}
\end{figure}

%     \begin{figure*}[h]
%     % \centering
%     \hspace*{-16pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/Angles_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
%             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
%         \end{tikzpicture}
%     \end{subfigure}
%     % \vspace{-10}
%     \caption
%     {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $1e-2$, indicating strong orthogonality between features from different classes assuming Neural Collapse property holds.}
%         \label{Fig:Deepnet_SCL_Geom_NC}
%     \label{Fig:Deepnet_SCL_Geom_GMu}
%     % \vspace{-15}
% \end{figure*}

     \noindent\textbf{Feature embedding heatmaps.}~
     %\vala{This part could be rephrased to only include the $\Hb^T\Hb$ score, unless we want to include the case with normalizing CE.}
     As a qualitative measure, we have generated heatmaps  that visually represent the learned embedding geometries; see Fig.~\ref{fig:GM matrices comparison}, \ref{fig:GM matrices comparison_old}, \ref{fig:GH matrices}. Specifically, we generate heatmaps of the Gram-matrices $\G_\M = \M^\top\M$ and $\G_\Hb = \Hb^\top\Hb$. In Fig.~\ref{fig:GM matrices comparison} we train ResNet-18 with the full MNIST dataset. In Fig.~\ref{fig:GM matrices comparison_old} we run on a subset of the dataset ($n = 10000$ total examples) with a batch size of 1000. Specifically for Fig.~\ref{fig:GM matrices comparison_old}, when optimizing with CE loss we modify the network (ResNet-18) such that it has a normalization layer before the linear classifier head. We consider this additional setting to allow for a comparison where CE features are constrained to the unit sphere akin to our SCL experiments. Lastly, in Fig.~\ref{fig:GH matrices} we plot the learned features Gram-matrix $\G_\Hb$ for a ResNet-18 trained on CIFAR10 ($n = 10000$ total examples) with a batch size of $1000$.\footnote{In both Fig.~\ref{fig:GH matrices} and Fig.~\ref{fig:GM matrices comparison_old} no batch duplication is used as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}.} This heatmap qualitatively shows a more complete picture as we are plotting $\G_\Hb = \Hb^\top \Hb$ rather than $\G_\M$, thus simultaneously illustrating both Neural Collapse and convergence to the k-OF structure.  
    \begin{figure*}[h]
        \centering
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{SCL}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
       % \vskip\baselineskip
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{CE}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GM]
        {$\G_\M$ Gram-matrices of mean-embeddings for various $R$-STEP imbalances at last epoch (350) of training with ResNet-18 on MNIST with $n = 10000$. To allow for fair comparison, the CE features are normalized before the classifier head akin to the SCL experiments.} 
        \label{fig:GM matrices comparison_old}
    \end{figure*}
  \begin{figure*}[h]
        \centering
        \hspace{-0.5in}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GH]
        {$\G_\Hb$ Gram-matrices of feature embeddings for various imbalances at last epoch (350) of training SCL with CIFAR10 and ResNet.} 
        \label{fig:GH matrices}
    \end{figure*}
\subsection{Optimization dynamics}

\noindent\textbf{Loss convergence.}~
     In order to compute the lower bounds shown in Fig.~\ref{fig:loss_convergence},  we use Thm.~\ref{thm:scl_full}, substituting $e^{-1}$ with $e^{-1/\tau}$ using $\tau = 0.1$ as employed in our experiments; this substitution is allowed thanks to  Remark \ref{rem:tau}. Furthermore, we compute the lower bounds and $\Lc(\Hb)$ on a per sample basis, thus we divide by $n = 1000$ which corresponds to the number of datapoints in our single batch. Lastly, as a method of maintaining numerical stability (as implemented in \cite{khosla2020supervised}) we apply a global scaling of the loss by a factor $\nicefrac{\tau}{\tau_b}$, where $\tau_b = 0.07$ is the base temperature \cite{khosla2020supervised}. The complete experiment, conducted over $2000$ epochs (with axes limited to $500$ epochs for clarity in Figure~\ref{fig:loss_convergence}), is available in Figure~\ref{fig:loss NC and angle convergence SM}.

      \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/LossCompToLowerBound.pdf}};
                 \node at (0.1,-1.97) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(a) Loss}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/NC.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.2,-1.8) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(b) NC}};
               %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/PairWiseAngles_corrected_small.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.13,-1.9) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(c) Angles}};
                %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a $\RT$-STEP imbalanced subset of MNIST of size $n=1000$. \textbf{(a)} Loss converges to the lower bound (dashed lines) computed in Thm.~\ref{thm:scl_full}. 
        \textbf{(b)} Within-class feature variation becomes negligible (NC). \textbf{(c)} The average pairwise cosine similarity of class-means approaches zero. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:loss NC and angle convergence SM} 
    \end{figure*}

\noindent\textbf{Effect of $\tau$.}~
%\vala{Maybe we should discuss this a bit}
As described in Sec.~\ref{sec:Deepnet_SCLGeom_exp} and Sec.~\ref{sec:full_batch_theory} the optimality of the OF geometry for the \ref{eq:SCL_UFM_full} is invariant to the choice of the temperature parameter $\tau$. However, we have found that the speed of convergence to the OF geometry is dependent on the choice of $\tau$. Shown in Fig.~\ref{fig:effect of tau full batch} is a full batch SCL experiment on $n=1000$ samples of MNIST trained on ResNet-18 with $\tau = 0.1, 1, 10$. It is clear from Fig.~\ref{fig:effect of tau full batch} that: (a) the within-class feature variation converges significantly faster for smaller $\tau$; (b) the angles converge to k-OF faster and smoother for smaller $\tau$ as well (see Fig.~\ref{fig:effect of tau full batch} (b)). In all cases, values of $\beta_\text{NC}$ and  $\alpha_{\text{sim}}(c,c')$ continue to decrease, and we anticipate further convergence if the networks are trained for longer. These results qualitatively agree with the findings of  \cite{khosla2020supervised} which suggest that smaller $\tau$ improves training speed. 
\begin{figure*}[h]
        \centering
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/NC.pdf}};
                 \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(a) NC}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                 \node at (-3,0.0)  [scale=0.9, rotate=90]{$\beta_\text{NC}
                 $};
            \end{tikzpicture}
        \end{subfigure}
       %\hfill
       \hspace{0.5in}
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/PairWiseAngles_corrected.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(b) Angles}};
               \node at (-3.4,0.0)  [scale=0.9, rotate=90]{$\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a subset of MNIST of size $n=1000$ with different temperature parameters $\tau$. \textbf{(a)} Within-class feature variation (NC). \textbf{(b)} Average pairwise cosine similarity of class-means. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:effect of tau full batch} 
    \end{figure*}

\subsection{Implications of batch-binding}
In this section, we describe examples where batching methods and batch-binding help improve the convergence speed of embeddings geometries to OF. 

\noindent\textbf{How batch-binding ensure unique OF geometry.}~ %In Fig.~\ref{fig:Binding_Examples_Visuals}, we provide a simple illustration to how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}. We believe that there may exist other methods to ensure conditions required for unique OF geometry; however, adding the same $k$ examples to each batch is a straightforward solution to ensuring OF and is usually computationally inexpensive as batch sizes tend to be larger than number of classes $k$. \vala{Rephrase ?} 
Fig.~\ref{fig:Binding_Examples_Visuals} provides a simple illustration demonstrating how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}.
While there are alternative approaches to satisfy the graph conditions stated in Cor.~\ref{cor:batch} for ensuring a unique OF geometry, the method of adding the same $k$ examples to each batch is a straightforward technique that is often computationally efficient, considering that batch sizes typically exceed the number of classes $k$.

\begin{figure}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.65\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_1.pdf} }}%
    \newline
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.36\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_2.pdf} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=0.32\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_3.pdf} }}%
    \caption{A simple illustration to explain how adding binding examples to each batch satisfies the requirements of Cor.~\ref{cor:batch}, thus leads to unique OF geometry. \textbf{(a)} Gives a $3$ class (black, grey and white) classification  example with 3 batches. In addition to the data for each batch (included in red), the binding examples $1,2,3$ are added to each batch. \textbf{(b)} Gives the Batch Interaction Graph for the induced subgraph $G_1$ of the class (black) of example $1$
    %class $G_{1}$ 
    and illustrates how all batches are connected through examples $1$, satisfying the first condition of Cor.~\ref{cor:batch}. \textbf{(c)} Elaborates on how all three class  graphs $G_1,G_2,G_3$ are connected through the interactions of data points $1,2,3$, satisfying the second condition of Cor.~\ref{cor:batch}.}
    \label{fig:Binding_Examples_Visuals}%
\end{figure}

\noindent\textbf{Improving convergence for CIFAR100.}~
In addition to the benchmark datasets previously explored, we consider the convergence of ResNet-18 embeddings to the OF geometry when trained with CIFAR100. The models are trained for $500$ epochs with a constant learning rate of $0.1$ and a batch size of 1024. With a large number of classes ($k = 100$ for CIFAR100) it becomes increasingly more likely for the randomly reshuffled batches to violate the conditions required for achieving unique OF based on  Cor.~\ref{cor:batch}. Particularly for large imbalance ratios (e.g., $R=100,50$), since the number of samples in each minority class could become as low as $5$-$10$, some batches might never encounter examples from minority classes. However, including the binding examples in each batch can improve the convergence of the feature geometry to OF. In Fig.~\ref{Fig:Deepnet_SCL_CIFAR100_GMu} we measure the convergence of ResNet-18 trained both with and without the batch-binding. Batch-binding considerably expedite and improve the convergence to the OF geometry. This is particularly noticeable for STEP-Imbalance and large imbalance ratios, where half of the classes are minorities, thus the inclusion of binding examples becomes crucial in ensuring that our theoretical convergence requirements for reaching the OF are satisfied.


\noindent\textbf{Improving DenseNet convergence by batch-binding.}~
When conducting our experiments for Fig.~\ref{fig:intro}, we have noticed that DenseNet-40 converges significantly slower  compared to ResNet-18. A potential reason for this may be related to the very different complexities of the two models: ResNet-18 has significantly more trainable parameters compared to DenseNet-40. In an attempt to improve the convergence speed, we have decided to reduce the batch size for DenseNet to $128$ in order to increase the number of possible back-propagation steps. We have also trained the DenseNet models for $500$ epochs instead of $350$ and we have reduced the learning rate from $0.1$ to $0.01$ at epoch $300$. Yet, we have observed that with much smaller batch sizes, the embedding geometry does not always converge to the OF geometry, especially when training with high imbalance ratios.  Specifically when training with randomly reshuffled batches, there is always a  chance that the Batch Interaction Graph does not meet the requirements of Cor.~\ref{cor:batch}, implying that the optimal solution for all batches is not necessarily OF. We hypothesize that this likelihood increases when using smaller batch sizes during training. In order to combat this effect, we have decided to run the DenseNet experiments with the addition of binding examples to every batch. 
As suggested by Fig.~\ref{Fig:DenseNet_BindingsComparison}, we find that adding such binding examples significantly improves the convergence to OF. This is particularly so when training on more complex datasets (CIFAR10 compared to MNIST) and under more severe imbalances (STEP imbalance with $R= 50,100$). These results emphasize the impact of batch-binding and provide further evidence regarding our claims in Sec.~\ref{sec:mini_batch_theory}. While the convergence values of $\Delta_{\G_\M}$ are higher when compared to ResNet-18, we deem them reasonable  considering the difference in the number of parameters between the two architectures. Similar to ResNet-18, we have provided geometric convergence results for DenseNet-40 in Fig.~\ref{Fig:Deepnet_SCL_DenseNet_Geom}.

\begin{figure}[h]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Cifar100/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.7) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.1) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.7) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of embeddings geometry to OF as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$ for a ResNet-18 models trained on imbalanced CIFAR100 with SCL. Models are trained with both random-shuffling and random-shuffling with batch-binding. We see how the inclusion of binding examples helps with convergence to OF, especially under $R$-STEP imbalance and large imbalance ratios.}
    \label{Fig:Deepnet_SCL_CIFAR100_GMu}
\end{figure}


 \begin{figure}[ht]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,2.07) [scale=0.9]{\textbf{Step}};
            \node at (2.6,2.07) [scale=0.9]{\textbf{Long-tail}};
            \node at (-6.25,0.0)  [scale=0.9, rotate=90]{$\Delta_{\G_\M}$};
            \node at (0.2,-2.07) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a ResNet-18 model trained on CIFAR10 under STEP imbalance, with data augmentation. Results represent the average run results over 5 versions of the experiments with randomly chosen binding examples from each class. 
    }
    \label{Fig:error_bars_plotGM}
\end{figure}




\begin{figure}[h]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots_compareBindings.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.8) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.3) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.8) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{CIFAR10}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{MNIST}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a DenseNet-40 model trained on CIFAR10 and MNIST under STEP imbalance with and without batch-binding. While the impact of batch-bindings is less noticeable when training on a simple dataset such as MNIST,  the convergence is significantly improved, particularly under imbalance, when training on a more complex dataset such as CIFAR10. %\vala{rewrite this ? add explanation in text} \ct{reads good !}
    }
    \label{Fig:DenseNet_BindingsComparison}
\end{figure}




\begin{figure*}[h]
    % \centering
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{$\G_\M$ Convergence to OF}
    \end{subfigure}
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/NC_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Neural Collapse}
    \end{subfigure}
    % \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Angles between class-means}
    \end{subfigure}
    \caption
    {Geometric convergence of embeddings (as based on Def.~\ref{def:nc}, Def.~\ref{def:of}, and Def.~\ref{def:ncof}) of DenseNet-40. We measure: \textbf{(a)} $\Delta_{\G_\M}$, \textbf{(b)} $\beta_{\text{NC}}$, and \textbf{(c)} $\text{Ave}_{c \neq c'} \alpha_{\text{sim}}(c,c')$ as defined in text.}
    \label{Fig:Deepnet_SCL_DenseNet_Geom}
\end{figure*}


\noindent\textbf{Impact of batch-binding on generalization.}~ 
To study the effect of binding examples on generalization, we  consider the \textit{Nearest Class Center} (NCC) classifier. For this, each test example is assigned the label of the class center $\mub_c$ learned during training that is closest to it (in Euclidean distance). We consider a simple setup of training a ResNet-18 model on CIFAR10 under imbalances $R = 10,100$ both with and without the binding examples. Models are trained with a batch size of $128$ for $350$ epochs. We start with a learning rate of $0.1$, which is reduced by a factor of 10 on epochs $250$ and $300$. Weight decay is set to $5\times10^{-4}$.
In addition, we apply data augmentation as it is common practice when considering generalization and test accuracy. In particular, rather than simply adding horizontally flipped images (as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}) we allow for generic augmentations that include simple horizontal or vertical flips and random cropping with a probability of $0.5$. %In order to help with the convergence speed, we implement the augmentation on the duplicate version of the batches which are added to each batch (previously, this duplicate batch simply included a horizontally flipped version of each data point). These augmentations include simple horizontal or vertical flips and random cropping with a probability of $0.5$.  
The NCC test accuracy was measured across $5$ versions of the experiment with the $k$ binding examples sampled randomly every time and $5$ versions without any batch-binding. The results for NCC balanced test accuracies are provided in Table~\ref{Tab:NCC_Bindings}. While making definitive conclusions regarding the impact of the embeddings geometries and binding examples on generalization requires further investigation, this preliminary investigation suggests that batch-bindingdoes \emph{not} negatively impact NCC test accuracy.
\begin{table}[ht]
  \caption{NCC test accuracy for Batch-Binding}
  \hspace*{-20pt}
  \label{Tab:NCC_Bindings}
  \centering
  \begin{tabular}{l|ll|ll}
  \toprule
    & \multicolumn{2}{c}{Step} & \multicolumn{2}{c}{Long-tail}\\ 
    \cmidrule(r){2-3} \cmidrule(r){4-5}
    Ratio \\ ($R$)      & Reshuffling  & Reshuffling & Reshuffling  & Reshuffling \\ & & + Batch-Binding &  & + Batch-Binding  \\ 
    \midrule
    $10$ & $83.31 \pm 0.65 \%$ &   $83.27 \pm 0.27 \%$  & $85.04 \pm 0.28 \%$  &  $85.03 \pm 0.57 \%$  \\
    $100$     & $64.07 \pm 1.79 \%$ & $64.18 \pm 1.25 \%$   &  $67.75 \pm 1.21 \%$ & $68.08 \pm 0.72 \%$\\
  \end{tabular}
\end{table}

Finally, Fig.~\ref{Fig:error_bars_plotGM} shows convergence of embeddings geometry to OF for the same experiments. As expected, the convergence is slightly slower in this case due to the inclusion of data augmentation (random crops and flips).

% \begin{table}
%   \caption{NCC test accuracy for Binding Examples}
%   \label{Tab:NCC_Bindings}
%   \centering
%   \begin{tabular}{lll}
%   \toprule
%     \multicolumn{3}{c}{Step} \\ 
%     \cmidrule(r){1-3}
%     Ratio ($\RT$)      & Random Reshuffling  & Random Reshuffling \\ & & + Binding Example  \\ 
%     \midrule
%     $10$ & $83.19 \%$ &   $83.27 \pm 0.27 \%$      \\
%     $100$     & $61.76 \%$       & $64.18 \pm 1.25 \%$  \\
%     \bottomrule
%     \multicolumn{3}{c}{Long-tail} \\
%     \cmidrule(r){1-3}
%     Ratio ($\RT$)      & Random Reshuffling  & Random Reshuffling \\ & & + Binding Example \\
%     \midrule
%     $10$ & $84.65 \%$ &   $85.03 \pm 0.57 \%$      \\
%     $100$     & $69.71 \%$       & $68.08 \pm 0.72 \%$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}




% \pagebreak 

==> sections_arxiv_v2/geometry.tex <==
\subsection{Centering}
In several previous works on the geometry of features learned by various loss functions \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring}, the theoretical model used, i.e. the UFM, did not constrain the sign of embedding coordinates. However, the experimental models often include several ReLU activations, leading to non-negativity constraints on the feature embeddings. To bridge this gap while comparing the geometry of empirical observations to the theoretical model predictions, a heuristic global mean centering is performed on the empirical embeddings. For the case of balanced labels, this \emph{centering} heuristic is as described as below \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring}:
\begin{align*}
    \mub_G &= \frac{1}{k}\sum_{c \in [k]}\mub_c,\ \ \Bar{\mub}_c = \mub_c - \mub_G,\ \ \Bar{\M} = \begin{bmatrix} \Bar{\mub}_1, \cdots, \Bar{\mub}_k \end{bmatrix}
\end{align*}
In our result, no such heuristic processing is required, as our model gives the geometry of embeddings as they are.

\subsection{OF vs ETF}
In this section we elaborate on the two geometries of interest- OF and ETF. Recall that our results show that the SCL with ReLU converges to the OF regardless of label distribution, whereas \cite{graf2021dissecting} showed that SCL without ReLU results in the ETF when label distribution is uniform. \new{For the reader's convenience, we recall the definition of simplex ETF from \cite{NC}:}
\new{
\begin{definition}[Simplex ETF]\label{def:etf}
    We say that $k$ vectors $\Vb = [\vb_1,\cdots,\vb_k] \in \R^{d\times k}$ form a simplex-ETF {if $\Vb^\top\Vb \propto \Id_k-\frac{1}{k}\ones_k\ones_k^\top$, i.e., for each pair of $(i,j)\in[k],$ $\|\vb_i\| = \|\vb_j\|$ and $\frac{\vb_i^T\vb_j}{\|\vb_i\|\|\vb_j\|} = \frac{-1}{k-1}$.} %\tina{need to define identity matrix somewhere earlier}
\end{definition}
}
\tina{I think for clarification, similar to OF, we need to mention that by ETF geometry we mean NC + mean-embeddings follow ETF. Have me mentioned this anywhere?}

\noindent\textbf{Mean-centered OF is ETF}: \new{The following straightforward lemma demonstrates that when a $k$-OF is centered, it transforms into an ETF.
\begin{lemma}
Suppose that a set of vectors $\{\vb_1,...,\vb_k\}$ form a $k$-OF in $\R^d$ with $d \geq k$, and their mean-centered counterparts are $\Bar{\vb}_c = \vb_c - \vb_G, \forall c \in [k]$, where $\vb_G = \frac{1}{k}\sum_{c\in[k]}\vb_c$.  Then, the centered embeddings $\{\Bar{\vb}_1,...,\Bar{\vb}_k\}$ form a simplex ETF spanning a $k-1$-dimensional subspace. 
\end{lemma}
\begin{proof}
Let $\Vb=\begin{bmatrix}
    \vb_1&\ldots&\vb_k
\end{bmatrix}$    and $\tilde\Vb=\begin{bmatrix}
    \tilde\vb_1&\ldots&\tilde\vb_k
\end{bmatrix}$. By definition of a $k$-OF, we know that $\Vb^\top\Vb\propto\Id$. Without loss of generality suppose the constant of proportionality is $1$ so that  $\Vb^\top\Vb=\Id\,.$ Since all $\vb_i$s are orthonormal, this then implies that $\Vb^T\vb_G=\frac{1}{k}\ones_k$ and $\vb_G^\top\vb_G=\frac{1}{k}\,.$ These put together gives the desired as follows:
\begin{align*}
    \tilde\Vb^\top\tilde\Vb &= \left(\Vb-\vb_G\ones_k^\top\right)^\top\left(\Vb-\vb_G\ones_k^\top\right) = \Vb^\top\Vb - \ones_k\vb_G^\top\Vb-\Vb^\top\vb_G\ones_k^\top+(\vb_G^\top\vb_G)\ones_k\ones_k^\top
    \\
    &=\Id_k - \frac{1}{k}\ones_k\ones_k^\top\,.
\end{align*}
\end{proof}
}

 Therefore, equivalently, the centered embeddings learned by deep-nets form an ETF. It is to be noted that our result shows this for an arbitrary label distribution, with balanced labels being a special case. 

On the other hand, it is not possible to obtain whether a set of vectors form an OF, given that their mean-centered versions make an ETF. This is because the unknown mean-vector can not be determined.


\subsection{UFM vs UFM$_+$: UFM fails to predict the geometry}
\tina{title?}

In this paper, we use the simplified \ref{eq:SCL_UFM_full} problem to describe the representations learned by deep-nets trained with SCL. Unlike many previous works studying the SCL or CE loss \cite{}, we impose ReLU (non-negativity) constraints on the embeddings in formulating the \ref{eq:SCL_UFM_full}. In Secs.~\ref{sec:Deepnet_SCLGeom_exp} and \ref{sec:theo_results}, we showed that regardless of the label configuration in the training set, the global optimizer of \ref{eq:SCL_UFM_full} is an OF and the embeddings learned by deep-nets converge to our prediction. On the other hand, when the training set is balanced, \citet{graf2021dissecting} showed that without the ReLU constraints, ETF minimizes the UFM. As discussed in Sec.~\ref{sec:}, we know that ETF is in fact the centered OF. Thus, in the balanced case, UFM provides a close prediction of the \emph{centered} embeddings. However, as we will show in the following lemma, the global optimizer of UFM is sensitive to label distribution in the training set, and ETF is not the global optimizer in the presence of imbalances. In other words, the difference between UFM and UFM$_+$ cannot be addressed by only considering the centering of the optimal embeddings.\tina{needs rewording}

\begin{lemma}
    Consider the \ref{eq:ufm} problem defined below. If classes in the training set are not balanced, % i.e., $\exists c,c'\in[k]$ such that $n_c\neq n_{c'}$, 
    the global solution of \ref{eq:ufm} is not necessarily an ETF. 

    \begin{align}\label{eq:ufm}
    \widehat{\Hb} \in \arg\min_{\Hb} \Lc_{\text{\emph{full}}}
    (\Hb)~~\text{\emph{subj. to}}~~\|\h_i\|^2 = 1,\, \forall i\in[n].
    \tag{$\text{UFM}$}
\end{align}
\end{lemma}
\begin{proof}
    To rule out the optimality of ETF in imbalanced setups, we show ETF does not minimize the loss in a $k=3$ class example. Specifically, consider a STEP-imbalanced training set with 3 classes of size $[\RT n_\text{min}, n_\text{min}, n_\text{min}]$ with $n_\text{min}\geq 2$ and $\RT \geq 10$. If $\Hb_\text{ETF}$ follows the ETF geometry, from Def.~\ref{def:etf} and the feasibility condition, for the mean-embeddings $\M_\text{ETF}$ we have $\M_\text{ETF}^\top\M_\text{ETF} = \frac{k}{k-1}(\Id_k - \frac{1}{k}\ones_k\ones_k^\top).$ Thus, the value of the loss function at ETF is as follows,
    \begin{align*}
        \Lc_{\text{{full}}}(\Hb_\text{ETF}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-\frac{3}{2}}\big) + 2\log\big(n_\text{min}-1+n_\text{min}(\RT+1)e^{-\frac{3}{2}}\big)\Big).
    \end{align*}
    Now, consider $\widetilde{\Hb} = [\widetilde{\mub}\otimes \ones_{\RT n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{ n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{n_\text{min}}^\top]$, where $\norm{\widetilde{\mub}}=1$ and thus $\widetilde{\Hb}$ is in the feasible set. With this choice of $\widetilde{\Hb}$, we have,
    \begin{align*}
        \Lc_{\text{{full}}}(\widetilde{\Hb}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-2}\big) + 2\log\big(2n_\text{min}-1+\RT n_\text{min}e^{-2}\big)\Big).
    \end{align*}
    It is easy to check that, for imbalance levels higher than $\RT\geq10$, $$\Lc_{\text{{full}}}(\widetilde{\Hb}) < \Lc_{\text{{full}}}(\Hb_\text{ETF}).$$ In other words, when the imbalance level is large enough, ETF does not attain the optimal cost in \ref{eq:ufm}.
\end{proof}

==> sections_arxiv_v2/geometry2.tex <==
Within this section, we provide an in-depth analysis
%, expanding upon our earlier discussions, 
of the disparities between the predictions generated by the UFM, commonly utilized in previous studies, and the refined version \ref{eq:SCL_UFM_full} that we employ in this work to study the embedding geometry of SCL.

The majority of previous works \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring} study the geometry of learned embeddings by investigating a proxy unconstrained features model (UFM). Specifically, the UFM drops the dependence of the learned embeddings $\Hb$ on the network parameters $\thetab$, and finds optimal $\widehat{\Hb}$ that minimizes the loss function. In case of SCL, as studied in e.g., \cite{graf2021dissecting}, the corresponding UFM is as follows,
% 
\begin{align}\label{eq:ufm}
    \arg\min_{\Hb} \Lc_{\text{{SCL}}}
    (\Hb)~~\text{{subj. to}}~~\|\h_i\|^2 = 1,\, \forall i\in[n].
    \tag{$\text{UFM}$}
\end{align}
% 
As explained in Sec.~\ref{sec:theo_results}, this paper employs a refined version of the UFM, namely \ref{eq:SCL_UFM_full}, to characterize the representations learned by SCL. Specifically, \ref{eq:SCL_UFM_full} further constrains the embeddings $\Hb$ to be non-negative, in this way accounting for the ReLU activation commonly used in several deep-net architectures. Thus the search for the optimal $\Hb$ is restricted to the non-negative orthant. 


%aim to connect and compare different aspects of these two theoretical models.

\subsubsection{Centering heuristic}\label{sec:centering}
Many deep neural network models incorporate ReLU activations, resulting in nonnegative feature embeddings at the last layer. In contrast, the UFM does not impose any constraints on the optimal $\Hb$, allowing it to contain negative entries.  To bridge this gap, previous works \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring,zhou2022optimization,seli,zhou2022all} apply a heuristic approach called \emph{global-mean centering} on the learned embeddings before comparing their arrangement with the theoretical prediction given by the UFM. Specifically, the centering heuristic is applied as follows: Prior to comparing the geometries, we subtract the global-mean embedding $\mub_G = \frac{1}{k}\sum_{c \in [k]}\mub_c$ from all class-mean embeddings $\mub_c$ to form the \emph{centered class-mean embeddings}  $\Bar{\mub}_c$:
\begin{align*}
    \Bar{\mub}_c = \mub_c - \mub_G,\ \qquad\ \Bar{\M} = \begin{bmatrix} \Bar{\mub}_1 & \cdots & \Bar{\mub}_k \end{bmatrix}\,.
\end{align*}
Indeed, this heuristic centering operation effectively ensures that the mean-embedding matrix $\bar{\M}$, after the necessary shifting, is centered at the origin, satisfying $\bar{\M}\ones_k=0$. This property also holds for the global optimizers of the UFM found in the previous work, which served as a motivation for the heuristic centering. 

Unlike the approach mentioned above, our findings do not necessitate any heuristic embedding processing for comparing the geometries. This is because our model directly provides the geometry of the embeddings in their original form.

\subsubsection{Centered OF is simplex ETF %Explaining relation to the result by \cite{graf2021dissecting}
}\label{ref:OFvsETF}
Focusing on the SCL, \citet{graf2021dissecting} have used the \ref{eq:ufm} to characterize the learned embeddings and have found that, for balanced classes, the simplex ETF geometry is the global optimizer of \ref{eq:ufm}. In other words, the optimal embeddings $\Hb$ adhere to the NC (Defn.~\ref{def:nc}), and the corresponding mean embeddings $\M$ form a simplex ETF.  {For the reader's convenience, we recall below the definition of simplex ETF from \cite{NC}.}
{
\begin{definition}[Simplex ETF]\label{def:etf}
    We say that $k$ vectors $\Vb = [\vb_1,\cdots,\vb_k] \in \R^{d\times k}$ form a simplex-ETF {if $\Vb^\top\Vb \propto \Id_k-\frac{1}{k}\ones_k\ones_k^\top$, i.e., for each pair of $(i,j)\in[k],$ $\|\vb_i\| = \|\vb_j\|$ and $\frac{\vb_i^T\vb_j}{\|\vb_i\|\|\vb_j\|} = \frac{-1}{k-1}$.} %\tina{need to define identity matrix somewhere earlier}
\end{definition}
}




In this paper, we show instead that the global optimizer of \ref{eq:SCL_UFM_full} is an OF. Remarkably, this result holds true regardless of the label-imbalance profile. However, for the purpose of comparison with the findings of \cite{graf2021dissecting}, let us specifically consider the scenario of balanced data. In this case, an intriguing question arises: 
\begin{center}
\emph{Specifically for balanced data, how does our discovery that embeddings with ReLU converge to an OF compare to the previous finding by \cite{graf2021dissecting} that embeddings without ReLU converge to an ETF?}    
\end{center}

The answer to this question lies on the centering trick discussed in Section \ref{sec:centering}. Specifically, stating that embeddings form an OF implies that \emph{centered} embeddings form an ETF. This straightforward fact is formalized in the following lemma.

%Thus, \citet{graf2021dissecting} used ETF as the reference geometry for describing their empirical observations in deep-net experiments. However, we use the OF geometry as the reference, since it minimizes \ref{eq:SCL_UFM_full} in the same balanced setup. The following straightforward lemma demonstrates that when an OF is centered, it transforms into an ETF.
\begin{lemma}\label{lem:OF2ETF}
Suppose that a set of vectors $\{\vb_1,...,\vb_k\}$ form a $k$-OF in $\R^d$ with $d \geq k$, and their mean-centered counterparts are $\Bar{\vb}_c = \vb_c - \vb_G, \forall c \in [k]$, where $\vb_G = \frac{1}{k}\sum_{c\in[k]}\vb_c$.  Then, the centered embeddings $\{\Bar{\vb}_1,...,\Bar{\vb}_k\}$ form a simplex ETF spanning a $k-1$-dimensional subspace. 
\end{lemma}
% \begin{proof}
% Let $\Vb=\begin{bmatrix}
%     \vb_1&\ldots&\vb_k
% \end{bmatrix}$    and $\bar\Vb=\begin{bmatrix}
%     \bar\vb_1&\ldots&\bar\vb_k
% \end{bmatrix}$. 
% %\todo{are these supposed to be tilde or bar?} 
% By definition of a $k$-OF, we know that $\Vb^\top\Vb\propto\Id$. Without loss of generality suppose the constant of proportionality is $1$ so that  $\Vb^\top\Vb=\Id\,.$ Since all $\vb_i$s are orthonormal, this then implies that $\Vb^\top\vb_G=\frac{1}{k}\ones_k$ and $\vb_G^\top\vb_G=\frac{1}{k}\,.$ These put together gives the desired as follows:
% \begin{align*}
%     \bar\Vb^\top\bar\Vb &= \left(\Vb-\vb_G\ones_k^\top\right)^\top\left(\Vb-\vb_G\ones_k^\top\right) = \Vb^\top\Vb - \ones_k\vb_G^\top\Vb-\Vb^\top\vb_G\ones_k^\top+(\vb_G^\top\vb_G)\ones_k\ones_k^\top=\Id_k - \frac{1}{k}\ones_k\ones_k^\top\,.
% \end{align*}
% \end{proof}
% 
 % Therefore, showing that embeddings learned by deep-nets form an OF, as demonstrated in this work, is essentially equivalent to the centered embeddings forming an ETF. However, we note that the results in \citet{graf2021dissecting} only holds when the training labels have a uniform distribution.
% 
Lemma \ref{lem:OF2ETF} states that based on our finding that embeddings form an OF, we can deduce that centered embeddings form an ETF. This conclusion aligns with the analysis conducted by \cite{graf2021dissecting} on the UFM (See Fig.~\ref{fig:CE_vs_SCL_OF_ETF} for a representative comparison). However, the UFM analysis itself does not provide information regarding the necessity of the centering technique, which remains heuristic. Additionally, it is important to note that it is unclear how to establish that (uncentered) embeddings form an OF if we initially know that centered embeddings form an ETF. This is due to the unknown vector used for centering, which cannot be determined. 
% This issue of identifiability is the underlying reason why the angle prediction eventually made by \cite{graf2021dissecting} in Fig.~\ref{fig:intro} deviates from the true value of ninety degrees, which corresponds to the OF.

% our finding and the finding by \cite{graf2021dissecting} are the same up to a global-mean centering of the embeddings. However, we remark that this 

%  \begin{remark}
%     Given that the centered version of a set of vectors form an ETF, it is not possible to obtain whether these vectors form an OF. This is because we cannot determine the unknown vector used for centering.     
%  \end{remark}


\subsubsection{UFM can fail to predict the true geometry}

\begin{wrapfigure}[20]{r}{0.38\textwidth} 
     \centering
            \vspace{-0.5in}\begin{tikzpicture}
                \node at (0.0,0.0) 
                {\includegraphics[width=0.35\textwidth]{Figs/CE_vs_SCL_OF_ETF/CE_vs_SCL_GMu_Convergence_plots_balanced.pdf}};
                 \node at (0.1,-2.3) [scale=0.7]{Epoch};
    			\node at (0.2,2.1) [scale=0.9]{$\G_\M$ \textbf{convergence}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
    \captionsetup{width=0.95\linewidth}
    \vspace{-0.1in}
    \caption{Convergence of embeddings geometries for SCL (in green) and CE (in blue)  on balanced CIFAR10 with ResNet-18. Solid lines track the distance of \emph{uncentered} embeddings to OF and  dashed lines track the distance of \emph{centered} embeddings to simplex ETF.  For CE, the learning rate and weight decay and batch size are set according to \cite{NC}. Note the convergence of SCL (solid green) to its implicit geometry is noticeably better compared to CE (dashed blue).}
    \label{fig:CE_vs_SCL_OF_ETF}
\end{wrapfigure}
In the previous section, we demonstrated that for balanced data, the solution found by the \ref{eq:ufm} does not predict the true geometry of the embeddings (i.e., OF) in presence of ReLU, but it can predict the geometry of the embeddings after the application of a global-mean centering heuristic (i.e., ETF). Naturally this raises the following question: 
\begin{center}
\emph{Does the \ref{eq:ufm} consistently provide accurate predictions for the geometry of the \emph{centered} embeddings? In other words, does the OF geometry predicted by our refined \ref{eq:SCL_UFM_full} always align with being a global optimizer of the UFM after centering?}    \end{center}

The lemma presented below demonstrates that the answer to this question is negative. Specifically, it shows that the global optimizer of \ref{eq:ufm} is sensitive to the label distribution of the training set, thus ETF is not necessarily a global optimizer in the presence of imbalances.  This is in contrast to \ref{eq:SCL_UFM_full}, for which we showed that the global optimizer  is consistently an OF, irrespective of the labels distribution. In other words, the difference between \ref{eq:ufm} and \ref{eq:SCL_UFM_full} cannot be addressed by only considering the centering of the optimal embeddings in general.

% for balanced data, that the \ref{eq:ufm} can predict the true geometry of embeddings up to a necessary global-mean centering heuristic

% As discussed in the previous section, when the training data is balanced, by considering the centering (as defined in Sec.~\ref{sec:centering}), both \ref{eq:ufm} and \ref{eq:SCL_UFM_full} provide a close characterization of the embeddings learned by deep-nets. However, as we will show in the following lemma, the global optimizer of \ref{eq:ufm} is sensitive to label distribution of the training set, and ETF is not necessarily the global optimizer in the presence of imbalances. This is in contrast to \ref{eq:SCL_UFM_full}, for which we showed the global optimizer, regardless of the training data distribution, is an OF. In other words, the difference between \ref{eq:ufm} and \ref{eq:SCL_UFM_full} cannot be addressed by only considering the centering of the optimal embeddings in general.


\begin{lemma}\label{lem:counterexample}
    If classes in the training set are not balanced, % i.e., $\exists c,c'\in[k]$ such that $n_c\neq n_{c'}$, 
    the global solution of \ref{eq:ufm} is not necessarily an ETF.  Thus, the solution of \ref{eq:SCL_UFM_full} (which according to Thm.~\ref{thm:scl_full} is an OF) is in general different to that of \ref{eq:ufm} even after centering is applied.
\end{lemma}
% \begin{proof}
%     To rule out the optimality of ETF in imbalanced setups, we show ETF does not minimize the loss in a $k=3$ class example. Specifically, consider a STEP-imbalanced training set with 3 classes of sizes $[\RT n_\text{min}, n_\text{min}, n_\text{min}]$ with $n_\text{min}\geq 2$ and $\RT \geq 10$. Suppose $\Hb_\text{ETF}$ follows the ETF geometry. Then, from Def.~\ref{def:etf} and the feasibility condition, for the mean-embeddings $\M_\text{ETF}$ we have $\M_\text{ETF}^\top\M_\text{ETF} = \frac{k}{k-1}(\Id_k - \frac{1}{k}\ones_k\ones_k^\top).$ Thus, the value of the loss function at ETF is 
%     \begin{align*}
%         \Lc_{\text{{full}}}(\Hb_\text{ETF}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-\frac{3}{2}}\big) + 2\log\big(n_\text{min}-1+n_\text{min}(\RT+1)e^{-\frac{3}{2}}\big)\Big).
%     \end{align*}
%     Now, consider $\widetilde{\Hb} = [\widetilde{\mub}\otimes \ones_{\RT n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{ n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{n_\text{min}}^\top]$, where {$\widetilde{\mub}$} is an arbitrary unit-norm vector. Since $\norm{\widetilde{\mub}}=1$, it follows that  $\widetilde{\Hb}$ is in the feasible set. With this choice of $\widetilde{\Hb}$, we have,
%     \begin{align*}
%         \Lc_{\text{{full}}}(\widetilde{\Hb}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-2}\big) + 2\log\big(2n_\text{min}-1+\RT n_\text{min}e^{-2}\big)\Big).
%     \end{align*}
%     It is easy to check that, for imbalance levels higher than $\RT\geq10$, $$\Lc_{\text{{full}}}(\widetilde{\Hb}) < \Lc_{\text{{full}}}(\Hb_\text{ETF}).$$ In other words, ETF does not always attain the optimal cost in \ref{eq:ufm}.
% \end{proof}

% \begin{remark}
% \tina{omit?}
%      While \citet{zhu2022balanced} acknowledge that the global optima of the UFM do not conform to the ETF geometry in the presence of class imbalance, they do not provide a formal proof to support this claim. In this context, Lemma \ref{lem:counterexample} fulfills this purpose.
% \end{remark}

\subsection{Comparing implicit Geometries: SCL vs CE -- A summary}
{We conclude this discussion by providing a summary of the observations on the contrasting implicit geometries of embeddings between the two loss functions: SCL and CE.
\\
\noindent~~\textbf{1. The SCL geometry with ReLU is robust to label-imbalances.} Specifically, the geometry of SCL embeddings exhibits symmetry consistently, whereas imbalances introduce distortions in the implicit geometry of SCL without ReLU and also for CE \citep{fang2021exploring,seli}.
\\
\noindent~~\textbf{2. The convergence of SCL to its implicit geometry is notably superior.} The measured geometry of SCL exhibits a faster decrease in distance from its analytic formula (i.e., OF) with each epoch, eventually reaching lower values. This holds true not only for label-imbalanced data, where \cite{seli} finds that the convergence of embeddings deteriorates as the imbalance ratio increases, but also for balanced data, where the convergence of embeddings with CE is inferior compared to classifiers \citep{NC}; see Fig. \ref{fig:CE_vs_SCL_OF_ETF} for visualization.
\\
\noindent~~\textbf{3. For SCL, batching  matters.}}~During CE training, when using any arbitrary batching method, there exists an implicit interaction among all the examples, that is facilitated by the inclusion of the classifier vectors in the loss objective. On the other hand, with SCL, the interactions between examples are explicitly controlled by the mini-batches. Specifically, our analysis of the role of batches in Secs.~\ref{sec:mini_batch_theory} and \ref{Sec:unique}, along with the batch-binding scheme presented in Sec. \ref{Sec:Binding_examples} reveal that the structure of mini-batches critically affects the geometry of the learnt embeddings. %Our batch-analysis and batch-binding scheme specifically emphasize the significance of batching in SCL.

\subsection{Batch-Binding}
In Sec.~\ref{sec:batching} we outlined a simple scheme called \emph{batch-binding} that ensures OF convergence starting from any given arbitrary set of mini-batches. The simple procedure is restated in Alg.~\ref{alg:binding} for simplicity.
 \begin{algorithm}
  \caption{Batch-binding}\label{alg:binding}
  \begin{algorithmic}[1]
    \Procedure{Batch-binding}{a set of mini-batches $\mathcal{B}$, number of classes $k$}
    \State \textbf{Binding examples}: A set of examples represents a set of binding examples if it includes exactly one example from every class. This set has, thus, $k$ elements. \label{def:binding}
\State To every batch $B\in\mathcal{B}$ add the chosen set of binding examples to create a new batch configuration $\mathcal{B}^\prime$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

==> sections_arxiv_v2/implicitBias.tex <==
%\subsection{Cross-entropy}
%
%\begin{propo}[simple modification of \cite{ji2021unconstrained}]
%Even with imbalances, minimizing CE loss \eqref{eq:CE} converges in direction to a KKT point of the following margin-maximization problem:
%\begin{align}\label{eq:svm_original_implicit_bias}
%\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
%\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
%\end{align}
%\end{propo}
%
%\ct{@Ganesh: check and sketch proof}
%

\subsection{VS-loss}

\begin{propo}[simple modification of \cite{ji2021unconstrained}]
Consider minimizing the VS-loss  
\begin{align}\label{eq:VS}
\Lc(\W,\Hb) = \sum_{i\in[n]} \log\Big(1+\sum_{c\neq y_i}e^{-\Delta_{y_i}(\w_{y_i}-\w_c)^T\h_i}\Big).
\end{align}
Then, gradient descent iterates CE loss \eqref{eq:CE} converges in direction to 
\begin{align}\label{eq:cssvm_original_implicit_bias}
\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\Delta_{y_i}\w_{y_i}-\Delta_c\w_c)^T\h_i \geq 1
\end{align}
\end{propo}

==> sections_arxiv_v2/implicit_bias.tex <==
\ct{@Ganesh: I moved the GD and logit regularization to Appendix, but feel free to reintroduce content in the main body as you see fit. Regarding logit regularization, where would this fit?}
\subsection{SVM solution is not a stationary direction of GD}

Let $\thetab := \vect(\W,\Hb) := [\w_1^T, \ldots, \w_k^T, \h_1^T, \ldots, \h_n^T]^T$ denote the vectorized representation of the embeddings and classifiers. Consider solving the unregularized  problem with gradient descent (GD) updates  $\thetab^{t+1} = \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)$, where $\Lc(\thetab^t):=\Lc(\W^t,\Hb^t)$ is the CE loss  in \eqref{eq:CE}. \cite{lyu2019gradient,ULPM} showed that the updates diverge in norm (i.e. $\|\thetab^t\|_2\rightarrow\infty$), but the normalized iterates $\thetab^t/\|\thetab^t\|_2$ converge to a  KKT point of \eqref{eq:SVM}. Since \eqref{eq:SVM} is nonconvex, it is unclear whether this point is a global optimum. Here, we use Theorem \ref{thm:global}  to show that a global minimizer $\hat\thetab$ of \eqref{eq:SVM} cannot be a converging direction of GD,  when classes are imbalanced. We start by formally defining the notion of a stationary direction below.

\begin{definition}[Stationary direction]
\label{defn:converging}
%We say a direction  $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction  of GD on $\Lc(\thetab)$ if and only if $\nicefrac{\nabla\Lc(\thetab)}{\|\nabla\Lc(\thetab)\|} = \nicefrac{-\thetab}{\|\thetab\|}$. 
We say $\thetab$ defines a stationary direction $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$
of GD on $\Lc(\thetab)$ if there exist constants $\kappa_1,\kappa_2>0$ such that $\nabla_\thetab\Lc(\kappa_1\thetab) = -\kappa_2\thetab$.
\end{definition}
%\gk{I think we have to refine the definition, or add assumptions- whether the relation should hold for all $\thetab$? What if for the same direction, some $\thetab$'s satisfy the condition while others do not?} \ct{Ok. Please  change and let's try to explain what's happening. Would something like the above work? I completed the proof and if I understand what you mean then it seems that the proof doesn't break.}
In words, a direction $\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction if the gradient descent update $\thetab^{+} = \thetab - \eta\nabla\Lc(\thetab)$ preserves this direction, i.e. $\nicefrac{\thetab^+}{\|\thetab^+\|_2}=\nicefrac{\thetab}{\|\thetab\|_2}$ , for any learning rate $\eta > 0$. 
\begin{definition}
	We say that $\nicefrac{\thetab}{\|\thetab\|}$ is a fixed direction under the GD update rule if and only if there exists an iteration $t$ such that $\frac{\thetab^{\tau}}{\|\thetab^{\tau}\|} = \frac{\thetab^{t}}{\|\thetab^{t}\|}, \quad\forall \quad\tau > t$.  \gk{tbd}
\end{definition}
\begin{lemma}
Suppose $\thetab$ is \emph{\underline{not}} a stationary direction of GD on $\Lc(\thetab)$. Then,
 	Under the GD update rule with finite learning rate $\eta >0$, $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is not a fixed direction 
	%\gk{to check if this term is good}
\end{lemma}
\begin{proof}
	Suppose $\thetab^t = \kappa\hat{\thetab}$ for some finite $\kappa >0$. Then, we show that $\thetab^{t+1}$, defined by an update of GD with a finite positive learning rate deviates from the direction $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$. Specifically, we will show that the projection of $\thetab^{t+1}$ onto the orthogonal complement of the subspace spanned by the vector $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is non-zero. Let $\Pbf_{\hat{\thetab}}$ and $\Pbf_{\hat{\thetab}}^\perp$ be the matrices projecting a vector onto $\hat{\thetab}$ and the orthogonal complement of $\hat{\thetab}$, respectively. Then, from the GD update equation we have, 
	\begin{align*}
		\thetab^{t+1} &= \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)\\
		\implies \Pbf_{\hat{\thetab}}^\perp\thetab^{t+1} &= \Pbf_{\hat{\thetab}}^\perp\thetab^t + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\thetab^t)\right)\\
		&= \Pbf_{\hat{\thetab}}^\perp\kappa\hat{\thetab} + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\kappa\hat{\thetab})\right)\\
		&= 0 + \frac{\eta\alpha_\kappa\kappa}{\alpha}\Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|\Pbf_{\hat{\thetab}}(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\right), \quad \text{where}\quad \beta = \frac{\eta\alpha_\kappa\kappa}{\alpha} > 0\\
		&= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\cos^2(\angle -\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &> 0, \quad \because \quad \angle \left(-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab}\right) \neq 0,\quad \text{from Proposition } \ref{propo:negative}.
	\end{align*}
\end{proof}
\gk{above, should we say explicitly that the angle is not 180 degrees either?}



With this definition, we now state the main result of this section. 



%\begin{assumption}\label{ass:align}
%\end{assumption}

\begin{propo}\label{propo:negative}
Assume imbalanced classes and $k>2$. Let $\hat\thetab=\vect(\What,\Hhat)$ be a global minimum of the non-convex SVM in \eqref{eq:SVM}. Then, $\nicefrac{\hat\thetab}{\|\hat\thetab\|}$ is \emph{not} a converging direction of GD on the CE loss.
\end{propo}
%\gk{I think we have to show this for all feasible scalar multiples of $\hat{\thetab}$? Related to how we define the convergence direction}

Proposition \ref{propo:negative} suggests that the KKT point to which GD converges to (in direction), is \emph{not} a global minimum of  \eqref{eq:SVM} when classes are imbalanced.
\footnote{Indeed, this statement can be formalized assuming that the GD path aligns with the gradients. While this statement is non-trivial, it has been proved (at least for $\eta\rightarrow0$) by \cite{} for binary data and we conjecture it to be true even for multiclass data (as already suggested by the results in \cite{}). 
 Specifically assume that $\lim_{t\rightarrow\infty}\inp{{\nbar{\thetab^t}}}{{-{\nbar{\nabla\Lc(\thetab^t)}}}}=1.$ If this is true, then Proposition \ref{propo:negative} and the gradient update rule yields  $\lim_{t\rightarrow\infty}\inp{\nbar{\thetab^t}}{\nicefrac{\hat\thetab}{\|\hat\thetab\|}}\neq1$. \ct{Check this!!!}% For the shake of contradiction assume this was not the case. Then, there exists $t_0$ such that for all $t\geq t_0$, $\|\nbar{\theta^t}-\nicefrac{\hat\thetab}{\|\hat\thetab\|}\|$
}. 
\ct{Also confirmed by our extended experiments in Figures ....} This is in stark to the balanced case, for which \cite{ULPM} showed that GD indeed converges to the global minimum of the non-convex SVM. Thus, \emph{even for a simple two-layer linear NN, it is in general \emph{not} true that GD converges to the global optimum of the corresponding max-margin optimization}. Specifically, while such a statement is always true for binary data as shown  by \cite{}, and for balanced multiclass data as shown by \cite{}, it fails for imbalanced multiclass data. 

\begin{remark} 
\ct{Check:}The proposition shows that the SVM solution is \emph{not} a converging direction of GD. From this, we can conclude that GD does not converge in that direction. On the other hand, note that showing a point $\thetab$ is a converging direction does \emph{not} imply that first-order methods necessariy converge in the direction of $\thetab$. This is because there might be a descending direction tangential to $\thetab$ (see for example \ref{unconstrained feature paper}).
\end{remark}



\paragraph{Proof.}
First, for arbitrary $\thetab$, denote the negative gradient of the CE loss as
	\begin{align}
		\g &:= -\nabla_\thetab\Lc(\thetab) = \sum_{i\in[n]}\sum_{c\neq y_i}\frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}\,\g_{i,c}\,,
	\end{align}
	where we denote the margins $s_{i,c} = (\w_{y_i}-\w_{c})^T\h_{i}$, and also, $\g_{i,c} = \nabla_\thetab s_{i,c}$. Specifically, using the shorthand $\alpha_{i,c} := \frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}$, we get $\g = \sum_{i\in[n]}\sum_{c\neq y_i}\alpha_{i,c}\g_{i,c}$. Here, note that $\g, \g_{i,c}, s_{i,c}$ are all functions of $\thetab$, but we suppress notation when clear from context.
	
Now, consider specific $\thetab = \kappa\hat{\thetab}$, where $\hat\thetab=\vect(\What,\Hhat)$, a global minimum of the non-convex SVM, and $\kappa >0$. From Theorem \ref{thm:global}\ref{thm:global_logits}, we know that $\hat\w_c^T\hat\h_i=\hat{z}_{ic}$ as defined in \eqref{eq:simplex}. Hence, the corresponding margins satisfy
\begin{align}
\forall i\in[n], c\neq y_i\,:\, s_{i,c}(\kappa\hat\thetab)=(\kappa\hat\w_{y_i}-\kappa\hat\w_{c})^T\kappa\hat\h_{i}=\kappa^2 \implies \alpha_{i,c}(\kappa\hat\thetab)=\alpha_\kappa>0,
\end{align}
Hence, $\g(\kappa\hat\thetab) = \alpha_\kappa\sum_{i\in[n]}\sum_{c\neq y_i}\g_{i,c}(\kappa\hat\thetab)$. In particular, evaluating $\g_{i,c}(\kappa\hat\thetab)=\nabla_\thetab s_{i,c}(\kappa\hat{\thetab})$ it follows that
\begin{subequations}\label{eq:grads_1}
	\begin{align}
\forall c \in [k]\,:\,~		-\nabla_{\w_{c}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\sum_{i: y_i=c}\hat\h_{i}-\sum_{i\in [n]}\hat\h_{i})\\
\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\hat\w_{y_i}-\sum_{c\in[k]}\hat\w_{c}).
	\end{align}
\end{subequations}
We now compute the angle between $\thetab = \kappa\hat{\thetab}$ and $-\nabla_{{\thetab}}\Lc(\kappa\hat{\thetab})$.
%\noindent\textbf{Angle between parameter and gradient:}
It can be checked that the gradient at $\kappa\hat{\thetab}$ is related to the gradient at $\hat{\thetab}$ as follows:
\begin{align*}
	\forall c \in [K]\,:\,~	 \nabla_{\w_{c}}\Lc(\kappa\hat{\thetab}) &=  -\alpha_\kappa\kappa^2\left(Kn_c\hat{\h_c}-\sum_{c}n_{c'}\hat{\h_{c'}}\right) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\w_{c}}\Lc(\hat{\thetab})\\
	\forall i \in [n]\,:\,~	
	\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab}) &= \alpha_\kappa\kappa^2K\hat{\w_{y_i}} =\frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\h_{i}}\Lc(\hat{\thetab})
\end{align*}	
where we used the following facts from Theorem \ref{thm:global} and $\alpha = \frac{\exp(-1)}{\left(1+(K-1)\exp(-1)\right)}$.
\begin{itemize}
	\item $\hat{\h}_{i} = \hat{\h}_{j}$ if $y_i = y_j$; denote $\hat{\h}_{i}$ by  $\hat{\h}_{c}$ when $y_i = c$
	\item $\sum_{c}\hat{\w}_c = 0$
\end{itemize}
Therefore, we get
$$\nabla_\thetab\Lc(\kappa\hat{\thetab}) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{{\thetab}}\Lc(\hat{\thetab}),
$$
Now, computing the inner products,
\begin{align*}
	-\nabla_{\w_{c}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2\left((K-1)n_c\hat{\h}_c^T\hat{\w}_{c}-\sum_{c'\neq c}n_{c'}\hat{\h}_{c'}^T\hat{\w}_{c}\right)\\
	&= \alpha_\kappa\kappa^2\left[(K-1)n_c\frac{K-1}{K}+\frac{n-n_c}{K}\right]\\
	&= \frac{\alpha_\kappa\kappa^2}{K}\left[\left((K-1)^2-1\right)n_c+n\right]\\
	-\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2K\hat{\w}_{y_i}^T\h_{i}\\
	&= \alpha_\kappa\kappa^2(K-1)
\end{align*}
Combining in $\thetab$ notation, we have
\begin{align*}
	-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab} &= \alpha_\kappa\kappa^2\left[n(K-1)+n\frac{(K-1)^2-1}{K}+n\right]\\
	&= \frac{\alpha_\kappa\kappa^2n}{K}(2K^2-2K)\\
	&= 2\alpha_\kappa\kappa^2n(K-1)
\end{align*}
Thus, we get the following for the cosine of the angle between the parameter and negative gradient at $\kappa\hat{\thetab}$:
\begin{align*}
	\cos(\angle -\nabla_\thetab\Lc(\kappa\hat{\thetab}),\kappa\hat{\thetab}) &= \frac{-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab}}{\|-\nabla_\thetab\Lc(\kappa\hat{\thetab})\|\kappa\hat{\thetab}\|}\\
	&= \frac{2\alpha_\kappa\kappa^2n(K-1)}{\frac{\alpha_\kappa\kappa^2}{\alpha}\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|}\\
	&= \frac{2n\alpha(K-1)}{\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|},
\end{align*}
which is independent of $\kappa$. This means that the angle between $\thetab$ and the negative gradient anywhere along the direction of $\hat{\thetab}$ remains a constant, irrespective of the magnitude of $\thetab$. Therefore, we can simplify the definition \ref{defn:converging} for $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ to be a stationary direction as there exists a $\gamma >0$ such that $\nabla\Lc(\hat{\thetab}) = -\gamma\hat{\thetab}$.
  


Next, suppose for the sake of contradiction that $\hat\thetab$ is a converging direction of GD. Following this (see Definition \ref{defn:converging}) and Equations \eqref{eq:grads_1}, there must exist $\kappa>0$ such that
\begin{subequations}\label{eq:grads_2}
	\begin{align}
\forall c \in [k]\,:\,~			-\nabla_{\w_{c}}\Lc(\hat\thetab) &= \alpha(k\sum_{i: y_i=c}\h_{i}-\sum_{i\in [N]}\h_{i}) = \gamma \w_{c} \label{eq:unreg_ce_grad_w_2}\\
	\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\hat\thetab) &= \alpha(K\w_{y_i}-\sum_{c\in[k]}\w_{c}) = \gamma\h_{i}\label{eq:unreg_ce_grad_h_2}\,.
	\end{align}
\end{subequations}
Also, from Theorem \ref{thm:global}\ref{thm:global_W} and the fact that $\Zhat^T\ones_k =0$, we have that
$
\sum_{c\in[k]}\w_c=\What\ones_k = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\ones_k = 0 \footnote{In fact, this property can alternatively be deduces from \eqref{eq:unreg_ce_grad_w_2} by summing for all $c\in[k].$}.
$ Therefore, \eqref{eq:unreg_ce_grad_h_2} gives
	\begin{align}
	\forall i \in [n]\,:\,~	\alpha(k\hat\w_{y_i}) = \gamma\hat\h_{i}
		\implies   \hat\h_{i}=\gamma'\hat\w_{y_i}=\gamma'\What\y_i \nn,
	\end{align}
	for some constant $\gamma'>0$ and one-hot encoding vector $\y_i=\eb_{y_i}.$ 
	Therefore, letting $\Y=[\y_1,\ldots,\y_n]_{k\times n}$ be the one-hot label matrix, we conclude that 
\begin{align*}
	\Hhat^T\Hhat=\gamma'\Hhat^T\What\Y &\implies (\Zhat^T\Zhat)^{1/2}=\gamma'\Zhat^T\Y,
	\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\Y\Y^T\Zhat,
		\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\diag(n_1,n_2,\ldots,n_k)\Zhat,
	\\
	&\implies \Zhat^T\big(\Id_k - (\gamma')^2\diag(n_1,n_2,\ldots,n_k)\big)\Zhat=\zeromat_{n\times n},
	\\
	&\implies \Zhat^T\diag({1-(\gamma')^2{n_1}},{1-(\gamma')^2{n_2}},\ldots,{1-(\gamma')^2{n_k}})\Z=\zeromat_{n\times n},
\end{align*}
where, the first implication follows by Theorem \ref{thm:global}\ref{thm:global_logits} and \ref{thm:global_gram}. Denote for convenience $\delta_{c}=1-(\gamma')^2{n_c}, c\in[k]$ and $\Delta=\sum_{c\in[k]}\delta_c.$ Then, from the last line above, it must be that
\begin{align*}
	&\forall i\in[n]\,:\, \Big(1-\frac{1}{k}\Big)^2\delta_{y_i}^2+\frac{1}{k^2}\sum_{c\neq y_i}^k\delta_c^2 =0 \implies \big(k-1\big)^2\delta_{y_i}^2+(\Delta-\delta_{y_i}^2) = 0
	\\
		\implies &\forall c\in[k]\,:\, \big(k-1\big)^2\delta_{c}^2+(\Delta-\delta_{c}^2) = 0 		\implies k(k-2)\delta_{c}^2=-\Delta.
			\\
			\stackrel{k>2}{\implies} 
			&\forall c\in[k]\,:\,\delta_{c}^2=-\Delta \implies \delta_{1}=\delta_2=\ldots\delta_k \implies n_1=n_2=\ldots=n_k=n/k.
%		&\implies \forall i\in[n]\,:\, \big(k-1\big)^2(1-(\kappa')^2{n_{y_i}})=\sum_{c\neq y_i}^k (1-(\kappa')^2{n_c}) = k - (\kappa')^2(n-n_{y_i}) ,
%			\\
%		&\implies \forall i\in[n]\,:\,  (\kappa')^2\big((k-1)^2+1\big)n_{y_i} = (k-1)^2 - k +n
\end{align*}
But data were assumed imbalanced, so we arrived at a contradiction completing the proof. Note also that in the last line, we used the assumption $k>2$.

%We now note that, along the direction of the SVM solution $\hat{\thetab}$ it is sufficient to consider the following simplified definition of converging direction \ref{defn:converging}: We say $\hat{\thetab}$ defines a stationary direction $\nbar{\hat{\thetab}}=\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$
%of GD on $\Lc(\thetab)$ if and only if there exists a constant $\kappa_3>0$ such that $\nabla\Lc(\hat{\thetab}) = -\kappa_3\hat{\thetab}$, which is used in the proof of Proposition \ref{propo:negative}
%This is due to the fact that $\nabla_\thetab\Lc(\kappa_1\hat{\thetab}) = \nicefrac{\alpha'\kappa_1}{\alpha}\nabla_\thetab\Lc(\hat{\thetab})$, where $\alpha' = \frac{\exp(-\kappa_1^2)}{1+(K-1)\exp(-\kappa_1^2)}$ which is described in the discussion below. The observation further shows that the angle between $\kappa_1\hat{\thetab}$ and $-\nabla_{\thetab}\Lc(\kappa_1\hat\thetab)$ is independent of $\kappa_1$.

%\gk{Plots of angle as functions of R, K etc} 
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm}
%		\caption{as a function of $R$}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm2}
%		\caption{Lorem ipsum}
	\end{subfigure}
	\caption{$\cos\left(\angle (-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)$ plotted against $R$ and $K$ respectively, with step imbalance on data. Note that the angle remains zero when $K=2$ or when $R=1$.}
\end{figure*}
%
%$$
%\forall c\in[k]\,,\, 1-(\kappa')^2{n_c} = 0 \implies n_1=n_2=\ldots=n_k.
%$$
%This contradicts our assumption that the dataset is imbalanced, completing the proof.


	%That is $\forall i\,:\, y_i=c$ the optimal feature $\hat\h_i$ aligns with the classifier $\hat\w_c$ of the corresponding class. 
	
	
%	Fix $i\in[n]$. Then from the display above and Theorem \ref{thm:global}\ref{thm:global_W},   
%	\begin{align}
%	\kappa'\hat\h_i = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}
%	Combining with Theorem \ref{thm:global}\ref{thm:global_Gram} (i.e. $\Hhat^T\Hhat=(\Zhat^T\Zhat)^{1/2}$), we conclude that
%	\begin{align}
%	\kappa'\Hhat^T\Hhat = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}	
	
	
%	But again from Theorem \ref{thm:global}\ref{thm:global_W} 
%$\w_c=\What\eb_c = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_c
%$

%	From \eqref{eq:h_opt} we have the relation between $\h_{i}^*$ and $\w_{y_i}^*$:
%	\begin{align*}
%		\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
%	\end{align*} 
%\gk{TBC}\ct{Need that $\w_{y_i}$ not aligned with $\h_i$.}



==> sections_arxiv_v2/lower_bound_proof_details.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
 For $c\in[k]$, let $\mathcal{C}_c = \{i: y_i = c\}$ be the set of examples belonging to class $c$, and define $\Lc_i(\Hb)$ as follows,
\begin{align}\label{eq:L_i}
  \Lc_i(\Hb) &= \sum_{{j\in\mathcal{C}_{y_i},j\neq i}}
  \log\Big(\sum_{{\ell\in[n],\ell\neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\Big)\nn\\
     &= \sum_{{j\in\mathcal{C}_{y_i},j\neq i}}\log\Big(\sum_{\ell\in\mathcal{C}_{y_i}, \ell\neq i}\exp{(\h_i^\top\h_\ell - \h_i^\top\h_j)}+\sum_{\ell\not\in \mathcal{C}_{y_i}}\exp{(\h_i^\top\h_\ell - \h_i^\top\h_j)}\Big).
\end{align}
Then, we can rewrite the full-batch SCL in \eqref{eq:SCL_full} as, 
\begin{align*}
    \Lc_\text{full}(\Hb)&= \sum_{i\in[n]}\frac{1}{n_{y_i}-1} \Lc_i(\Hb) = \sum_{c \in [k]}\frac{1}{n_{c}-1} \sum_{i\in\mathcal{C}_c}\Lc_i(\Hb).
\end{align*}
 Now for $c\in[k]$, consider example $i\in\mathcal{C}_c$, and define $$\mathbf{a}_i := \frac{1}{n_c-1}\sum_{\ell\in\mathcal{C}_{c}, \ell\neq i}
\h_\ell, \quad \mathbf{b}_i := \frac{1}{n - n_c}\sum_{\ell\not\in\mathcal{C}_{c}}
\h_\ell.$$ 
Note $\mathbf{a}_i$ is the mean-embedding of all examples in class $c$ but $i$, and $\mathbf{b}_i$ is the mean-embedding of all examples not in class $c$. Starting from \eqref{eq:L_i}, by applying Jensen's inequality to the strictly convex function $f_1(x) := \exp(x - \h_i^\top\h_j)$ we have,
 % 
 % Since $\forall i,j\in[n]$, $f(x) := \exp(x - \h_i^\top\h_j)$ is a strictly convex function, by applying Jensen's inequality to \eqref{eq:L_i}, we have,
 \begin{align}\label{eq:jensen_1}
 \Lc_i(\Hb) 
 % &= \sum_{{j\in\mathcal{C}_{c},j\neq i}}\log\Big(\sum_{\ell\in\mathcal{C}_{c}, \ell\neq i}\exp{(\h_i^\top\h_\ell - \h_i^\top\h_j)}+\sum_{\ell\not\in \mathcal{C}_{c}}\exp{(\h_i^\top\h_\ell - \h_i^\top\h_j)}\Big)\nn\\
 %%%%%%%%%
 &\geq \sum_{{j\in\mathcal{C}_{c},j\neq i}}\log\Big( (n_c-1) \exp{(\h_i^\top\mathbf{a}_i - \h_i^\top\h_j)}  +  (n-n_c) \exp{(\h_i^\top\mathbf{b}_i - \h_i^\top\h_j)}\Big)\nn\\
 % 
&=\sum_{{j\in\mathcal{C}_{c},j\neq i}}\log\Big( \big((n_c-1)\exp{(\h_i^\top\mathbf{a}_i)}  +  (n-n_c) \exp{(\h_i^\top\mathbf{b}_i})\big) \exp{(- \h_i^\top\h_j)}\Big)\nn\\
&\stackrel{(i)}{=}\sum_{{j\in\mathcal{C}_{c},j\neq i}}\log\Big(\alpha_i \exp{(- \h_i^\top\h_j)}\Big)\nn\\
&\stackrel{(ii)}{=}(n_c-1)\log\Big(\alpha_i \exp{(- \h_i^\top(\frac{1}{n_c-1}\sum_{{j\in\mathcal{C}_{c},j\neq i}}\h_j))}\Big)\nn\\
&= (n_c-1)\log(\alpha_i \exp(-\h_i^\top\mathbf{a}_i))\nn\\
&= (n_c-1)\log\Big((n_c-1) + (n-n_c)\exp\big(\frac{1}{n-n_c}\h_i^\top \sum_{\ell \not\in \mathcal{C}_c} \h_\ell - \frac{1}{n_c-1} \h_i^\top \sum_{\ell \in \mathcal{C}_c, \ell\neq i} \h_\ell\big)\Big),
 \end{align}
 where in $(i)$, we define $\alpha_i := (n_c-1)\exp{(\h_i^\top\mathbf{a}_i)}  +  (n-n_c) \exp{(\h_i^\top\mathbf{b}_i})$, and in $(ii),$ we use the fact that the function $f_2(x):=\log(\alpha_i\exp(x))$ is an affine function. Now consider all samples $i\in\mathcal{C}_c$. From \eqref{eq:jensen_1}, \begin{align}\label{eq:Jensen_L_i}
 \frac{1}{n_c-1}\sum_{i\in\mathcal{C}_c} &\Lc_i(\Hb) \geq \sum_{i\in\mathcal{C}_c} \log\Big((n_c-1) + (n-n_c)\exp\big(\frac{1}{n-n_c}\h_i^\top \sum_{\ell \not\in \mathcal{C}_c} \h_\ell - \frac{1}{n_c-1} \h_i^\top \sum_{\ell \in \mathcal{C}_c, \ell\neq i} \h_\ell\big)\Big)\nn\\
 %
 &\geq n_c\log\Big((n_c-1) + (n-n_c)\exp\big(\frac{1}{n_c(n-n_c)} \sum_{\substack{i\in\mathcal{C}_c \\ \ell \not\in \mathcal{C}_c}} \h_i^\top \h_\ell - \frac{1}{n_c(n_c-1)} \sum_{\substack{i\in\mathcal{C}_c \\ \ell \in \mathcal{C}_c, \ell\neq i}} \h_i^\top \h_\ell\big)\Big).
 \end{align}
 In the last line we use Jensen's inequality on  $f_3(x):=\log((n_c-1)+(n-n_c)\exp(x))$ which is strictly convex since 
 $n_c>1$ and $n-n_c>0$. 

 By the ReLU constraints we have $\h_i \geq 0,\, i\in[n]$, which implies $\h_i^\top\h_j\geq 0,\,\forall i,j\in[n]$. Further, by Cauchy-Schwarz inequality $\h_i^\top\h_j \leq \norm{\h_i}\norm{\h_j}=1$, with equality achieved if and only if $\h_i=\h_j$. Since $f_3$ is non-decreasing, we can simplify the bound in \eqref{eq:Jensen_L_i} as follows,
 \begin{align}\label{eq:cauchy}
     \frac{1}{n_c-1}\sum_{i\in\mathcal{C}_c} &\Lc_i(\Hb) \geq n_c\log\Big((n_c-1) + (n-n_c)e^{- 1}\Big).
 \end{align}
 Summing over all classes $c\in[k]$, we get the final bound on the full-batch SCL:
\begin{align*}
    \Lc_\text{full}(\Hb) = \sum_{c\in[k]}\frac{1}{n_c-1}\sum_{i\in\mathcal{C}_c} \Lc_i(\Hb) \geq \sum_{c\in[k]} n_c\log\Big((n_c-1) + (n-n_c)e^{- 1}\Big).
\end{align*}
To achieve the lower-bound, from \eqref{eq:cauchy}, we require $\h_i=\h_j$ if $y_i=y_j$ and $\h_i^\top\h_j=0$ otherwise. This requirement also satisfies the equality condition for the Jensen inequalities applied in \eqref{eq:jensen_1} and \eqref{eq:Jensen_L_i}. Thus, any $\Hb$ achieving the lower-bound follows an OF geometry (Def.~\ref{def:ncof}), which exists as long as $d\geq k$. 

% \gk{sounds like only one $\Hb$, needs rewording} \tina{@GK: changed 'the only' to 'any' :D Sounds better now?}

% \tina{double check for details}

% \ct{Is there an ``easy'' way to show that the UFM solution is not an ETF when data are balanced?}

==> sections_arxiv_v2/num_results.tex <==
% Structure: 
% \begin{itemize}
%     \item 3 datasets, exp + step for Resnet discuss convergence to OF 
%     \item Ganesh's proof + discussion with ReLU, without ReLU (graf) 
%     \item Lowerbound full batch to loss convergence 
%     \item GM plots here CE vs SCL 
%     \item Ganesh's batch argument 
%     \item regular batch vs Vala - Batch experiments, discussion of larger batchsizes (small batch with same examples vs large batches...) 
%     \item Test accuracy Augmentation vs Augmentation and vala batch, VS Loss, CE comparison 
%     \item Consider including other models if vala batching helps, consider other sampling 
%     \item relu last layer vs whole architecture relu 
%     \item wSCL (not that promising), any UFM results 
% \end{itemize}






\gk{is this section for anything in particular?}

==> sections_arxiv_v2/outlook.tex <==
%\vspace{-0.25cm}
We propose \emph{\ref{SELI}} as the class-imbalance-invariant geometry of classifiers and embeddings learnt by overparameterized models when trained beyond zero training error. We arrive at it after showing that the UF-SVM global minimizers follow this geometry. Subsequently, we conjecture that: (C1) GD on the UFM leads to solutions approaching the SELI geometry asymptotically in the number of epochs; (C2) training of deep-nets beyond zero training error learns models that approach the SELI geometry. 

Statement (C1) is a conjecture and does not follow from Theorem~\ref{thm:SVM}. This is because GD is only known to converge to KKT points of the non-convex UF-SVM \cite{lyu2019gradient,ULPM}, which are not necessarily global minima.  Thus, while Proposition~\ref{propo:reg_path} combined with the benign landscape of the corresponding ridge-regularized minimization, as well as, our experiments suggest its validity, the conjecture remains to be further investigated.\footnote{Relying on \citep{ji2020directional}, \citet{vardi2021margin} showed gradient flow  finds global minimizers in deep linear nets. However, these only apply to binary classification. We show that interesting behaviors might occur (e.g. in the role of regularization and geometry) when $k>2$ and $R>1$ calling  further studies.} We also note that convergence rates appear slower with increasing imbalance levels; a feature which is interesting to study further. 

Regarding conjecture (C2), we deem our experiments encouraging: the classifiers' and embeddings' geometries get closer to the SELI geometry as neural-network training progresses. Specifically, the Gram matrices $\G_\W$ and $\G_\Hb$ of the classifiers and embeddings, respectively, align increasingly better with their SELI counterparts $\Vb\Lambdab\Vb^T$ and $\Ub\Lambdab\Ub^T$; see Fig.~\ref{fig:}. Also, Fig. \ref{fig:} shows that Lemma \ref{lem:} is able to make predictions regarding the norms of majorities versus minorities. We note that, similar to the UFM experiments, convergence appears slower for larger imbalance ratios. Also, we observe better convergence for classifiers compared to embeddings \ct{and for norm predictions compared to angle predictions}. Overall, we hope our results motivate further experimental investigations, especially since data imbalances appear frequently across applications. 
 %\new{In our experiments, we use optimization-parameter choices (e.g. learning rate, weight-decay, momentum) that are consistent with previous works in the literature.} 

 Beyond that, we believe that further similar studies on identifying geometrical structures of learned embeddings and classifiers could offer new perspectives on generalization. For example, our results could pave that way since they uncover different geometries (aka SELI for different $R$ values), each leading to different generalization (worse for increasing $R$ \cite{byrd2019effect}). %On one hand, CE on balanced data leads to ETF geometry, and, is known to generalize well. On the other hand, CE on imbalanced data changes the geometry, and, is known to achieve poor generalization  in terms of (say) balanced error \cite{byrd2019effect}. since having access to different geometries  each leading to different generalization might help uncovering connections between train geometries and generalization. 
 Relatedly, we envision that further such studies lead to algorithmic contributions in deep imbalanced learning as they can facilitate studying the implicit bias effect of CE adjustments and post-hoc techniques tailored to imbalanced data \cite{TengyuMa,Menon,CDT,KimKim,kang2020decoupling,ganesh,autobalance}.


\ct{
Future work:
\begin{itemize}
\item general imbalance (beyond step)
\item other losses, e.g. square loss?
\end{itemize}
}

%\paragraph{Rethinking implicit bias: Imbalance trouble}  \ct{needs rewriting}A series of works that examine the implicit bias of gradient descent (and of its variants, such as stochastic GD, gradient flow, etc.) yield characterizations of the preferred minimizer that roughly take the following format: the model weights found by GD converge to a KKT point of an optimization program that minimizes a certain norm of the weights subject to an interpolation constraint. In the simplest and cleanest setting of a linear model trained with either square-loss or cross-entropy, the resulting optimization is convex and minimizes the $\ell_2$ norm of the weights subject to either an interpolation constraint or a linear separability constraint \cite{}. For example, GD on cross-entropy loss in a linear setting converges (in direction) to the max-margin classifier \cite{}. We note that in general nonlinear settings, the norm that is minimized can depend on the model architecture \cite{}. Perhaps more importantly, beyond the linear setting, the resulting optimization program is non-convex. This naturally raises the question of whether the KKT point preferred by GD is a global minimizer. Our first finding shows that the answer is in general negative even in the simplest setting beyond the standard linear model, that of a 2-layer linear network:
% 
%\begin{finding}
%Consider training of a 2-layer linear network with gradient flow (GF) on cross-entropy (CE) loss without explicit regularization. There exists multiclass imbalanced dataset such that the global minimizer of the (non-convex) max-margin optimization is \emph{not} a convergence direction of GF.
%\end{finding}
%\begin{figure}[ht!]
%	\centering
%	\includegraphics[width=\linewidth]{Figures/G_errors_CE}
%\end{figure}
%\ct{@Ganesh: One plot -two curves. One for balanced. one for imbalanced. distance to G cvx (which corresponds to global optimum) over epochs. In the LPM model.}


%We believe these questions are important since data imbalances appear more frequently, than not, across applications \cite{}. Beyond that, answering these questions might offer a new perspective in better understanding potential connections of NC to generalization. On the one hand, CE entropy on balanced data leads to the symmetric geometry characterized by NC1--3, and also, it is known to achieve good generalization. On the other hand, as we will see, the presence of imbalances drastically changes the geometry, and also, it is known to achieve poor generalization, measured in terms of (say) balanced error \cite{}. Having access to different geometries that each leads to different generalization levels might shed light in understand wether a connection between NC and generalization can be formalized. Relatedly, we envision that our study leads to algorithmic contributions in imbalanced learning with overparameterized models as it can be used to study changes to NC geometry when training with losses other than CE that are tailored to imbalanced data.

==> sections_arxiv_v2/proof_thm2.tex <==
% \tina{small detail: should I add the previous section inside a proof environment or should we remove it here?}\ct{No need for proof environment when the entire section is the proof}

    Consider the mini-batch SCL in \eqref{eq:scl_batch}, repeated below for convenience:
 \begin{align*}
     \Lc_{\text{batch}}(\Hb):=\sum_{B \in \mathcal{B}}\sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\bigg(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\bigg),
 \end{align*}
 Denoting the loss over a batch $B$ by 
 \begin{align*}
     \Lc_{B}(\Hb) := \sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\bigg(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\bigg),
 \end{align*}
 we have $\Lc_{\text{batch}}(\Hb)=\sum_{B \in \mathcal{B}}\Lc_{B}(\Hb)$.
 Now, for a given batch $B$, we apply Thm.~\ref{thm:scl_full} to get the lower bound and conditions for equality:
 \begin{align*}
      \Lc_B(\Hb) \geq \sum_{c \in [k]}n_{B,c}\log\left(n_{B,c}-1+(n_{B}-n_{B,c})e^{-1}\right).
  \end{align*}
  Moreover, equality holds if and only if for every pair of samples $i,j\in B$: $\h_i^\top\h_j=0$ if $y_i\neq y_j$ and $\h_i=\h_j$ if $y_i=y_j$. With this, the overall loss can be bounded from below by summing the individual lower bounds over different batches:
  \begin{align*}
      \Lc_\text{{batch}}(\Hb) \geq \sum_{B \in \mathcal{B}}\sum_{c \in [k]}n_{B,c}\log\left(n_{B,c}-1+(n_{B}-n_{B,c})e^{-1}\right),
  \end{align*}
  with equality achieved if and only if for every $B\in\mathcal{B}$ and every pair of samples $i,j\in B$, $\h_i^\top\h_j=0$ if $y_i\neq y_j$ and $\h_i=\h_j$ if $y_i=y_j$. As long as $d \geq k$, the equality conditions of every individual batch can be satisfied simultaneously.



\subsection{Proof of Cor.~\ref{cor:batch}}
% \new{As seen from the motivating example in Sec.~\ref{sec:mini_batch_theory}, the equality conditions in Thm.~\ref{thm:scl_mini} can be satisfied by many configurations for an arbitrary batching scheme. In Cor.~\ref{cor:batch}, we define the requirements of a batching scheme in order for the global optimal of the mini-batch SCL to be unique (up to global rotations), and match the optimal of the full-batch SCL. }

% \new{From the proof of Thm.~\ref{thm:scl_mini}, the conditions for equality for the overall problem depend on how individual batch conditions interact with each other. We prove the :}
% \begin{itemize}
%     \item \new{\textit{similar examples:} we know that at equality, within every batch $B$, for every pair of similar examples (aka belonging to the same class), $i,j \in B, y_i = y_j$, $\h_i = \h_j$. Consider another batch $B^\prime$. In the same way, for equality, we have that for every pair $l,m \in B^\prime$, $\h_l = \h_m$. }
    
%     \new{If for some $c \in [k]$, $\{i \in B: y_i = c\}  \cap \{i \in B^\prime: y_i = c\} \neq \phi$, let $u \in B\cap B^\prime: y_u = c$, then the equality conditions for both the batches imply that $\h_i = \h_u = \h_l, \forall i \in B:y_i = c, \forall l \in B^\prime: y_l = c$. Extending the argument to all mini-batches, in terms of our definition of the Batch Interaction Graph (\ref{def:big}), we have that the induced sub-graph $G_c$ is connected.}
    
%     \new{On the other hand, cf for a $c \in [k]$, $\{i \in B: y_i = c\}  \cap \{i \in B^\prime: y_i = c\} = \phi$, then the equality of embeddings belonging to the two batches is not guaranteed, even if their labels are equal. This occurs when $G_c$ is not connected.}
%     \item \new{\textit{contrasting examples:} Similar to the equality conditions, we now consider the interaction of examples from two different classes. If there is at least one batch, say $B$, there exist at least one example each from classes $c$ and $c^\prime$, respectively, the batch-wise equality conditions from Thm.~\ref{thm:scl_mini} state that $\h_u \perp \h_v$, where $y_u = c, y_c = c^\prime$. In terms of the graph notation, this occurs when $G_c$ and $G_{c^\prime}$ are connected. }
    
%     \new{However, if no such batch exists for the pair of classes $c$ and $c^\prime$, then the orthogonality of embeddings from these two classes is not guaranteed. In terms of the graph notation, this occurs when $G_c$ and $G_{c^\prime}$ are not connected.}
% \end{itemize}

% Therefore, the global minimizer will be uniquely an OF if and only if the batching scheme satisfies both the conditions stated above.


% ************************
% \todo{another option}********

{From Thm.~\ref{thm:scl_mini}, the optimal configuration of embeddings in \ref{eq:SCL_UFM_full} under the mini-batch SCL depends on how batch conditions interact with each other. Specifically, recall that the equality in \eqref{eq:scl_mini_lb} is achieved if and only if for any batch $B\in\mathcal{B}$, and each pair of samples $(i,j)\in B$, $\h_i=\h_j$ if $y_i=y_j$, and $\h_i^\top\h_j = 0$ otherwise. The OF geometry clearly satisfies all these conditions and achieves the minimal cost of \ref{eq:SCL_UFM_full}. However, as discussed in Sec.~\ref{sec:mini_batch_theory}, these equality conditions may be satisfied by configurations other than OF for an arbitrary batching scheme. So, in Cor.~\ref{cor:batch}, we specify the requirements of a batching scheme in order for the global optimal of the mini-batch SCL to be unique (up to global rotations), and match the optimal of the full-batch SCL, which is the OF geometry. }

% {As discussed in Sec.~\ref{sec:mini_batch_theory}, the equality conditions of Thm.~\ref{thm:scl_mini} may be satisfied by configurations other than OF for an arbitrary batching scheme. In Cor.~\ref{cor:batch}, we define the requirements of a batching scheme in order for the global optimal of the mini-batch SCL to be unique (up to global rotations), and match the optimal of the full-batch SCL, which is the OF geometry. }
% 
% 
% From proof of Thm.~\ref{thm:scl_mini}, the conditions for equality for the overall problem depend on how individual batch conditions interact with each other. 
To prove the corollary, we separately address the `IF' and `ONLY IF' parts of the  Cor.~\ref{cor:batch}. 
% We prove {separately the `IF' and `ONLY IF' parts of the } Cor.~\ref{cor:batch}.




\noindent$\bullet$~\textbf{`IF' direction.}~{Assume the batching scheme satisfies both conditions of Cor.~\ref{cor:batch}: {1) $\forall c\in[k]$, the induced subgraph $G_c$ is connected, and 2) $\forall c\neq c'\in[k]$, there exists an edge between $G_c$ and $G_{c'}$.} We show below that under these two conditions the optimum of \ref{eq:SCL_UFM_full} under mini-batch SCL follows an OF geometry. {In other words, we show that the optimal embeddings align if they belong to the same class (NC) and are orthogonal if they have different labels (mean-embeddings follow k-OF). (See Def.~\ref{def:ncof}.)}}

   {%\textit{Similar examples:} 
   \textit{{NC:}} Consider a class $c$. From our assumption, the induced subgraph $G_c$ is connected. Thus, a path exists from any node (representing corresponding example) to any other node in $G_c$. 
   %\new{If $G_c$ contains only two nodes, say $i,j$, then by Definition \ref{def:big} of the Batch Interaction Graph, both are present in the same batch, say $B_1$. Thus, from Thm.~\ref{thm:scl_mini}, we can infer that at the optimal solution, we have $\h_i = \h_j$, due to equality conditions for batch $B_1$. Thus, suppose in the following that the graph has at least}
   Consider three nodes\footnote{{The same arguments and considerations apply when $G_c$ consists of only two nodes.}} along a path, indexed by $i,j,l$ that belong to class $c$. Let there be an edge between $i,j$ and $j,l$ each. By Def.~\ref{def:big} of the Batch Interaction Graph, examples $i$ and $j$ are present in a batch, say $B_1$, and examples $j,l$ belong to a batch $B_2$ that is possibly different from $B_1$. From Thm.~\ref{thm:scl_mini}, we can infer that at the optimal solution, we have $\h_i = \h_j$, due to equality conditions for batch $B_1$. Also, $\h_j = \h_l$, due to equality conditions for batch $B_2$. Thus, by transitivity, we have $\h_i = \h_j = \h_l$. Repeating this argument along any path in $G_c$ for every $c \in [k]$, we obtain the NC property: $\h_i = \h_j, \forall i,j:y_i = y_j=c$ for every class $c \in [k]$.}
    
    %\textit{Contrasting examples:} 
    \textit{$k$-OF:} From our assumption, for any pair of classes $c_1$ and $c_2$, there exists an edge between $G_{c_1}$ and $G_{c_2}$ {connecting}
    %at 
    at least one pair of nodes $i,j: i\in G_{c_1}, j \in G_{c_2}$. By definition of the Batch Interaction Graph, we know that examples $i$ and $j$ belong in at least one batch. {Thus,} by Thm.~\ref{thm:scl_mini}, at the optimal solution, we have $\h_i \perp \h_j$ since examples $y_i=c_1\neq c_2=y_j$. Now, {by NC,  $\h_i=\mub_{c_1}$, $\h_j=\mub_{c_2}$, and thus, $\mub_{c_1}\perp \mub_{c_2}$. This holds for every pair of classes $c_1\neq c_2 \in [k]$. Therefore, the matrix $\M=[\mub_1,...,\mub_k]$ of class-mean embeddings forms a $k-$OF.}
     
    % along with the argument about \emph{similar examples} in the previous paragraph and repeating for every pair of classes, we can deduce that $\h_i \perp \h_j, \forall i \in c_1, j\in c_2$. 
    

    {Combining the two statements above, we conclude that at the global optimal solution, the embeddings follow the OF geometry, as desired.}


\noindent$\bullet$~\textbf{`ONLY IF' direction.} For the other direction, it suffices to show that if either of the two conditions in Cor.~\ref{cor:batch} does not hold, then there exists an optimizer that does not follow the OF geometry. 
Specifically, we show that when either of the two conditions is violated {and $d\geq k+1$}, there exists an embeddings matrix $\widetilde{\Hb}$ attaining the loss lower-bound that does not satisfy one of the two requirements of the OF geometry: 1) $\widetilde{\Hb}$ does not follow NC, or 2) the corresponding mean-embeddings $\widetilde{\M}$ do not arrange as a $k$-OF.

\textit{Case 1.} Suppose for a $c\in[k]$, the induced subgraph $G_c$ is not connected, and without loss of generality, assume $c=1$. This means that $G_1$ has at least two separate components. Denote the nodes in each of the two component by $V_1^1$ and $V_1^2$ respectively, and recall for $c\geq 2$, $V_c=\{i:y_i=c\}$. As $d\geq k+1$, we can choose a set of $k+1$ vectors $[\widetilde{\mub}_1^1, \widetilde{\mub}_1^2, \widetilde{\mub}_2, \widetilde{\mub}_3,...,\widetilde{\mub}_k]$ such that they form a $(k+1)-$OF. Define $\widetilde{\Hb}=[\widetilde{\h}_1,...,\widetilde{\h}_n]$ as follows: 
\begin{align*}
    \forall i \in V_1^1, &\quad \widetilde{\h}_i = \widetilde{\mub}_1^1\\
    \forall i \in V_1^2, &\quad \widetilde{\h}_i = \widetilde{\mub}_1^2\\
    \forall i \in V_c,\,c\in[k], &\quad \widetilde{\h}_i = \widetilde{\mub}_c\,.
\end{align*}
Then, $\widetilde{\Hb}$ satisfies the equality conditions in Thm.~\ref{thm:scl_mini} since there is no edge between the nodes in $V_1^1$ and $V_1^2$ by the assumption. However, the embeddings in class $y=1$ do not align, since $\widetilde{\mub}_1^1$ is orthogonal to $\widetilde{\mub}_1^2$. Thus, $\widetilde{\Hb}$ optimizes \ref{eq:SCL_UFM_full} while it does not satisfy NC and differs from the OF geometry.

\textit{Case 2.} Suppose there exists $c_1\neq c_2\in[k]$ for which there is no edges between $G_{c_1}$ and $G_{c_2}$, and without loss of generality, assume $c_1=1, c_2=2$. Consider an embedding matrix $\widetilde{\Hb}$ that satisfies NC, and the corresponding mean-embedding matrix $\widetilde{\M}=[\widetilde{\mub}_1,\widetilde{\mub}_2,...,\widetilde{\mub}_k]$ is such that $\forall c\neq c'\in\{2,...,k\}$, $\widetilde{\mub}_c^\top\widetilde{\mub}_{c'}=0$ and $\widetilde{\mub}_1=\widetilde{\mub}_2$. Such an $\widetilde{\M}$ exists as $d\geq k$ and all we need is to have $[\widetilde{\mub}_2,...,\widetilde{\mub}_k]$ be a $(k-1)-$OF in the non-negative orthant. Since, there is no edge between $G_1$ and $G_2$, there is no $B\in\mathcal{B}$ that includes samples from classes $y=1$ and $y=2$ simultaneously. Equivalently, to achieve the lower-bound of Thm.~\ref{thm:scl_mini}, we do not require orthogonality between any pairs of samples $i\in\mathcal{C}_1$ and $j\in\mathcal{C}_2$. Therefore, $\widetilde{\Hb}$ is an optimal solution of the \ref{eq:SCL_UFM_full}. However, the mean-embeddings do not follow a $k-$OF. In fact, this optimal geometry, does not distinguish the samples in classes $y=1$ and $y=2$.


    




% \tina{old:}    
    % \textbf{`ONLY IF' direction.} {Assume that $G_c$ is not connected from some $c \in [k]$, \new{i.e., there exist two nodes $i,j \in G_c$ between which there is no path in the graph.} We will show that an optimal solution does not necessarily form an OF geometry.}
    
    % {We use the following example: Suppose $k=2, n_1 = n_2 = 4, \mathcal{B} = \{\{1,2,5,6\},\{3,4,7,8\}\}$, with labels $y_1 = y_2 = y_3 = y_4 = 1, y_5 = y_6 = y_7 = y_8 = 2$. With this batching, from Thm.~\ref{thm:scl_mini}, at a global optimum we have: $\h_1 = \h_2 \perp \h_5 = \h_6$ and $\h_3 = \h_4 \perp \h_7 = \h_8$. Now, suppose $d = 4$, then the following is a valid minimizing feature configuration: $\h_1 = \h_2 = [1 \ 0 \ 0 \ 0]^T, \h_3 = \h_4 = [0 \ 1 \ 0 \ 0]^T, \h_5 = \h_6 = [0 \ 0 \ 1 \ 0]^T, \h_7 = \h_8 = [0 \ 0 \ 0 \ 1]^T$. 
  % Therefore, although this is an optimal feature configuration, NC is not satisfied, with examples from the same class being arbitrarily separated from each other, and the features do not form an OF geometry. On the other hand, another optimal feature configuration given by $\h_1 = \h_2 =  \h_3 = \h_4 = [1 \ 0 \ 0 \ 0]^T, \h_5 = \h_6 = \h_7 = \h_8 = [0 \ 1 \ 0 \ 0]^T$ satisfies NC and forms an OF geometry. 
    % Therefore, the optimum is not uniquely an OF geometry.}

    % {Or, let there be a pair of classes $c_1$ and $c_2$ such that $G_{c_1}$ is not connected to $G_{c_2}$. Again, we will show
% that an optimal solution does not necessarily form an OF geometry.}

% {We consider the following example: Suppose $k=4, n_1 = n_2 = n_3 = n_4 = 2, \mathcal{B} = \{\{1,2,3,4\},\{5,6,7,8\}\}$, with labels $y_1 = y_2 = 1, y_3 = y_4 = 2, y_5 = y_6 = 3, y_7 = y_8 = 4$. With this batching, from Thm.~\ref{thm:scl_mini} we have: $\h_1 = \h_2 \perp \h_3 = \h_4$ and $\h_5 = \h_6 \perp \h_7 = \h_8$. Now, suppose $d = 4$, then the following is an optimal feature configuration: $\h_1 = \h_2 = [1 \ 0 \ 0 \ 0]^T, \h_3 = \h_4 = [0 \ 1 \ 0 \ 0]^T, \h_5 = \h_6 = [\nicefrac{1}{\sqrt{2}} \ \nicefrac{1}{\sqrt{2}} \ 0 \ 0]^T, \h_7 = \h_8 = [0 \ 0 \ \nicefrac{1}{\sqrt{2}} \ \nicefrac{1}{\sqrt{2}}]^T$. Therefore, although this is an optimal feature configuration and NC is satisfied, every class is not contrasted against every other class, thus resulting in non-orthogonal embeddings. On the other hand, another optimal solution given by $\h_1 = \h_2 = [1 \ 0 \ 0 \ 0]^T, \h_3 = \h_4 = [0 \ 1 \ 0 \ 0]^T, \h_5 = \h_6 = [0 \ 0 \ 1 \ 0]^T, \h_7 = \h_8 = [0 \ 0 \ 0 \ 1]^T$ follows an OF geometry. Therefore, an optimal solution does not necessarily form an OF geometry.} 


Therefore, the global minimizer will be uniquely an OF if and only if the batching scheme satisfies both the conditions stated in Cor.~\ref{cor:batch}.


% \tina{instead of giving counter example for the other direction:\\
% if Gc is not connected (assuming d>=k+1), a k+1-OF is also optimal: Gc has at least two separate connected components. assign two separate vectors $\mub_{c,1}$ and $\mub_{c,2}$ to each. if these two with the rest of the mean-embeddings form a (k+1)-OF, the equality conditions are satisfied.\\
% if Gc1 and Gc2 are not connected: consder a (k-1)-OF where $\mub_{c1}=\mub_{c2}$ and they form a k-1-OF with rest of the mean-embeddings . This should satisfy the equality conditions and is hence optimal.\\
% So optimal solution not unique. and either NC or orthogonality of class-means can be violated
% }

\subsection{Batch analysis for \ref{eq:SCL_UFM_full} vs UFM}
\label{rem:compare_graf}

{\citet[Thm.~2]{graf2021dissecting} studies the UFM without ReLU constraints and with balanced labels, and proves that the global solution is a simplex ETF. The authors note that their proof relies on the batch construction as the set of all combinations of a given size.
In contrast, we have proved that for \ref{eq:SCL_UFM_full}  the global solution is an OF for a wider range of batching scenarios (specifically, as long as they satisfy the interaction properties characterized in Cor.~\ref{cor:batch}). Without ReLU, as noted by \citet[Fig.~5]{graf2021dissecting}, the optimal configuration of examples in each batch can have a different geometry, depending on the label distribution of the examples within the batch. However, \emph{with} ReLU, the optimal configuration of every batch is an OF over the classes whose examples are present in the batch. In particular, there is no contradiction between two mini-batches having both overlapping and mutually exclusive classes, since the optimal configuration of one batch does not violate the optimal configuration of another. Furthermore, the overall batch construction can have a unique OF as the optimal configuration provided the conditions in Cor.~\ref{cor:batch} are satisfied. The conditions include the batching assumed by \citet{graf2021dissecting} as a special case, while being applicable in less restrictive scenarios. {Sec.~\ref{Sec:Binding_examples} explored the implications of this finding, by studying the criteria for a batching scheme to lead to a unique minimizer geometry and further suggesting a simple scheme to convert an arbitrary batching to one satisfying these criteria.} }

% \begin{remark}[Comparison to analysis of \citet{graf2021dissecting}]\label{rem:compare_graf_app} {In \ref{rem:compare_graf}, we have commented on the differences between our proof showing the optimization of mini-batch SCL under \ref{eq:SCL_UFM_full} and that of \citet{graf2021dissecting} under the UFM. We further elaborate with an illustrative example below: when optimizing the loss decomposed over a set of mini-batches, it is crucial to consider whether the individual batch minimizers are also overall optimal solutions. }

% Consider a simple example: $k= d = 3, y_1 = 1, y_2 = 2, y_3 = 3, B_1 = \{1,2\}, B_2 = \{1,3\}, B_3 = \{2,3\}, \mathcal{B} = \{B_1, B_2, B_3\}$. Let us identify the optimal embeddings for the two scenarios with and without non-negativity constraints on the embedding coordinates.
% \begin{enumerate}
%     \item Without non-negativity (UFM): the optimal embedding configurations can be shown to be ETF with $2$ vectors for every batch, which is simply an antipodal structure. In other words, the batch-wise optimal solutions are $\h_1 = -\h_2, \h_1 = -\h_3$ and $\h_2 = -\h_3$, for the batches $B_1, B_2$ and $B_3$, respectively. However, the batch-wise optimal solutions are infeasible due to their contradictory nature. From \cite{graf2021dissecting}, it can be deduced that the overall optimal configuration is instead an ETF with $3$ vectors. This example underscores the difficulty in optimizing the loss over every batch separately in case of SCL without non-negativity. See (a) in Fig.~\ref{fig:remark}.
%     \item With non-negativity \eqref{eq:SCL_UFM_full}: our results imply that the optimal embeddings form a $2$-OF for every batch, i.e., $\h_1 \perp \h_2, \h_1 \perp\h_3$ and $\h_2 \perp\h_3$, for the batches $B_1, B_2$ and $B_3$, respectively. The three conditions are compatible with each other and the fact that the overall optimal solution is a $3$-OF in $\R^3$. Therefore, we were able to break down the overall optimization into individual batches. See (b) in Fig.~\ref{fig:remark}.
% \end{enumerate}
% \end{remark} 

\begin{figure*}
        \centering
        \begin{subfigure}{0.99\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[clip, trim=1cm 13cm 1cm 13.3cm, width = \textwidth]{Figs/etf.pdf}};
                \node at (0.0,-1.3) [scale=0.9]{\textbf{(a)} UFM optimal embeddings};
                \node at (-4.5,-0.8) [scale=0.9]{\textbf{(i)}};
                \node at (-1.3,-0.8) [scale=0.9]{\textbf{(ii)}};
                \node at (1.85,-0.8) [scale=0.9]{\textbf{(iii)}};
                \node at (4.9,-0.8) [scale=0.9]{\textbf{(iv)}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.99\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[clip, trim=1cm 12cm 1cm 12.3cm, width = \textwidth]{Figs/of.pdf}};
                \node at (0.0,-1.3) [scale=0.9]{\textbf{(b)} UFM$_+$ optimal embeddings};
                \node at (-4.5,-0.8) [scale=0.9]{\textbf{(i)}};
                \node at (-1.3,-0.8) [scale=0.9]{\textbf{(ii)}};
                \node at (1.85,-0.8) [scale=0.9]{\textbf{(iii)}};
                \node at (4.9,-0.8) [scale=0.9]{\textbf{(iv)}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \captionsetup{width= \linewidth}
        \caption[remark]
        {Rem.~\ref{rem:compare_graf_app} visualized, \textbf{(a)(i,ii,iii)} indicate the antipodal structure of the optimal embeddings under UFM in each of the 3 mini-batches respectively, whereas the overall optimal geometry is an ETF \textbf{(a)(iv)}. This contrasts the optimal embeddings under UFM$_+$ where each mini-batch \textbf{(b)(i,ii,iii)} is consistent with the overall optima \textbf{(b)(iv)}.}
        \label{fig:remark} 
    \end{figure*}


==> sections_arxiv_v2/proofs_for_discussion_sec.tex <==
\section{Proofs for Section \ref{sec:UFMvsUFM+}}

\subsection{Proof of Lemma \ref{lem:OF2ETF}}

Let $\Vb=\begin{bmatrix}
    \vb_1&\ldots&\vb_k
\end{bmatrix}$    and $\bar\Vb=\begin{bmatrix}
    \bar\vb_1&\ldots&\bar\vb_k
\end{bmatrix}$. 
%\todo{are these supposed to be tilde or bar?} 
By definition of a $k$-OF, we know that $\Vb^\top\Vb\propto\Id$. Without loss of generality suppose the constant of proportionality is $1$ so that  $\Vb^\top\Vb=\Id\,.$ Since all $\vb_i$s are orthonormal, this then implies that $\Vb^\top\vb_G=\frac{1}{k}\ones_k$ and $\vb_G^\top\vb_G=\frac{1}{k}\,.$ These put together gives the desired as follows:
\begin{align*}
    \bar\Vb^\top\bar\Vb &= \left(\Vb-\vb_G\ones_k^\top\right)^\top\left(\Vb-\vb_G\ones_k^\top\right) = \Vb^\top\Vb - \ones_k\vb_G^\top\Vb-\Vb^\top\vb_G\ones_k^\top+(\vb_G^\top\vb_G)\ones_k\ones_k^\top=\Id_k - \frac{1}{k}\ones_k\ones_k^\top\,.
\end{align*}


\subsection{Proof of Lemma \ref{lem:counterexample}}

    To rule out the optimality of ETF in imbalanced setups, we show ETF does not minimize the loss in a $k=3$ class example. Specifically, consider a STEP-imbalanced training set with 3 classes of sizes $[R n_\text{min}, n_\text{min}, n_\text{min}]$ with $n_\text{min}\geq 2$ and $R \geq 10$. Suppose $\Hb_\text{ETF}$ follows the ETF geometry. Then, from Def.~\ref{def:etf} and the feasibility condition, for the mean-embeddings $\M_\text{ETF}$ we have $\M_\text{ETF}^\top\M_\text{ETF} = \frac{k}{k-1}(\Id_k - \frac{1}{k}\ones_k\ones_k^\top).$ Thus, the value of the loss function at ETF is 
    \begin{align*}
        \Lc_{\text{{full}}}(\Hb_\text{ETF}) = n_\text{min} \Big(R \log\big(R n_\text{min}-1+2n_\text{min}e^{-\frac{3}{2}}\big) + 2\log\big(n_\text{min}-1+n_\text{min}(R+1)e^{-\frac{3}{2}}\big)\Big).
    \end{align*}
    Now, consider $\widetilde{\Hb} = [\widetilde{\mub}\otimes \ones_{R n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{ n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{n_\text{min}}^\top]$, where {$\widetilde{\mub}$} is an arbitrary unit-norm vector. Since $\norm{\widetilde{\mub}}=1$, it follows that  $\widetilde{\Hb}$ is in the feasible set. With this choice of $\widetilde{\Hb}$, we have,
    \begin{align*}
        \Lc_{\text{{full}}}(\widetilde{\Hb}) = n_\text{min} \Big(R \log\big(R n_\text{min}-1+2n_\text{min}e^{-2}\big) + 2\log\big(2n_\text{min}-1+R n_\text{min}e^{-2}\big)\Big).
    \end{align*}
    It is easy to check that, for imbalance levels higher than $R\geq10$, $$\Lc_{\text{{full}}}(\widetilde{\Hb}) < \Lc_{\text{{full}}}(\Hb_\text{ETF}).$$ In other words, ETF does not always attain the optimal cost in \ref{eq:ufm}.


==> sections_v2/Deepnet_SCLGeom_exp.tex <==
% \vspace{-0.5cm}
% \vspace{0.2cm}
\noindent\textbf{Experimental setup.}~ Following the setup of \citet{graf2021dissecting}, our models consist of a backbone (ResNet, DenseNet, etc) with a normalizing layer to output features with unit norm. For all geometric convergence results, we apply a ReLU on output features before normalization. We employ {Stochastic Gradient Descent} (SGD) with a learning rate of $0.1$, momentum set to $0.9$ and with no weight decay.  Furthermore, as in \citet{graf2021dissecting,khosla2020supervised}, we set the temperature parameter $\tau = 0.1$ as \citet{khosla2020supervised} have found that it yields optimal performance. In addition, we empirically find that convergence to OF is not highly dependent on $\tau$ for values near $0.1$, yet the specific choice affects the speed of convergence.

We study the behavior of models trained with SCL under, {1)} $R$-\textit{STEP} imbalance having $k/2$ majority classes with $n_\maj$ examples per class and $k/2$ minority classes with $n_{\min} = \nicefrac{n_{\maj}}{R}$ examples per class, and {2)} $R$-\textit{Long-tailed} (LT) imbalance where the number of training datapoints exponentially decreases across classes such that $n_c = n_1 R^{-(c-1/k-1)}$, for $c \in [k]$. Regardless of the imbalance ratio $R$, we ensure that $n_c \geq 2$ by adding a vertically flipped version of each image as a method of batch duplication. Unless stated, we do not perform any additional data augmentation on the datasets, and use a batch size of $1024$ with random reshuffling. 

Finally, when studying the impact of ReLU on generalization, we use a Nearest Center Classifier (NCC) on the output features to evaluate model performance. For such experiments, following the setup of \cite{khosla2020supervised}, we employ a projection head by adding a 2 layer non-linear MLP (with or without ReLU at the last layer) and compare the test accuracy under difference imbalance ratios.

% 
% \begin{wrapfigure}[17]{t}{0.40\textwidth} 
%         \centering
%         %\hspace*{-20pt}
%             \centering
%             \vspace{-0.2in}\begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=0.38\textwidth]{Figs/Gm_Heatmap_Plots/Heatmap_2_fixed.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (-1.3,2.4) [scale=0.9]{\textbf{R = 1}};
%            	\node at (0.8,2.4) [scale=0.9]{\textbf{R = 100}};
%                 \node at (-2.8,-0.9)  [scale=0.9, rotate=90]{\textbf{CE}};
%                 \node at (-2.8,1.2)  [scale=0.9, rotate=90]{\textbf{SCL}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \captionsetup{width=1\linewidth}
%         \caption[GM]
%         {$\G_\M$ at last epoch (350) for ResNet-18 trained on $R$-STEP imbalanced MNIST. See text for details. %Each $\G_\M$ normalized to have a maximum value of 1. 
%         % For comparability, values plotted are divided by the max value in each $\G_\M$ matrix.
%         } %\todo{Do deepnet CE and compare its to the SCL , maybe plot SCL first, keep only R 1 and 100, state that this is with a normalizing layer}} 
%         \label{fig:GM matrices comparison}
% \end{wrapfigure}
% \vspace{5pt}
% \begin{wrapfigure}[19]{t}{0.40\textwidth} 
%         \centering
%         %\hspace*{-20pt}
%             \centering
%             \vspace{-0.2in}\begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=0.38\textwidth]{Figs/Gm_Heatmap_Plots/Heatmap_ICLR.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (-1.3,3.4) [scale=0.9]{\textbf{R = 1}};
%            	\node at (0.7,3.4) [scale=0.9]{\textbf{R = 100}};
%                 \node at (-3.15,-1.8)  [scale=0.9, rotate=90]{\textbf{CE}};
%                 \node at (-3.15,2.1)  [scale=0.9, rotate=90]{\textbf{SCL + ReLU}};
%                 \node at (-3.15,0.2)  [scale=0.9, rotate=90]{\textbf{SCL}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \captionsetup{width=1\linewidth}
%         \caption[GM]
%         {$\G_\M$ at epoch 350 for ResNet-18 trained on $R$-STEP imbalanced MNIST. See text. %Each $\G_\M$ normalized to have a maximum value of 1. 
%         % For comparability, values plotted are divided by the max value in each $\G_\M$ matrix.
%          } %\todo{Do deepnet CE and compare its to the SCL , maybe plot SCL first, keep only R 1 and 100, state that this is with a normalizing layer}} 
%         \label{fig:GM matrices comparison}
% \end{wrapfigure}

 % Link to the codebase to reproduce  experiments is provided \href{https://github.com/valavakilian/SCL_Geometry_And_Batching.git}{here}. %We maintain a batch size of \todo{insert bsz} with a constant learning rate of 0.1.  %\new{While working with SCL, we noticed that the geometry convergence was not affected by changes in }
 %\new{While working with SCL, we noticed that the geometry convergence was not affected by changes in optimization hyper-parameters}. \tina{is this sentence needed given what comes next?}


%In order to focus on the geometry convergence, we do not perform data augmentation on the datasets. However, in order to comply with the batches SCL requirement (each batch must include at least 2 datapoints from each class \cite{graf2021dissecting}), we add a augmented  each batch by adding a x-axis flipped version of each image from the batch.

%\tina{Are we showing any NC in the main body? we can delete the metric then. But need to shortly mention that NC occurs and we show in SM (we will show right?) so we focus on class-means with these metrics} 
%\tina{+I think it's worth emphasizing that GM is for last-layer features here again}

% \vspace{5pt}
\begin{wraptable}[11]{r}{0.4\textwidth}\label{Fig:Heatmaps_SCL_CE}
\vspace*{-5pt}
    \centering
    \resizebox{0.4\columnwidth}{!}{%
    \begin{tabular}{|l|l|l|}
        \cline{1-3}
        \multicolumn{1}{|c}{Imbalance Ratio (R)} & \multicolumn{1}{|c}{w/o ReLU} & \multicolumn{1}{|c|}{w/ ReLU} \\ \hline
        1 & \multicolumn{1}{c}{72.17 $\pm$ 0.23}  & \multicolumn{1}{|c|}{72.32 $\pm$ 0.60} \\ \hline
        10 (Step) & 56.58 $\pm$ 0.50 & 58.16 $\pm$ 0.76\\ \hline
        10 (LT) & 57.10 $\pm$ 1.04 & 57.88 $\pm$ 1.05 \\ \hline
        100 (Step) & 43.49 $\pm$ 0.30 & 43.80 $\pm$ 0.25 \\ \hline
        100 (LT) & 37.19 $\pm$ 2.50 & 39.71 $\pm$ 0.09 \\ \hline
    \end{tabular}
    }
    \captionsetup{width=\linewidth}
    \caption{Test accuracy comparison for a ResNet-18 trained using SCL on CIFAR100 with and without ReLU after the projection head. We use NCC for classification. Note that the addition of ReLU does not compromise the accuracy. For details, see \ref{sec:generalization} in SM.} %\tina{what is mlp here? haven't been explained in text before. (maybe just say with and without relu)}}
    \label{tab:cifar100_main}
\end{wraptable}
\noindent\textbf{Metrics.}~Since in all experiments we observe the within-class variations of the last-layer embeddings ($\h_i$) become negligible towards the end of training (see NC plots in Fig.~\ref{fig:Deepnet_SCL_Geom_NC} in SM), we focus here on the geometry of class-mean embeddings $\M$. 
Thus, to measure the distance of learned embedding to the OF geometry, we compute the distance metric $\Delta_{\G_\M} := \|\frac{\G_\M}{\|\G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$.
%In addition, we measure the pairwise cosine similarity \todo{fig 1 has different notation should be consistent}$\alpha_{\text{sim}}(c,c'):= \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for $c\neq c'\in[k]$.

% \todo{maybe move NC}By Def. \ref{def:ncof}, given NC, the Gram matrix for the $k$-OF is the identity matrix, $\Id_{k} \in \R^{k \times k}$. We measure convergence to OF by calculating a distance metric between $\G_\M$ for the last layer features and the k-OF geometry,  $\Delta_{\G_\M} := \|\frac{\G_\M}{\|\G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$. Moreover, we quantify the collapse of features, $\h_i, i \in [n]$, to their class-means (NC) through $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ \cite{NC}.\footnote{Here, $\Sigma_B= \sum_{c\in [k]}(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})^T$ is the between class covariance matrix, $\boldsymbol{\mu}_G = \frac{1}{k}\sum_{c\in[k]}\boldsymbol{\mu}_c$ is the weighted global mean, and $\Sigma_W  = \sum_{i\in [n]}(\h_i - \boldsymbol{\mu}_{y_i})(\h_i - \boldsymbol{\mu}_{y_i})^T$ is the within class covariance matrix.}  In addition, we measure the pairwise cosine similarity $\alpha_{\text{sim}}(c,c'):= \nicefrac{\mub_c^T\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ between feature class-means $\mub_c,\mub_{c'}, c\neq c'\in[k]$. Finally, for ease of comparison with results \cite{graf2021dissecting}, we also compute the corresponding angular distance $\Delta_\text{ang}:=1 - \nicefrac{1}{\pi}\arccos(\alpha_{\text{sim}}(c,c'))$.% adopted by \cite{graf2021dissecting}. to measure the orthogonality of frame independent of the NC.

\noindent\textbf{Observations on Geometry.}~In Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}, we plot the distance $\Delta_{\G_\M}$ between the learned feature-embeddings and the OF geometry as training progresses. We consistently observe that the learned features during training converge to the OF geometry, irrespective of the imbalance level $R$ of the training set and the imbalance pattern (STEP or LT). This suggests that the feature geometry learned by SCL
is invariant to the training label distribution. 

Interestingly, the invariance that is revealed by our study is distinct for SCL with ReLU as opposed to the case of SCL without ReLU, and that of CE and MSE loss. CE and MSE are known to be sensitive to imbalances \citep{seli, fang2021exploring, liu2023inducing, behnia2023implicit, dang2023neural}. Additionally, for different values of $R$, there is no significant difference between the speed of convergence, unlike the CE loss \citep{seli}, where it is empirically observed that the rate worsens with larger imbalance.

\noindent\textbf{Generalization.} To ensure that ReLU does not yield any adverse effects on test accuracy, we trained ResNet-18 (with a projection head) with and without ReLU on CIFAR10, CIFAR100, Tiny Imagenet and evaluated the balanced test accuracy when training under label imbalance. Following \citep{zhu2022balanced,khosla2020supervised,chen2020simple}, we consider the features before a projection head for evaluating the test accuracy of the models. Our results, e.g. in Tab.~\ref{tab:cifar100_main}, indicate that the addition of ReLU does \emph{not} compromise test accuracy. For a detailed discussion on the results see \ref{sec:generalization} in SM.

% \begin{wraptable}[12]{r}{0.6\textwidth}
%     \centering
%     \resizebox{0.6\columnwidth}{!}{%
%     \begin{tabular}{|l|l|l|l|l|}
%         \cline{2-5}
%         \multicolumn{1}{c}{} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \hline
%         R & Step & LongTail & Step & LongTail \\ \hline
%         1 & \multicolumn{2}{|c}{72.17 +/- 0.23}  & \multicolumn{2}{|c|}{72.32 +/- 0.60} \\ \hline
%         10 & 56.58 +/- 0.50 & 57.10 +/- 1.04 & 58.16 +/- 0.76 & 57.88 +/- 1.05 \\ \hline
%         100 & 43.49+/- 0.30 & 37.19 +/- 2.50 & 43.80 +/- 0.25 & 39.71 +/- 0.09 \\ \hline
%     \end{tabular}
%     }
%     \captionsetup{width=\linewidth}
%     \caption{Test accuracy comparison for a ResNet-18 trained using SCL on CIFAR100 with and without ReLU after the MLP. As per \cite{khosla2020supervised} the pre-projection features are used for accuracy comparison and we use Nearest Class Center for classification. We note that the addition of ReLU does not compromise the accuracy. For details, see \ref{sec:generalization} in SM.}
% \end{wraptable}



% \new{Fig.~\ref{fig:heatmap} illustrates how , in case of CE and SCL, with high imbalance ratio $R$, the class-mean embeddings representing different minority classes form smaller angles, making the minority classes less distinguishable and potentially impacting performance. Compared to that, SCL with ReLU; produces the same OF geometry between all classes, including minorities, regardless of imbalance. See Fig.~\ref{fig:heatmap}, $R = 10,100$.}



%\begin{wraptable}{17}[0.38\textwidt]
%  \begin{table}[!ht]
%  \fontsize{9pt}{15pt}\selectfont
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \cline{2-5}
%          \multicolumn{1}{c}{} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \hline
%         R & Step & LongTail & Step & LongTail \\ \hline
%           1 & \multicolumn{2}{|c}{72.17 +/- 0.23}  & \multicolumn{2}{|c|}{72.32 +/- 0.60} \\ \hline
%         10 & 56.58 +/- 0.50 & 57.10 +/- 1.04 & 58.16 +/- 0.76 & 57.88 +/- 1.05 \\ \hline
%         100 & 43.49+/- 0.30 & 37.19 +/- 2.50 & 43.80 +/- 0.25 & 39.71 +/- 0.09 \\ \hline
%     \end{tabular}
%     \caption{Test accuracy comparison for a ResNet-18 model trained using SCL on CIFAR100 both with an without ReLU after the MLP. As per \cite{khosla2020supervised} the pre-projection fetures is used for test accuracy comparison and use Nearest Class Center for classification. The results suggest that the addition of ReLU does not compromise the test accuracy. For more analysis, see \ref{sec:generalization} in SM.}
% \end{table}
%\end{wraptable}



% \begin{wraptable}{r}{0.5\textwidth}
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%         \cline{2-5}
%         \multicolumn{1}{c}{} & \multicolumn{2}{|c}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \hline
%         R & Step & LongTail & Step & LongTail \\ \hline
%         1 & \multicolumn{2}{|c}{72.17 +/- 0.23}  & \multicolumn{2}{|c|}{72.32 +/- 0.60} \\ \hline
%         10 & 56.58 +/- 0.50 & 57.10 +/- 1.04 & 58.16 +/- 0.76 & 57.88 +/- 1.05 \\ \hline
%         100 & 43.49+/- 0.30 & 37.19 +/- 2.50 & 43.80 +/- 0.25 & 39.71 +/- 0.09 \\ \hline
%     \end{tabular}
% \end{wraptable}

% \FloatBarrier

% \section{\ref{eq:scl+} does not compromise Accuracy}\label{sec:generalization}
% \new{Having discussed the symmetry-preserving value of ReLU activation in SCL training, we now turn towards the impact on generalization accuracy. While the exact relationship between the training feature geometry and generalization is an open question, it is conceivable that maintaining symmetry in features is beneficial to generalization \citep{behnia2023implicit, zhu2022balanced}. In fact, our experiments with class-imbalance reveal that ReLU improves the test accuracy significantly in a subset of the cases, while not deteriorating in others. There have been suggestions of loss function modifications in such a way that the feature geometry is symmetric in presence of class-imbalance, consequently also achieving improvements in generalization \cite{behnia2023implicit, zhu2022balanced}. Since the role of a projector block is of interest when training with SCL, we compare the experimental test accuracies both when the projector is retained (aka post-projection) as well as discarded (aka pre-projection) during inference.}

% \new{We consider the effect of ReLU in two representative settings, (i) linear layer projector (ii) two-layer MLP projector. The details on the projector structure are deferred to the SM.}

% \todo{only two tables from below to be retained in main body}

% \begin{table}[!ht]
% \fontsize{9pt}{5pt}\selectfont
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%     \hline
%          & \multicolumn{4}{|c|}{Pre-Projection}   & \multicolumn{4}{|c|}{Post-Projection}   \\  \hline 
%         R & \multicolumn{2}{|c|}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} & \multicolumn{2}{|c|}{MLP} & \multicolumn{2}{|c|}{MLP + ReLU} \\ \hline
%          & Step & LT & Step & LT & Step & LT & Step & LT \\ \hline
%         1 & \multicolumn{2}{|c|}{62.53 +/- 1.23}  & \multicolumn{2}{|c|}{62.26 +/- 0.37} & \multicolumn{2}{|c|}{62.71 +/- 1.10} & \multicolumn{2}{|c|}{62.48 +/- 0.40} \\ \hline
%         10 \text{ (Step) } & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \hline
%         10 \text{ (LT) } & 51.22 +/- 1.94 & 49.81 +/- 0.82 & 50.99 +/- 1.83 & 48.76 +/- 1.18 \\ \hline
%         100 \text{ (Step) } & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%         100 \text{ (LT) } & 36.06 +/- 0.89 & 35.84 +/- 1.33 & 34.57 +/- 0.95 & 33.78 +/- 1.34 \\ \hline
%     \end{tabular}
%     \caption{\vala{New Tables} Post-projection, Tiny ImageNet}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.91 +/- 0.23 \% & 91.79 +/- 0.21 \% & \textbf{91.88 +/- 0.29} \% & 91.86 +/- 0.32 \% \\ \hline
%         10 & 82.12 +/- 1.06 \% & 83.29 +/- 0.49 \% & \textbf{83.70 +/- 1.09} \% & 83.41 +/- 0.64 \% \\ \hline
%         100 & 61.25 +/- 0.64 \% & 62.98 +/- 0.68 \% & 60.19 +/- 1.75 \% & \textbf{67.12 +/- 1.04} \% \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR10-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.89 +/- 0.26 \% & 91.81 +/- 0.24 \% & 91.88 +/- 0.23 \% & \textbf{91.94 +/- 0.40} \% \\ \hline
%         10 & 81.11 +/- 1.24 \% & 81.02 +/- 0.60 \% & \textbf{82.35 +/- 0.67} \% & 80.81 +/- 1.01 \% \\ \hline
%         100 & 55.74 +/- 1.08 \% & 57.07 +/- 0.60 \% & 55.31 +/- 1.98 \% & \textbf{59.83 +/- 1.75} \% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR10-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.17 +/- 0.23 \% & \textbf{72.32 +/- 0.60\%} \\ \hline
%         10 & 56.58 +/- 0.50 \% & \textbf{58.16 +/- 0.76\%} \\ \hline
%         100 & 43.49 +/- 0.30\% & \textbf{43.80 +/- 0.25\%} \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR100-STEP}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & \textbf{72.30 +/- 0.57} \% & 72.25 +/- 0.35\% \\ \hline
%         10 & 54.57 +/- 0.49 \% & \textbf{55.35 +/- 0.33\%} \\ \hline
%         100 & \textbf{40.29 +/- 0.33\%} & 39.93 +/- 0.14\% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR100-STEP}
% \end{table}



% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.73 +/- 0.30\% & 91.96 +/- 0.26\% & \textbf{92.04 +/- 0.10\%} & 91.79 +/- 0.13\% \\ \hline
%         10 & 83.25 +/- 0.55\% & 84.02 +/- 0.68\% & 83.70 +/- 0.70\% & \textbf{84.40 +/- 0.79\%} \\ \hline
%         100 & 68.40 +/- 1.35\% & 67.88 +/- 1.21\% & \textbf{68.75 +/- 0.31\%} & 68.57 +/- 1.69\% \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR10-LT}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%         R & Linear & Linear + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 91.73 +/- 0.29\% & 91.81 +/- 0.36\% & \textbf{92.04 +/- 0.13\%} & 91.91 +/- 0.17\% \\ \hline
%         10 & 82.55 +/- 0.64\% & 82.98 +/- 0.98\% & 82.97 +/- 0.83\% & \textbf{82.99 +/- 1.03\%} \\ \hline
%         100 & 63.64 +/- 0.99\% & 63.51 +/- 1.39\% & \textbf{63.67 +/- 0.77\%} & 62.65 +/- 2.37\% \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR10-LT}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.25 +/- 0.33 \% & \textbf{72.30 +/- 0.19\%} \\ \hline
%         10 & 57.10 +/- 1.04 \% & \textbf{57.88 +/- 1.05\%} \\ \hline
%         100 & 37.19 +/- 2.50\% & \textbf{39.71 +/- 0.09\%} \\ \hline
%     \end{tabular}
%     \caption{Pre-projection, CIFAR100-LT}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|}
%     \hline
%         R & MLP & MLP + ReLU \\ \hline
%         1 & 72.37 +/- 0.32 \% & \textbf{72.44 +/- 0.29\%} \\ \hline
%         10 & 56.27 +/- 0.45 \% & \textbf{57.08 +/- 0.82\%} \\ \hline
%         100 & 35.29 +/- 1.64\% & \textbf{37.21 +/- 0.51\%} \\ \hline
%     \end{tabular}
%     \caption{Post-projection, CIFAR100-LT}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|}
%     \hline
%          & \multicolumn{2}{|c|}{Pre-Projection}   & \multicolumn{2}{|c|}{Post-Projection}   \\  \hline 
%         R & MLP & MLP + ReLU & MLP & MLP + ReLU \\ \hline
%         1 & 62.53 +/- 1.23  & 62.26 +/- 0.37 & 62.71 +/- 1.10 & 62.48 +/- 0.40 \\ \hline
%         10 \text{ (Step) } & 50.17 +/- 1.44 & 49.78 +/- 0.67 & 48.93 +/- 1.64 & 46.93 +/- 0.53 \\ \hline
%         10 \text{ (LT) } & 51.22 +/- 1.94 & 49.81 +/- 0.82 & 50.99 +/- 1.83 & 48.76 +/- 1.18 \\ \hline
%         100 \text{ (Step) } & 39.13 +/- 0.63 & 40.02 +/- 0.62  & 37.41 +/- 0.29 &  37.19 +/- 0.68 \\ \hline
%         100 \text{ (LT) } & 36.06 +/- 0.89 & 35.84 +/- 1.33 & 34.57 +/- 0.95 & 33.78 +/- 1.34 \\ \hline
%     \end{tabular}
%     \caption{\vala{New Tables} Post-projection, Tiny ImageNet}
% \end{table}


% \new{Thus, as noted in Tables \ref{tab:} we make a remarkable observation that simply adding ReLU to the network can yield significant improvements in test accuracy in certain cases, while at least matching that of the case without ReLU in others. In light of this, our finding of the insensitivity of the embedding geometry in presence of ReLU serves a potential explanation. Our analysis therefore paves an important direction for future empirical investigations into the role of the activation functions in the projector network on generalization of SCL} 






% \begin{figure*}
%         % \centering
%         \hspace*{-40pt}
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_CIFAR10_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{CIFAR10}};
%                 \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{Step Imbalance}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \hspace{-0.5cm}
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_MNIST_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{MNIST}};
%                \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \hspace{-0.5cm} 
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_FMNIST_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{FMNIST}};
%                 \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \vskip\baselineskip
%        %  \vspace{-0.5cm}
%        %  \begin{subfigure}[b]{0.3\textwidth}
%        %      \centering
%        %      \begin{tikzpicture}
%        %          \node at (0.0,0) 
%        %          {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_CIFAR10_exp_SCL_ReLU_noAugment.pdf}};
%        %          % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% % \node at (0.0,2.0) [scale=0.7]{\textbf{CIFAR10}};
%        %          \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{Longtail Imbalance}};
%        %          % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%        %      \end{tikzpicture}
%        %  \end{subfigure}
%        %  \hfill
%        %  \begin{subfigure}[b]{0.3\textwidth}
%        %      \centering
%        %      \begin{tikzpicture}
%        %          \node at (0,0) 
%        %          {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_MNIST_exp_SCL_ReLU_noAugment.pdf}};
%        %          % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% % \node at (0.0,2.0) [scale=0.7]{\textbf{MNIST}};
%        %         \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%        %         % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%        %      \end{tikzpicture}
%        %  \end{subfigure}
%        %  \hfill
%        %  \begin{subfigure}[b]{0.3\textwidth}
%        %      \centering
%        %      \begin{tikzpicture}
%        %          \node at (0,0) 
%        %          {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_FMNIST_exp_SCL_ReLU_noAugment.pdf}};
%        %          % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% % \node at (0.0,2.0) [scale=0.7]{\textbf{FMNIST}};
%        %          \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%        %          % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%        %      \end{tikzpicture}
%        %  \end{subfigure}
        
%         \caption
%         {Measured convergence of the Gram matrix of class means, $\G_\M$, to the OF geometry as described in Sec.\ref{sec:setup}. \ct{Larger legend?}}
%         \label{Fig:Deepnet_SCL_Geom_GMu}
%     \end{figure*}

%Lastly, Figure~\ref{fig:GM matrices comparison} shows a heat plot of $\G_\M$ learned by SCL compared with those learned by CE. Avoiding minority collapse: from our empirical observations, if the features converge to an OF regardless of the label distribution, it can be inferred that the models trained with SCL may be more resilient to the issues such as the minority collapse \cite{fang2021exploring}. \todo{In relation to figure 3 comparing to CE, we will discuss this after the remark}





%####################################################################


% \begin{figure*}
%         \centering
%         % \hspace{-0.5cm}
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_CIFAR10_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{CIFAR10}};
%                 \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{Step Imbalance}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \hspace{-0.5cm}
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_MNIST_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{MNIST}};
%                \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \hspace{-0.5cm} 
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_FMNIST_step_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,2.0) [scale=0.9]{\textbf{FMNIST}};
%                 \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         % \vskip\baselineskip
%         \vspace{-0.5cm}
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_CIFAR10_exp_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% \node at (0.0,2.0) [scale=0.7]{\textbf{CIFAR10}};
%                 \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{Longtail Imbalance}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_MNIST_exp_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% \node at (0.0,2.0) [scale=0.7]{\textbf{MNIST}};
%                \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/Deepnet_Geometry_GMu_Plots/ResNet18_FMNIST_exp_SCL_ReLU_noAugment.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			% \node at (0.0,2.0) [scale=0.7]{\textbf{FMNIST}};
%                 \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
        
%         \caption
%         {Measured convergence of the Gram matrix of class means, $\G_\M$, to the OF geometry as described in Sec.\ref{sec:setup}. \ct{Larger legend?}}
%         \label{Fig:Deepnet_SCL_Geom_GMu}
%     \end{figure*}

% Figure \ref{fig:GM matrices comparison} shows a heat plot of the Gram matrix of class-mean of features learned by SCL and compare with those learned by CE in a similar setup.... Avoiding minority collapse: from our empirical observations, if the features converge to an OF regardless of the label distribution, it can be inferred that the models trained with SCL may be more resilient to the issues such as the minority collapse \cite{fang2021exploring}. \todo{In relation to figure 3 comparing to CE, we will discuss this after the remark}

% \begin{figure*}
%         \centering
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 1}};
%                 \node at (-2.4,0.0)  [scale=0.9, rotate=90]{\textbf{SCL}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 10}};
%                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 100}};
%                 \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%        % \vskip\baselineskip
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1CE.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 1}};
%                 \node at (-2.4,0.0)  [scale=0.9, rotate=90]{\textbf{CE}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10CE.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 10}};
%                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.3\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100CE.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.8) [scale=0.9]{\textbf{R = 100}};
%                 \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%         \end{subfigure}
%         \caption[GM]
%         {$\G_\M$ matrices for various $(R)$-STEP imbalances at last epoch of training with ResNet-18 on MNIST with 10000 total examples. The CE features are normalized before the classifier head to allow for fair comparison. \todo{Do deepnet CE and compare its to the SCL , maybe plot SCL first}} 
%         \label{fig:GM matrices comparison}
%     \end{figure*}

%     \todo{Add NC plots}
% \begin{figure*}
%     % \centering
%     \hspace*{-20pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-4.2,3.1) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.5,3.1) [scale=0.9]{\textbf{MNIST}};
%             \node at (4.8,3.1) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-7.3,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-7.3,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%         \end{tikzpicture}
%     \end{subfigure}
%     \caption
%     {Following the same setup as Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu} we analyse the NC property.We observe that our NC metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ in on an order of $0.01$ suggesting that the class features are well concentrated around their respected means $\mu_c$. \tina{can't we have this merged with GM figure, and have smaller plots to take the same space?}}
%     \label{Fig:Deepnet_SCL_Geom_NC}
% \end{figure*}

==> sections_v2/SMroadmap.tex <==

\section*{Roadmap to the Supplementary material}

%{\color{darkblue} 
The SM contains the following. In Section \ref{sec:SEL_mat_properties} we derive several useful properties of the simplex-encoded-label (\SEL)~matrix, which we then use  in Section \ref{sec:SELI_properties} to present  closed-form characterizations of the embeddings and classifiers geometries. Notably, these include explicit expressions for the norms and angles of both majority and minority classes, which we accompany with numerical illustrations shedding further light on the features of the proposed \emph{\ref{SELI}} geometry. Next, in Section \ref{sec:proofs_UF-SVM}, we use the derived properties of the \SEL~matrix to prove our main Theorem \ref{thm:SVM} and its corollaries. In Section \ref{sec:nuc_norm_SM} we derive several useful properties of the nuclear-norm penalized CE minimization, which we then use in Section \ref{sec:proofs_regularization} to prove the statements of Section \ref{Sec:reg}. Section \ref{sec:UFM} contains additional numerical results on the UFM, such as experiments with varying weight-decay and regularization choices. Additional experiments on real data (such as, isolated minority/majority geometry investigations, and classifiers/embeddings norm ratios), as well as further implementation details, are included in Section \ref{sec:real_exp_SM}. In Section \ref{sec:minority} we show how results relate to minority collapse providing additional theoretical justifications and novel perspectives to empirical observations reported by previous work. Finally, an elaborate discussion on additional related works is contained in Section \ref{sec:rel2}.
%}

==> sections_v2/abstract.tex <==
Supervised contrastive loss (SCL) is a competitive and often superior alternative to the cross-entropy loss for classification. While prior studies have demonstrated that both losses yield symmetric training representations under balanced data, this symmetry breaks under class imbalances. This paper presents an intriguing discovery: the introduction of a ReLU activation at the final layer effectively restores the symmetry in SCL-learned representations. We arrive at this finding analytically, by establishing that the global minimizers of an unconstrained features model with SCL loss and entry-wise non-negativity constraints form an orthogonal frame. Extensive experiments conducted across various datasets, architectures, and imbalance scenarios corroborate our finding.  Importantly, our experiments reveal that the inclusion of the ReLU activation restores symmetry without compromising test accuracy. This constitutes the first geometry characterization of SCL under imbalances. Additionally, our analysis and experiments underscore the pivotal role of batch selection strategies in representation geometry. By proving necessary and sufficient conditions for mini-batch choices that ensure invariant symmetric representations, we introduce batch-binding as an efficient strategy that guarantees these conditions hold. 




% \new{In this paper we ask: how does class-imbalance and the presence of an activation function at the  influence the learned representations of SCL?} To address this question, \new{we find that the geometry of embeddings learned by SCL with ReLU activations in the last hidden layer} consistently form an orthogonal frame (OF). Remarkably, this holds true regardless of the distribution of training labels. \new{\gk{could be confusing} Effectively, incorporating ReLU enforces a symmetry in the embedding geometry. Our work is the first to characterize the geometry of training features of SCL under imbalances. \gk{this line can go}This fact suggests that adding ReLU activations to the features is sufficient if one aims to design a training scheme that produces symmetric distribution of learned features.} In contrast,  previous work has shown that embeddings geometries for CE loss are highly dependent on the class sizes. We arrive at our finding theoretically, by proving that the global minimizers of an unconstrained features model with SCL loss and entry-wise non-negativity constraints form an OF. We then validate the model's prediction by conducting experiments with standard deep-learning models on benchmark vision datasets. \new{Our experiments indicate that the straightforward addition of ReLU not only helps in the embedding geometry, but also holds potential to improve test accuracy, particularly when dealing with label-imbalanced training data.} Finally, our analysis and experiments reveal that the batching scheme chosen during SCL training plays a critical role in {determining the quality of} convergence to the OF geometry. \new{Notably,  we characterize the set of mini-batch choices that lead to an OF minimizer. This latter finding highlights the critical role of batching and leads to a concrete algorithmic contribution of a sampling strategy (batch-binding) that leads to significant improvements on geometry convergence.} 

% Supervised contrastive loss (SCL) is a competitive and often superior alternative to the cross-entropy (CE) loss for classification. \new{In this paper we ask: how does class-imbalance and the presence of an activation function influence the learned representations of SCL?} To address this question, \new{we find that the geometry of embeddings learned by SCL with ReLU activations in the last hidden layer} consistently form an orthogonal frame (OF). Remarkably, this holds true regardless of the distribution of training labels. \new{\gk{could be confusing} Effectively, incorporating ReLU enforces a symmetry in the embedding geometry. Our work is the first to characterize the geometry of training features of SCL under imbalances. \gk{this line can go}This fact suggests that adding ReLU activations to the features is sufficient if one aims to design a training scheme that produces symmetric distribution of learned features.} In contrast,  previous work has shown that embeddings geometries for CE loss are highly dependent on the class sizes. We arrive at our finding theoretically, by proving that the global minimizers of an unconstrained features model with SCL loss and entry-wise non-negativity constraints form an OF. We then validate the model's prediction by conducting experiments with standard deep-learning models on benchmark vision datasets. \new{Our experiments indicate that the straightforward addition of ReLU not only helps in the embedding geometry, but also holds potential to improve test accuracy, particularly when dealing with label-imbalanced training data.} Finally, our analysis and experiments reveal that the batching scheme chosen during SCL training plays a critical role in {determining the quality of} convergence to the OF geometry. \new{Notably,  we characterize the set of mini-batch choices that lead to an OF minimizer. This latter finding highlights the critical role of batching and leads to a concrete algorithmic contribution of a sampling strategy (batch-binding) that leads to significant improvements on geometry convergence.} 

% we show that thanks to the non-negativity constraints (modeling the ReLU), not only is the minimizing geometry stable, but also
% This finding motivates a simple algorithm wherein the addition of a few  \textit{binding examples} in each batch significantly speeds up the occurrence of the OF geometry. \gk{alternatively}


%\new{Guided by our finding on the relation between the batching strategy and feature geometry, we propose that a simple scheme with a fixed number of \textit{binding examples} improves convergence.}
% Supervised contrastive loss (SCL) is a proposed alternative to the cross-entropy (CE) loss with the heuristic of incorporating semantics in the representations. %We study the properties of the learned representations (features) in large models from the perspective of implicit bias.
% We show that the geometry of features learned by SCL form an orthogonal frame (OF) irrespective of the training data distribution. Taking inspiration from existing work on implicit bias in models trained with CE loss, we study the empirical risk minimization (ERM) with SCL on the unconstrained features model (UFM). We characterize its global minimizers with ReLU activation modeled with non-negativity constraints on the learned features. %We complement the global solution structure by proving that SCL has a benign loss landscape under the UFM.
% Conducting experiments on standard deep-learning models for vision on benchmark datasets, we show that our analytical characterizations predict the geometry of representations. We provide a geometric understanding of the trained models, thereby providing a qualitative comparison with models trained with CE loss. %A key differentiating factor of our characterization is that we show OF to be the unique minimizing geometry independent of label imbalance and reweighting of the loss.
% Further, we study the effect of batch construction on the global minimizers wherein we prove the OF to be the solution for a wide class of batch constructions, which leads to a simple scheme for batch construction which yields better convergence to the OF geometry without requiring all combinations of examples or random reshuffling during optimization. 
% \gk{not all results. Bring UFM later, then verified in experiments}


 

==> sections_v2/analysis.tex <==
\section{Analysis}

\begin{lemma}\label{lem:centering}
 Any global minimizer $(\hat\W,\hat\Hb)$ of \eqref{eq:svm_original} is such that $\sum_{c\in[k]}\hat\w_c=\zeros$.
\end{lemma}

\begin{proof}
For the sake of contradiction assume that $\bar\w:=\frac{1}{k}\sum_{c\in[k]}\hat\w_c\neq \zeros$, that is $\|\bar\w\|_2>0$. Consider the pair $({\Vb},\hat\Hb)$ where the columns of $\Vb$ are defined each such that $\vb_c=\hat\w_c-\bar\w$. Clearly, the new pair is feasible, since $(\hat\W,\hat\Hb)$ is feasible. But, 
$$
\sum_{c\in[k]}\|\vb_c\|^2 = \sum_{c\in[k]}\|\w_c\|^2 + k\|\bar\w\|^2 - \inp{\bar\w}{\sum_{c\in[k]}\w_c} =  \sum_{c\in[k]}\|\w_c\|^2 - k\|\bar\w\|^2 <\sum_{c\in[k]}\|\w_c\|^2,
$$
which contradicts optimality of $(\hat\W,\hat\Hb)$. Hence, it must be that $\bar\w=\zeros$.
\end{proof}


Consider first the minimization over $\Hb$ for any fixed $\W$:
\begin{align}
\Hb(\W):=\arg\min_{\Hb}~\frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
\end{align}
Note that this optimization is separable over the rows of $\Hb$ and each row of $\Hb(\W)$ is found by minimizing the following:
\begin{align}\label{eq:hi_sep}
\min_{\h}~\frac{1}{2}\|\h_i\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1\quad\forall c\neq y_i
\end{align}
The above optimization is strongly convex. Slater's conditions hold, thus KKT conditions are necessary and sufficient. Therefore the solution $\hat\h_i:=\h_i(\W)$ of the problem  above is unique and satisfies:
\begin{align}\label{eq:hi_KKT}
\hat\h_i = \A_{-{y_i}}^T\lab_i , \qquad \lab_i\geq \zeros,  \qquad \A_{y_i}\hat\h_i\geq \ones, \qquad \lab_i^T(\ones-\A_{-{y_i}}\hat\h_i)=0
\end{align}
for some optimal dual variable $\lab_i\in\R^{k-1}$. Also, from strong duality, the minimization in \eqref{eq:hi_sep} is equivalent to the following maximization
\begin{align}
\max_{\lab} ~-\frac{1}{2}\|\A_{y_i}^T\lab\|^2+\lab^T\ones \quad\quad\text{sub. to}\quad \lab \geq 0.
\end{align}

\begin{remark}
Note that {if $\A_{y_i}\A_{y_i}^T$ is invertible and $\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\geq \zeros$,} then the primal dual pair:
\begin{align}
 \hat\h_i=\A_{y_i}^T\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\qquad{\text{and}}\qquad\lab_i=\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones
\end{align}
 satisfies the KKT and is thus optimal. However, this might not be true for the optimal $\W$. Thus, we consider below the general case.
 \end{remark}
 
 In general, \eqref{eq:svm_original} reduces to the following min-max optimization
 \begin{align}\label{eq:cvx_onlyW}
\min_{\substack{\W\\
\A_{y_i}=\ones\w_{y_i}^T-\W_{-y_i}^T
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\|\W\|^2 -\frac{1}{2}\sum_{i\in[n]}\|\A_{y_i}^T\lab_i\|^2 + \sum_{i\in[n]}\lab_i^T\ones.
\end{align}
From Lemma \ref{lem:centering}, the optimization above does not change when we impose the additional constraint $\sum_c\w_c=\zeros$. Using this, note that $\w_c = -\W_{-c}\ones, \forall c\in[k]$. Therefore, 
\begin{align}
\A_c = \ones\w_c^T-\W_{-c}^T = -\ones\left(\W_{-c}\ones\right)^T-\W_{-c}^T = -\left(\Id+\ones\ones^T\right)\W_{-c}^T
\end{align}
Therefore,
$$
\A_c\A_c^T = \left(\Id+\ones\ones^T\right)\W_{-c}^T\W_{-c}\left(\Id+\ones\ones^T\right).
$$
Recalling the notation of the Gram matrix $\G$ and its submatrices $\G_{-c}, c$ and recognizing that $\G_{-c}=\W_{-c}^T\W_{-c}$, we can rewrite the optimization in \eqref{eq:cvx_onlyW} as follows
 \begin{align}\label{eq:cvx_onlyG}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{i\in[n]}\lab_i^T\left(\Id+\ones\ones^T\right)\G_{-y_i}\left(\Id+\ones\ones^T\right)\lab_i + \sum_{i\in[n]}\lab_i^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W \succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \sum_{c\in[k]}\w_c=\zeros \nn
\end{align}
By symmetry, for all $i: y_i=c$ it holds that $\la_i=\la_c$. Also, note that
$$
(\W^T\W\ones = \zeros ~~\text{ OR }~~ \ones^T\W^T\W = \zeros^T) \Leftrightarrow \W\ones=\zeros.
$$
 Using these, we can further reduce the above to the following
 \begin{align}\label{eq:cvx_onlyG_c}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_c\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\left(\Id+\ones\ones^T\right)\G_{-c}\left(\Id+\ones\ones^T\right)\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W\succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \G\ones=\zeros,~~ \ones^T\G=\zeros^T \nn
\end{align}
Finally, we can exploit the lemma below, to write the optimization only in terms of Gram matrices.
\begin{lemma}\label{lem:chol}
Consider arbitrary $\G\succeq\zeros_{k\times k}$ with $\G\ones=\zeros.$
%with $\rm{rank}(G)=r$. 
Assume $d\geq k-1$. Then, there exists $\W\in\R^{d\times k}$ such that $\G=\W^T\W$.
\end{lemma}
\begin{proof}
Recall that any positive semidefinite matrix $\G\succ\zeros_{k\times k}$ with $\rm{rank}(G)=r$ has a  Cholesky factorization $\G=\Lb\Lb^T$ with $\Lb\in\R^{k\times k}$ lower triangular with exactly $r$ positive diagonal elements and $k-r$ columns containing all zeros. Note since $\G\ones=\zeros$, $r\leq k-1$ in our case. Thus, $\Lb$ has at least one column containing all zeros. Remove that column and with some abuse of notation let $\Lb\in\R^{k\times (k-1)}$ be the remaining Cholesky factor. Then, for all $d\geq k-1$, we can choose $\W = \begin{bmatrix} \Lb^T \\ \zeros_{(d-(k-1))\times k} \end{bmatrix}$, which completes the proof.
 \end{proof}
 Indeed, using Lemma \eqref{lem:chol}, the optimziation in \eqref{eq:cvx_onlyG_c} is equivalent \footnote{Here, equivalence is in the following sense. If $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, then $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}. Also, if $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}, then $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, where here $\hat\W$ is such that $\hat\W^T\hat\W=\hat\G$ and its existence is guaranteed by Lemma \ref{lem:chol}.}
  to the following:
\begin{align}\label{eq:cvx_G}
&\min_{\substack{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}
}} ~\max_{\lab_c\geq \zeros }~~F(\G,\lab_c) :=\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\widetilde\J_c\G\widetilde\J_c^T\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones,
\end{align}
where we set $\widetilde\J_c:=\left(\Id_{k-1}+\ones\ones^T\right)\J_c.$

 
 We can write the inner maximization in \eqref{eq:cvx_G} using strong duality as follows
 \begin{align}
& \min_{\mub_c\geq \zeros}\max_{\lab_c}~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\tilde\J_c\G\tilde\J_c^T\lab_c + \sum_{c\in[k]}\lab_c^T\left(n_c\ones + \mub_c\right)\\
=&\min_{\mub_c\geq \zeros}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),
 \end{align}
 where we recall that $\G_{-c}:=\J_c\G\J_c^T.$
 
 \begin{propo}\label{eq:h_opt}
 	Let $(\hat\W,\hat\Hb)$ be any global minimizer of \eqref{eq:svm_original}. Then, the Gram matrix $\hat\G:=\hat\W^T\hat\W$ is a minimizers of the following convex SDP:
 \begin{align}\label{eq:SDP}
 &\min_{\G,\G_{-c},\mub_c}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right) 
 \\
 \nn
 &~~\text{sub. to}\quad \G\succeq \zeros_{k\times k},~~\G_{-c}=\J_c\G\J_c^T,~~\mub_c\geq\zeros_{k-1},~~\G\ones=(\ones^T\G)^T=\zeros.
 \end{align}
 Moreover, letting $\hat\mub_c, c\in[k]$ denote minimizers of the convex program above and defining $$\hat\lab_c = \frac{1}{n_c}\left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),$$
 it holds for all $i\in[n]$ that,
 $$
\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
 $$
 \end{propo}
 
 \begin{remark}
Solving \eqref{eq:SDP} in CVX gives $\hat\mub_c = 0, \forall c\in[k]$. Hence, $\lab_{c}>\zeros$, which would imply that all constraints are active. Unfortunately, we know that this is NOT true if we run GD. \red{Our conjecture (?) is that GD converges to a KKT point of \eqref{eq:SDP} that is NOT a global optimum.}
 \end{remark}
 
 \subsection{The Dual problem}

 \begin{propo}
 The dual of \eqref{eq:svm_original} is the following (convex) SDP:
 \begin{align}
& \max_{\lab_c\in\R^{k-1}, c\in[k]}~~\sum_{c\in[k]}n_c\lab_c^T\ones_{k-1}\\
& ~~~\text{sub. to}~~~~~ \lab_c \geq 0\nn\\
& \qquad\qquad\qquad \Pb_k\left(\Id_k - \sum_{c\in[k]}n_c\J_c^T\left(\Id_{k-1}+\ones\ones^T\right)\lab_c\lab_c^T\left(\Id_{k-1}+\ones\ones^T\right)\J_c\right)\Pb_k\succeq 0\nn
 \end{align}
 where we set $\Pb_k:=\Id_k-\frac{1}{k}\ones\ones.$ 
 \end{propo}

Remark: A fast way to see the above is from \eqref{eq:cvx_G}. The second constraint can be written in an SDP form using Schur complement.


\subsection{A direct tight convex relaxation}
The following program is a convex relaxation of \eqref{eq:svm_original} found by setting
\begin{align}\label{eq:X_rel}
\X_{2k \times 2k} = \begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix},
\end{align}
for $\bar\Hb_{d \times k}=[\bar\h_1, \ldots, \bar\h_k]$ the feature matrix. Here, we note in \eqref{eq:svm_original} that at the optimal $\h_i=\bar\h_{y_i}$ for all $i\in[n].$

\begin{align}\label{eq:cvx_X2}
&\min_{\X\in\R^{{2k \times 2k}}}~~\sum_{c\in[k]}\X[c,c] + \sum_{c\in[k]}n_c\X[k+c,k+c]\\
&~\text{sub.~to}~~~~\X[c,k+c]-\X[c',k+c]\geq 1,~c'\neq c, c\in[k] \\
&\qquad\qquad\quad\X\succeq 0_{2k\times 2k}
\end{align}

It is not hard to see that the relaxation is tight provided that $d\geq 2k$ \ct{(This is loose. The $\X$ matrix is not gonna be full rank at the optimal. For example, we can add without loss of generality the constraint that row-column sum of top $k\times k$ block is $0$)}. Indeed, for any $d\geq 2k$, we can decompose an optimal $\hat\X$ in factors $\hat\W$ and $\hat\Hb$ using Cholesky decomposition (see Lemma \ref{lem:chol}). It is easy to verify that these factors $\hat\W$ and $\hat\Hb$ are feasible in \eqref{eq:cvx_G}. Hence they are optimal.


 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%% December 6 -- optimize first over G, then over \la
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \subsection{Old}
%% Interestingly, the min-max problem in \eqref{eq:cvx_G} is convex-concave. {Also, it should be possible (check?) to show that the minimization can be equivalently performed in a bounded set.} Thus, by Sion's min-max theorem, we can flip the order of min-max. 
%%
%%For convenience, denote $\tilde\J_c:=\left(\Id+\ones\ones^T\right)\J_c$, $c\in[k].$ The objective can be written as 
%%$$
%%F(\G,\lab_c)= \frac{1}{2}\tr\left(\G \X \right) + \sum_{c\in[k]}n_c\lab_c^T\ones,
%%$$
%%where we defined
%%\begin{align}
%%\X := \Id - \sum_{c\in[k]} n_c \tilde\J_c^T\lab_c\lab_c^T\tilde\J_c.
%%\end{align}
%%
%%\begin{lemma}\label{lem:Gmin}
%%The following is true about the minimization over $G$:
%%\begin{align}
%%\min_{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}}\tr\left({\G\X}\right)=\begin{cases}
%%0 & \Pb^\perp_k\X\Pb^\perp_k\succeq \zeros \\
%%-\infty & \text{o.w.}
%%\end{cases}
%%\end{align}
%% \end{lemma}
%% Using Lemma \ref{lem:Gmin}, \eqref{eq:cvx_G} is reduces to the following maximization
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad \sum_{c\in[k]}n_c\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)^T\preceq \Pb^\perp_k
%% \end{align}
%% Using Schur-complement, we can write this as an SDP:
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad 
%% \begin{bmatrix} 
%%\Id_{k\times k}  & \sqrt{n_1}\tilde\J_1^T\lab_1 & \sqrt{n_2}\tilde\J_2^T\lab_2 & \cdots & \sqrt{n_k}\tilde\J_2^T\lab_2 \\
%% \sqrt{n_1}\lab_1^T\tilde\J_1  & 1 & 0 & \cdots & 0 \\  \sqrt{n_2}\lab_2^T\tilde\J_2  & 0 & 1 & \cdots & 0 \\  
%%\vdots & \vdots & \vdots & \cdots & \vdots \\
%%\\  \sqrt{n_k}\lab_k^T\tilde\J_1  & 0 & 0 & \cdots & 1  
%%  \end{bmatrix} \succeq \zeros_{2k \times 2k}
%% \end{align} 




%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\subsection{KKT conditions}
The Lagrangian of the convex problem of \eqref{eq:svm_original} is the following, for dual variables $\{\la_{i,c}\}, i\in[n], c\in[k], c\neq y_i$:
\begin{equation}
	\Ellc(\W, \Hb, \{\lambda_{i,c}\}) = \frac{1}{2}\sum_{c=1}^{K}\|\w_{c}\|^2+ \frac{1}{2}\sum_{i=1}^{N}\|\h_{i}\|^2 + \sum_{i\in[n]}\sum_{c'\neq y_i}\la_{i,c'}(1-\w_{y_i}^T\h_{i}+\w_{c'}^T\h_i)
\end{equation}
The KKT conditions are then as follows:
\begin{subequations}\label{eq:KKT}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}+\sum_{i:y_i\neq c}\la_{i,c}\h_i -\sum_{i:y_i=c}\Big(\sum_{c'\neq y_i} \la_{i,c'}\Big)\h_i = 0\\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{i\in[n]}\Big(\sum_{c'\neq y_i}\lambda_{i,c'}\Big)\w_{y_i}+\sum_{i\in[n]}\sum_{c'\neq y_i}\lambda_{i,c'}\w_{c'} = 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\lambda_{i,c} \geq 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \lambda_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}

The KKT conditions can be rewritten equivalently with respect to an augmented dual variable representation $\beta_{i,c}, i\in[n], c\in[k]$ as follows:
\begin{subequations}\label{eq:KKT_beta}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}-\sum_{i\in[n]}\beta_{i,c}\h_i  = 0 \,\Leftrightarrow\,  \W_{d\times k} = \Hb_{d\times n}\Bb^T_{n\times k} \\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{c\in[k]}\beta_{i,c}\w_c = 0\,\Leftrightarrow\,  \Hb_{d\times n} = \W_{d\times k}\Bb_{k\times n} \\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\beta_{i,c} \leq 0 \label{eq:beta_new}
	\\
	\forall i\in[n] \,&:\,\beta_{i,y_i} = -\sum_{c\neq y_i}\beta_{i,c}\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \beta_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}
To see that these are equivalent, set for all $i\in[n]$: $\beta_{i,c}=\begin{cases} \sum_{c'\neq c}\lambda_{i,c'} & c=y_i \\ -\lambda_{i,c} & c\neq y_i\end{cases}.$ Above, we have also defined an $k\times n$ matrix $\Bb$ with entries $[\Bb]_{c,i}=\beta_{i,c}.$ From constraint \eqref{eq:beta_new} it follows that $\Bb$ has column-sum equal to zero, i.e. $\Bb^T\ones_{k}=0.$ For instance this immediately yields $\W\ones_{k}=0$ (which we proved from first principles in Lemma \ref{lem:centering}).

Also, note that the first two conditions imply
\begin{align}
\Hb^T\W = \Hb^T\Hb \Bb^T \qquad\text{and}\qquad \W^T\Hb = \W^T\W\Bb.
\end{align}
Hence,
\begin{align}
\X_{(k+n)\times (k+n)}:=\begin{bmatrix}\W^T\W & \W^T\Hb \\ \Hb^T\W & \Hb^T\Hb\end{bmatrix}=\begin{bmatrix}\W^T\W & \zeros_{k\times n} \\ \zeros_{n\times k} &\Hb^T\Hb\end{bmatrix}
\underbrace{\begin{bmatrix}\Id_{k\times k} & \Bb_{k\times n} \\ \Bb^T_{n\times k} & \Id_{n\times n}\end{bmatrix}
}_{\widetilde{\Bb}}.
\end{align}
and
\begin{align}
\tr\Big(\widetilde{\Bb}^T\X \Big) = \tr\Big(\widetilde{\Bb}\cdot {\rm{bldiag}}(\W^T\W,\Hb^T\Hb) \cdot\widetilde{\Bb}\Big)
\end{align}




%A possibly interesting observation here is the following.
%\begin{lemma} Suppose $(\W,\Hb,\Bb)$ satisfy the KKT conditions \eqref{eq:KKT_beta}. If $\Bb$ is such that $\Id_{k\times k} \succeq \Bb\Bb^T$, then the matrix $\X=\begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix}$ is a solution to the SDP in \eqref{eq:cvx_X}.
%\end{lemma}




==> sections_v2/commands.tex <==
% Alternative minipage environment, renders better in terms of spacing

%\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsfig,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,multirow,comment, boldline}
\usepackage{hyperref,graphicx,amsmath,amsfonts,amssymb,bm,url,breakurl,epsf,color,MnSymbol,mathbbol,fmtcount,semtrans,caption,multirow,comment, boldline}
%\usepackage[]{algorithm2e}
%\usepackage[noend]{algpseudocode}
\usepackage{wrapfig}
\usepackage{enumitem}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{dsfont}

\usepackage{xcolor}

\newlist{myitemize}{enumerate}{1}
\setlist[myitemize]{font=\color{darkred}\bfseries\itshape}

  \usepackage{mathtools}
% \DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\usepackage{titlesec}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}

\usepackage{movie15}

\usepackage{caption}
\usepackage[bottom,hang,flushmargin]{footmisc} 

\setlength{\captionmargin}{30pt}

\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

\newcommand{\darkred}{\color{darkred}}
\newcommand{\darkgreen}{\color{darkgreen}}
\newcommand{\darkblue}{\color{darkblue}}

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}
  
\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}

%------- new notation
\newcommand{\delmaj}{\delta_{\text{maj}}}
\newcommand{\delmin}{\delta_{\text{minor}}}

\newcommand{\LDT}{\text{LDT}}
\newcommand{\CDT}{\text{CDT}}
\newcommand{\CE}{\text{CE,binary}}
\newcommand{\SVM}{\text{SVM}}

\newcommand{\ibar}{\overline{i}}
\newcommand{\Xib}{\mathbf{\Xi}}
\newcommand{\Lcvs}{\Lc_{\text VS}}
\newcommand{\Zhatd}{\Zhat_{\deltab}}
\newcommand{\Ubd}{\Ub_{\deltab}}
\newcommand{\Vbd}{\Vb_{\deltab}}
\newcommand{\Lambdabd}{\Lambdab_{\deltab}}
\newcommand{\Zhateff}{\Zhat^\text{eff}}
\newcommand{\Ubeff}{\Ub^\text{eff}}
\newcommand{\Vbeff}{\Vb^\text{eff}}
\newcommand{\Lambdabeff}{\Lambdab^\text{eff}}
\newcommand{\nceff}{n_c^\text{eff}}
\newcommand{\neff}{n^\text{eff}}
\newcommand{\nbeff}{\mathbf{n}^\text{eff}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\Top}{\mathcal{T}}
\newcommand{\Reff}{R^\text{eff}}
\newcommand{\heff}{\h^\text{eff}}
\newcommand{\Hbeff}{\Hb^\text{eff}}
\newcommand{\Mbeff}{\M^\text{eff}}
% \newcommand{\Lambdabeff}{\Lambdab^\text{eff}}
\newcommand{\Whatcdt}{\What_\text{CDT}}
\newcommand{\Hhatcdt}{\Hhat_\text{CDT}}
\newcommand{\Whatldt}{\What_\text{LDT}}
\newcommand{\Hhatldt}{\Hhat_\text{LDT}}
\newcommand{\htildei}{\tilde{\h}_i}
\newcommand{\htilde}{\tilde{\h}}
\newcommand{\Hbtilde}{\tilde{\Hb}}
\newcommand{\Hbbar}{\overline{\Hb}}
\newcommand{\Mbbar}{\overline{\M}}
\newcommand{\Mbhat}{\hat{\M}}
\newcommand{\Hbbareff}{\overline{\Hb}^\text{eff}}
\newcommand{\Mbbareff}{\overline{\M}^\text{eff}}
\newcommand{\I}{\mathbf{I}}
%--------------
\newtheorem{observation}{Observation}
\newtheorem{finding}{Finding}
% \newtheorem{theorem}{Theorem}
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}{Lemma}[section]
%\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{propo}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}

%\newtheorem{remark}{Remark}[section]
%\newtheorem{remarks}[subsection]{Remarks}
%\newtheorem{example}{Example}

%------------------------

\newcommand{\Cos}[2]{\operatorname{cos}(#1,#2)}
\newcommand{\Coss}[2]{\operatorname{cos}\left(#1,#2\right)}

\newcommand{\wmaj}{\w_{\rm{maj}}}
\newcommand{\wmin}{\w_{\rm{minor}}}
\newcommand{\hmaj}{\h_{\rm{maj}}}
\newcommand{\hmin}{\h_{\rm{minor}}}

\newcommand{\mubmaj}{\boldsymbol{\mu}_{\rm{maj}}}
\newcommand{\mubmin}{\boldsymbol{\mu}_{\rm{minor}}}

\newcommand{\Q}{\mathbf{Q}}

\newcommand{\minor}{{\text{minor}}}
\newcommand{\maj}{{\text{maj}}}

\newcommand{\rank}{\operatorname{rank}}

\newcommand{\Ghat}{\hat{\G}}

\newcommand{\der}{\mathrm{d}}
\newcommand{\dert}{\mathrm{d}t}

\newcommand{\nbar}[1]{\overline{#1}}

\newcommand{\nmin}{n_{\text{min}}}

\newcommand{\Deltab}{\boldsymbol{\Delta}}

\newcommand{\rhobar}{\overline{\rho}}

\newcommand{\SEL}{{SEL}}
\newcommand{\SELd}{$\deltab$-{SEL}}
\newcommand{\SELI}{{SELI}}
\newcommand{\ETFmat}{\M^\star}

\newcommand{\dmin}{\delta_{\operatorname{minor}}}
\newcommand{\dmaj}{\delta_{\operatorname{maj}}}

\newcommand{\Sec}{Sec.}
\newcommand{\SM}{SM}

\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\diag}{diag}

\newcommand{\vbtilde}{\widetilde{\vb}}

\newcommand{\widesim}[2][1.5]{
  \mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}
}
\newcommand{\cut}[1]{\textcolor{red}{}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Ub}{\mathbf{U}}
% \newcommand{\nb}{\mathbf{n}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\Rb}{\mathbf{R}}

\newcommand{\Ellc}{\mathcal{L}}


\newcommand{\Wopt}{\W^*}
\newcommand{\Hopt}{\Hb^*}
\newcommand{\Mopt}{\Mb^*}
\newcommand{\wopt}{\w^*}
\newcommand{\hopt}{\h^*}
\newcommand{\mopt}{\mub^*}
\newcommand{\Hb}{{\mathbf{H}}}
\newcommand{\Mb}{{\mathbf{M}}}
\newcommand{\Hhat}{{\hat{\Hb}}}
\newcommand{\What}{{\hat{\W}}}
\newcommand{\what}{{\hat{\w}}}
\newcommand{\hhat}{{\hat{\h}}}
\newcommand{\Ubhat}{{\hat{\Ub}}}
\newcommand{\Vbhat}{{\hat{\Vb}}}
\newcommand{\Labhat}{{\hat{\Lambdab}}}
\newcommand{\Zhat}{{\hat{\Z}}}
\newcommand{\zhat}{{\hat{\z}}}
%\newcommand{\G}{{G}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\XXb}{\overline{\mathbf{X}}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Pb}{\mathds{P}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Qbf}{\mathbf{Q}}
\newcommand{\Pibf}{\boldsymbol{\Pi}}
\newcommand{\Xibf}{\boldsymbol{\Xi}}

\newcommand{\omegab}{\boldsymbol{\omega}}

\newcommand{\pbf}{\mathbf{p}}
\newcommand{\qbf}{\mathbf{q}}



%Bold lower
\newcommand{\lab}{\boldsymbol{\la}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\mubhat}{\hat{\boldsymbol{\mu}}}
\newcommand{\thetab}{{\boldsymbol{\theta}}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\ellb}{\boldsymbol{\ell}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\zo}{\overline{\mathbf{z}}}
\newcommand{\bseta}{{\boldsymbol{\eta}}}
\newcommand{\Iden}{\mathbf{I}}
\newcommand{\cb}{\mathbf{c}}  
\newcommand{\ab}{\mathbf{a}}
\newcommand{\oneb}{\mathbf{1}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\betab}{\boldsymbol{\beta}}
% \newcommand{\nceff}{n_c^\text{eff}}
%\newcommand{\tb}{\mathbf{t}}


%Calligraphic
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Ps}{\mathcal{P}}
\newcommand{\Rs}{\mathcal{R}}
\newcommand{\Tc}{{\mathcal{T}}}
\newcommand{\Sc}{{\mathcal{S}}}
\newcommand{\Bc}{{\mathcal{B}}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Zc}{\mathcal{Z}}
%\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Gc}{{\mathcal{G}}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Qc}{\mathbb{Q}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Ic}{\mathcal{I}}

%hat, tilde, etc
\newcommand{\vh}{\hat{v}}
%\newcommand{\alh}{\hat{\al}}
\newcommand{\thh}{\hat{\tau_{h}}}
\newcommand{\tgh}{\hat{\tau_{g}}}
%...

%Equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{align}}
\newcommand{\eea}{\end{align}}

\newcommand{\vp}{\vspace{5pt}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\nn}{\notag}

\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}

\newcommand{\rP}{\stackrel{{P}}{\longrightarrow}}

%% Greek
\newcommand{\al}{\alpha}
 \newcommand{\om}{\omega}
% \newcommand{\betabh}{\hat{\boldsymbol\beta}}
    \newcommand{\gammab}{\boldsymbol\gamma}
%        \newcommand{\etab}{\boldsymbol\eta}
 \newcommand{\chib}{\boldsymbol\chi}
 \newcommand{\Sigb}{\boldsymbol\Sigma}
  \newcommand{\Sigmab}{\boldsymbol\Sigma}
    \newcommand{\rhob}{\boldsymbol\rho}
  \newcommand{\la}{{\lambda}}                     % lambda
  \newcommand{\eps}{\epsilon}
    \newcommand{\Lambdab}{\boldsymbol{\Lambda}}                     % lambda
\newcommand{\Xhat}{\hat{\X}}
 \newcommand{\deltab}{\boldsymbol\delta}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% FAIRNESS paper %%%%%%%%%%%%%%
\newcommand{\Rcbal}{\Rc_{\text{bal}}}
\newcommand{\Rco}{\overline\Rc}
\newcommand{\Rcbalinf}{\overline{\Rc}_{\text{bal}}}
\newcommand{\Rtrain}{\Rc_{\text{train}}}
\newcommand{\Rdeo}{\Rc_{\text{deo}}}
\newcommand{\wh}{\hat{\w}}
\newcommand{\bh}{\hat{b}}
\newcommand{\ind}[1]{\mathds{1}[#1]}

\newcommand{\bt}{\tilde b}
\newcommand{\qt}{\tilde q}
\newcommand{\rhobt}{\tilde \rhob}
\newcommand{\rhot}{\tilde \rho}

\newcommand{\bomega}{\bar\omega}

\newcommand{\vbh}{\hat\vb}

%\newcommand{\wt}{\overline}

\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\newcommand{\Del}{\Delta}
%\newcommand{\om}{\omega}
%\newcommand{\wt}{\widetilde\w}

\newcommand{\wt}{\widetilde}

\newcommand{\B}{\mathbf{B}}

\newcommand{\Id}{\mathds{I}}
\newcommand{\Jd}{\mathds{J}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\zeromat}{{[0]}}
\newcommand{\zeros}{\mathbf{0}}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\abs}[1]{\lvert#1\rvert}

\newcommand{\wte}{\widetilde}

==> sections_v2/conclusions.tex <==
\vspace{-0.3cm}
We have shown consistent empirical and theoretical evidence that SCL learns training embeddings that converge to the OF geometry irrespective of the level of class imbalance. We believe this finding contributes a unique result to the growing literature of neural-collapse / implicit-geometry phenomena. For balanced data, we extend the contributions of \citet{graf2021dissecting} to the case in presence of ReLU activations. Further, our results identify exact conditions on the mini-batch selection to achieve the OF geometry, allowing for a wider set of possibilities in batching than found by \cite{graf2021dissecting} for SCL without ReLU. For imbalanced data, our results are the first explicit characterization of the geometry, concluding that imbalances do \emph{not} alter the geometry if a ReLU activation is added at the last layer. In both cases, these advancements are achieved by analyzing a refined UFM model, \ref{eq:SCL_UFM_full}, that closely aligns with experimental conditions by constraining embeddings to the non-negative orthant. This model also leads to new findings about the intricate role of batching in SCL optimization, that may be of independent interest. A future investigation of exact characterization of the geometry with imbalances and without ReLU can help complete the understanding of the implicit-geometry of SCL. Although the majority of implicit geometry characterizations in the literature require $d>k$, it is interesting to extend our findings to settings where $d<k$ following the steps of \cite{gao2023study} for the CE loss. Likewise, our finding regarding the crucial role of batching in geometry opens the door to further investigations aimed at devising efficient batch strategies in cases with a large number of classes.
Finally, like most studies on neural-collapse phenomena, our results share a common limitation: they only provide insights into the behavior during training. On the other hand, there is a line of research that explores algorithmic modifications to SCL \citep{gunel2020supervised,jitkrittum2022elm,samuel2021distributional,li2022targeted,kang2021exploring,li2022targeted}, often rooted but not explicitly connected to geometric principles, to enhance generalization under imbalances. Ultimately, we envision the two research streams merging through the ongoing exchange of ideas.

% \todo{below is OLD; refer to Graf Conclusion- nicely written}We find that training with the supervised contrastive loss results in training features that exhibit neural collapse and form an orthogonal frame. Importantly, this phenomenon is insensitive to changes to the distribution of labels in the training set. We provide empirical evidence through experiments on standard vision models. The invariance stands in contrast with the behavior of features learned by the cross entropy loss. Studying the UFM with SCL optimization in the non-negative orthant, thus incorporating the impact of ReLU activations, we prove that the OF minimizes the loss. We expect that this observation has practical significance in helping guide appropriate training methodology, in addition to the existing empirical evidence on the superior quality of SCL. Through analytical arguments, we discover favorable nature of batching of examples, and demonstrate an effective scheme to ensure OF features in any given batching.

==> sections_v2/convex_forms.tex <==
\subsection{Convex Equivalent form: Nuclear norm}\label{eq:svm_z_nuc}
\begin{align*}
	&\quad  \min_{\Z}~\|\Z\|_*
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\Z}~\left[\min_{\W,\Hb \ \text{s.t.} \ \W\Hb = \Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)\right]
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1
\end{align*}

%\subsection{Equality of margins/activeness of constraints:}
%\begin{center}
%	\begin{tabular}{||c ||c | c|| c | c ||} 
%		\hline
%		& BalERM-CE & BalSVM & ImbalERM-CE & ImbalSVM \\ [0.5ex] 
%		\hline\hline
%		$(\W,\Hb)$ & Equal & Active & Unequal & Active \\ 
%		\hline
%		$\Z$ & Equal & Active & Equal & Active \\ 
%		\hline
%		$\X$ &  &  &  &  \\ [1ex] 
%		\hline
%	\end{tabular}
%\end{center}


==> sections_v2/exp_appex_old.tex <==
\subsection{Details on the main experimental setup}\label{sec:exp_details_SM}
In our deep-net experiments, we focus on two common network architectures, ResNet and DenseNet. Specifically, we use ResNet-18 and DenseNet-40 with approximately $11$ million and $200$ thousand trainable parameters, respectively. For both models, we replace the last layer linear classifier with a normalization layer (normalizing such that $\| \h_i\|=1$ for $i \in [n]$) of feature dimension $d=512$. Specifically, following  \cite{graf2021dissecting}, we  directly optimize the normalized features that are then used for inference. (We note this is slightly different compared to \cite{khosla2020supervised}, where the authors train the output features of a projection head, then discard this projection head at inference time). We remark that both ResNet and DenseNet architectures include ReLU activations before the final output, which enforces a non-negativity on the learned embeddings. Resnet-18 models with CIFAR10, MNIST and FashionMNIST have been trained for 350 epochs with a constant learning rate of $0.1$, no weight decay, batch size of $1024$, and SCL temperature parameter $\tau = 0.1$ (consistent with the choice of $\tau$ made in \cite{khosla2020supervised,graf2021dissecting}). For all experiments with other models or datasets, we provide experimental details in the following sections. All models, regardless of architecture or dataset, have been trained on a single Tesla V100 GPU machine. 

% All ResNet models were trained for 350 epochs with a constant learning rate of $0.1$ and no weight decay. On the other hand, we observed slower convergence to OF geometry when training our DenseNet models on more complex datasets such as CIFAR10, and larger imbalance ratios $\RT$. To combat this, we increased the number of training epochs to 500 while annealing the learning rate by a factor of 0.1 on epoch 300, reduced to batch size to 128 to increase number of back-propagation iterations, and used binding examples to improve convergence speed. 

%\todo{Remove the following?}
%Given our focus on feature geometry, we did not perform any data augmentation to increase convergence speed.  \vala{mention this ? We did perform experiments with common-practice data augmentation techniques which showed general convergence towards OF, but more iterations for better convergence}.

% \vala{Do we need further specific detail for each ? }

% \noindent\textbf{Details for Fig.~\ref{fig:intro}} 

% \noindent\textbf{Details for Fig.~\ref{fig:GM matrices comparison}}

\subsection{Additional geometric analysis}
     
     In addition to analyzing the convergence of the Gram-matrix of class-mean embeddings $\G_\M$ to the OF geometry (as provided in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}), we also keep track of Neural Collapse (Defn.~\ref{def:nc}) of individual embeddings and orthogonality of their class-means (Defn.~\ref{def:of}) separately. Furthermore, we qualitatively study the Gram matrices $\G_\M$ and $\G_\Hb$  and compare them to corresponding matrices for the CE loss under imbalances. 
     
     \noindent\textbf{Neural Collapse.}~
     In order to quantify the collapse (NC) of embeddings, $\h_i, i \in [n]$, to their class-means,  we measure $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ \cite{NC}. Here, $\Sigma_B= \sum_{c\in [k]}(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})^\top$ is the between class covariance matrix, $\boldsymbol{\mu}_G = \frac{1}{k}\sum_{c\in[k]}\boldsymbol{\mu}_c$ is the  global mean, and $\Sigma_W  = \sum_{i\in [n]}(\h_i - \boldsymbol{\mu}_{y_i})(\h_i - \boldsymbol{\mu}_{y_i})^\top$ is the within class covariance matrix.

     For the experiments shown in Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu} and Fig.~\ref{fig:loss_convergence} in the main body, the corresponding values of $\beta_\text{NC}$ can be found in Fig.~\ref{fig:Deepnet_SCL_Geom_NC} and Fig.~\ref{fig:loss NC and angle convergence SM}(b) respectively.

     
    % \begin{figure*}[h]
    %     % \centering
    %     \hspace*{-16pt}
    %     \begin{subfigure}[b]{\textwidth}
    %         \centering
    %         \begin{tikzpicture}
    %             \node at (0.0,0) 
    %             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
    %             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    %             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
    %             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
    %             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
    %             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
    %             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
    %             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
    %         \end{tikzpicture}
    %     \end{subfigure}
    %     % \vspace{-10}
    %     \caption
    %     {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values }
    %     \label{Fig:Deepnet_SCL_Geom_NC}
    %     % \vspace{-15}
    % \end{figure*}

    \begin{figure}[t]
    % \centering
    %\hspace*{-20pt}
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Exp/NC_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.3) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.3) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.3) [scale=0.9]{\textbf{FMNIST}};
            \node at (-7.8,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-7.8,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.3) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Neural Collapse metric $\beta_\text{NC}:=\tr(\Sigma_W\Sigma_B^\dagger)/k$ for corresponding ResNet-18 training results from Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Values are usually on the order of $10^{-3}$ suggesting strong convergence of embeddings to their class means.}
    \label{fig:Deepnet_SCL_Geom_NC}
\end{figure}

    \noindent\textbf{Angular convergence.}~
    Having confirmed convergence of embeddings to their respective class-means via NC ($\h_i \approx \mub_c $ for $i:y_i = c$), we can now compare the feature geometry to the OF geometry by calculating the average $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ between each pair of classes. Fig.~\ref{fig:Deepnet_SCL_Geom_angles} plots the average cosine similarity $\text{Ave}_{c\neq c'}\alpha_{\text{sim}}(c,c')$ between class means for the same experiment as that 
 of Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. The graphs indicate strong convergence to orthogonality between feature representations of different classes. Similarly, results for angular convergence corresponding to Fig.~\ref{fig:loss_convergence} are provided in Fig.~\ref{fig:loss NC and angle convergence SM}(c), indicating similar convergence to OF for the full-batch experiments.

    \begin{figure}[h]
    % \centering
    %\hspace*{-20pt}
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.975\textwidth]{Figs/Deepnet_Geometry_Exp/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.3) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.3) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.3) [scale=0.9]{\textbf{FMNIST}};
            \node at (-7.6,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-7.6,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.3) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $10^{-2}$, indicating strong orthogonality between class-mean embeddings.}
    \label{fig:Deepnet_SCL_Geom_angles}
\end{figure}

%     \begin{figure*}[h]
%     % \centering
%     \hspace*{-16pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/Angles_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-3.2,2.5) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.3,2.5) [scale=0.9]{\textbf{MNIST}};
%             \node at (3.5,2.5) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-5.6,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-5.6,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
%         \end{tikzpicture}
%     \end{subfigure}
%     % \vspace{-10}
%     \caption
%     {Average cosine similarity between different class means $\alpha_{\text{sim}}(c,c') := \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_c\|\|\mub_{c'}\|}$ for corresponding results from ~\ref{Fig:Deepnet_SCL_Geom_GMu}. Final values are mostly on the order of $1e-2$, indicating strong orthogonality between features from different classes assuming Neural Collapse property holds.}
%         \label{Fig:Deepnet_SCL_Geom_NC}
%     \label{Fig:Deepnet_SCL_Geom_GMu}
%     % \vspace{-15}
% \end{figure*}

     \noindent\textbf{Feature embedding heatmaps.}~
     %\vala{This part could be rephrased to only include the $\Hb^T\Hb$ score, unless we want to include the case with normalizing CE.}
     As a qualitative measure, we have generated heatmaps  that visually represent the learned embedding geometries; see Fig.~\ref{fig:GM matrices comparison}, \ref{fig:GM matrices comparison_old}, \ref{fig:GH matrices}. Specifically, we generate heatmaps of the Gram-matrices $\G_\M = \M^\top\M$ and $\G_\Hb = \Hb^\top\Hb$. In Fig.~\ref{fig:GM matrices comparison} we train ResNet-18 with the full MNIST dataset. In Fig.~\ref{fig:GM matrices comparison_old} we run on a subset of the dataset ($n = 10000$ total examples) with a batch size of 1000. Specifically for Fig.~\ref{fig:GM matrices comparison_old}, when optimizing with CE loss we modify the network (ResNet-18) such that it has a normalization layer before the linear classifier head. We consider this additional setting to allow for a comparison where CE features are constrained to the unit sphere akin to our SCL experiments. Lastly, in Fig.~\ref{fig:GH matrices} we plot the learned features Gram-matrix $\G_\Hb$ for a ResNet-18 trained on CIFAR10 ($n = 10000$ total examples) with a batch size of $1000$.\footnote{In both Fig.~\ref{fig:GH matrices} and Fig.~\ref{fig:GM matrices comparison_old} no batch duplication is used as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}.} This heatmap qualitatively shows a more complete picture as we are plotting $\G_\Hb = \Hb^\top \Hb$ rather than $\G_\M$, thus simultaneously illustrating both Neural Collapse and convergence to the k-OF structure.  
    \begin{figure*}[h]
        \centering
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{SCL}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        %\hspace*{-20pt}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2.2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
       % \vskip\baselineskip
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm1CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.5,0.0)  [scale=0.9, rotate=90]{\textbf{CE}};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm10CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
               \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.29\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gm_Heatmap_Plots/Gm100CE.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,1.8) [scale=0.9]{\textbf{}};
                \node at (-2.4,0.0)  [scale=0.9, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GM]
        {$\G_\M$ Gram-matrices of mean-embeddings for various $R$-STEP imbalances at last epoch (350) of training with ResNet-18 on MNIST with $n = 10000$. To allow for fair comparison, the CE features are normalized before the classifier head akin to the SCL experiments.} 
        \label{fig:GM matrices comparison_old}
    \end{figure*}
  \begin{figure*}[h]
        \centering
        \hspace{-0.5in}
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh1.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 1}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh10.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 10}};
               \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Gh_Heatmap_Plots/Gh100.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
    			\node at (0.0,2) [scale=0.9]{\textbf{R = 100}};
                \node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \caption[GH]
        {$\G_\Hb$ Gram-matrices of feature embeddings for various imbalances at last epoch (350) of training SCL with CIFAR10 and ResNet.} 
        \label{fig:GH matrices}
    \end{figure*}
\subsection{Optimization dynamics}

\noindent\textbf{Loss convergence.}~
     In order to compute the lower bounds shown in Fig.~\ref{fig:loss_convergence},  we use Thm.~\ref{thm:scl_full}, substituting $e^{-1}$ with $e^{-1/\tau}$ using $\tau = 0.1$ as employed in our experiments; this substitution is allowed thanks to  Remark \ref{rem:tau}. Furthermore, we compute the lower bounds and $\Lc(\Hb)$ on a per sample basis, thus we divide by $n = 1000$ which corresponds to the number of datapoints in our single batch. Lastly, as a method of maintaining numerical stability (as implemented in \cite{khosla2020supervised}) we apply a global scaling of the loss by a factor $\nicefrac{\tau}{\tau_b}$, where $\tau_b = 0.07$ is the base temperature \cite{khosla2020supervised}. The complete experiment, conducted over $2000$ epochs (with axes limited to $500$ epochs for clarity in Figure~\ref{fig:loss_convergence}), is available in Figure~\ref{fig:loss NC and angle convergence SM}.

      \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/LossCompToLowerBound.pdf}};
                 \node at (0.1,-1.97) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(a) Loss}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/NC.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.2,-1.8) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(b) NC}};
               %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.325\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/PairWiseAngles_corrected_small.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.13,-1.9) [scale=0.7]{Epoch};
    			\node at (0.0,1.95) [scale=0.9]{\textbf{(c) Angles}};
                %\node at (-2.7,0.0)  [scale=0.7, rotate=90]{};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a $\RT$-STEP imbalanced subset of MNIST of size $n=1000$. \textbf{(a)} Loss converges to the lower bound (dashed lines) computed in Thm.~\ref{thm:scl_full}. 
        \textbf{(b)} Within-class feature variation becomes negligible (NC). \textbf{(c)} The average pairwise cosine similarity of class-means approaches zero. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:loss NC and angle convergence SM} 
    \end{figure*}

\noindent\textbf{Effect of $\tau$.}~
%\vala{Maybe we should discuss this a bit}
As described in Sec.~\ref{sec:Deepnet_SCLGeom_exp} and Sec.~\ref{sec:full_batch_theory} the optimality of the OF geometry for the \ref{eq:SCL_UFM_full} is invariant to the choice of the temperature parameter $\tau$. However, we have found that the speed of convergence to the OF geometry is dependent on the choice of $\tau$. Shown in Fig.~\ref{fig:effect of tau full batch} is a full batch SCL experiment on $n=1000$ samples of MNIST trained on ResNet-18 with $\tau = 0.1, 1, 10$. It is clear from Fig.~\ref{fig:effect of tau full batch} that: (a) the within-class feature variation converges significantly faster for smaller $\tau$; (b) the angles converge to k-OF faster and smoother for smaller $\tau$ as well (see Fig.~\ref{fig:effect of tau full batch} (b)). In all cases, values of $\beta_\text{NC}$ and  $\alpha_{\text{sim}}(c,c')$ continue to decrease, and we anticipate further convergence if the networks are trained for longer. These results qualitatively agree with the findings of  \cite{khosla2020supervised} which suggest that smaller $\tau$ improves training speed. 
\begin{figure*}[h]
        \centering
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0.0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/NC.pdf}};
                 \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(a) NC}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                 \node at (-3,0.0)  [scale=0.9, rotate=90]{$\beta_\text{NC}
                 $};
            \end{tikzpicture}
        \end{subfigure}
       %\hfill
       \hspace{0.5in}
        \begin{subfigure}[b]{0.4\textwidth}
            \centering
            \begin{tikzpicture}
                \node at (0,0) 
                {\includegraphics[width=\textwidth]{Figs/tau_fullbatch/PairWiseAngles_corrected.pdf}};
                % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
                \node at (0.0,-2.4) [scale=0.7]{Epoch};
    			\node at (0.0,2.47) [scale=0.9]{\textbf{(b) Angles}};
               \node at (-3.4,0.0)  [scale=0.9, rotate=90]{$\text{Ave}_{c \neq c'}\text{ }\alpha_{\text{sim}(c,c')}$};
               % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
            \end{tikzpicture}
        \end{subfigure}
        \captionsetup{width= \linewidth}
        \caption[loss]
        {Full-batch SCL: ResNet-18 trained on a subset of MNIST of size $n=1000$ with different temperature parameters $\tau$. \textbf{(a)} Within-class feature variation (NC). \textbf{(b)} Average pairwise cosine similarity of class-means. Each epoch is equivalent to one iteration of gradient descent.}
        \label{fig:effect of tau full batch} 
    \end{figure*}

\subsection{Implications of batch-binding}
In this section, we describe examples where batching methods and batch-binding help improve the convergence speed of embeddings geometries to OF. 

\noindent\textbf{How batch-binding ensure unique OF geometry.}~ %In Fig.~\ref{fig:Binding_Examples_Visuals}, we provide a simple illustration to how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}. We believe that there may exist other methods to ensure conditions required for unique OF geometry; however, adding the same $k$ examples to each batch is a straightforward solution to ensuring OF and is usually computationally inexpensive as batch sizes tend to be larger than number of classes $k$. \vala{Rephrase ?} 
Fig.~\ref{fig:Binding_Examples_Visuals} provides a simple illustration demonstrating how adding binding examples can satisfy the requirements of Cor.~\ref{cor:batch}.
While there are alternative approaches to satisfy the graph conditions stated in Cor.~\ref{cor:batch} for ensuring a unique OF geometry, the method of adding the same $k$ examples to each batch is a straightforward technique that is often computationally efficient, considering that batch sizes typically exceed the number of classes $k$.

\begin{figure}%
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.65\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_1.pdf} }}%
    \newline
    \centering
    \subfloat[\centering]{{\includegraphics[width=0.36\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_2.pdf} }}%
    \qquad
    \subfloat[\centering]{{\includegraphics[width=0.32\linewidth]{Figs/BindingExamples_visuals/BatchConnectivity_3.pdf} }}%
    \caption{A simple illustration to explain how adding binding examples to each batch satisfies the requirements of Cor.~\ref{cor:batch}, thus leads to unique OF geometry. \textbf{(a)} Gives a $3$ class (black, grey and white) classification  example with 3 batches. In addition to the data for each batch (included in red), the binding examples $1,2,3$ are added to each batch. \textbf{(b)} Gives the Batch Interaction Graph for the induced subgraph $G_1$ of the class (black) of example $1$
    %class $G_{1}$ 
    and illustrates how all batches are connected through examples $1$, satisfying the first condition of Cor.~\ref{cor:batch}. \textbf{(c)} Elaborates on how all three class  graphs $G_1,G_2,G_3$ are connected through the interactions of data points $1,2,3$, satisfying the second condition of Cor.~\ref{cor:batch}.}
    \label{fig:Binding_Examples_Visuals}%
\end{figure}

\noindent\textbf{Improving convergence for CIFAR100.}~
In addition to the benchmark datasets previously explored, we consider the convergence of ResNet-18 embeddings to the OF geometry when trained with CIFAR100. The models are trained for $500$ epochs with a constant learning rate of $0.1$ and a batch size of 1024. With a large number of classes ($k = 100$ for CIFAR100) it becomes increasingly more likely for the randomly reshuffled batches to violate the conditions required for achieving unique OF based on  Cor.~\ref{cor:batch}. Particularly for large imbalance ratios (e.g., $R=100,50$), since the number of samples in each minority class could become as low as $5$-$10$, some batches might never encounter examples from minority classes. However, including the binding examples in each batch can improve the convergence of the feature geometry to OF. In Fig.~\ref{Fig:Deepnet_SCL_CIFAR100_GMu} we measure the convergence of ResNet-18 trained both with and without the batch-binding. Batch-binding considerably expedite and improve the convergence to the OF geometry. This is particularly noticeable for STEP-Imbalance and large imbalance ratios, where half of the classes are minorities, thus the inclusion of binding examples becomes crucial in ensuring that our theoretical convergence requirements for reaching the OF are satisfied.


\noindent\textbf{Improving DenseNet convergence by batch-binding.}~
When conducting our experiments for Fig.~\ref{fig:intro}, we have noticed that DenseNet-40 converges significantly slower  compared to ResNet-18. A potential reason for this may be related to the very different complexities of the two models: ResNet-18 has significantly more trainable parameters compared to DenseNet-40. In an attempt to improve the convergence speed, we have decided to reduce the batch size for DenseNet to $128$ in order to increase the number of possible back-propagation steps. We have also trained the DenseNet models for $500$ epochs instead of $350$ and we have reduced the learning rate from $0.1$ to $0.01$ at epoch $300$. Yet, we have observed that with much smaller batch sizes, the embedding geometry does not always converge to the OF geometry, especially when training with high imbalance ratios.  Specifically when training with randomly reshuffled batches, there is always a  chance that the Batch Interaction Graph does not meet the requirements of Cor.~\ref{cor:batch}, implying that the optimal solution for all batches is not necessarily OF. We hypothesize that this likelihood increases when using smaller batch sizes during training. In order to combat this effect, we have decided to run the DenseNet experiments with the addition of binding examples to every batch. 
As suggested by Fig.~\ref{Fig:DenseNet_BindingsComparison}, we find that adding such binding examples significantly improves the convergence to OF. This is particularly so when training on more complex datasets (CIFAR10 compared to MNIST) and under more severe imbalances (STEP imbalance with $R= 50,100$). These results emphasize the impact of batch-binding and provide further evidence regarding our claims in Sec.~\ref{sec:mini_batch_theory}. While the convergence values of $\Delta_{\G_\M}$ are higher when compared to ResNet-18, we deem them reasonable  considering the difference in the number of parameters between the two architectures. Similar to ResNet-18, we have provided geometric convergence results for DenseNet-40 in Fig.~\ref{Fig:Deepnet_SCL_DenseNet_Geom}.

\begin{figure}[h]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Cifar100/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.7) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.1) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.7) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of embeddings geometry to OF as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$ for a ResNet-18 models trained on imbalanced CIFAR100 with SCL. Models are trained with both random-shuffling and random-shuffling with batch-binding. We see how the inclusion of binding examples helps with convergence to OF, especially under $R$-STEP imbalance and large imbalance ratios.}
    \label{Fig:Deepnet_SCL_CIFAR100_GMu}
\end{figure}


 \begin{figure}[ht]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,2.07) [scale=0.9]{\textbf{Step}};
            \node at (2.6,2.07) [scale=0.9]{\textbf{Long-tail}};
            \node at (-6.25,0.0)  [scale=0.9, rotate=90]{$\Delta_{\G_\M}$};
            \node at (0.2,-2.07) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a ResNet-18 model trained on CIFAR10 under STEP imbalance, with data augmentation. Results represent the average run results over 5 versions of the experiments with randomly chosen binding examples from each class. 
    }
    \label{Fig:error_bars_plotGM}
\end{figure}




\begin{figure}[h]
    % \centering
    \hspace*{-5pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots_compareBindings.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-2.4,3.8) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,4.3) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (2.6,3.8) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (-6.2,1.6)  [scale=0.9, rotate=90]{\textbf{CIFAR10}};
            \node at (-6.2,-1.2)  [scale=0.9, rotate=90]{\textbf{MNIST}};
            \node at (0.2,-3.8) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \caption
    {Convergence of $\G_\M$ to the OF geometry for a DenseNet-40 model trained on CIFAR10 and MNIST under STEP imbalance with and without batch-binding. While the impact of batch-bindings is less noticeable when training on a simple dataset such as MNIST,  the convergence is significantly improved, particularly under imbalance, when training on a more complex dataset such as CIFAR10. %\vala{rewrite this ? add explanation in text} \ct{reads good !}
    }
    \label{Fig:DenseNet_BindingsComparison}
\end{figure}




\begin{figure*}[h]
    % \centering
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/GMu_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{$\G_\M$ Convergence to OF}
    \end{subfigure}
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/NC_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Neural Collapse}
    \end{subfigure}
    % \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=\textwidth]{Figs/DenseNet_Geometry/Angles_Convergence_plots.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.2,3.5) [scale=0.9]{\textbf{CIFAR10}};
            \node at (0.4,3.5) [scale=0.9]{\textbf{MNIST}};
            \node at (4.8,3.5) [scale=0.9]{\textbf{FMNIST}};
            \node at (-8.2,1.5)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-8.2,-1.3)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.4,-3.37) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
        \caption{Angles between class-means}
    \end{subfigure}
    \caption
    {Geometric convergence of embeddings (as based on Def.~\ref{def:nc}, Def.~\ref{def:of}, and Def.~\ref{def:ncof}) of DenseNet-40. We measure: \textbf{(a)} $\Delta_{\G_\M}$, \textbf{(b)} $\beta_{\text{NC}}$, and \textbf{(c)} $\text{Ave}_{c \neq c'} \alpha_{\text{sim}}(c,c')$ as defined in text.}
    \label{Fig:Deepnet_SCL_DenseNet_Geom}
\end{figure*}


\noindent\textbf{Impact of batch-binding on generalization.}~ 
To study the effect of binding examples on generalization, we  consider the \textit{Nearest Class Center} (NCC) classifier. For this, each test example is assigned the label of the class center $\mub_c$ learned during training that is closest to it (in Euclidean distance). We consider a simple setup of training a ResNet-18 model on CIFAR10 under imbalances $R = 10,100$ both with and without the binding examples. Models are trained with a batch size of $128$ for $350$ epochs. We start with a learning rate of $0.1$, which is reduced by a factor of 10 on epochs $250$ and $300$. Weight decay is set to $5\times10^{-4}$.
In addition, we apply data augmentation as it is common practice when considering generalization and test accuracy. In particular, rather than simply adding horizontally flipped images (as described in Sec.~\ref{sec:Deepnet_SCLGeom_exp}) we allow for generic augmentations that include simple horizontal or vertical flips and random cropping with a probability of $0.5$. %In order to help with the convergence speed, we implement the augmentation on the duplicate version of the batches which are added to each batch (previously, this duplicate batch simply included a horizontally flipped version of each data point). These augmentations include simple horizontal or vertical flips and random cropping with a probability of $0.5$.  
The NCC test accuracy was measured across $5$ versions of the experiment with the $k$ binding examples sampled randomly every time and $5$ versions without any batch-binding. The results for NCC balanced test accuracies are provided in Table~\ref{Tab:NCC_Bindings}. While making definitive conclusions regarding the impact of the embeddings geometries and binding examples on generalization requires further investigation, this preliminary investigation suggests that batch-bindingdoes \emph{not} negatively impact NCC test accuracy.
\begin{table}[ht]
  \caption{NCC test accuracy for Batch-Binding}
  \hspace*{-20pt}
  \label{Tab:NCC_Bindings}
  \centering
  \begin{tabular}{l|ll|ll}
  \toprule
    & \multicolumn{2}{c}{Step} & \multicolumn{2}{c}{Long-tail}\\ 
    \cmidrule(r){2-3} \cmidrule(r){4-5}
    Ratio \\ ($R$)      & Reshuffling  & Reshuffling & Reshuffling  & Reshuffling \\ & & + Batch-Binding &  & + Batch-Binding  \\ 
    \midrule
    $10$ & $83.31 \pm 0.65 \%$ &   $83.27 \pm 0.27 \%$  & $85.04 \pm 0.28 \%$  &  $85.03 \pm 0.57 \%$  \\
    $100$     & $64.07 \pm 1.79 \%$ & $64.18 \pm 1.25 \%$   &  $67.75 \pm 1.21 \%$ & $68.08 \pm 0.72 \%$\\
  \end{tabular}
\end{table}

Finally, Fig.~\ref{Fig:error_bars_plotGM} shows convergence of embeddings geometry to OF for the same experiments. As expected, the convergence is slightly slower in this case due to the inclusion of data augmentation (random crops and flips).

% \begin{table}
%   \caption{NCC test accuracy for Binding Examples}
%   \label{Tab:NCC_Bindings}
%   \centering
%   \begin{tabular}{lll}
%   \toprule
%     \multicolumn{3}{c}{Step} \\ 
%     \cmidrule(r){1-3}
%     Ratio ($\RT$)      & Random Reshuffling  & Random Reshuffling \\ & & + Binding Example  \\ 
%     \midrule
%     $10$ & $83.19 \%$ &   $83.27 \pm 0.27 \%$      \\
%     $100$     & $61.76 \%$       & $64.18 \pm 1.25 \%$  \\
%     \bottomrule
%     \multicolumn{3}{c}{Long-tail} \\
%     \cmidrule(r){1-3}
%     Ratio ($\RT$)      & Random Reshuffling  & Random Reshuffling \\ & & + Binding Example \\
%     \midrule
%     $10$ & $84.65 \%$ &   $85.03 \pm 0.57 \%$      \\
%     $100$     & $69.71 \%$       & $68.08 \pm 0.72 \%$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}




% \pagebreak 

==> sections_v2/geometry.tex <==
\subsection{Centering}
In several previous works on the geometry of features learned by various loss functions \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring}, the theoretical model used, i.e. the UFM, did not constrain the sign of embedding coordinates. However, the experimental models often include several ReLU activations, leading to non-negativity constraints on the feature embeddings. To bridge this gap while comparing the geometry of empirical observations to the theoretical model predictions, a heuristic global mean centering is performed on the empirical embeddings. For the case of balanced labels, this \emph{centering} heuristic is as described as below \cite[e.g.,][]{NC,zhu2021geometric,fang2021exploring}:
\begin{align*}
    \mub_G &= \frac{1}{k}\sum_{c \in [k]}\mub_c,\ \ \Bar{\mub}_c = \mub_c - \mub_G,\ \ \Bar{\M} = \begin{bmatrix} \Bar{\mub}_1, \cdots, \Bar{\mub}_k \end{bmatrix}
\end{align*}
In our result, no such heuristic processing is required, as our model gives the geometry of embeddings as they are.

\subsection{OF vs ETF}
In this section we elaborate on the two geometries of interest- OF and ETF. Recall that our results show that the SCL with ReLU converges to the OF regardless of label distribution, whereas \cite{graf2021dissecting} showed that SCL without ReLU results in the ETF when label distribution is uniform. \new{For the reader's convenience, we recall the definition of simplex ETF from \cite{NC}:}
\new{
\begin{definition}[Simplex ETF]\label{def:etf}
    We say that $k$ vectors $\Vb = [\vb_1,\cdots,\vb_k] \in \R^{d\times k}$ form a simplex-ETF {if $\Vb^\top\Vb \propto \Id_k-\frac{1}{k}\ones_k\ones_k^\top$, i.e., for each pair of $(i,j)\in[k],$ $\|\vb_i\| = \|\vb_j\|$ and $\frac{\vb_i^T\vb_j}{\|\vb_i\|\|\vb_j\|} = \frac{-1}{k-1}$.} %\tina{need to define identity matrix somewhere earlier}
\end{definition}
}
\tina{I think for clarification, similar to OF, we need to mention that by ETF geometry we mean NC + mean-embeddings follow ETF. Have me mentioned this anywhere?}

\noindent\textbf{Mean-centered OF is ETF}: \new{The following straightforward lemma demonstrates that when a $k$-OF is centered, it transforms into an ETF.
\begin{lemma}
Suppose that a set of vectors $\{\vb_1,...,\vb_k\}$ form a $k$-OF in $\R^d$ with $d \geq k$, and their mean-centered counterparts are $\Bar{\vb}_c = \vb_c - \vb_G, \forall c \in [k]$, where $\vb_G = \frac{1}{k}\sum_{c\in[k]}\vb_c$.  Then, the centered embeddings $\{\Bar{\vb}_1,...,\Bar{\vb}_k\}$ form a simplex ETF spanning a $k-1$-dimensional subspace. 
\end{lemma}
\begin{proof}
Let $\Vb=\begin{bmatrix}
    \vb_1&\ldots&\vb_k
\end{bmatrix}$    and $\tilde\Vb=\begin{bmatrix}
    \tilde\vb_1&\ldots&\tilde\vb_k
\end{bmatrix}$. By definition of a $k$-OF, we know that $\Vb^\top\Vb\propto\Id$. Without loss of generality suppose the constant of proportionality is $1$ so that  $\Vb^\top\Vb=\Id\,.$ Since all $\vb_i$s are orthonormal, this then implies that $\Vb^T\vb_G=\frac{1}{k}\ones_k$ and $\vb_G^\top\vb_G=\frac{1}{k}\,.$ These put together gives the desired as follows:
\begin{align*}
    \tilde\Vb^\top\tilde\Vb &= \left(\Vb-\vb_G\ones_k^\top\right)^\top\left(\Vb-\vb_G\ones_k^\top\right) = \Vb^\top\Vb - \ones_k\vb_G^\top\Vb-\Vb^\top\vb_G\ones_k^\top+(\vb_G^\top\vb_G)\ones_k\ones_k^\top
    \\
    &=\Id_k - \frac{1}{k}\ones_k\ones_k^\top\,.
\end{align*}
\end{proof}
}

 Therefore, equivalently, the centered embeddings learned by deep-nets form an ETF. It is to be noted that our result shows this for an arbitrary label distribution, with balanced labels being a special case. 

On the other hand, it is not possible to obtain whether a set of vectors form an OF, given that their mean-centered versions make an ETF. This is because the unknown mean-vector can not be determined.


\subsection{UFM vs UFM$_+$: UFM fails to predict the geometry}
\tina{title?}

In this paper, we use the simplified \ref{eq:SCL_UFM_full} problem to describe the representations learned by deep-nets trained with SCL. Unlike many previous works studying the SCL or CE loss \cite{}, we impose ReLU (non-negativity) constraints on the embeddings in formulating the \ref{eq:SCL_UFM_full}. In Secs.~\ref{sec:Deepnet_SCLGeom_exp} and \ref{sec:theo_results}, we showed that regardless of the label configuration in the training set, the global optimizer of \ref{eq:SCL_UFM_full} is an OF and the embeddings learned by deep-nets converge to our prediction. On the other hand, when the training set is balanced, \citet{graf2021dissecting} showed that without the ReLU constraints, ETF minimizes the UFM. As discussed in Sec.~\ref{sec:}, we know that ETF is in fact the centered OF. Thus, in the balanced case, UFM provides a close prediction of the \emph{centered} embeddings. However, as we will show in the following lemma, the global optimizer of UFM is sensitive to label distribution in the training set, and ETF is not the global optimizer in the presence of imbalances. In other words, the difference between UFM and UFM$_+$ cannot be addressed by only considering the centering of the optimal embeddings.\tina{needs rewording}

\begin{lemma}
    Consider the \ref{eq:ufm} problem defined below. If classes in the training set are not balanced, % i.e., $\exists c,c'\in[k]$ such that $n_c\neq n_{c'}$, 
    the global solution of \ref{eq:ufm} is not necessarily an ETF. 

    \begin{align}\label{eq:ufm}
    \widehat{\Hb} \in \arg\min_{\Hb} \Lc_{\text{\emph{full}}}
    (\Hb)~~\text{\emph{subj. to}}~~\|\h_i\|^2 = 1,\, \forall i\in[n].
    \tag{$\text{UFM}$}
\end{align}
\end{lemma}
\begin{proof}
    To rule out the optimality of ETF in imbalanced setups, we show ETF does not minimize the loss in a $k=3$ class example. Specifically, consider a STEP-imbalanced training set with 3 classes of size $[\RT n_\text{min}, n_\text{min}, n_\text{min}]$ with $n_\text{min}\geq 2$ and $\RT \geq 10$. If $\Hb_\text{ETF}$ follows the ETF geometry, from Def.~\ref{def:etf} and the feasibility condition, for the mean-embeddings $\M_\text{ETF}$ we have $\M_\text{ETF}^\top\M_\text{ETF} = \frac{k}{k-1}(\Id_k - \frac{1}{k}\ones_k\ones_k^\top).$ Thus, the value of the loss function at ETF is as follows,
    \begin{align*}
        \Lc_{\text{{full}}}(\Hb_\text{ETF}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-\frac{3}{2}}\big) + 2\log\big(n_\text{min}-1+n_\text{min}(\RT+1)e^{-\frac{3}{2}}\big)\Big).
    \end{align*}
    Now, consider $\widetilde{\Hb} = [\widetilde{\mub}\otimes \ones_{\RT n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{ n_\text{min}}^\top, -\widetilde{\mub}\otimes \ones_{n_\text{min}}^\top]$, where $\norm{\widetilde{\mub}}=1$ and thus $\widetilde{\Hb}$ is in the feasible set. With this choice of $\widetilde{\Hb}$, we have,
    \begin{align*}
        \Lc_{\text{{full}}}(\widetilde{\Hb}) = n_\text{min} \Big(\RT \log\big(\RT n_\text{min}-1+2n_\text{min}e^{-2}\big) + 2\log\big(2n_\text{min}-1+\RT n_\text{min}e^{-2}\big)\Big).
    \end{align*}
    It is easy to check that, for imbalance levels higher than $\RT\geq10$, $$\Lc_{\text{{full}}}(\widetilde{\Hb}) < \Lc_{\text{{full}}}(\Hb_\text{ETF}).$$ In other words, when the imbalance level is large enough, ETF does not attain the optimal cost in \ref{eq:ufm}.
\end{proof}

==> sections_v2/implicitBias.tex <==
%\subsection{Cross-entropy}
%
%\begin{propo}[simple modification of \cite{ji2021unconstrained}]
%Even with imbalances, minimizing CE loss \eqref{eq:CE} converges in direction to a KKT point of the following margin-maximization problem:
%\begin{align}\label{eq:svm_original_implicit_bias}
%\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
%\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
%\end{align}
%\end{propo}
%
%\ct{@Ganesh: check and sketch proof}
%

\subsection{VS-loss}

\begin{propo}[simple modification of \cite{ji2021unconstrained}]
Consider minimizing the VS-loss  
\begin{align}\label{eq:VS}
\Lc(\W,\Hb) = \sum_{i\in[n]} \log\Big(1+\sum_{c\neq y_i}e^{-\Delta_{y_i}(\w_{y_i}-\w_c)^T\h_i}\Big).
\end{align}
Then, gradient descent iterates CE loss \eqref{eq:CE} converges in direction to 
\begin{align}\label{eq:cssvm_original_implicit_bias}
\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\Delta_{y_i}\w_{y_i}-\Delta_c\w_c)^T\h_i \geq 1
\end{align}
\end{propo}

==> sections_v2/implicit_bias.tex <==
\ct{@Ganesh: I moved the GD and logit regularization to Appendix, but feel free to reintroduce content in the main body as you see fit. Regarding logit regularization, where would this fit?}
\subsection{SVM solution is not a stationary direction of GD}

Let $\thetab := \vect(\W,\Hb) := [\w_1^T, \ldots, \w_k^T, \h_1^T, \ldots, \h_n^T]^T$ denote the vectorized representation of the embeddings and classifiers. Consider solving the unregularized  problem with gradient descent (GD) updates  $\thetab^{t+1} = \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)$, where $\Lc(\thetab^t):=\Lc(\W^t,\Hb^t)$ is the CE loss  in \eqref{eq:CE}. \cite{lyu2019gradient,ULPM} showed that the updates diverge in norm (i.e. $\|\thetab^t\|_2\rightarrow\infty$), but the normalized iterates $\thetab^t/\|\thetab^t\|_2$ converge to a  KKT point of \eqref{eq:SVM}. Since \eqref{eq:SVM} is nonconvex, it is unclear whether this point is a global optimum. Here, we use Theorem \ref{thm:global}  to show that a global minimizer $\hat\thetab$ of \eqref{eq:SVM} cannot be a converging direction of GD,  when classes are imbalanced. We start by formally defining the notion of a stationary direction below.

\begin{definition}[Stationary direction]
\label{defn:converging}
%We say a direction  $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction  of GD on $\Lc(\thetab)$ if and only if $\nicefrac{\nabla\Lc(\thetab)}{\|\nabla\Lc(\thetab)\|} = \nicefrac{-\thetab}{\|\thetab\|}$. 
We say $\thetab$ defines a stationary direction $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$
of GD on $\Lc(\thetab)$ if there exist constants $\kappa_1,\kappa_2>0$ such that $\nabla_\thetab\Lc(\kappa_1\thetab) = -\kappa_2\thetab$.
\end{definition}
%\gk{I think we have to refine the definition, or add assumptions- whether the relation should hold for all $\thetab$? What if for the same direction, some $\thetab$'s satisfy the condition while others do not?} \ct{Ok. Please  change and let's try to explain what's happening. Would something like the above work? I completed the proof and if I understand what you mean then it seems that the proof doesn't break.}
In words, a direction $\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction if the gradient descent update $\thetab^{+} = \thetab - \eta\nabla\Lc(\thetab)$ preserves this direction, i.e. $\nicefrac{\thetab^+}{\|\thetab^+\|_2}=\nicefrac{\thetab}{\|\thetab\|_2}$ , for any learning rate $\eta > 0$. 
\begin{definition}
	We say that $\nicefrac{\thetab}{\|\thetab\|}$ is a fixed direction under the GD update rule if and only if there exists an iteration $t$ such that $\frac{\thetab^{\tau}}{\|\thetab^{\tau}\|} = \frac{\thetab^{t}}{\|\thetab^{t}\|}, \quad\forall \quad\tau > t$.  \gk{tbd}
\end{definition}
\begin{lemma}
Suppose $\thetab$ is \emph{\underline{not}} a stationary direction of GD on $\Lc(\thetab)$. Then,
 	Under the GD update rule with finite learning rate $\eta >0$, $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is not a fixed direction 
	%\gk{to check if this term is good}
\end{lemma}
\begin{proof}
	Suppose $\thetab^t = \kappa\hat{\thetab}$ for some finite $\kappa >0$. Then, we show that $\thetab^{t+1}$, defined by an update of GD with a finite positive learning rate deviates from the direction $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$. Specifically, we will show that the projection of $\thetab^{t+1}$ onto the orthogonal complement of the subspace spanned by the vector $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is non-zero. Let $\Pbf_{\hat{\thetab}}$ and $\Pbf_{\hat{\thetab}}^\perp$ be the matrices projecting a vector onto $\hat{\thetab}$ and the orthogonal complement of $\hat{\thetab}$, respectively. Then, from the GD update equation we have, 
	\begin{align*}
		\thetab^{t+1} &= \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)\\
		\implies \Pbf_{\hat{\thetab}}^\perp\thetab^{t+1} &= \Pbf_{\hat{\thetab}}^\perp\thetab^t + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\thetab^t)\right)\\
		&= \Pbf_{\hat{\thetab}}^\perp\kappa\hat{\thetab} + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\kappa\hat{\thetab})\right)\\
		&= 0 + \frac{\eta\alpha_\kappa\kappa}{\alpha}\Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|\Pbf_{\hat{\thetab}}(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\right), \quad \text{where}\quad \beta = \frac{\eta\alpha_\kappa\kappa}{\alpha} > 0\\
		&= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\cos^2(\angle -\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &> 0, \quad \because \quad \angle \left(-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab}\right) \neq 0,\quad \text{from Proposition } \ref{propo:negative}.
	\end{align*}
\end{proof}
\gk{above, should we say explicitly that the angle is not 180 degrees either?}



With this definition, we now state the main result of this section. 



%\begin{assumption}\label{ass:align}
%\end{assumption}

\begin{propo}\label{propo:negative}
Assume imbalanced classes and $k>2$. Let $\hat\thetab=\vect(\What,\Hhat)$ be a global minimum of the non-convex SVM in \eqref{eq:SVM}. Then, $\nicefrac{\hat\thetab}{\|\hat\thetab\|}$ is \emph{not} a converging direction of GD on the CE loss.
\end{propo}
%\gk{I think we have to show this for all feasible scalar multiples of $\hat{\thetab}$? Related to how we define the convergence direction}

Proposition \ref{propo:negative} suggests that the KKT point to which GD converges to (in direction), is \emph{not} a global minimum of  \eqref{eq:SVM} when classes are imbalanced.
\footnote{Indeed, this statement can be formalized assuming that the GD path aligns with the gradients. While this statement is non-trivial, it has been proved (at least for $\eta\rightarrow0$) by \cite{} for binary data and we conjecture it to be true even for multiclass data (as already suggested by the results in \cite{}). 
 Specifically assume that $\lim_{t\rightarrow\infty}\inp{{\nbar{\thetab^t}}}{{-{\nbar{\nabla\Lc(\thetab^t)}}}}=1.$ If this is true, then Proposition \ref{propo:negative} and the gradient update rule yields  $\lim_{t\rightarrow\infty}\inp{\nbar{\thetab^t}}{\nicefrac{\hat\thetab}{\|\hat\thetab\|}}\neq1$. \ct{Check this!!!}% For the shake of contradiction assume this was not the case. Then, there exists $t_0$ such that for all $t\geq t_0$, $\|\nbar{\theta^t}-\nicefrac{\hat\thetab}{\|\hat\thetab\|}\|$
}. 
\ct{Also confirmed by our extended experiments in Figures ....} This is in stark to the balanced case, for which \cite{ULPM} showed that GD indeed converges to the global minimum of the non-convex SVM. Thus, \emph{even for a simple two-layer linear NN, it is in general \emph{not} true that GD converges to the global optimum of the corresponding max-margin optimization}. Specifically, while such a statement is always true for binary data as shown  by \cite{}, and for balanced multiclass data as shown by \cite{}, it fails for imbalanced multiclass data. 

\begin{remark} 
\ct{Check:}The proposition shows that the SVM solution is \emph{not} a converging direction of GD. From this, we can conclude that GD does not converge in that direction. On the other hand, note that showing a point $\thetab$ is a converging direction does \emph{not} imply that first-order methods necessariy converge in the direction of $\thetab$. This is because there might be a descending direction tangential to $\thetab$ (see for example \ref{unconstrained feature paper}).
\end{remark}



\paragraph{Proof.}
First, for arbitrary $\thetab$, denote the negative gradient of the CE loss as
	\begin{align}
		\g &:= -\nabla_\thetab\Lc(\thetab) = \sum_{i\in[n]}\sum_{c\neq y_i}\frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}\,\g_{i,c}\,,
	\end{align}
	where we denote the margins $s_{i,c} = (\w_{y_i}-\w_{c})^T\h_{i}$, and also, $\g_{i,c} = \nabla_\thetab s_{i,c}$. Specifically, using the shorthand $\alpha_{i,c} := \frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}$, we get $\g = \sum_{i\in[n]}\sum_{c\neq y_i}\alpha_{i,c}\g_{i,c}$. Here, note that $\g, \g_{i,c}, s_{i,c}$ are all functions of $\thetab$, but we suppress notation when clear from context.
	
Now, consider specific $\thetab = \kappa\hat{\thetab}$, where $\hat\thetab=\vect(\What,\Hhat)$, a global minimum of the non-convex SVM, and $\kappa >0$. From Theorem \ref{thm:global}\ref{thm:global_logits}, we know that $\hat\w_c^T\hat\h_i=\hat{z}_{ic}$ as defined in \eqref{eq:simplex}. Hence, the corresponding margins satisfy
\begin{align}
\forall i\in[n], c\neq y_i\,:\, s_{i,c}(\kappa\hat\thetab)=(\kappa\hat\w_{y_i}-\kappa\hat\w_{c})^T\kappa\hat\h_{i}=\kappa^2 \implies \alpha_{i,c}(\kappa\hat\thetab)=\alpha_\kappa>0,
\end{align}
Hence, $\g(\kappa\hat\thetab) = \alpha_\kappa\sum_{i\in[n]}\sum_{c\neq y_i}\g_{i,c}(\kappa\hat\thetab)$. In particular, evaluating $\g_{i,c}(\kappa\hat\thetab)=\nabla_\thetab s_{i,c}(\kappa\hat{\thetab})$ it follows that
\begin{subequations}\label{eq:grads_1}
	\begin{align}
\forall c \in [k]\,:\,~		-\nabla_{\w_{c}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\sum_{i: y_i=c}\hat\h_{i}-\sum_{i\in [n]}\hat\h_{i})\\
\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\hat\w_{y_i}-\sum_{c\in[k]}\hat\w_{c}).
	\end{align}
\end{subequations}
We now compute the angle between $\thetab = \kappa\hat{\thetab}$ and $-\nabla_{{\thetab}}\Lc(\kappa\hat{\thetab})$.
%\noindent\textbf{Angle between parameter and gradient:}
It can be checked that the gradient at $\kappa\hat{\thetab}$ is related to the gradient at $\hat{\thetab}$ as follows:
\begin{align*}
	\forall c \in [K]\,:\,~	 \nabla_{\w_{c}}\Lc(\kappa\hat{\thetab}) &=  -\alpha_\kappa\kappa^2\left(Kn_c\hat{\h_c}-\sum_{c}n_{c'}\hat{\h_{c'}}\right) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\w_{c}}\Lc(\hat{\thetab})\\
	\forall i \in [n]\,:\,~	
	\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab}) &= \alpha_\kappa\kappa^2K\hat{\w_{y_i}} =\frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\h_{i}}\Lc(\hat{\thetab})
\end{align*}	
where we used the following facts from Theorem \ref{thm:global} and $\alpha = \frac{\exp(-1)}{\left(1+(K-1)\exp(-1)\right)}$.
\begin{itemize}
	\item $\hat{\h}_{i} = \hat{\h}_{j}$ if $y_i = y_j$; denote $\hat{\h}_{i}$ by  $\hat{\h}_{c}$ when $y_i = c$
	\item $\sum_{c}\hat{\w}_c = 0$
\end{itemize}
Therefore, we get
$$\nabla_\thetab\Lc(\kappa\hat{\thetab}) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{{\thetab}}\Lc(\hat{\thetab}),
$$
Now, computing the inner products,
\begin{align*}
	-\nabla_{\w_{c}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2\left((K-1)n_c\hat{\h}_c^T\hat{\w}_{c}-\sum_{c'\neq c}n_{c'}\hat{\h}_{c'}^T\hat{\w}_{c}\right)\\
	&= \alpha_\kappa\kappa^2\left[(K-1)n_c\frac{K-1}{K}+\frac{n-n_c}{K}\right]\\
	&= \frac{\alpha_\kappa\kappa^2}{K}\left[\left((K-1)^2-1\right)n_c+n\right]\\
	-\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2K\hat{\w}_{y_i}^T\h_{i}\\
	&= \alpha_\kappa\kappa^2(K-1)
\end{align*}
Combining in $\thetab$ notation, we have
\begin{align*}
	-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab} &= \alpha_\kappa\kappa^2\left[n(K-1)+n\frac{(K-1)^2-1}{K}+n\right]\\
	&= \frac{\alpha_\kappa\kappa^2n}{K}(2K^2-2K)\\
	&= 2\alpha_\kappa\kappa^2n(K-1)
\end{align*}
Thus, we get the following for the cosine of the angle between the parameter and negative gradient at $\kappa\hat{\thetab}$:
\begin{align*}
	\cos(\angle -\nabla_\thetab\Lc(\kappa\hat{\thetab}),\kappa\hat{\thetab}) &= \frac{-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab}}{\|-\nabla_\thetab\Lc(\kappa\hat{\thetab})\|\kappa\hat{\thetab}\|}\\
	&= \frac{2\alpha_\kappa\kappa^2n(K-1)}{\frac{\alpha_\kappa\kappa^2}{\alpha}\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|}\\
	&= \frac{2n\alpha(K-1)}{\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|},
\end{align*}
which is independent of $\kappa$. This means that the angle between $\thetab$ and the negative gradient anywhere along the direction of $\hat{\thetab}$ remains a constant, irrespective of the magnitude of $\thetab$. Therefore, we can simplify the definition \ref{defn:converging} for $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ to be a stationary direction as there exists a $\gamma >0$ such that $\nabla\Lc(\hat{\thetab}) = -\gamma\hat{\thetab}$.
  


Next, suppose for the sake of contradiction that $\hat\thetab$ is a converging direction of GD. Following this (see Definition \ref{defn:converging}) and Equations \eqref{eq:grads_1}, there must exist $\kappa>0$ such that
\begin{subequations}\label{eq:grads_2}
	\begin{align}
\forall c \in [k]\,:\,~			-\nabla_{\w_{c}}\Lc(\hat\thetab) &= \alpha(k\sum_{i: y_i=c}\h_{i}-\sum_{i\in [N]}\h_{i}) = \gamma \w_{c} \label{eq:unreg_ce_grad_w_2}\\
	\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\hat\thetab) &= \alpha(K\w_{y_i}-\sum_{c\in[k]}\w_{c}) = \gamma\h_{i}\label{eq:unreg_ce_grad_h_2}\,.
	\end{align}
\end{subequations}
Also, from Theorem \ref{thm:global}\ref{thm:global_W} and the fact that $\Zhat^T\ones_k =0$, we have that
$
\sum_{c\in[k]}\w_c=\What\ones_k = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\ones_k = 0 \footnote{In fact, this property can alternatively be deduces from \eqref{eq:unreg_ce_grad_w_2} by summing for all $c\in[k].$}.
$ Therefore, \eqref{eq:unreg_ce_grad_h_2} gives
	\begin{align}
	\forall i \in [n]\,:\,~	\alpha(k\hat\w_{y_i}) = \gamma\hat\h_{i}
		\implies   \hat\h_{i}=\gamma'\hat\w_{y_i}=\gamma'\What\y_i \nn,
	\end{align}
	for some constant $\gamma'>0$ and one-hot encoding vector $\y_i=\eb_{y_i}.$ 
	Therefore, letting $\Y=[\y_1,\ldots,\y_n]_{k\times n}$ be the one-hot label matrix, we conclude that 
\begin{align*}
	\Hhat^T\Hhat=\gamma'\Hhat^T\What\Y &\implies (\Zhat^T\Zhat)^{1/2}=\gamma'\Zhat^T\Y,
	\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\Y\Y^T\Zhat,
		\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\diag(n_1,n_2,\ldots,n_k)\Zhat,
	\\
	&\implies \Zhat^T\big(\Id_k - (\gamma')^2\diag(n_1,n_2,\ldots,n_k)\big)\Zhat=\zeromat_{n\times n},
	\\
	&\implies \Zhat^T\diag({1-(\gamma')^2{n_1}},{1-(\gamma')^2{n_2}},\ldots,{1-(\gamma')^2{n_k}})\Z=\zeromat_{n\times n},
\end{align*}
where, the first implication follows by Theorem \ref{thm:global}\ref{thm:global_logits} and \ref{thm:global_gram}. Denote for convenience $\delta_{c}=1-(\gamma')^2{n_c}, c\in[k]$ and $\Delta=\sum_{c\in[k]}\delta_c.$ Then, from the last line above, it must be that
\begin{align*}
	&\forall i\in[n]\,:\, \Big(1-\frac{1}{k}\Big)^2\delta_{y_i}^2+\frac{1}{k^2}\sum_{c\neq y_i}^k\delta_c^2 =0 \implies \big(k-1\big)^2\delta_{y_i}^2+(\Delta-\delta_{y_i}^2) = 0
	\\
		\implies &\forall c\in[k]\,:\, \big(k-1\big)^2\delta_{c}^2+(\Delta-\delta_{c}^2) = 0 		\implies k(k-2)\delta_{c}^2=-\Delta.
			\\
			\stackrel{k>2}{\implies} 
			&\forall c\in[k]\,:\,\delta_{c}^2=-\Delta \implies \delta_{1}=\delta_2=\ldots\delta_k \implies n_1=n_2=\ldots=n_k=n/k.
%		&\implies \forall i\in[n]\,:\, \big(k-1\big)^2(1-(\kappa')^2{n_{y_i}})=\sum_{c\neq y_i}^k (1-(\kappa')^2{n_c}) = k - (\kappa')^2(n-n_{y_i}) ,
%			\\
%		&\implies \forall i\in[n]\,:\,  (\kappa')^2\big((k-1)^2+1\big)n_{y_i} = (k-1)^2 - k +n
\end{align*}
But data were assumed imbalanced, so we arrived at a contradiction completing the proof. Note also that in the last line, we used the assumption $k>2$.

%We now note that, along the direction of the SVM solution $\hat{\thetab}$ it is sufficient to consider the following simplified definition of converging direction \ref{defn:converging}: We say $\hat{\thetab}$ defines a stationary direction $\nbar{\hat{\thetab}}=\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$
%of GD on $\Lc(\thetab)$ if and only if there exists a constant $\kappa_3>0$ such that $\nabla\Lc(\hat{\thetab}) = -\kappa_3\hat{\thetab}$, which is used in the proof of Proposition \ref{propo:negative}
%This is due to the fact that $\nabla_\thetab\Lc(\kappa_1\hat{\thetab}) = \nicefrac{\alpha'\kappa_1}{\alpha}\nabla_\thetab\Lc(\hat{\thetab})$, where $\alpha' = \frac{\exp(-\kappa_1^2)}{1+(K-1)\exp(-\kappa_1^2)}$ which is described in the discussion below. The observation further shows that the angle between $\kappa_1\hat{\thetab}$ and $-\nabla_{\thetab}\Lc(\kappa_1\hat\thetab)$ is independent of $\kappa_1$.

%\gk{Plots of angle as functions of R, K etc} 
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm}
%		\caption{as a function of $R$}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm2}
%		\caption{Lorem ipsum}
	\end{subfigure}
	\caption{$\cos\left(\angle (-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)$ plotted against $R$ and $K$ respectively, with step imbalance on data. Note that the angle remains zero when $K=2$ or when $R=1$.}
\end{figure*}
%
%$$
%\forall c\in[k]\,,\, 1-(\kappa')^2{n_c} = 0 \implies n_1=n_2=\ldots=n_k.
%$$
%This contradicts our assumption that the dataset is imbalanced, completing the proof.


	%That is $\forall i\,:\, y_i=c$ the optimal feature $\hat\h_i$ aligns with the classifier $\hat\w_c$ of the corresponding class. 
	
	
%	Fix $i\in[n]$. Then from the display above and Theorem \ref{thm:global}\ref{thm:global_W},   
%	\begin{align}
%	\kappa'\hat\h_i = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}
%	Combining with Theorem \ref{thm:global}\ref{thm:global_Gram} (i.e. $\Hhat^T\Hhat=(\Zhat^T\Zhat)^{1/2}$), we conclude that
%	\begin{align}
%	\kappa'\Hhat^T\Hhat = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}	
	
	
%	But again from Theorem \ref{thm:global}\ref{thm:global_W} 
%$\w_c=\What\eb_c = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_c
%$

%	From \eqref{eq:h_opt} we have the relation between $\h_{i}^*$ and $\w_{y_i}^*$:
%	\begin{align*}
%		\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
%	\end{align*} 
%\gk{TBC}\ct{Need that $\w_{y_i}$ not aligned with $\h_i$.}



==> sections_v2/intro.tex <==
 \vspace{-0.2cm}

% \subsection{Motivation}

The prevalence of deep-neural networks (DNNs) has led to a growing research interest in understanding their underlying mechanisms. 
%This has resulted in significant progress and new insights being generated.
A recent research thread, focusing on classification tasks, explores whether it is possible to describe the structure of weights learned by DNNs when trained beyond zero-training error. The specific characteristics of this structure will depend on the DNN being used, the dataset being trained on, and the chosen optimization hyperparameters. Yet, \emph{is it possible to identify macroscopic structural characteristics that are common among these possibilities?}

In an inspiring study, \cite{NC} demonstrates this is possible for the classifiers and for the embeddings when training with cross-entropy (CE) loss and balanced datasets. Through extensive experiments over multiple architectures and datasets with an equal number of examples per class, they found that the geometries of  classifiers and of centered class-mean embeddings {(outputs of  the last hidden layer)} consistently converge during training to a common simplex equiangular tight frame (ETF), a structure composed of vectors that have equal norms and equal angles between them, with the angles being the maximum possible. Moreover, they observed neural-collapse (NC), a property where embeddings of individual examples from each class converge to their class-mean embedding. 
%
% This discovery has become the foundation for research endeavors in multiple directions over the past couple of years. Among 

Numerous follow-up studies have delved deeper into explaining this phenomenon and further investigating how the converging geometry changes with class imbalances. 
The unconstrained-features model (UFM), proposed independently by \cite{mixon2020neural,fang2021exploring,graf2021dissecting,lu2020neural}, plays a central role in the majority of these follow-up studies. Specifically, the UFM serves as a theoretical abstraction for DNN training, in which the network architecture is viewed as a powerful black-box that generates embeddings without any restrictions in the last {(hidden)} layer. For CE loss, the UFM minimizes $\min_{\w_c\in\R^d,\h_i \in\R^d} \Lc_{\text{CE}}\big(\{\w_c\}_{c\in[k]},\{\h_i\}_{i\in[n]}\big)$ in which both classifiers $\w_c$ for the $k$ classes and  embeddings $\h_i$ for the $n$ training examples are unconstrainedly optimized over $\R^d$. \cite{zhu2021geometric,graf2021dissecting,fang2021exploring} have verified that the global minimum of this non-convex problem satisfies NC and follows the ETF geometry observed in DNN experiments by \cite{NC}. Recent works by \cite{seli, fang2021exploring,behnia2023implicit} have demonstrated that the global optimum of the UFM changes when classes are imbalanced. Yet, the new solution still predicts the geometry observed in DNN experiments, providing evidence that, despite its oversimplification, the UFM is valuable in predicting structural behaviors. 


%A subtle issue in those studies that will nevertheless prove central to our study is the fact that
% \resizebox{0.9\textwidth}{!}{
% \begin{figure*}
%         % \centering
%         \hspace{-10pt}
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Graf_contribution/both_models/Graff_Boxplot_R1.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.2) [scale=0.9]{\textbf{R = 1}};
%                 \node at (0.0,1.7) [scale=1.1]{\textbf{Balanced}};
%                 \node at (-1.25, 0.5)  [scale=0.8, rotate=0]{\textbf{DenseNet}};
%                 \node at (-1.4,-0.1)  [scale=0.8, rotate=0]{\textbf{ResNet}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%             \vspace{-0.3in}
%             % \caption{}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Graf_contribution/both_models/Graff_Boxplot_R10.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.2) [scale=0.9]{\textbf{R = 10}};
%                \node at (2.3,1.7) [scale=1.1]{\textbf{Imbalanced}};
%                % \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%             \vspace{-0.3in}
%             % \caption{}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.32\textwidth}
%             \centering
%             \begin{tikzpicture}
%                 \node at (0,0) 
%                 {\includegraphics[width=\textwidth]{Figs/Graf_contribution/both_models/Graff_Boxplot_R100.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (0.0,1.2) [scale=0.9]{\textbf{\textbf{R = 100}}};
%                 % \node at (-2.7,0.0)  [scale=0.9, rotate=90]{};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{};
%             \end{tikzpicture}
%             \vspace{-0.3in}
%             % \caption{}
%         \end{subfigure}
%         \vspace{2pt}
%         \caption
%         {\gk{change to histogram on cosines} Experimental validation of our key finding: SCL learns orthogonal class-mean embeddings irrespective of class imbalances. Shown are box plots of pairwise angular distance $\Delta_\text{ang}=1 - \nicefrac{1}{\pi}\arccos\big(\nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_{c'}\|\|\mub_c\|}\big)$ between class-mean embeddings $\mub_c,\mub_{c'}, c\neq c'\in[k]$ of a ResNet-18 (bottom) and DenseNet-40 (top) trained with SCL on $R$-STEP-imbalanced CIFAR-10. In all three cases, our prediction highlighted in green and corresponding to an orthogonal angle is remarkably close to the measurements. Compare to the red line predicted by \cite{graf2021dissecting} for balanced data. No explicit characterization has been known previously for imbalanced data. %\vala{Increase axis font as well ? }
%         %\ct{Looks like spacing of figure headers is a bit meshed up and same for most plots}
%         } 
%         \vspace{-0.2in}
%         \label{fig:intro}
%     \end{figure*}
%     % }

% \begin{figure*}
%         \begin{subfigure}[b]{0.99\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.9\textwidth]{Figs/Histogram_Graff_CosAngles.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-4.4,2.2) [scale=0.9]{\textbf{R = 1}};
%             \node at (0.0,2.2) [scale=0.9]{\textbf{R = 10}};
%             \node at (4.4,2.2) [scale=0.9]{\textbf{R = 100}};
%             \node at (-6.9,1.0)  [scale=0.9, rotate=90]{\textbf{No-ReLU}};
%             \node at (-6.9,-0.7)  [scale=0.9, rotate=90]{\textbf{ReLU}};
%         \end{tikzpicture}
%     \end{subfigure}
%         \vspace*{-10pt}
%         \hfill
%         \captionsetup{width= 0.95\linewidth}
%         \caption[histogram]
%         {Experimental validation of our key finding: SCL learns orthogonal class-mean embeddings irrespective of class imbalances. Shown are histograms of pairwise cosine similarities $\cos(\mub_c, \mub_{c'}) = \nicefrac{\mub_c^\top\mub_{c'}}{\|\mub_{c'}\|\|\mub_c\|}$  between class-mean embeddings $\mub_c,\mub_{c'}, c\neq c'\in[k]$ of a ResNet-18 trained with SCL on $R$-STEP-imbalanced CIFAR-10. Values with ReLU applied to the output features (bottom) and without ReLU (top). In all three cases with ReLU (bottom), our prediction ({\color{red}red}) corresponding to an orthogonal angle is remarkably close to the measurements. No explicit characterization has been known previously for imbalanced data with or without ReLU. }
%         % Also interestingly, the empirical distribution of the cosine similarities with imbalance and without ReLU is dispersed over a range of values, as opposed to either the balanced data or (im)balanced data with ReLU.}
%         \label{fig:histogram} 
%     \end{figure*}



% \begin{figure*}
%     % \centering
%     \begin{subfigure}[b]{0.50\textwidth}
%     % \centering
%     \begin{tikzpicture}
%         \node at (0.0,0) 
%         {\includegraphics[width=\textwidth]{Figs/Heatmap_ICLR_new.pdf}};
%         \node at (-2.2,3.5) [scale=0.9]{\textbf{SCL + ReLU}};
%         \node at (-0.2,3.5) [scale=0.9]{\textbf{SCL}};
%         \node at (1.9,3.5) [scale=0.9]{\textbf{CE}};
%         \node at (-4.2,2.2)  [scale=0.9, rotate=90]{\textbf{R = 1}};
%         \node at (-4.2,0.1)  [scale=0.9, rotate=90]{\textbf{R = 10}};
%         \node at (-4.2,-1.9)  [scale=0.9, rotate=90]{\textbf{R = 100}};
%     \end{tikzpicture}
% \end{subfigure}
%     \vspace*{-10pt}
%     \hfill
%     \captionsetup{width= 0.95\linewidth}
%     \caption[histogram]
%         {\vala{ Explanation!!! }\gk{Pairwise cosine similarities between class-means of learned feature embeddings, with ResNet-18 on CIFAR-10. \textbf{SCL+ReLU:} the mean feature embeddings for different classes are mutually orthogonal, forming an OF, regardless of imbalance (imbalance ratio $R=1,10,100$)}. This invariance does not hold in the absence of ReLU for \textbf{SCL}. Further, \textbf{CE} feature geometry is also sensitive to imbalance. The label distribution is STEP imbalanced, with classes $0-4$ are majorities and $5-9$ are minorities. \tina{mention how to read the heatmap: the last five classes are minorities etc}  }
%     % Also interestingly, the empirical distribution of the cosine similarities with imbalance and without ReLU is dispersed over a range of values, as opposed to either the balanced data or (im)balanced data with ReLU.}
%     % \label{fig:histogram} 
%     \label{fig:heatmap} 
% \end{figure*}


Expanding beyond the scope of CE minimization, \cite{graf2021dissecting} also used the UFM to determine whether optimizing with the supervised-contrastive loss (SCL)  results in any alterations to the geometric structure of the learned embeddings.\footnote{SCL is designed to train only embeddings and is an extension of the well-known contrastive loss used for unsupervised learning, adapted to supervised datasets \citep{khosla2020supervised}; see Equation \eqref{eq:SCL_full}.}
% 
% \begin{wrapfigure}[26]{r}{0.4\textwidth} 
%      \centering
%             % \vspace{-0.07in}
%             \begin{tikzpicture}
%                 \node at (0.0,0.0) 
%                 {\includegraphics[width=0.4\textwidth]{Figs/Heatmap_ICLR_new.pdf}};
%                  \node at (-2.0,2.8) [scale=0.7]{\textbf{SCL + ReLU}};
%                 \node at (-0.2,2.8) [scale=0.7]{\textbf{SCL}};
%                 \node at (1.5,2.8) [scale=0.7]{\textbf{CE}};
%                 \node at (-3.2,1.9)  [scale=0.7, rotate=90]{\textbf{R = 1}};
%                 \node at (-3.2,0.1)  [scale=0.7, rotate=90]{\textbf{R = 10}};
%                 \node at (-3.2,-1.6)  [scale=0.7, rotate=90]{\textbf{R = 100}};
%                 %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%     \captionsetup{width=0.95\linewidth}
%     \caption{Gram matrices, $\G_\M/\max_{i,j}|\G_\M[i,j]|$, of class-means of learned feature embeddings at last epoch of training, with ResNet-18 on MNIST. \textbf{SCL+ReLU:} the mean feature embeddings for different classes are mutually orthogonal, forming an OF, regardless of imbalance (imbalance ratio $R=1,10,100$). This invariance does not hold in the absence of ReLU for \textbf{SCL} or \textbf{CE}. The label distribution is STEP imbalanced, with the first five classes as majorities and the rest as minorities.}
%     \vspace{0.03in}
%     \label{fig:heatmap}
%     \vspace{-1.0cm}
% \end{wrapfigure}

\begin{wrapfigure}[26]{r}{0.5\textwidth} 
     \centering
            \vspace{-20pt}
            \begin{tikzpicture}
                \node at (0.0,0.0) 
                {\includegraphics[width=0.5\textwidth]{Figs/Heatmap_ICLR_new_CEcentered.pdf}};
                 \node at (-2.4,3.3) [scale=0.9]{\textbf{SCL + ReLU}};
                \node at (-0.2,3.3) [scale=0.9]{\textbf{SCL}};
                \node at (1.9,3.3) [scale=0.9]{\textbf{CE}};
                \node at (-3.7,2.2)  [scale=0.9, rotate=90]{\textbf{R = 1}};
                \node at (-3.7,0.1)  [scale=0.9, rotate=90]{\textbf{R = 10}};
                \node at (-3.7,-1.9)  [scale=0.9, rotate=90]{\textbf{R = 100}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
    \captionsetup{width=0.95\linewidth}
    \caption{Gram matrices, $\G_\M/\max_{i,j}|\G_\M[i,j]|$, of class-means of learned feature embeddings at last epoch of training, with ResNet-18 on MNIST. \textbf{SCL+ReLU:} the mean feature embeddings for different classes are mutually orthogonal, forming an OF, regardless of imbalance (imbalance ratio $R=1,10,100$). This invariance does not hold in the absence of ReLU for \textbf{SCL}. Further, \textbf{CE} feature geometry is also sensitive to imbalance. The label distribution is STEP imbalanced, with the first five classes as majorities and the rest as minorities. See Sec.\ref{sec:exp_fig1_detail} in SM for more information.}
    \vspace{0.03in}
    \label{fig:heatmap}
    \vspace{-1.0cm}
\end{wrapfigure}

% 
% Moving a step beyond CE minimization, and in an effort to explore how the learned geometry is affected by the loss being optimized, \cite{graf2021dissecting} also used the UFM to determine whether optimizing instead with the supervised-contrastive loss (SCL)  results in any alterations to the geometric structure of the learned embeddings.
%In an effort to explore how the learned geometry is affected by the loss being optimized \cite{graf2021dissecting} also used the UFM to determine whether optimizing with the supervised-contrastive loss (SCL)  instead of the CE loss results in any alterations to the geometric structure of the learned embeddings.
% 
\vspace{-4pt}
They proved for balanced datasets that the global solution of $\min_{\h_i\in\R^d}\Lc_{\text{SCL}}\big(\{\h_i\}_{i\in[n]}\big)$ remains a simplex ETF, suggesting that CE and SCL find the same embedding geometries. In Fig.~\ref{fig:heatmap}, we investigate the geometry of class-means in presence of class-imbalance. The prediction in \cite{graf2021dissecting} only applies to balanced data (SCL with $R=1$ in Fig.~\ref{fig:heatmap}) and no prior work has explicitly characterized the geometry of SCL {with} class imbalances. Observing the middle column of the figure, note that the geometry of embeddings changes drastically\footnote{Analogous finding is reported by \cite{zhu2022balanced}, although not visualized as done here.} as the imbalance ratio $R$ increases. This behavior of SCL is consistent with the CE embeddings geometry, which, as discussed previously,  also changes with the imbalance; see last column of Fig.~\ref{fig:heatmap}.

In this paper, we arrive at a surprising finding: simply introducing a ReLU activation at the final layer restores the symmetry in SCL-trained representations. This phenomenon is clearly illustrated in the first column of Fig.~\ref{fig:heatmap}. Below is a detailed description of our contributions.

% \ct{remove paragraph below if happy with above}
% \new{In  we present a visualization of feature geometries learned by SCL with and without ReLU, and by CE when training ResNet-18 on imbalanced MNIST with different imbalance ratios $R$.} 
% % \gk{to be changed for new fig} In Fig.~\ref{fig:histogram}(a), we present a histogram illustrating the distribution of the measured pairwise cosine similarities of the class-means $\mub_c,\mub_{c'}$ for $c\neq c'$. 
% \new{The prediction in \cite{graf2021dissecting} only applies to balanced data (SCL with $R=1$ in Fig.~\ref{fig:heatmap}) and no prior work has explicitly characterized the geometry of SCL loss {with} class imbalances.} 
% In this paper, we propose surprisingly simple modifications to SCL training to restore symmetry in the learned features regardless of imbalance. 
% This paper reveals the surprising finding that applying ReLU to the last-layer features restores the symmetry in features learned by SCL. Our claim is supported with theoretical and empirical findings.

%\begin{center}
% \emph{what is the geometry of the embeddings under imbalances?} Ultimately, \emph{\textbf{is the implicit geometry of embeddings the same when optimizing with either the CE or the SCL loss?}} Additionally, \emph{when classes are balanced, what could account for the difference between the UFM prediction from \cite{graf2021dissecting} and the experimental values in Fig.~\ref{fig:histogram}(a)? Is the UFM unable to accurately predict the geometry learned by SCL?} 
%\end{center}

% \ct{Add a few sentences about batching being essential in SCL (can motivate as differentiating factor to CE). Say that to best of our knowledge whether the specific bathcing scheme choice has any impact on what and how fast SCL learns has not been thoroughly investigated. Raise this as an additional motivating question adding to the above.}

% \new{A key characteristic of optimizing a model with SCL is that the batching scheme can potentially lead to different optimal solutions depending on the choice of mini-batches. To the best of our knowledge, there is a lack of understanding on whether a specific batching scheme has any impact of what and how fast SCL learns optimal embeddings. Through our analysis of batching requirements and usefulness of the proposed simple yet effective scheme, for achieving a unique solution that is same as that given by full-batch SCL, we hope to motivate further studies into this aspect.} 

% For illustrationWe then run the same experiment only this time over a STEP-imbalanced version of CIFAR 10 with 5 majority/minority classes and imbalance ratio $R=10, 100$. The measured cosine similarities are depicted in Figure \ref{fig:intro}(Left). 




\subsection{Summary of contributions}
% \new{We find that we can learn class-mean embeddings that are pairwise orthogonal, hence they form an orthogonal frame (OF), a structure composed of vectors that have equal norms and are mutually orthogonal to each other when training the models with SCL. Interestingly,  this geometry remains consistent regardless of the label distribution, i.e., the number of examples per class. The emergence of this symmetric structure relies on adding ReLU activations at the final embedding layer and the choice of batching scheme.}

We conduct an in-depth examination of the geometry of training representations (embeddings) of SCL, particularly in relation to varying levels of dataset imbalances. Our study leads us to identify and capture, both analytically and empirically, and for the first time, the impact on the representation geometry of: (i) a straightforward architectural modification, specifically the incorporation of a ReLU activation at the final layer, and (ii) the batch-selection strategy.

% \ct{remove this if you like the above instead}Our analysis focuses on modifications to SCL which would help models retain a symmetric feature geometry, regardless of imbalance. We demonstrate that one such modification yields an orthogonal frame (OF), a structure composed of class-mean embedding vectors that have equal norms and are mutually orthogonal to each other. In particular, we study: 

\noindent\textbf{Impact of ReLU.}~We find that the addition of a ReLU activation to the last-layer of the architecture results in an orthogonal frame (OF) geometry. That is, a  geometry structure composed of class-mean embedding vectors that have equal norms and are mutually orthogonal to each other. A preliminary experimental validation of this finding is illustrated in Fig.~\ref{fig:heatmap}. The experiments correspond to STEP-imbalanced MNIST data with five majority/minority classes and imbalance ratio $R=1,10, 100$. Each heatmap represents the pairwise inner products between the class-means of learned feature embeddings. 
%While not shown in this figure, we first note (see  Fig.~\ref{fig:Deepnet_SCL_Geom_NC}, Sec.~\ref{app:exp_appex} in SM) that all features of a given class collapse to their mean, i.e. \emph{neural-collapse} occurs. More importantly, 
The figure (first column) reveals that with the addition of ReLU at the last layer, SCL  learns orthogonal features \emph{regardless of class imbalance.} This is in stark contrast to the varying geometries of vanilla SCL (optimized commonly without ReLU) and CE loss.
%Contrary to this, the feature geometries learned by SCL without ReLU and CE loss are sensitive to imbalance. As imbalance ratio increases, the angles between minority classes become smaller, making minority classes centers less distinguishable. 
Extensive additional experiments for Long-tailed (LT) distributions, other datasets and architectures, are presented in Sec.~\ref{sec:Deepnet_SCLGeom_exp} and also Sec.~\ref{app:exp_appex} in the SM. We also present experimental findings that confirm ReLU symmetrises the geometry without compromising test accuracy.
% .In addition to the main finding of convergence to OF geometry, our empirical results show that adding ReLU to the last layer does not compromise test accuracy of SCL.}

\begin{figure}[t!]
    % \centering
    \hspace*{-16pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.85\textwidth]{Figs/GMu_Convergence_plots_ICLR_Fig2.pdf}};
            % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
            \node at (-4.4,2.35) [scale=0.9]{\textbf{MNIST}};
            \node at (-1.4,2.35) [scale=0.9]{\textbf{CIFAR10}};
            \node at (1.5,2.35) [scale=0.9]{\textbf{CIFAR100}};
            \node at (4.4,2.35) [scale=0.9]{\textbf{Tiny ImageNet}};
            \node at (-6.2,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
            \node at (-6.2,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
            \node at (0.1,-2.4) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    % \vspace{-10pt}
    \captionsetup{width= 0.95\linewidth}
    \caption
    {
    Distance of learned embeddings to the OF geometry as measured by $\|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$ where $\G_\M=\M^\top\M$ is the Gram matrix of class-mean embeddings. For MNIST and CIFAR10 we use ResNet-18 and for the more complex CIFAR100 and Tiny-ImageNet, we use ResNet-34 and train using batch-binding (see Sec.~\ref{sec:batching}). Regardless of the imbalance level $R$, the embeddings consistently converge to the OF geometry.
    % 
    % 
    % Deepnet models trained on imbalanced datasets with SCL. Convergence of embeddings to the OF geometry as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$, where $\G_\M=\M^\top\M$ is the Gram matrix of class-mean embeddings. For MNSIT and CIFAR10 we used a ResNet-18 and for CIFAR100 and Tiny-ImageNet, having been more complex dataests, we use ResNet-34 and train using batch-binding. We observe that $\Delta_{\G_\M}$ is consistently on the order of $10^{-2}$ regardless of dataset or imbalance.
    }
    \label{Fig:Deepnet_SCL_Geom_GMu}
\end{figure}

We support this finding by theoretically  investigating the global minimizers of an extended version, denoted as \ref{eq:SCL_UFM_full}, of the original unconstrained-features model (UFM). This refinement accounts for the presence of ReLU activations which we impose on the last-layer by minimizing SCL over the non-negative orthant. Concretely, we show that all global solutions of $\min_{\h_i\geq 0}\Lc_{\text{SCL}}\big(\{\h_i\}_{i\in[n]}\big)$ satisfy NC and the corresponding class-mean features form an OF. This explains the  convergence of feature geometry to an OF as consistently observed in our experiments; for example, see Fig. \ref{Fig:Deepnet_SCL_Geom_GMu}. %eliminating the requirement for a heuristic centering of the class-mean embeddings as implemented in the majority of prior studies. 
% \tina{omitted the sentence on centering for now... }

\noindent\textbf{Batching and its implications.}~Furthermore, we identify the crucial impact of batch selection strategies  during SCL training in shaping the learned embedding geometry. Concretely, by analyzing the \ref{eq:SCL_UFM_full}, we establish straightforward criteria for the batching scheme, ensuring that any global minimizer of \ref{eq:SCL_UFM_full} forms an OF. These conditions explain the substantial degradation in convergence towards an OF when employing a fixed batch partition instead of randomly reshuffling the batches at each training epoch. Intriguingly, we demonstrate that any arbitrary batching partition can be transformed into one that fulfills our theoretical conditions by performing so-called \textit{batch-binding}. Through extensive experiments in Sec.~\ref{Sec:Binding_examples} and in the SM, we show that batch-binding consistently accelerates the convergence of the learned geometry towards an OF and even improves convergence to ETF geometry under balanced training in the absence of ReLU.



% \noindent\textbf{Notation.}~
% For a positive integer $n$, we denote $[n] := \{1,2,3,...,n\}$. For matrix $\Vb\in\R^{m\times n}$, $\Vb[i,j]$ denotes its $(i,j)$-th entry, $\vb_j$ denotes the $j$-th {column}, $\Vb^\top$ its transpose. We denote $\|\Vb\|_F$ the Frobenius norm of $\Vb$. We use $\Vb \propto \mathbf{X}$ whenever the two matrices are equal up to a scalar constant. We use $\Vb \geq 0$ to denote the entry-wise non-negativity of the elements of $\Vb$, i.e., $\Vb[i,j] \geq 0, \forall i \in [m],j \in [n]$. Finally, $\Id_m$ denotes the identity matrix of size $m$.






% \vspace{-0.1in}
% \subsection{Summary of contributions}
% % \vspace{-0.1in}
% % This paper answers all the above questions. 
% % \vp
% \noindent\textbf{Key finding.}~We find that SCL with ReLU activations learns class-mean embeddings that are pairwise orthogonal, hence forming an orthogonal frame (OF), a structure composed of vectors that have equal norms and are mutually orthogonal to each other. Interestingly,  this geometry remains consistent regardless of the label distribution, i.e., the number of examples per class. 
% \new{ We are the first to characterize the geometry of SCL features under imbalances.} 
% % \todo{move to conclusion: while the answer to this in absence of ReLU still remains open}
% % This finding highlights a notable distinction between SCL and CE loss, as the geometry of embeddings learnt with CE is known to be highly-influenced by the label distribution.

% % \vp
% \noindent\textbf{Experimental justification.}~An experimental validation of our finding is illustrated in Fig.~\ref{fig:heatmap}. The experiments correspond to STEP-imbalanced  CIFAR-10 data with five majority/minority classes and imbalance ratio $R=1,10, 100$. \new{Each heatmap represents the pairwise cosine similarities between the class-means of learned feature embeddings. While not shown in this figure, we first note (see Sec.~\ref{app:exp_appex} in SM) that all features of a given class collapse to their mean, i.e. \emph{neural collapse} occurs. More importantly, the figure shows that SCL with ReLU learns orthogonal features regardless of imbalance in data $R=10,100$. This is distinct from SCL without ReLU as well as CE loss, where the feature geometry is sensitive to imbalance, as shown in the figure.}
% % \new{The red line highlights the cosine of orthogonal angles (corresponding to an OF), which is $0$, and remarkably aligns with the measured angles for \emph{all} values of the imbalance ratio $R$}.
% Extensive additional experiments for Long-tailed (LT) distributions, other datasets, and architectures, are presented in Sec.~\ref{sec:Deepnet_SCLGeom_exp} and Sec.~\ref{app:exp_appex} in the SM. \new{In addition to the main finding of convergence to OF geometry, our empirical results show that adding ReLU to the last layer does not compromise the test accuracy of SCL, while in fact improving it in certain cases of imbalance.}

% % \vp
% % \noindent\new{\textbf{ReLU does not compromise test accuracy of SCL.}~Earlier works using SCL have found that having a projector block during training, that is later dropped during inference helps improve the accuracy. Our experiments with and without ReLU activations in the projector reveal that ReLU helps achieve a higher test accuracy in presence of class imbalance in a subset of our experiments without any other changes to the training process. This is consistent with our finding of symmetry in the feature geometry irrespective of imbalanced data} 
% % \ct{probably Sec. 5.2 should be added?}

% % \vp
% \noindent\textbf{Theoretical justification.}~Our finding emerged through theoretical analysis by investigating the global minimizers of an extended version, denoted as \ref{eq:SCL_UFM_full}, of the original unconstrained-features model (UFM). This refinement accounts for the presence of ReLU activations in the last hidden layer by minimizing the SCL over the non-negative orthant. Concretely, we show that all global solutions of $\min_{\h_i\geq 0}\Lc_{\text{SCL}}\big(\{\h_i\}_{i\in[n]}\big)$ satisfy NC and the corresponding class-mean features form an OF. This explains the implicit geometry observed in our experiments, eliminating the requirement for a heuristic centering of the class-mean embeddings as implemented in the majority of prior studies.

% % \vp
% \noindent\textbf{Analysis of batching and implications.}~Finally, we examine the impact of batching on determining the learned embedding geometry. By utilizing the \ref{eq:SCL_UFM_full}, we establish straightforward criteria for the batching scheme, ensuring that any global minimizer forms an OF. By utilizing these conditions, we provide an explanation for the observed substantial degradation in convergence towards an OF when employing a fixed batch partition instead of randomly reshuffling the batches at each training epoch. Intriguingly, we demonstrate that any arbitrary batching partition can be transformed into one that fulfills our theoretical conditions by performing so-called ``batch-binding'' in each batch. Moreover, {as verified in Sec.~\ref{Sec:Binding_examples}}, this approach consistently accelerates the convergence of the learned geometry towards an OF.

% % \gk{todo: remove}
% % \subsection{Organization}

% % {The remaining portion of the paper is organized as follows. In Sec.~\ref{sec:setup}, we formally introduce the SCL and provide an overview of the OF geometry. Sec. \ref{sec:Deepnet_SCLGeom_exp} presents and discusses the experimental evidence that supports our main finding. The theoretical justification for our finding is presented in Sec.~\ref{sec:theo_results}, where we analyze both full-batch and mini-batch SCL scenarios. Building upon the insights gained from the analysis of mini-batch SCL, Sec.~\ref{sec:batching} explores the critical role of batching and proposes a binding-examples scheme aimed at enhancing the convergence quality of the implicit geometry. To position our results in the context of related works, Sec.~\ref{sec:discussion} further discusses the most closely related studies and presents a detailed comparison between the \ref{eq:SCL_UFM_full} model, which we rely on in this paper, and the previously-used UFM. Sec.~\ref{sec:conclusions} concludes the paper by reflecting on the contribution of our findings and discussing their implications at the intersection of the literature on neural-collapse phenomena and contrastive-type losses. The appendix contains all the proofs, along with additional experimental details and supplementary experiments.}

% % \vspace{5pt}

% % \todo{more related work? Currently in SM. bring important ones to the end of the paper.}













==> sections_v2/num_results.tex <==
% Structure: 
% \begin{itemize}
%     \item 3 datasets, exp + step for Resnet discuss convergence to OF 
%     \item Ganesh's proof + discussion with ReLU, without ReLU (graf) 
%     \item Lowerbound full batch to loss convergence 
%     \item GM plots here CE vs SCL 
%     \item Ganesh's batch argument 
%     \item regular batch vs Vala - Batch experiments, discussion of larger batchsizes (small batch with same examples vs large batches...) 
%     \item Test accuracy Augmentation vs Augmentation and vala batch, VS Loss, CE comparison 
%     \item Consider including other models if vala batching helps, consider other sampling 
%     \item relu last layer vs whole architecture relu 
%     \item wSCL (not that promising), any UFM results 
% \end{itemize}






\gk{is this section for anything in particular?}

==> sections_v2/old_gk.tex <==
\tina{old proof:}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:jensen_exp_sim}

    \begin{align}
        \sum_{m:y_m = y_i, m\neq i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)} \geq (n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \h_i^T\h_j\right)}    
    \end{align}
    where equality holds if and only if $\h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2 \neq i: y_{m_1} = y_{m_2} = y_i$
 \end{lemma}
 \begin{proof}
     For a given $i,j$, let $\h_i^T\h_m := x_{m}, \h_i^T\h_j = \alpha$. Then,
     \begin{align}
         \sum_{m:y_m = y_i, m\neq i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)} &= \sum_{m:y_m = y_i, m\neq i}\exp{\left(x_m - \alpha\right)}\\
         &= \exp{\left(-\alpha\right)}\sum_{m:y_m = y_i, m\neq i}\exp{\left(x_m\right)}\\
         &= \exp{\left(-\alpha\right)}(n_c-1)\frac{1}{(n_c-1)}\sum_{m:y_m = y_i, m\neq i}\exp{\left(x_m\right)}\\
         &\geq \exp{\left(-\alpha\right)}(n_c-1)\exp{\left(\frac{1}{(n_c-1)}\sum_{m:y_m = y_i, m\neq i}x_m\right)},\label{eq:jensen_exp}\\
         & \text{where the Jensen's inequality is applied on $\exp{(x)}$} \nonumber\\
         &= (n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \h_i^T\h_j\right)}
     \end{align}
     Due to the strict convexity of $\exp{(x)}$ on $x$, the inequality in Eq. \ref{eq:jensen_exp} holds with equality if and only if $x_{m_1} = x_{m_2}, \forall m_1,m_2 \neq i: y_{m_1} = y_{m_2} = y_i$.
 \end{proof}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{lemma}\label{lem:jensen_exp_con}
    \begin{align}
        \sum_{m:y_m \neq y_i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)} \geq (n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \h_i^T\h_j\right)}    
    \end{align}
    where equality holds if and only if $\h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} \neq y_i$
 \end{lemma}
 \begin{proof}
     For a given $i,j$, let $\h_i^T\h_m := x_{m}, \h_i^T\h_j = \alpha$. Then,
     \begin{align}
         \sum_{m:y_m \neq y_i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)} &= {m:y_m \neq y_i}\exp{\left(x_m - \alpha\right)}\\
         &= \exp{\left(-\alpha\right)}\sum_{m:y_m \neq y_i}\exp{\left(x_m\right)}\\
         &= \exp{\left(-\alpha\right)}(n-n_c)\frac{1}{(n-n_c)}\sum_{m:y_m \neq y_i}\exp{\left(x_m\right)}\\
         &\geq \exp{\left(-\alpha\right)}(n-n_c)\exp{\left(\frac{1}{(n-n_c)}\sum_{m:y_m \neq y_i}x_m\right)},\label{eq:jensen_exp}\\
         & \text{where the Jensen's inequality is applied on $\exp{(x)}$} \nonumber\\
         &= (n-n_c)\exp{\left(\frac{1}{(n-n_c)}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \h_i^T\h_j\right)}
     \end{align}
     Due to the strict convexity of $\exp{(x)}$ on $x$, the inequality in Eq. \ref{eq:jensen_exp} holds with equality if and only if $x_{m_1} = x_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} \neq y_i$.
 \end{proof}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{lemma}\label{lem:jensen_log1p}
     \begin{align}
         &\sum_{i\in\mathcal{C}_c}\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)\\
         & \ \ n_c\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n_c(n-n_c)}\left(\sum_{i\in[n]}\sum_{m:y_m \neq y_i}\h_i^T\h_m\right) - \frac{1}{n_c(n_c-1)}\left(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\right)\right)}\right)
     \end{align}
 \end{lemma}
 \begin{proof}
     For a given $c\in [k]$, let $n_c-1 := a > 0, n-n_c := b > 0$ \gk{do we need $n_c > 1$? maybe indicator takes care of it} and $x_i := \left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)$. Then,
     \begin{align}
         &\sum_{i\in\mathcal{C}_c}\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)\\
         &= \sum_{i\in\mathcal{C}_c}\log\left(a +b\exp{(x_i)}\right)\\
         &\geq n_c\log\left(a +b\exp{\left(\frac{1}{n_c}\sum_{i\in\mathcal{C}_c}x_i\right)}\right),\label{eq:jensen_log1p}\\
         &\text{where the Jensen's inequality is applied on $\log(a+b\exp(x))$} \nonumber\\
         &= n_c\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n_c(n-n_c)}\left(\sum_{i\in[n]}\sum_{m:y_m \neq y_i}\h_i^T\h_m\right) - \frac{1}{n_c(n_c-1)}\left(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\right)\right)}\right)
     \end{align}
     Due to the strict convexity of $\log(a+b\exp{(x)})$ on $x$, the inequality in Eq. \ref{eq:jensen_log1p} holds with equality if and only if $x_{i_1} = x_{i_2}, \forall i_1,i_2 \in \mathcal{C}_c$.
 \end{proof}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:affine}
For a given $i$,
    \begin{align}
    &\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \h_i^T\h_j\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \h_i^T\h_j\right)}\Bigg]\nonumber\\
     &= \log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\right)\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\Bigg]\nonumber\\
    \end{align}
\end{lemma}
\begin{proof}
    Let $a:= (n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right)\right)}$ and $b:=(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right)\right)}$. Then,
    \begin{align}
    &\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log\Bigg((n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \h_i^T\h_j\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \h_i^T\h_j\right)}\Bigg)\nonumber\\
    &=  \frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log\Bigg(a\exp{\left(- \h_i^T\h_j\right)}+b\exp{\left(- \h_i^T\h_j\right)}\Bigg)\nonumber\\   
    &= \frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i} \left(- \h_i^T\h_j\right) + \frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log(a+b)\nonumber\\
    &= \log\left(\exp\left(\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i} \left(- \h_i^T\h_j\right)\right)\right) + \log(a+b)\nonumber\\
    &= \log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\right)\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\Bigg]\nonumber\\
    \end{align}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:log1p_non_dec}
    The function $f:\R \rightarrow \R, f(x) =\log(a+b\exp(x)), a,b \in \R_+$ is non-decreasing in the argument $x \in \R$
\end{lemma}
\begin{proof}
    Consider the derivative of $f(x)$: $f'(x) = \frac{b\exp(x)}{a+b\exp(x)} > 0, \  \forall x \in \R$. Therefore, $f(x)$ is a non-decreasing function of $x$.
\end{proof}


\subsection{Proof of Thm.~\ref{thm:scl_full}}


\begin{proof}

 \begin{align}
     \Lc(\Hb)&:=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{{j\in\mathcal{C}_{y_i},j\neq i}}
     \log\Big(\sum_{{\ell\in[n],\ell\neq i}}\exp{\left(\h_i^T\h_\ell - \h_i^T\h_j\right)}\Big)\nonumber\\
     %
     &= \sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{{j\in\mathcal{C}_{y_i},j\neq i}}\log\left(\sum_{\ell\in\mathcal{C}_{y_i}, \ell\neq i}\exp{\left(\h_i^T\h_\ell - \h_i^T\h_j\right)}+\sum_{\ell\not\in \mathcal{C}_c}\exp{\left(\h_i^T\h_\ell - \h_i^T\h_j\right)}\right)\nonumber\\
     %
     &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{c}-1}\sum_{j\in\mathcal{C}_c, j \neq i}\log\left(\sum_{\ell\in\mathcal{C}_{y_i}, \ell\neq i}\exp{\left(\h_i^T\h_\ell - \h_i^T\h_j\right)}+\sum_{\ell\not\in\mathcal{C}_c}\exp{\left(\h_i^T\h_ell - \h_i^T\h_j\right)}\right)\nonumber
     \end{align}
% Now, we apply Jensen's inequality twice to the strictly convex functions $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$ and $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$, over the variable $m$, for a given $i$ and $j$: 
Now, applying Lemma \ref{lem:jensen_exp_sim} and \ref{lem:jensen_exp_con}, we use Jensen's inequality twice to the strictly convex functions $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$ and $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$, over the variable $m$, for a given $i$ and $j$:
 \begin{align}
     \Lc(\Hb) &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\bigg(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\bigg) - \h_i^T\h_j\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \h_i^T\h_j\right)}\Bigg]\nonumber
     \end{align}
Applying Lemma \ref{lem:affine}, we use that fact that the function $\log\bigg(a\exp{\left(- \h_i^T\h_j\right)}+b\exp{\left(- \h_i^T\h_j\right)}\bigg)$ is affine over its arguments $\h_i^T\h_j$ for a given $i$ and constants $a$ and $b$:
 \begin{align}
     \Lc(\Hb) &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\bigg(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\bigg)\right)}\nonumber\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\bigg)\right)}\Bigg]\nonumber\\
     &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log\Bigg[(n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\bigg)\right)}\Bigg]\nonumber
     \end{align}
% Now, we apply Jensen's inequality to the function $\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)$, over the variable $i$, and constants $a,b_i,c,d_i$, for a given $i$ : \gk{todo:check strict convexity } 
Now, applying Lemma \ref{lem:jensen_log1p}, where we use the Jensen's inequality again:
 \begin{align}
     \Lc(\Hb)&\geq \sum_{c \in [k]}n_c\log\Bigg[(n_c-1) +(n-n_c)\exp\Bigg(\frac{1}{n_c(n-n_c)}\bigg(\sum_{i\in[n]}\sum_{m:y_m \neq y_i}\h_i^T\h_m\bigg)\nonumber\\
     & \ \ \ - \frac{1}{n_c(n_c-1)}\bigg(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\bigg)\Bigg)\Bigg]\nonumber
     \end{align}
Now, we use the following facts
\begin{itemize}
    \item $\h_i^T\h_m \geq 0, \ \text{since} \ h_{i,p} \geq 0, h_{j,p} \geq 0$, with equality if and only if $\h_i^T\h_m = 0$, i.e. $\h_i$ and $\h_m$ are orthogonal to each other.
    \item $\h_i^T\h_j \leq \|\h_i\|\|\h_j\| = 1$, due to Cauchy-Schwartz inequality, with equality if and only if $\h_i = \h_j$.
    \item The function $f:\R \rightarrow \R, f(x) =\log\big(a+b\exp(x)\big), a,b \in \R_+$ is non-decreasing in the argument $x \in \R$ (see Lemma \ref{lem:log1p_non_dec})
\end{itemize}
Using the above we get the lower bound on the SCL:
 \begin{align}
     \Lc(\Hb)&\geq \sum_{c \in [k]}n_c\log\big(n_c-1+(n-n_c)e^{-1}\big)\nonumber
 \end{align}
 \noindent\textbf{Conditions for equality:}
 where equality is achieved if and only if the following hold:
 \begin{itemize}
     \item Last step: $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$
     \item Lemma \ref{lem:jensen_exp_sim}: $\forall i \in [n], \h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} = y_i$. Note that this condition is already implied by $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$. 
     \item Lemma \ref{lem:jensen_exp_con}: $\forall i \in [n], \h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} \neq y_i$. Similar to above, this condition is implied by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$.
     \item Lemma \ref{lem:jensen_log1p}: 
     \begin{align}
         & \frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right) \nonumber\\
         & \ \ = \frac{1}{n-n_c}\left(\h_l^T\sum_{m:y_m \neq y_l}\h_m\right) - \frac{1}{n_c-1}\left(\h_l^T\sum_{j:y_j = y_l,j \neq l}\h_j\right), \forall i,l : y_i = y_l\nonumber
     \end{align}
     Once again, this condition is implied by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$
 \end{itemize}
 Therefore, the condition for equality of the lower bound is given by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$. Further, this implies that the features form an $k$-OF, whose existence is guaranteed because $d \geq k$.  
 % \gk{todo: elaborate}
 \end{proof}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% earlier version
%  \begin{proof}

%  \begin{align}
%      \Lc(\Hb)&:=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{\substack{j\in\mathcal{C}_{y_i}\\j\neq i}
%      }\log\left(\sum_{m:m\neq i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}\right)\nonumber\\
%      &= \sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{m:y_m = y_i, m\neq i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}+\sum_{m:y_m \neq y_i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}\right)\nonumber\\
%      &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{m:y_m = y_i, m\neq i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}+\sum_{m:y_m \neq y_i}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}\right)\nonumber
%      \end{align}
% % Now, we apply Jensen's inequality twice to the strictly convex functions $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$ and $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$, over the variable $m$, for a given $i$ and $j$: 
% Now, applying Lemma \ref{lem:jensen_exp_sim} and \ref{lem:jensen_exp_con}, we use Jensen's inequality twice to the strictly convex functions $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$ and $\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}$, over the variable $m$, for a given $i$ and $j$:
%  \begin{align}
%      \Lc(\Hb) &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\bigg(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\bigg) - \h_i^T\h_j\right)}\nonumber\\
%      & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \h_i^T\h_j\right)}\Bigg]\nonumber
%      \end{align}
% Applying Lemma \ref{lem:affine}, we use that fact that the function $\log\bigg(a\exp{\left(- \h_i^T\h_j\right)}+b\exp{\left(- \h_i^T\h_j\right)}\bigg)$ is affine over its arguments $\h_i^T\h_j$ for a given $i$ and constants $a$ and $b$:
%  \begin{align}
%      \Lc(\Hb) &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log\Bigg[(n_c-1)\exp{\left(\frac{1}{n_c-1}\bigg(\h_i^T\sum_{m:y_m = y_i, m\neq i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\bigg)\right)}\nonumber\\
%      & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\bigg)\right)}\Bigg]\nonumber\\
%      &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log\Bigg[(n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\bigg(\h_i^T\sum_{m:y_m \neq y_i}\h_m\bigg) - \frac{1}{n_c-1}\bigg(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\bigg)\right)}\Bigg]\nonumber
%      \end{align}
% % Now, we apply Jensen's inequality to the function $\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)$, over the variable $i$, and constants $a,b_i,c,d_i$, for a given $i$ : \gk{todo:check strict convexity } 
% Now, applying Lemma \ref{lem:jensen_log1p}, where we use the Jensen's inequality again:
%  \begin{align}
%      \Lc(\Hb)&\geq \sum_{c \in [k]}n_c\log\Bigg[(n_c-1) +(n-n_c)\exp\Bigg(\frac{1}{n_c(n-n_c)}\bigg(\sum_{i\in[n]}\sum_{m:y_m \neq y_i}\h_i^T\h_m\bigg)\nonumber\\
%      & \ \ \ - \frac{1}{n_c(n_c-1)}\bigg(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\bigg)\Bigg)\Bigg]\nonumber
%      \end{align}
% Now, we use the following facts
% \begin{itemize}
%     \item $\h_i^T\h_m \geq 0, \ \text{since} \ h_{i,p} \geq 0, h_{j,p} \geq 0$, with equality if and only if $\h_i^T\h_m = 0$, i.e. $\h_i$ and $\h_m$ are orthogonal to each other.
%     \item $\h_i^T\h_j \leq \|\h_i\|\|\h_j\| = 1$, due to Cauchy-Schwartz inequality, with equality if and only if $\h_i = \h_j$.
%     \item The function $f:\R \rightarrow \R, f(x) =\log\big(a+b\exp(x)\big), a,b \in \R_+$ is non-decreasing in the argument $x \in \R$ (see Lemma \ref{lem:log1p_non_dec})
% \end{itemize}
% Using the above we get the lower bound on the SCL:
%  \begin{align}
%      \Lc(\Hb)&\geq \sum_{c \in [k]}n_c\log\big(n_c-1+(n-n_c)\exp(-1)\big)\nonumber
%  \end{align}
%  \noindent\textbf{Conditions for equality:}
%  where equality is achieved if and only if the following hold:
%  \begin{itemize}
%      \item Last step: $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$
%      \item Lemma \ref{lem:jensen_exp_sim}: $\forall i \in [n], \h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} = y_i$. Note that this condition is already implied by $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$. 
%      \item Lemma \ref{lem:jensen_exp_con}: $\forall i \in [n], \h_i^T\h_{m_1} = \h_i^T\h_{m_2}, \forall m_1,m_2: y_{m_1} = y_{m_2} \neq y_i$. Similar to above, this condition is implied by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$.
%      \item Lemma \ref{lem:jensen_log1p}: 
%      \begin{align}
%          & \frac{1}{n-n_c}\left(\h_i^T\sum_{m:y_m \neq y_i}\h_m\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right) \nonumber\\
%          & \ \ = \frac{1}{n-n_c}\left(\h_l^T\sum_{m:y_m \neq y_l}\h_m\right) - \frac{1}{n_c-1}\left(\h_l^T\sum_{j:y_j = y_l,j \neq l}\h_j\right), \forall i,l : y_i = y_l\nonumber
%      \end{align}
%      Once again, this condition is implied by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$
%  \end{itemize}
%  Therefore, the condition for equality of the lower bound is given by $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$. Further, this implies that the features form an $k$-OF, whose existence is guaranteed because $d \geq k$.  
%  % \gk{todo: elaborate}
%  \end{proof}
 

 \subsection{Unnormalized SCL UFM}
 Conjecture: convergence in the direction of global minima of following ``SVM''
 \begin{align}\label{eq:scl_svm}
 \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i.
 \end{align}

 Conjecture: convergence in the direction of global minima of following ``ReLU-SVM''
 \begin{align}\label{eq:scl_relu_svm}
 \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i, \G[i,j] \geq 0, \forall i,j \in \left[n\right].
 \end{align}

 \subsection{Claims}
 \begin{itemize}
    \item CVX solution with full batch gives ETF for balanced labels:
    \begin{align}
        \arg\min_{\G \succeq 0} \Lc(\G)~~\text{\emph{subj. to}}~\G[i,i] = 1, i\in[n] = I_n - \frac{1}{n}.
    \end{align}
    \item The non-negativity (due to ReLU) constraint on coordinates of features $\h_i$ leads to non-negativity constraints on elements of $\G$ matrix. Corresponding CVX program yields OF for imbalanced labels:
    \begin{align}
        \arg\min_{\G \succeq 0} \Lc(\G)~~\text{\emph{subj. to}}~\G[i,i] = 1, i\in[n], \G[i,j] \geq 0, \forall i,j \in \left[n\right] = I_n.
    \end{align}
    \item SCL ReLU UFM with imbalance empirically converges to OF, suggesting the non-negativity constraint on $\G$ is tight
    \item Prop. \ref{prop:scl_of_lb}: SCL ReLU type loss of \cite{lu2020neural} has OF as its global minimum, in addition to having ETF as the solution without ReLU constraint
    \item To do: prove that SCL with ReLU on imbalance has OF as global minimum for any imbalance - lower bounds?
    \item Unnormalized SCL converges in the direction of SCL SVM? What is the global solution here?
    Ball constraint, growing ball
    \item Solution of \eqref{eq:scl_svm} is the ETF for balanced labels
    \item Solution of \eqref{eq:scl_relu_svm} is the OF (for any imbalance?)
    
 \end{itemize}
 \begin{propo}\label{propo:scl_svm}
 Solution of \eqref{eq:scl_svm} is the ETF with balanced labels
     \begin{align}
 \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,k]\geq 1, i\in[n], y_j = y_i, y_{k}=\neq y_i; = I_n - \frac{1}{n}, \text{when} \ n_c=1, \forall c \in [k] 
 \end{align}
 \end{propo}
 \noindent\textbf{Proof:}\\
 The Lagrangian is
 \begin{align}
     L(\alpha,\G) &= \text{tr}(\G) + \sum_i\sum_{j\neq i}\alpha_{i,j} + \sum_i\sum_{j\neq i}\alpha_{i,j}(-G_{ii}+G_{ij})\\
     &= \sum_i\sum_{j\neq i}\alpha_{i,j} + \text{tr}(\A\G)
 \end{align}
 where 
 \begin{align}
    A_{ij} = \begin{cases}
    -\sum_{j'\neq i}\alpha_{i,j'} , & j = i\\
    \alpha_{i,j}, & j \neq i 
\end{cases} 
 \end{align}
 The dual function is
 \begin{equation}
     \max_{\alpha_{i,j}\geq 0} \sum_i\sum_{j\neq i}\alpha_{i,j} \ \text{sub. to. } \mathbf{I}_n+\A \succeq 0
 \end{equation}
 This can be transformed into
  \begin{equation}
     \max_{B} \text{tr}(\Zhat B) \ \text{sub. to. } B \preceq I, B1_n = 0, B \odot \Zhat \geq 0
 \end{equation}


\noindent~\textbf{General $n_c$:} For a generic $n_c$, the dual is:
\begin{equation}
     \max_{\alpha_{i,j,k}\geq 0} \sum_i\sum_{j: y_j=y_i}\sum_{k:y_k \neq y_i}\alpha_{i,j,k} \ \text{sub. to. } \mathbf{I}_n+\A \succeq 0
 \end{equation}
 where
  \begin{align}
    A_{ij} = \begin{cases}
    -\sum_{k:y_k \neq y_i}\alpha_{i,j,k} , & y_j = y_i\\
    \sum_{j':y_j' = y_i}\alpha_{i,j',j}, & y_j \neq y_i 
\end{cases} 
 \end{align}
 Let $\Bb = -\A$, i.e. 
   \begin{align}
    B_{ij} = \begin{cases}
    \sum_{k:y_k \neq y_i}\alpha_{i,j,k} , & y_j = y_i\\
    -\sum_{j':y_j' = y_i}\alpha_{i,j',j}, & y_j \neq y_i 
\end{cases} 
 \end{align}
 Then, it holds that $\Bb1_n = 0$. The dual becomes
\begin{equation}
     \max_{B} \text{tr}(\Zhat B^T) \ \text{sub. to. } B \preceq I, B1_n = 0,  B \odot \Zhat \geq 0  \ \text{todo:last constraint}
 \end{equation}
 where
 \begin{align}
    \Zhat_{ij} = \begin{cases}
    1 - 1/k , & y_j = y_i\\
    -1/k, & y_j \neq y_i 
\end{cases} 
 \end{align}
 
 \begin{propo}\label{propo:scl_relu_svm}
 Solution of \eqref{eq:scl_svm} is the OF (imbalance?)
     \begin{align}
 \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i, \G[i,j] \geq 0, \forall i,j \in \left[n\right] = I_n
 \end{align}
 \end{propo}

\subsection{Useful Lemmas}
 \begin{lemma}\label{lem:motivation}
    Given a symmetric matrix $\G \succeq 0$ and $\G_{ii} = 1, \forall i$, it follows that $|\G_{ij}| \leq 1$.
Consider a vector $\ab = [a_1 \ a_2 \ ... \ a_n]^T$, where $a_i = 1, a_j = -\G_{ij}, a_k = 0, \forall k \neq i,j$. Since $\G \succeq 0$, we have the following
\begin{align*}
    \ab^T\G\ab = 1 - \G_{ij}^2 &\geq 0 \\
    \implies |\G_{ij}| &\leq 1
\end{align*}
\end{lemma}







\subsection{Optimality of OF}
\subsubsection{ReLU SCL with only dissimilar examples}
First, consider the setting of \cite{lu2020neural}. Here, $n_c = 1, \forall c \in [k]$, and we use the following objective.
\begin{align}\label{eq:fu}
    \Lc_\tau(\Hb):=\sum_{i\in[n]}\log(1+\sum_{j\neq i}\exp{(\h_j^T\h_i -1)})
\end{align}
where $\h_i\in \R^{d}$
\cite{lu2020neural} proves that the global minimizers of the following problem form a simplex ETF:
\begin{align}
 \arg\min_\Hb \Lc_T(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, i\in[n].
 \end{align}
 where $d \geq n-1$ and $T > 0$. The proof involves finding a lower bound for the loss and identifying the conditions for achievability of the lower bound. We consider the following modification of the problem, corresponding to the presence of ReLU units in the last hidden-layer of a DNN.
\begin{align}\label{eq:scl_relu}
 \arg\min_\Hb \Lc_\tau(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
 \end{align}
 
 \begin{propo}\label{prop:scl_of_lb}
 The following lower bound holds for the objective function of \eqref{eq:scl_relu} with $\tau>0$ and $d\geq n$:
  \begin{align}
      \Lc_\tau(\Hb) \geq n\log(1+(n-1)\exp{(-\tau)}),
  \end{align}
  and the equality is achieved if and only if
  $\h_i^T\h_j = 0, \ \forall i\neq j$.
 \end{propo}
 \begin{proof}
 
 \end{proof}
 Thus, the global minimizers form an OF. Note that this result required that the dimension of the representation space be at least $n$, as opposed to $n-1$, unlike earlier. This is due to the fact that an OF exists if and only if $d\geq n$.

% \subsection{SCL with similar and dissimilar examples}
%  With setting of \cite{pmlr-v139-graf21a}, we have the following SCL loss:
%   \begin{align}\label{eq:scl_loss}
%      \Lc(\Hb):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j' \neq i, j' \neq j}\exp{-(\h_i^T\h_j - \h_i^T\h_j')})
%  \end{align}
%  We consider the following convex relaxation:
%  \begin{align}\label{eq:scl_loss_cvx}
%      \Lc(\G):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j' \neq i, j' \neq j}\exp{-(\G(i,j) - \G(i,j'))})
%  \end{align}
%  Split the inner sum into two types of terms: similar and dissimilar examples
%  \begin{align}
%      \Lc(\G):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j': y_{j'} \neq y_i}\exp{-(\G(i,j) - \G(i,j'))}+\sum_{j': y_{j'} = y_i, j' \neq i, j' \neq j}\exp{-(\G(i,j) - \G(i,j'))})
%  \end{align}
% check if loss goes to sum log(1+ {similar terms}
% todo:check the following bound holds if labels are balanced. We know this for $n_c = 1,2$:
% \begin{align}
%       \Lc_(\G) \geq n\log((n_c-1)+(n-n_c)\exp{(-1)}),
%   \end{align}
\subsubsection{SCL reduction with 2 examples each}
\gk{assuming the symmetry argument, we consider below the reduced objective function for a balanced dataset with 2 representative examples for every class.} Consider the setting of ReLU SCL optimization. For an example $i$, let $\ibar$ be its similar example, i.e., $y_{\ibar} = y_i$.
\begin{align}\label{eq:scl_red}
     \Lc(\Hb):=\sum_{i\in[2k]}\log\left(1+\sum_{y_j \neq y_i}\exp{\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right)}\right)
 \end{align}
 We solve the following minimization:
 \begin{align}\label{eq:scl_relu_red}
 \arg\min_\Hb \Lc(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
 \end{align}
  \begin{propo}\label{prop:scl_relu_red}
 The following lower bound holds for the objective function of \eqref{eq:scl_red} with $d\geq n$:
  \begin{align}
      \Lc(\Hb) \geq 2k\log\left(1+(2k-2)\exp(-1)\right),
  \end{align}
  and the equality is achieved if and only if
  $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_{\ibar}, \forall i \in [2k]$.
 \end{propo}
 \begin{proof}
 Consider the loss function
 \begin{align}
     \Lc(\Hb):=\sum_{i\in[2k]}\log\left(1+\sum_{y_j \neq y_i}\exp{\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right)}\right)
 \end{align}
 Due to Jensen's inequality, we have
 \begin{align}
     \frac{1}{2k-2}\sum_{y_j\neq y_i}\exp\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right) \geq \exp\left(\frac{1}{2k-2}\h_i\right)
 \end{align}
 \gk{todo}
 \end{proof}

 \subsubsection{SCL with general balanced dataset}
 Setting of \cite{pmlr-v139-graf21a}:
 \begin{align}\label{eq:scl_bal}
     \Lc(\Hb):=\sum_{i\in[n]}\frac{1}{n_c-1}\sum_{j \neq i, y_j = y_i}\log\left(1+\sum_{k:y_k \neq y_i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)
 \end{align}
We solve the following minimization:
 \begin{align}\label{eq:scl_relu_bal_old}
 \arg\min_\Hb \Lc(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
 \end{align}
  \begin{propo}\label{prop:scl_relu_bal}
 The following lower bound holds for the objective function of \eqref{eq:scl_bal} with $d\geq n$:
  \begin{align}
      \Lc(\Hb) \geq n\log\left(n_c-1+(n-n_c)\exp(-1)\right),
  \end{align}
  and the equality is achieved if and only if
  $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$.
 \end{propo}
 \begin{proof}
 Consider the loss function
 \begin{align}
     \Lc(\Hb)&:=\sum_{i\in[n]}\frac{1}{n_c-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{k:k\neq i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)\\
     &= \sum_{i\in[n]}\frac{1}{n_c-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{k:y_k = y_i, k\neq i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}+\sum_{k:y_k \neq y_i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)\\
     &\geq \sum_{i\in[n]}\frac{1}{n_c-1}\sum_{j \neq i, y_j = y_i}\log((n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{k:y_k = y_i, k\neq i}\h_k\right) - \h_i^T\h_j\right)}\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \h_i^T\h_j\right)})\\
     &\geq \sum_{i\in[n]}\log((n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{k:y_k = y_i, k\neq i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\right)\right)}\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)})\\
     &= \sum_{i\in[n]}\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)\\
     &\geq n\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n(n-n_c)}\left(\sum_{i\in[n]}\sum_{k:y_k \neq y_i}\h_i^T\h_k\right) - \frac{1}{n(n_c-1)}\left(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\right)\right)}\right)\\
     &\geq n\log\left(n_c-1+(n-n_c)\exp(-1)\right)
 \end{align}
 where equality is achieved if and only if $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$.
 \gk{todo: elaborate}
 \end{proof}

 \subsubsection{SCL with imbalanced dataset}
 Setting of \cite{pmlr-v139-graf21a}:
 \begin{align}\label{eq:scl_imbal}
     \Lc(\Hb):=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(1+\sum_{k:y_k \neq y_i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)
 \end{align}
We solve the following minimization:
 \begin{align}\label{eq:scl_relu_bal_old}
 \arg\min_\Hb \Lc(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
 \end{align}
  \begin{propo}\label{prop:scl_relu_bal}
 The following lower bound holds for the objective function of \eqref{eq:scl_bal} with $d\geq n$:
  \begin{align}
      \Lc(\Hb) \geq \sum_{c \in [k]}n_c\log\left(n_c-1+(n-n_c)\exp(-1)\right),
  \end{align}
  and the equality is achieved if and only if
  $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$.
 \end{propo}
 \begin{proof}
 Identical to the above proof.
 \begin{align}
     \Lc(\Hb)&:=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{k:k\neq i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)\\
     &= \sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{k:y_k = y_i, k\neq i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}+\sum_{k:y_k \neq y_i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)\\
     &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(\sum_{k:y_k = y_i, k\neq i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}+\sum_{k:y_k \neq y_i}\exp{\left(\h_i^T\h_k - \h_i^T\h_j\right)}\right)\\
     &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\frac{1}{n_{c}-1}\sum_{j \neq i, y_j = y_i}\log((n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{k:y_k = y_i, k\neq i}\h_k\right) - \h_i^T\h_j\right)}\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \h_i^T\h_j\right)})\\
     &\geq \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log((n_c-1)\exp{\left(\frac{1}{n_c-1}\left(\h_i^T\sum_{k:y_k = y_i, k\neq i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i, j \neq i}\h_j\right)\right)}\\
     & \ \ \ +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)})\\
     &= \sum_{c \in [k]}\sum_{i\in\mathcal{C}_c}\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n-n_c}\left(\h_i^T\sum_{k:y_k \neq y_i}\h_k\right) - \frac{1}{n_c-1}\left(\h_i^T\sum_{j:y_j = y_i,j \neq i}\h_j\right)\right)}\right)\\
     &\geq \sum_{c \in [k]}n_c\log\left((n_c-1) +(n-n_c)\exp{\left(\frac{1}{n_c(n-n_c)}\left(\sum_{i\in[n]}\sum_{k:y_k \neq y_i}\h_i^T\h_k\right) - \frac{1}{n_c(n_c-1)}\left(\sum_{i\in[n]}\sum_{j:y_j = y_i,j \neq i}\h_i^T\h_j\right)\right)}\right)\\
     &\geq \sum_{c \in [k]}n_c\log\left(n_c-1+(n-n_c)\exp(-1)\right)
 \end{align}
 where equality is achieved if and only if $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i \in [n]$.
 \gk{todo: elaborate}
 \end{proof}


==> sections_v2/outlook.tex <==
%\vspace{-0.25cm}
We propose \emph{\ref{SELI}} as the class-imbalance-invariant geometry of classifiers and embeddings learnt by overparameterized models when trained beyond zero training error. We arrive at it after showing that the UF-SVM global minimizers follow this geometry. Subsequently, we conjecture that: (C1) GD on the UFM leads to solutions approaching the SELI geometry asymptotically in the number of epochs; (C2) training of deep-nets beyond zero training error learns models that approach the SELI geometry. 

Statement (C1) is a conjecture and does not follow from Theorem~\ref{thm:SVM}. This is because GD is only known to converge to KKT points of the non-convex UF-SVM \cite{lyu2019gradient,ULPM}, which are not necessarily global minima.  Thus, while Proposition~\ref{propo:reg_path} combined with the benign landscape of the corresponding ridge-regularized minimization, as well as, our experiments suggest its validity, the conjecture remains to be further investigated.\footnote{Relying on \citep{ji2020directional}, \citet{vardi2021margin} showed gradient flow  finds global minimizers in deep linear nets. However, these only apply to binary classification. We show that interesting behaviors might occur (e.g. in the role of regularization and geometry) when $k>2$ and $R>1$ calling  further studies.} We also note that convergence rates appear slower with increasing imbalance levels; a feature which is interesting to study further. 

Regarding conjecture (C2), we deem our experiments encouraging: the classifiers' and embeddings' geometries get closer to the SELI geometry as neural-network training progresses. Specifically, the Gram matrices $\G_\W$ and $\G_\Hb$ of the classifiers and embeddings, respectively, align increasingly better with their SELI counterparts $\Vb\Lambdab\Vb^T$ and $\Ub\Lambdab\Ub^T$; see Fig.~\ref{fig:}. Also, Fig. \ref{fig:} shows that Lemma \ref{lem:} is able to make predictions regarding the norms of majorities versus minorities. We note that, similar to the UFM experiments, convergence appears slower for larger imbalance ratios. Also, we observe better convergence for classifiers compared to embeddings \ct{and for norm predictions compared to angle predictions}. Overall, we hope our results motivate further experimental investigations, especially since data imbalances appear frequently across applications. 
 %\new{In our experiments, we use optimization-parameter choices (e.g. learning rate, weight-decay, momentum) that are consistent with previous works in the literature.} 

 Beyond that, we believe that further similar studies on identifying geometrical structures of learned embeddings and classifiers could offer new perspectives on generalization. For example, our results could pave that way since they uncover different geometries (aka SELI for different $R$ values), each leading to different generalization (worse for increasing $R$ \cite{byrd2019effect}). %On one hand, CE on balanced data leads to ETF geometry, and, is known to generalize well. On the other hand, CE on imbalanced data changes the geometry, and, is known to achieve poor generalization  in terms of (say) balanced error \cite{byrd2019effect}. since having access to different geometries  each leading to different generalization might help uncovering connections between train geometries and generalization. 
 Relatedly, we envision that further such studies lead to algorithmic contributions in deep imbalanced learning as they can facilitate studying the implicit bias effect of CE adjustments and post-hoc techniques tailored to imbalanced data \cite{TengyuMa,Menon,CDT,KimKim,kang2020decoupling,ganesh,autobalance}.


\ct{
Future work:
\begin{itemize}
\item general imbalance (beyond step)
\item other losses, e.g. square loss?
\end{itemize}
}

%\paragraph{Rethinking implicit bias: Imbalance trouble}  \ct{needs rewriting}A series of works that examine the implicit bias of gradient descent (and of its variants, such as stochastic GD, gradient flow, etc.) yield characterizations of the preferred minimizer that roughly take the following format: the model weights found by GD converge to a KKT point of an optimization program that minimizes a certain norm of the weights subject to an interpolation constraint. In the simplest and cleanest setting of a linear model trained with either square-loss or cross-entropy, the resulting optimization is convex and minimizes the $\ell_2$ norm of the weights subject to either an interpolation constraint or a linear separability constraint \cite{}. For example, GD on cross-entropy loss in a linear setting converges (in direction) to the max-margin classifier \cite{}. We note that in general nonlinear settings, the norm that is minimized can depend on the model architecture \cite{}. Perhaps more importantly, beyond the linear setting, the resulting optimization program is non-convex. This naturally raises the question of whether the KKT point preferred by GD is a global minimizer. Our first finding shows that the answer is in general negative even in the simplest setting beyond the standard linear model, that of a 2-layer linear network:
% 
%\begin{finding}
%Consider training of a 2-layer linear network with gradient flow (GF) on cross-entropy (CE) loss without explicit regularization. There exists multiclass imbalanced dataset such that the global minimizer of the (non-convex) max-margin optimization is \emph{not} a convergence direction of GF.
%\end{finding}
%\begin{figure}[ht!]
%	\centering
%	\includegraphics[width=\linewidth]{Figures/G_errors_CE}
%\end{figure}
%\ct{@Ganesh: One plot -two curves. One for balanced. one for imbalanced. distance to G cvx (which corresponds to global optimum) over epochs. In the LPM model.}


%We believe these questions are important since data imbalances appear more frequently, than not, across applications \cite{}. Beyond that, answering these questions might offer a new perspective in better understanding potential connections of NC to generalization. On the one hand, CE entropy on balanced data leads to the symmetric geometry characterized by NC1--3, and also, it is known to achieve good generalization. On the other hand, as we will see, the presence of imbalances drastically changes the geometry, and also, it is known to achieve poor generalization, measured in terms of (say) balanced error \cite{}. Having access to different geometries that each leads to different generalization levels might shed light in understand wether a connection between NC and generalization can be formalized. Relatedly, we envision that our study leads to algorithmic contributions in imbalanced learning with overparameterized models as it can be used to study changes to NC geometry when training with losses other than CE that are tailored to imbalanced data.

==> sections_v2/related_work.tex <==
%\ct{add citation to this pls: https://arxiv.org/pdf/2305.13165.pdf}\ct{If done pls delete my comments}

%\ct{Shall we }
% \vspace{-17}
The simple concept behind SCL, introduced as an extension of the contrastive loss \citep[e.g.,][]{chen2020simple, tian2019contrastive} to the fully supervised setting by \citet{khosla2020supervised},  involves pulling together the normalized features of examples belonging to the same class while pushing them away from examples of other classes.  Despite its simplicity, SCL offers a generalization of existing loss functions like the triplet loss \citep{weinberger2005distance} and the N-pair loss \citep{sohn2016improved}, and surpasses the performance of the CE loss on standard vision classification datasets,  while also being more robust to natural corruptions in the data and less sensitive to hyperparameters \citep{khosla2020supervised}. 
% Further studies have also highlighted the resilience of SCL and variants alike to distribution shifts, particularly in scenarios involving training with imbalanced data \citep{gunel2020supervised,jitkrittum2022elm,samuel2021distributional,li2022targeted,kang2021exploring,li2022targeted}. These studies commonly involve training a combination of CE and SCL-type losses.

% In recent years, there has been a notable increase in interest regarding the properties of the embedding space and weight vectors learned through unsupervised and supervised contrastive losses, as well as CE. Of particular importance is the endeavor to uncover the fundamental distinctions between these losses, which could be essential in order to effectively harness the respective strengths of each method and formalize principled ways to combine them.
% Specifically, an increasing series of recent works have focused on uncovering the embedding geometry of CE, Mean-Squared Error (MSE) losses, and their variants \citep{NC,zhu2021geometric,zhou2022optimization,zhou2022all,lu2020neural,seli,yaras2022neural,behnia2023implicit,gao2023study,zhou2022all,graf2021dissecting,tirer2022extended,han2021neural,fang2021exploring,sukenik2023deep}. In addition to the scientific curiosity surrounding such  studies, this exploration has paved the way for novel CE-based approaches to training DNNs on imbalanced data \citep{behnia2023implicit,liang2023inducing,xie2023neural,sharma2023learning,dang2023neural}. 

In recent years, there has been a notable interest regarding the properties of the embedding space and weights learned through unsupervised/supervised contrastive losses, as well as CE. 
Of particular importance is the endeavor to uncover the fundamental distinctions between these losses to effectively harness each of their strengths and formalize principled ways to combine them.
Specifically, starting by \cite{NC}, an increasing series of recent works have focused on uncovering the embedding geometry of CE, Mean-Squared Error (MSE) losses, and their variants. We highlighted some of these works in Sec.~\ref{sec:intro} while numerous other works contribute to these investigation \citep[e.g.,][]{zhou2022optimization,zhou2022all,yaras2022neural,gao2023study,han2021neural,sukenik2023deep}. In addition to the scientific curiosity surrounding such  studies, this exploration has paved the way for novel CE-based approaches to training DNNs on imbalanced data \citep{behnia2023implicit,liang2023inducing,xie2023neural,sharma2023learning,dang2023neural,yang2022inducing}. 

However, less attention has been devoted in the existing literature to a comparable set of results for the SCL. \citet{graf2021dissecting} is the first to study the embedding geometry of SCL for balanced data and comparing it to that of CE. To tackle the imbalances, and inspired by \citet{graf2021dissecting}
that suggests balanced data is crucial for obtaining symmetric embeddings, 
\citet{zhu2022balanced} have recently proposed and investigated a modification of the SCL that boosts performance under class imbalances.  
% Our work extends the study of \citet{graf2021dissecting} to imbalanced data and complements the findings of \citet{zhu2022balanced} by showing that SCL with ReLU can actually learn symmetric embedding structure even in the presence of imbalances. 
Our work extends  and complements these two studies by showing that SCL with ReLU can actually learn symmetric embedding structure even in the presence of imbalances. While preparing the manuscript of our paper, we became aware of a recent work \citep{cho2023mini}, where the authors consider the mini-batch optimization of the unsupervised contrastive loss and propose a loss-based choice of mini-batches to speed up convergence to ETF. Since their setting is different, it would be interesting to see how our ideas can benefit their findings and vice versa.

% However, less attention has been devoted in the existing literature to a comparable set of comprehensive results for the SCL. \citet{graf2021dissecting} is the first study  that explicitly delves into understanding the embedding geometry of SCL and comparing it to that of CE. While this study is pioneering, we note two limitations. Their investigation primarily focuses on balanced data. To tackle this, and inspired by suggestions in \citet{graf2021dissecting} that balanced data is crucial for obtaining symmetric embeddings geometries, \citet{zhu2022balanced} have very recently proposed and investigated a modification of the SCL that boosts performance under class imbalances.  


% %\citet{li2022targeted} is also motivated by similar feature-geometry considerations when dealing with imbalanced data and devise an approach aiming at mapping the features to specified targets for improved performance. 
%Other recent works have also attempted to find hybrid methods combining traditional supervised methods with contrastive techniques for various classification tasks \citep[e.g.,][]{kang2021exploring,gunel2020supervised}.

% Our work extends the study of \citet{graf2021dissecting} to imbalanced data and complements the findings of \citet{zhu2022balanced} by showing that SCL with ReLU can actually learn symmetric embedding structure even in the presence of imbalances. While preparing the manuscript of our paper, we were made aware of a recent work \citep{cho2023mini}, where the authors consider the mini-batch optimization of the unsupervised contrastive loss and propose a loss-based choice of mini-batches to speed up convergence to ETF.

%proposes methods to combine CE with SCL and also find evidence in favor of SCL over CE in learning from imbalanced data.} 
% \todo{maybe omit this?}Among the emerging works demonstrating the benefits of supervised contrastive learning in training neural networks, \citet{gunel2020supervised} propose to combine the CE and SCL losses for fine-tuning pre-trained language models.} %This work is motivated by the stability issues of the CE loss in fine-tuning tasks in natural language processing applications.

%Over the past few years, there has been a surge of interest in understanding the properties of the feature space and weight vectors learned by unsupervised and supervised contrastive losses and CE. Especially significant is a quest to reveal the key differences between the approaches. Such an understanding can be crucial for aiding meaningful ways to utilize the combined strengths of the two.


%\new{In an attempt to understand the geometry of features learned by the SCL, \citet{graf2021dissecting} studied the global optima of the loss function under the Unconstrained Features Model (UFM), with balanced label distribution. By ``geometry'' of features, we refer to the (relative) norms and pairwise angles of feature-embeddings in the feature space. It was shown that under the setup where the ERM consists of the aggregate loss over all combinations of batches of a given size (possibly with overlapping examples), that the global minimizers form the Simplex Equiangular Tight Frame (ETF). This result (\citep[Thm.~2]{graf2021dissecting}) uncovered that the geometry of training features is closely related to that learned by the CE loss in UFM under balanced label distribution. \citet{zhu2022balanced} is motivated by the observation in \citet{graf2021dissecting} that balanced data is necessary for the optimal feature geometry to have symmetric structure, and they propose a modification of the SCL that is observed to help in learning from imbalanced data. The authors of \citet{li2022targeted} are also motivated by the feature geometry in presence of imbalanced data and devise an approach that is aimed at mapping the features to specified targets. Recent works have also attempted to find hybrid methods combining traditional supervised methods with contrastive techniques for various classification tasks \citep[e.g.,][]{kang2021exploring,gunel2020supervised}.}
% NC of CE \citep{gao2023study,zhou2022all,yaras2022neural}\citep{NC,zhu2021geometric,zhou2022optimization,zhou2022all,lu2020neural,seli,behnia2023implicit,yaras2022neural,zhong2023understanding}
% \citep{kasarla2022maximum}
% Imbalance \todo{elaborate} \citep{liu2023inducing,liang2023inducing,xie2023neural,sharma2023learning,dang2023neural}

% %To the best of our knowledge, there only 
% %Our findings are novel since to the best of our knowledge no previous work derived . 
% %The authors of \citet{NC} discovered and formalized the Neural collapse phenomenon. Their formalization involved four NC properties. The first property concerns the collapse of class embeddings to their corresponding means. Properties two and three concern the geometry of class-means and classifier-weights, specifically their alignment and convergence to a simplex ETF geometry. Property four is a consequence of the other three properties, hence is less important in the formalization and we do not discuss it further. 
% %Motivated by our findings, we propose and use here a regrouping/renaming of the aforementioned three properties. We refer to the first property as the \emph{\ref{NC}} property, and, to the second and third properties as the \emph{\ref{ETF}} property. We argue that this distinction is important towards a formulation that is invariant across class-imbalances, by showing that the ETF property is \emph{note} invariant and replacing it with the \emph{\ref{\SELI}}~property. For balanced data, the \SELI~property simplifies to the ETF property. 
% \vspace{-0.2cm}
% \gk{todo} The original contribution by  \citet{NC} has attracted lots of attention resulting  in numerous followups within short time period, e.g., \citep{zhu2021geometric,ULPM,fang2021exploring,han2021neural,lu2020neural,mixon2020neural,graf2021dissecting,zhou2022optimization}. (See also \citep[Sec.~E]{han2021neural} for a  review of the recent literature.) Several works have proposed and/or used the UFM with CE training to 
% analyze theoretical abstractions of NC  \citep{zhu2021geometric,ULPM,fang2021exploring,graf2021dissecting}. We drove particular inspiration from \citet{zhu2021geometric}, who  presented a particularly transparent and complete analysis of the optimization landscape of ridge-regularized CE minimization for the UFM under balanced data.  In the same spirit, we also relied on the UFM.  
% %\footnote{We first came across the UFM idea thanks to \citet{mixon2020neural}; thus, we chose to maintain their naming of the model. Other works adapt the name Layer Peeled Model, originally proposed in \citet{fang2021exploring}.}
%  However, our work is, to the best of our knowledge, the first explicit geometry analysis for class-imbalanced data. See also Table \ref{table:intro} for a comparison. %Also, it appears that none of these previous works identid
% %The only previous work considering class imbalances is \citet{fang2021exploring}, which we discuss separately below.
% %A close inspection of  their proof made us realize that their landscape results remain invariant to imbalances after appropriate reformulation (compare Thm. \ref{thm:regularized} here to \citet[Thm.~3.2]{zhu2021geometric}). Nevertheless, 
% %Here, we found that, with imbalances, not only   ETF geometry changes, but also, the change is  sensitive to the regularization strenfth. Motivated by this and the practice of training with very small weight-decay, we established the limit of solutions for vanishing regularization and we analyzed their geometry. 

% %Notably, our technical analysis is also new compared to the common underlying techniques used in \emph{all} previous works %\citep{zhu2021geometric}. In fact, it is different compared to all aforementioned analyses \citep{zhu2021geometric,ULPM,graf2021dissecting,lu2020neural}; see also Remark~\ref{remark:comparison}. \citet{ULPM} is the only previous work that studied the UF-SVM (aka zero regularization). However, their result holds only for balanced data and is a special case of Thm.~\ref{thm:SVM}. See also Table \ref{table:intro}.

% %Those works relied on lower bounding the CE loss combining Jensen's and Cauchy-Schwartz inequalities. It is not clear how to extend that technique to class-imbalance settings. Intuitively, the challenge is that those inequalities are tight only when symmetric structures occur (e.g. classifiers align with embeddings, which does not hold under imbalances) . Notably, the difference also applies when comparing our results to \citet{ULPM}, the only previous work that studied the UF-SVM. Not only does their results hold for balanced data, but also, their analysis is again based on the use of same inequalities. Instead, we use convex relaxations and duality to directly analyze the UF-SVM and our results hold for all imbalance levels. 


% The only previous work on neural collapse with imbalances is  
% \citet{fang2021exploring}, which was the first to note that collapse of the embeddings is preserved, but otherwise the geometry might skew away from ETF. Also, \citet{fang2021exploring} first proposed studying the new geometry using the UFM and appropriate convex relaxations. With this setup, they presented an intriguing finding, which they termed \emph{minority collapse}: for large imbalance levels, the minorities' classifiers collapse to the same vector. As  mentioned above, our focus is on the, particularly relevant for deep-learning practice, zero-training error scenarios. This excludes minority collapse by definition. More importantly, we derive an explicit geometric characterization of \emph{both}  embeddings and  classifiers for \emph{both} majorities and minorities and for \emph{all} imbalance levels.  {Specializing these findings to vanishing regularization and imbalance ratio growing to infinity recovers and gives new insights to minority collapse. 
% %see \Sec~\ref{sec:minority} for an elaborate discussion.
% }

% % There are two key differences to our findings. First, we focus on zero training-error regime where CE solutions perfectly separate the data. This is \emph{not} the case under minority collapse, since training accuracy is then zero for minorities. Second, and most important, we derive an explicit characterization of the geometry of both the embeddings and the classifiers that also holds for \emph{all} imbalance levels. In the SM and in Sec.~ \ref{sec:experiments} we also show  that minority collapse is \emph{not} observed  for finite levels of imbalance and sufficiently small regularization. 

% Our results also draw from and relate to the literatures on implicit bias, matrix factorization, and imbalanced deep-learning.  {We defer a detailed discussion on these to Sec. \ref{sec:rel2} of the Supplementary Material. }
















==> sections_v2/scl_temp.tex <==
% \section{Optimality of OF}
% \subsection{ReLU SCL with only dissimilar examples}
% First, consider the setting of \cite{lu2020neural}. Here, $n_c = 1, \forall c \in [k]$, and we use the following objective.
% \begin{align}\label{eq:fu}
%     \Lc_\tau(\Hb):=\sum_{i\in[n]}\log(1+\sum_{j\neq i}\exp{(\h_j^T\h_i -1)})
% \end{align}
% where $\h_i\in \R^{d}$
% \cite{lu2020neural} proves that the global minimizers of the following problem form a simplex ETF:
% \begin{align}
%  \arg\min_\Hb \Lc_T(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, i\in[n].
%  \end{align}
%  where $d \geq n-1$ and $T > 0$. The proof involves finding a lower bound for the loss and identifying the conditions for achievability of the lower bound. We consider the following modification of the problem, corresponding to the presence of ReLU units in the last hidden-layer of a DNN.
% \begin{align}\label{eq:scl_relu}
%  \arg\min_\Hb \Lc_\tau(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
%  \end{align}
 
%  \begin{propo}\label{prop:scl_of_lb}
%  The following lower bound holds for the objective function of \eqref{eq:scl_relu} with $\tau>0$ and $d\geq n$:
%   \begin{align}
%       \Lc_\tau(\Hb) \geq n\log(1+(n-1)\exp{(-\tau)}),
%   \end{align}
%   and the equality is achieved if and only if
%   $\h_i^T\h_j = 0, \ \forall i\neq j$.
%  \end{propo}
%  \begin{proof}
 
%  \end{proof}
%  Thus, the global minimizers form an OF. Note that this result required that the dimension of the representation space be at least $n$, as opposed to $n-1$, unlike earlier. This is due to the fact that an OF exists if and only if $d\geq n$.

% \subsection{SCL with similar and dissimilar examples}
%  With setting of \cite{pmlr-v139-graf21a}, we have the following SCL loss:
%   \begin{align}\label{eq:scl_loss}
%      \Lc(\Hb):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j' \neq i, j' \neq j}\exp{-(\h_i^T\h_j - \h_i^T\h_j')})
%  \end{align}
%  We consider the following convex relaxation:
%  \begin{align}\label{eq:scl_loss_cvx}
%      \Lc(\G):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j' \neq i, j' \neq j}\exp{-(\G(i,j) - \G(i,j'))})
%  \end{align}
%  Split the inner sum into two types of terms: similar and dissimilar examples
%  \begin{align}
%      \Lc(\G):=\sum_{i\in[n]}\sum_{j:y_j = y_i}\log(1+\sum_{j': y_{j'} \neq y_i}\exp{-(\G(i,j) - \G(i,j'))}+\sum_{j': y_{j'} = y_i, j' \neq i, j' \neq j}\exp{-(\G(i,j) - \G(i,j'))})
%  \end{align}
% check if loss goes to sum log(1+ {similar terms}
% todo:check the following bound holds if labels are balanced:
% \begin{align}
%       \Lc_(\G) \geq n\log(1+(k-1)\exp{(-1)}),
%   \end{align}
% \subsection{SCL reduction with 2 examples each}
% \gk{assuming the symmetry argument, we consider below the reduced objective function for a balanced dataset with 2 representative examples for every class.} Consider the setting of ReLU SCL optimization. For an example $i$, let $\ibar$ be its similar example, i.e., $y_{\ibar} = y_i$.
% \begin{align}\label{eq:scl_red}
%      \Lc(\Hb):=\sum_{i\in[2k]}\log\left(1+\sum_{y_j \neq y_i}\exp{\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right)}\right)
%  \end{align}
%  We solve the following minimization:
%  \begin{align}\label{eq:scl_relu_red}
%  \arg\min_\Hb \Lc(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
%  \end{align}
%   \begin{propo}\label{prop:scl_relu_red}
%  The following lower bound holds for the objective function of \eqref{eq:scl_red} with $d\geq n$:
%   \begin{align}
%       \Lc(\Hb) \geq 2k\log\left(1+(2k-2)\exp(-1)\right),
%   \end{align}
%   and the equality is achieved if and only if
%   $\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_{\ibar}, \forall i \in [2k]$.
%  \end{propo}
%  \begin{proof}
%  Consider the loss function
%  \begin{align}
%      \Lc(\Hb):=\sum_{i\in[2k]}\log\left(1+\sum_{y_j \neq y_i}\exp{\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right)}\right)
%  \end{align}
%  Due to Jensen's inequality, we have
%  \begin{align}
%      \frac{1}{2k-2}\sum_{y_j\neq y_i}\exp\left(\h_i^T\h_j - \h_i^T\h_{\ibar}\right) \geq \exp\left(\frac{1}{2k-2}\h_i\right)
%  \end{align}
%  \gk{todo}
%  \end{proof}
%  \subsection{SCL UFM results}
%  Add plots showing convergence to OF in UFM-ReLU for any imbalance.

%  \subsection{Unnormalized SCL UFM}
%  Conjecture: convergence in the direction of global minima of following ``SVM''
%  \begin{align}\label{eq:scl_svm}
%  \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i.
%  \end{align}

%  Conjecture: convergence in the direction of global minima of following ``ReLU-SVM''
%  \begin{align}\label{eq:scl_relu_svm}
%  \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i, \G[i,j] \geq 0, \forall i,j \in \left[n\right].
%  \end{align}

%  \subsection{Claims}
%  \begin{itemize}
%     \item CVX solution with full batch gives ETF for balanced labels:
%     \begin{align}
%         \arg\min_{\G \succeq 0} \Lc(\G)~~\text{\emph{subj. to}}~\G[i,i] = 1, i\in[n] = I_n - \frac{1}{n}.
%     \end{align}
%     \item The non-negativity (due to ReLU) constraint on coordinates of features $\h_i$ leads to non-negativity constraints on elements of $\G$ matrix. Corresponding CVX program yields OF for imbalanced labels:
%     \begin{align}
%         \arg\min_{\G \succeq 0} \Lc(\G)~~\text{\emph{subj. to}}~\G[i,i] = 1, i\in[n], \G[i,j] \geq 0, \forall i,j \in \left[n\right] = I_n.
%     \end{align}
%     \item SCL ReLU UFM with imbalance empirically converges to OF, suggesting the non-negativity constraint on $\G$ is tight
%     \item Prop. \ref{prop:scl_of_lb}: SCL ReLU type loss of \cite{lu2020neural} has OF as its global minimum, in addition to having ETF as the solution without ReLU constraint
%     \item To do: prove that SCL with ReLU on imbalance has OF as global minimum for any imbalance - lower bounds?
%     \item Unnormalized SCL converges in the direction of SCL SVM? What is the global solution here?
%     Ball constraint, growing ball
%     \item Solution of \eqref{eq:scl_svm} is the ETF for balanced labels
%     \item Solution of \eqref{eq:scl_relu_svm} is the OF (for any imbalance?)
    
%  \end{itemize}
%  \begin{propo}\label{propo:scl_svm}
%  Solution of \eqref{eq:scl_svm} is the ETF with balanced labels
%      \begin{align}
%  \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,k]\geq 1, i\in[n], y_j = y_i, y_{k}=\neq y_i; = I_n - \frac{1}{n}, \text{when} \ n_c=1, \forall c \in [k] 
%  \end{align}
%  \end{propo}
%  \noindent\textbf{Proof:}\\
%  The Lagrangian is
%  \begin{align}
%      L(\alpha,\G) &= \text{tr}(\G) + \sum_i\sum_{j\neq i}\alpha_{i,j} + \sum_i\sum_{j\neq i}\alpha_{i,j}(-G_{ii}+G_{ij})\\
%      &= \sum_i\sum_{j\neq i}\alpha_{i,j} + \text{tr}(\A\G)
%  \end{align}
%  where 
%  \begin{align}
%     A_{ij} = \begin{cases}
%     -\sum_{j'\neq i}\alpha_{i,j'} , & j = i\\
%     \alpha_{i,j}, & j \neq i 
% \end{cases} 
%  \end{align}
%  The dual function is
%  \begin{equation}
%      \max_{\alpha_{i,j}\geq 0} \sum_i\sum_{j\neq i}\alpha_{i,j} \ \text{sub. to. } \mathbf{I}_n+\A \succeq 0
%  \end{equation}
%  This can be transformed into
%   \begin{equation}
%      \max_{B} \text{tr}(\Zhat B) \ \text{sub. to. } B \preceq I, B1_n = 0, B \hada \odot \Zhat \geq 0
%  \end{equation}


% \noindent~\textbf{General $n_c$:} For a generic $n_c$, the dual is:
% \begin{equation}
%      \max_{\alpha_{i,j,k}\geq 0} \sum_i\sum_{j: y_j=y_i}\sum_{k:y_k \neq y_i}\alpha_{i,j,k} \ \text{sub. to. } \mathbf{I}_n+\A \succeq 0
%  \end{equation}
%  where
%   \begin{align}
%     A_{ij} = \begin{cases}
%     -\sum_{k:y_k \neq y_i}\alpha_{i,j,k} , & y_j = y_i\\
%     \sum_{j':y_j' = y_i}\alpha_{i,j',j}, & y_j \neq y_i 
% \end{cases} 
%  \end{align}
%  Let $\Bb = -\A$, i.e. 
%    \begin{align}
%     B_{ij} = \begin{cases}
%     \sum_{k:y_k \neq y_i}\alpha_{i,j,k} , & y_j = y_i\\
%     -\sum_{j':y_j' = y_i}\alpha_{i,j',j}, & y_j \neq y_i 
% \end{cases} 
%  \end{align}
%  Then, it holds that $\Bb1_n = 0$. The dual becomes
% \begin{equation}
%      \max_{B} \text{tr}(\Zhat B^T) \ \text{sub. to. } B \preceq I, B1_n = 0,  B \hada \odot \Zhat \geq 0  \ \text{todo:last constraint}
%  \end{equation}
%  where
%  \begin{align}
%     \Zhat_{ij} = \begin{cases}
%     1 - 1/k , & y_j = y_i\\
%     -1/k, & y_j \neq y_i 
% \end{cases} 
%  \end{align}
 
%  \begin{propo}\label{propo:scl_relu_svm}
%  Solution of \eqref{eq:scl_svm} is the OF (imbalance?)
%      \begin{align}
%  \arg\min_{\G\succeq 0}  \text{tr}(\G)~~\text{\emph{subj. to}}~\G[i,j] - \G[i,i']\geq 1, i\in[n], y_j = y_i, y_{i'}=\neq y_i, \G[i,j] \geq 0, \forall i,j \in \left[n\right] = I_n
%  \end{align}
%  \end{propo}

% \subsection{Useful PSD Properties}
%  \begin{lemma}\label{lem:motivation}
%     Given a symmetric matrix $\G \succeq 0$ and $\G_{ii} = 1, \forall i$, it follows that $|\G_{ij}| \leq 1$.
% Consider a vector $\ab = [a_1 \ a_2 \ ... \ a_n]^T$, where $a_i = 1, a_j = -\G_{ij}, a_k = 0, \forall k \neq i,j$. Since $\G \succeq 0$, we have the following
% \begin{align*}
%     \ab^T\G\ab = 1 - \G_{ij}^2 &\geq 0 \\
%     \implies |\G_{ij}| &\leq 1
% \end{align*}
% \end{lemma}

==> sections_v2/setup.tex <==
% \subsection{Supervised Contrastive Loss}
% \vspace{-0.2cm}
% 
% \noindent\textbf{Notation.}~
% For a positive integer $n$, we denote $[n] := \{1,2,3,...,n\}$. For matrix $\Vb\in\R^{m\times n}$, $\Vb[i,j]$ denotes its $(i,j)$-th entry, $\vb_j$ denotes the $j$-th {column}, $\Vb^\top$ its transpose. We denote $\|\Vb\|_F$ the Frobenius norm of $\Vb$. We use $\Vb \propto \mathbf{X}$ whenever the two matrices are equal up to a scalar constant. We use $\Vb \geq 0$ to denote the entry-wise non-negativity of the elements of $\Vb$, i.e., $\Vb[i,j] \geq 0, \forall i \in [m],j \in [n]$. Finally, $\Id_m$ denotes the identity matrix of size $m$.
% 
%We use $\ones_m$ to denote an  $m$-dimensional vector of all ones and $\Id_m$ for the $m$-dimensional identity matrix. For vectors/matrices with all zero entries, we simply write $0$, as dimensions are easily understood from context.
% 
% \vspace{-3pt}

% \vp

% \vp
\noindent\textbf{Notation.}~
For a positive integer $n$, $[n] := \{1,2,3,...,n\}$. For matrix $\Vb\in\R^{m\times n}$, $\Vb[i,j]$ denotes its $(i,j)$-th entry, $\vb_j$ denotes the $j$-th {column}, $\Vb^\top$ its transpose. We denote $\|\Vb\|_F$ the Frobenius norm of $\Vb$. We use $\Vb \propto \mathbf{X}$ whenever the two matrices are equal up to a scalar constant. We use $\Vb \geq 0$ to denote the entry-wise non-negativity, i.e., $\Vb[i,j] \geq 0, \forall i \in [m],j \in [n]$. Finally, $\Id_m$ denotes the identity matrix of size $m$.

Consider $k$-class classification and training set $S=\{(\x_i,y_i)\}_{i = 1}^{n}$ where $\x_i\in\R^d,\,y_i\in[k]$ represent  data samples and  corresponding class labels. We use $n_c$ to denote the number of examples in class $c\in[k]$, and $\h_\thetab(\cdot)$ to denote the 
 last-layer feature-embeddings of a deep-net parameterized by $\thetab$. We compute the SCL on a given batch $B\subseteq[n]$ of training examples as follows,
% Given a $k$-class classification task, for a batch $B$, we write the ERM problem with SC as:
     \begin{align}\label{eq:scl_main}
     % \min_{\thetab} \ 
     \Lc_B(\thetab) := \sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B \\ y_j = y_i, j\neq i}}\log\bigg(1+\sum_{\ell \neq i,j}\exp{\Big(\frac{1}{\tau}\big({\h_\thetab(\x_i)^\top\h_\thetab(\x_\ell) - \h_\thetab(\x_i)^\top\h_\thetab(\x_j)}\big)\Big)}\bigg),
 \end{align}
 % Note that \cite{khosla2020supervised} proposed two variations of SupCon. We present the version that was argued by the authors to be superior for supervised classification.
%\vspace{-0.1in}
where $\tau$ is a positive scalar temperature hyper-parameter,
%as described by \cite{khosla2020supervised}
{and $n_{B,y_i}$ is the number of examples in batch $B$ belonging to class $c= y_i$. To train a deep-net, we minimize SCL \eqref{eq:scl_main} over the network parameters $\thetab$ on a set of batches $\mathcal{B}$ chosen from the training set. As introduced by \citet{khosla2020supervised}, SCL requires normalized features, so we assume $\norm{\h_{\thetab}(\x_i)} = 1$}.
% }
%\tina{do we need the following here?} We will consider SCL under both \textit{mini-batch} and \textit{full-batch} with the latter involving a single batch including all datapoints ($n_{B,y_i} = n$)}. Following previous literature on UFM \cite{mixon2020neural,fang2021exploring} \new{For a datapoint $x_i,y_i$, we will define $h_i = h_{\theta}(x_i)$ as the $d \geq k$ dimensional extracted feature, that is normalized to possess unit norm. \tina{up to here} 
Furthermore, we assume that $d\geq k$ and $n_c, n_{B,c}\geq2, c\in[k]$.\footnote{When using SCL, it is common practice to add an augmented version of the datapoints in each batch to itself \citep{khosla2020supervised,graf2021dissecting}. This practice, referred to as \textit{batch duplication}, helps ensure that each datapoint in a batch has at least one other example in the same class to compare to during training.}
% \begin{figure*}
%     % \centering
%     \hspace*{-16pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Exp/GMu_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-3.2,2.65) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.3,2.65) [scale=0.9]{\textbf{MNIST}};
%             \node at (4.0,2.65) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-6.2,1.2)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-6.2,-1.1)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             \node at (0.1,-2.6) [scale=0.9]{\textbf{Epoch}};
%         \end{tikzpicture}
%     \end{subfigure}
%     % \vspace{-10}
%     \caption
%     {ResNet-18 trained on imbalanced datasets with SCL. Convergence of embeddings to the OF geometry as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$, where $\G_\M=\M^\top\M$ is the Gram matrix of class-mean embeddings. $\Delta_{\G_\M}$ is consistently on the order of $0.01$ regardless of dataset or imbalance.}
%     \label{Fig:Deepnet_SCL_Geom_GMu}
%     % \vspace{-15}
% \end{figure*}
{We let $\HT_{d \times n} = \begin{bmatrix} \hT_1, \cdots, \hT_n \end{bmatrix}$ denote an embeddings matrix where each column corresponds to one of the examples in the training set, {i.e., $\h_i:=\h_\thetab(\x_i)$.  The \emph{embeddings geometry} or so-called  \emph{implicit geometry}\footnote{
The specific terminology is adopted from \cite{behnia2023implicit}.} refers to the norms and pairwise-angles of these vectors $\h_i, i\in[n]$. Note these quantities correspond exactly to the entries of the
Gram matrix $\Hb^\top\Hb$.} To characterize the geometry, we need the following definitions.} 
% \todo{no need for SCL+. we impose Relu, unless ow stated, this holds} 
% \new{Since our focus is on studying the feature geometry with non-negative values for feature coordinates, we refer to training a model with non-negative features using SCL as \textbf{SCL$_+$}. The optimization objective for such a training is:}
% \begin{align}\label{eq:scl+}
%     \min_{\thetab \ \text{s.t.} \ \h_\thetab(\x) \geq 0} \sum_{B \in \mathcal{B}}\Lc_B(\thetab) \tag{$\text{SCL}_+$}
% \end{align}

%\tina{This is more of an experiment detail not setup. Move it to the next section. Or see Christos' comment in the file he shared} 

% In order to characterize our target geometry, we will use the following definition: 
\begin{definition}[Neural Collapse (NC)]\label{def:nc}
    NC occurs if $\h_i = \h_j, \ \forall \ i,j: y_i = y_j$. %In other words, the within class variation of features becomes negligible \tina{is negligible same as features being exactly equal? }.
\end{definition} 
\begin{definition}[$k$-Orthogonal Frame ($k$-OF)]\label{def:of}
    We say that $k$ vectors $\Vb = [\vb_1,\cdots,\vb_k] \in \R^{d\times k}$ form a $k$-OF {if $\Vb^\top\Vb \propto \Id_k$, i.e., for each pair of $(i,j)\in[k],$ $\|\vb_i\| = \|\vb_j\|$ and $\vb_i^\top\vb_j = 0$.} %\tina{need to define identity matrix somewhere earlier}
\end{definition}
{When the within-class variation of embeddings is negligible, i.e., $\Hb$ satisfies NC, it suffices to focus on the class-mean embeddings ${\mub}_c = \frac{1}{n_c}\sum_{i: y_i = c} \h_i, c\in[k]$ and the respective matrices $\MT_{d\times k} =  \begin{bmatrix} {\mub}_1, \cdots, {\mub}_k \end{bmatrix}$ and $\G_\M = \M^\top\M$ instead of $\Hb$ and $\Hb^\top\Hb.$ With these, we can formally define the OF geometry for embeddings.}
% {When  the within-class variation of embeddings is negligible, i.e., $\Hb$ satisfies NC, it suffices to focus on the class-mean embeddings ${\mub}_c = \frac{1}{n_c}\sum_{i: y_i = c} \h_i, c\in[k]$ and their respective matrix $\MT_{d\times k} =  \begin{bmatrix} {\mub}_1, \cdots, {\mub}_k \end{bmatrix}$. That is, it is adequate to study $\G_\M = \M^\top\M$ instead of $\Hb^\top\Hb.$ With these, we can formally define the OF geometry for embeddings $\Hb$ as follows.}
%In our theoretical and experimental analysis, we measure the Gram matrix of class means $\G_\M = \M^T\M \in \R^{k \times k}$. 
% Further, we define a geometric structure: 

% With this, we are ready to define the reference geometry of features:
\begin{definition}[OF geometry] \label{def:ncof}
    We say that a feature-embedding matrix $\Hb$ follows an OF geometry if it satisfies NC and the class-means form a $k$-OF, i.e., $\G_\M\propto\Id_k$.
\end{definition}
% We can now proceed to discuss our results using the definitions above.


% \begin{wrapfigure}[18]{r}{0.40\textwidth} 
%         \centering
%         %\hspace*{-20pt}
%             \centering
%             \vspace{-0.0in}\begin{tikzpicture}
%                 \node at (0.0,0) 
%                 {\includegraphics[width=0.38\textwidth]{Figs/Gm_Heatmap_Plots/Heatmap_2_fixed.pdf}};
%                 % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%     			\node at (-1.3,2.4) [scale=0.9]{\textbf{R = 1}};
%            	\node at (0.8,2.4) [scale=0.9]{\textbf{R = 100}};
%                 \node at (-2.8,-0.9)  [scale=0.9, rotate=90]{\textbf{CE}};
%                 \node at (-2.8,1.2)  [scale=0.9, rotate=90]{\textbf{SCL}};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%         \captionsetup{width=1\linewidth}
%         \caption[GM]
%         {$\G_\M$ at last epoch (350) for ResNet-18 trained on $\RT$-STEP imbalanced MNIST. Each $\G_\M$ normalized to have a maximum diagonal value of 1.
%         % For comparability, values plotted are divided by the max value in each $\G_\M$ matrix.
%         } %\todo{Do deepnet CE and compare its to the SCL , maybe plot SCL first, keep only R 1 and 100, state that this is with a normalizing layer}} 
%         \label{fig:GM matrices comparison}
% \end{wrapfigure}

% % \begin{wrapfigure}[18]{r}{0.40\textwidth} 
% \begin{figure}
%     % \centering
%     \hspace*{-13pt}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=0.66\textwidth]{Figs/Deepnet_Geometry_Exp/GMu_Convergence_plots.pdf}};
%             % \node at (-5.7,2.4) [scale=0.7]{\textbf{Norm Ratios}};
%             \node at (-2.8,2.1) [scale=0.9]{\textbf{CIFAR10}};
%             \node at (0.1,2.1) [scale=0.9]{\textbf{MNIST}};
%             \node at (3.2,2.1) [scale=0.9]{\textbf{FMNIST}};
%             \node at (-4.8,1)  [scale=0.9, rotate=90]{\textbf{Step}};
%             \node at (-4.8,-0.8)  [scale=0.9, rotate=90]{\textbf{Long-tail}};
%             % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%         \end{tikzpicture}
%     \end{subfigure}
%     % \vspace{-10}
%     \caption
%     {ResNet-18 models trained on imbalanced datasets with SCL. Convergence of features to the OF geometry as measured by $\Delta_{\G_\M} := \|\frac{\G_\M}{\| \G_\M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$.  $\Delta_{\G_\M}$ is consistently on the order of $0.01$ regardless of dataset or imbalance.}%Shows the convergence of feature geometry for a ResNet-18 model trained using SCL to NC-OF by calculating $\Delta_{\G_\M} := \|\frac{\M^T \M}{\| \M^T \M\|_F} - \frac{\Id_{k}}{\|\Id_{k}\|_F}\|_F$. Amazingly, $\Delta_{\G_\M}$ is mostly on the order of $0.01$ regardless of imbalance or dataset.}
%     \label{Fig:Deepnet_SCL_Geom_GMu}
%     % \vspace{-15}
%     \vspace{-0.1in}
% \end{figure}
% % \end{wrapfigure}





==> sections_v2/theo_results.tex <==
In this section, we analytically justify the convergence of the embeddings learned by SCL to the OF geometry. For our theoretical analysis, we use the Unconstrained Features Model (UFM) \citep{mixon2020neural,fang2021exploring,graf2021dissecting,ULPM,lu2020neural,tirer2022extended}, where we treat the last-layer features $\Hb$ as free variables, removing the dependence to the network parameters $\thetab$. However, we refine the UFM, and consider the SCL minimization over the non-negative orthant to accommodate for the presence of ReLU activations in the last layer.\footnote{\cite{tirer2022extended} (and several follow ups, e.g. \cite{sukenik2023deep}) has also studied incorporating the ReLU activation in the UFM, albeit focusing on MSE loss.} Following \citet{khosla2020supervised}, we further constrain the embeddings $\h_i$ to be normalized. We prove, irrespective of the labels distribution, that the global optimizers form an OF. Formally, consider the following refined UFM for SCL, which we call {$\text{UFM}_+$} for convenience:
%
% To this end, we adopt a refined Unconstrained Features Model (UFM) \cite{mixon2020neural,fang2021exploring,graf2021dissecting,ULPM,lu2020neural,tirer2022extended} for our theoretical study and we show, irrespective of the training data distribution, the global optimizers of UFM trained by SCL is the OF. In the UFM, we. treat the last-layer features as free variables, by abstracting out the mapping from the input to the features. We consider the minimization of the SCL over the non-negative orthant to accommodate the presence of ReLU activations in the feature layer of many common architectures:
\begin{align}\label{eq:SCL_UFM_full}
    \widehat{\Hb} \in \arg\min_{\Hb} \Lc_{\text{SCL}}
    (\Hb)~~\text{{subj. to}}~~\Hb \geq 0\,\text{ and }\|\h_i\|^2 = 1,\, \forall i\in[n].
    \tag{$\text{UFM}_+$}
\end{align}
Recall $\Hb\geq 0$ denotes entry-wise non-negativity. We begin our analysis by considering the full-batch loss in Sec.~\ref{sec:full_batch_theory}, and extend our results to the SCL minimized on mini-batches in Sec.~\ref{sec:mini_batch_theory}. We provide specific conditions that mini-batches must satisfy in order to have the same global optimum as the full-batch version. 
 % Throughout this section, we assume the dimension of the feature space $d\geq k$, and that for each class $c\in[k]$, $n_c \geq 2$. \vala{repeated on purpose ?}


% \subsection{Optimal feature configuration of SCL with non-negative features} 
\subsection{Full-batch SCL}\label{sec:full_batch_theory}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Specifically, we consider the following problem of optimizing the SCL under the UFM with non-negative features. (\cite{graf2021dissecting}) The assumption of non-negative features holds true whenever the ReLU activation is applied at the layer producing the features of interest. We prove that the global optimal of the norm-constrained SCL with non-negative features is achieved by the Orthogonal Frame (OF), whenever the feature space has dimensions at least $k$, the number of classes in the training data. The following result holds for an arbitrary label distribution \gk{todo:do we need at least two examples?} 
%  \begin{align}\label{eq:scl_imbal}
%      \Lc(\Hb):=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\left(1+\sum_{m \neq i,j}\exp{\left(\h_i^T\h_m - \h_i^T\h_j\right)}\right)
%  \end{align}
% We solve the following minimization:
%  \begin{align}\label{eq:scl_relu_bal}
%  \arg\min_\Hb \Lc(\Hb)~~\text{\emph{subj. to}}~\|\h_i\| = 1, h_{i,l} \geq 0, i\in[n], l \in [d].
%  \end{align}

% % \begin{definition}{$k$-Orthogonal Frame (OF)}\gk{needs to go earlier}
% %     We say that $k$ vectors $\vb_1,...,\vb_k$ in $\R^d$ form a $k$-OF if for each pair of samples $i,j\in[k]$ $\|\vb_i\| = \|\vb_i\|,$ and $\vb_i^T\vb_j = 0$.
% % \end{definition}
% % \begin{definition}{Neural Collapse (NC)} \gk{may not be needed if we define in intro}
% %     For a feature configuration described by $\Hb$, we say that NC occurs if $\h_i = \h_j, \ \forall \ i,j: y_i = y_j$.
% % \end{definition}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Here, we focus on the full-batch SCL, where the entire training set is treated as a single batch. Specifically, we consider \ref{eq:SCL_UFM_full} 
% \begin{align}\label{eq:SCL_UFM_full}
%     \hat{\Hb} \in \arg\min_\Hb \Lc%_{\text{full}}
%     (\Hb)~~\text{{subj. to}}~~\Hb \geq 0\,\text{ and }\|\h_i\|^2 = 1,\, \forall i\in[n],
% \end{align}
with $\Lc_{\text{SCL}}
(\Hb)$ being the full-batch SCL defined as,
% 
\begin{align}\label{eq:SCL_full}
    \Lc_\text{full}(\Hb):=\sum_{i\in[n]}\frac{1}{n_{y_i}-1}\sum_{j \neq i, y_j = y_i}\log\Big(\sum_{\ell \neq i}\exp{\big(\h_i^\top\h_\ell - \h_i^\top\h_j\big)}\Big).
\end{align}
Thm.~\ref{thm:scl_full} specifies the optimal cost and optimizers of \ref{eq:SCL_UFM_full} with the full-batch SCL \eqref{eq:SCL_full}.


\begin{theorem}[Full-batch SCL minimizers]\label{thm:scl_full} Let $d\geq k$.
%\footnote{\todo{Discuss with Christos, consider removing} Note that this result required that the dimension of the representation space be at least $k$, as opposed to $k-1$, unlike without non-negativity. This is due to the fact that a $k$-OF exists in $\R^d$ if and only if $d\geq k$.}
For any $\Hb$ feasible in \ref{eq:SCL_UFM_full}, it holds,
  \begin{align}\label{eq:scl_full_lb}
      \Lc_\text{\emph{full}}(\Hb) \geq \sum_{c \in [k]}n_c\log\left(n_c-1+(n-n_c)e^{-1}\right).
  \end{align}
  Moreover, equality is achieved if and only if $\Hb$ satisfies NC and the class-means form a k-OF.
\end{theorem}
% \begin{remark}\label{rem:tau}
%     The normalization of the embeddings in \ref{eq:SCL_UFM_full} corresponds to SCL with temperature $\tau=1$. More generally, the normalization becomes $\norm{\h_i}^2=1/\tau$. The conclusion of Thm.~\ref{thm:scl_full} is insensitive to the choice of $\tau$, thus stated above for $\tau=1$ without loss of generality. Although the value of $\tau$ does not affect the global optimizers of \ref{eq:SCL_UFM_full}, we have empirically observed that it impacts the speed of convergence during training.
% \end{remark}
% \gk{bring Graf discussion}


We defer the proof details to Sec.~\ref{app:proof_details} in SM. The bound relies on successive uses of Jensen's inequality and the fact that for feasible $\Hb$, each pair of training samples $i,j\in[n]$ satisfies $0\leq\h_i^\top\h_j\leq 1$. We complete the proof by verifying that equality is attained only if $\h_i^\top\h_j=1$ when $y_i=y_j$ and $\h_i^\top\h_j=0$ when $y_i\neq y_j$. Rather, to achieve the optimal cost, features with similar labels must align (NC) and the class-mean features must form an OF.

\begin{wrapfigure}[11]{r}{0.28\textwidth} 
     \centering
            \vspace{-0.3in}\begin{tikzpicture}
                \node at (0.0,0.0) 
                {\includegraphics[width=0.28\textwidth]{Figs/Loss_convergence/LossCompToLowerBound_partial.pdf}};
                 \node at (0.1,-1.6) [scale=0.7]{Epoch};
    			\node at (0.0,1.6) [scale=0.9]{\textbf{Loss}};
                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
            \end{tikzpicture}
    \captionsetup{width=0.95\linewidth}
    \vspace{-20pt}
    \caption{Full-batch SCL converges to the lower bound (dashed lines) in Thm.~\ref{thm:scl_full}.}
    \vspace{0.03in}
    \label{fig:loss_convergence}
\end{wrapfigure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}
%     The proof proceeds by repeated application of the Jensen's inequality and finally employing the Cauchy-Schwartz inequality on the appropriate inner products of feature vectors. We further use the fact that the non-negativity constraints on the feature imply the non-negativity of the inner products. We conclude by identifying the conditions of attaining the lower bound with equality by noting the equality conditions for the inequalities used in the proof at various steps.   
% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textit{Label imbalance does not impact the geometry of features learned by SCL with ReLU}: in case of CE, several works \cite{zhu2021geometric,zhou2022optimization,graf2021dissecting} showed that the loss learns an implicit geometry characterized by the ETF under balanced data. In case of imbalanced label distribution, \cite{seli} showed that the geometry is no longer the ETF, and described the features and classifiers by the SELI geometry. In case of the SCL, \cite{graf2021dissecting} proved the global optimality of the ETF on the SCL with UFM without ReLU modeling. Based on numerical and empirical observations, the geometry with imbalanced label distribution is not longer the ETF when ReLU is not taken into account. However, with the modeling of ReLU activations, our results demonstrate that the label distribution does not impact the feature geometry.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Thm.~\ref{thm:scl_full} shows that any optimal embedding geometry learned by the full-batch SCL with ReLU constraints uniquely follows the OF geometry (Defn. \ref{def:ncof}) and the conclusion is independent of the training label distribution.
We have already seen in Sec.~\ref{sec:Deepnet_SCLGeom_exp}, that  this conclusion is empirically verified by deep-net experiments.
 To further verify the lower bound on the cost of the SCL loss given by the theorem, we compare it in Fig.~\ref{fig:loss_convergence} with the empirical loss of a  ResNet-18 model trained with full-batch SCL \eqref{eq:SCL_full} on $R$-STEP MNIST dataset and $n=1000$ total examples. Note the remarkable convergence of the loss to the lower bound (dashed horizontal lines) as training progresses.


% \new{To verify Thm.~\ref{thm:scl_full}, we train ResNet-18 model with full-batch SCL \eqref{eq:SCL_full} on the MNIST dataset. For each imbalance ratio $\RT$, we choose an $\RT$-STEP imbalanced subset of MNIST of size $n=1000$ as the training set. We do not apply batch duplication or data augmentation in this experiments. Fig.~\ref{fig:loss_convergence} illustrates the convergence of the loss to the lower-bound described by the theorem. Since we train over the full-batch loss, each epoch (one pass of the training set) is equivalent to one iteration of gradient descent.}

% To support Thm.~\ref{thm:scl_full} we conduct experiments akin to Sec.~\ref{sec:Deepnet_SCLGeom_exp} on a subset of MNIST with ResNet-18. Specifically, using 1000 total examples we vary the label distribution in a $(\RT)$-STEP imbalanced manner maintaining a (full) batch size of 1000, without batch duplication or applying any augmentation to the data. Furthermore, we measure the $\Lc(\Hb)$ through training and compare it to the lower bound of Thm.~\ref{thm:scl_full} (see Fig.~\ref{fig:loss NC and angle convergence} (a)). To confirm convergence to NC-OF geometry we measure both the NC through $\beta_{NC}=\tr(\Sigma_W\Sigma_B^\dagger)/k$, and the average pairwise cosine similarity between class means, $\text{Ave}_{c \neq c'} \alpha_{\text{sim}}(c,c')$, defined in Sec.~\ref{sec:Deepnet_SCLGeom_exp} (see Fig.~\ref{fig:loss NC and angle convergence} (b,c)).%\footnote{Here, $\Sigma_B= \sum_{c\in [k]}(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})(\boldsymbol{\mu}_c - \boldsymbol{\mu}_{G})^T$ is the between class covariance matrix, $\boldsymbol{\mu}_G = \frac{1}{k}\sum_{c\in[k]}\boldsymbol{\mu}_c$ is the weighted global mean, and $\Sigma_W  = \sum_{i\in [n]}(\h_i - \boldsymbol{\mu}_{y_i})(\h_i - \boldsymbol{\mu}_{y_i})^T$ is the within class covariance matrix.}
% It is clear in Fig.~\ref{fig:loss NC and angle convergence} that the empirically achieved loss proceeds to the lower bound as training progresses while the within class variation approaches zero and the cosine similarities tend to $0$. \tina{rewrite}
 
 % \begin{figure*}
 %        \centering
 %        \begin{subfigure}[b]{0.325\textwidth}
 %            \centering
 %            \begin{tikzpicture}
 %                \node at (0.0,0) 
 %                {\includegraphics[width=\textwidth]{Figs/Loss_convergence/LossCompToLowerBound_partial.pdf}};
 %                 \node at (0.1,-1.8) [scale=0.7]{Epoch};
 %    			\node at (0.0,1.85) [scale=0.9]{\textbf{Loss}};
 %                %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
 %                % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
 %            \end{tikzpicture}
 %        \end{subfigure}
 %        \hfill
 %        \captionsetup{width= \linewidth}
 %        \caption[loss]
 %        {\new{Full-batch SCL: ResNet-18 trained on a $\RT$-STEP imbalanced subset of MNIST of size $n=1000$. Loss converges to the lower bound (dashed lines) computed in Thm.~\ref{thm:scl_full}. Each epoch is equivalent to one iteration of gradient descent.} }
 %        \label{fig:loss NC and angle convergence} 
 %    \end{figure*}
% \noindent\textbf{Invariance to label imbalance with ReLU constraints.} Thm.~\ref{thm:scl_full} shows that any optimal feature geometry learned by the full-batch SCL under ReLU constraints uniquely follows the OF geometry and is independent on the training label distribution. This contrasts with CE and mean-squared loss, where the learned features form an ETF with balanced data \cite{zhu2021geometric,zhou2022optimization,graf2021dissecting,NC,tirer2022extended} but their geometry significantly changes under imbalanced label distribution \cite{seli, fang2021exploring, liu2023inducing, behnia2023implicit, dang2023neural} \ct{cite more imbalanced papers}. 
% 
% \todo{rewrite}Moreover, in case of the SCL without ReLU activations, \cite{graf2021dissecting} proves the optimality of the ETF for balanced training set. However, in the presence of imbalances, several works \cite{graf2021dissecting,zhu2022balanced} argue that under imbalanced label distribution, the optimal geometry is no longer an ETF.




%On the other hand, a prediction on only the centered features does not specify the geometry if the features are not arbitrarily centered.
%Although \cite{graf2021dissecting} acknowledges the issue of geometry comparisons arising from the presence of ReLU activations in deep neural networks, their theoretical model does not adequately account for this factor. Thus, \cite[Fig. 7]{graf2021dissecting} shows a substantial gap between the theoretical prediction and empirical observations; \red{compare also the red to green lines Fig. \ref{fig:intro}(a)}. 
 %\todo{Cite BCL and Graf for imbalance invariance}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Batch optimized SCL} 
\subsection{Mini-batch SCL}\label{sec:mini_batch_theory}
Thm.~\ref{thm:scl_full} shows that minimizing SCL over the training set as a single batch recovers an OF in the feature space, regardless of the training label distribution. However, in practice, SCL optimization is performed over batches chosen from training set \citep{khosla2020supervised, graf2021dissecting}. Specifically, we have a set of batches $\mathcal{B}$ and we compute the loss on each batch $B\in\mathcal{B}$ as in \eqref{eq:scl_main}. While in the full-batch SCL \eqref{eq:SCL_full}, all pairs of training samples interact with each other, in the mini-batch version, two samples $(i,j)$ interact only if there exists a batch $B\in\mathcal{B}$ such that $i,j\in B$. A natural question is whether the mini-batch construction impacts the embeddings learned. In this section, we study the role of batching on the embeddings geometry more closely.


Similar to the previous section, we consider \ref{eq:SCL_UFM_full}, where we directly optimize the SCL over embeddings $\Hb$. However, this time we study the mini-batch SCL defined as follows,
% 
 \begin{align}\label{eq:scl_batch}
     \Lc_{\text{batch}}(\Hb):=\sum_{B \in \mathcal{B}}\sum_{i\in B}\frac{1}{n_{B,y_i}-1}\sum_{\substack{j\in B\\j \neq i, y_j = y_i}}\log\bigg(\sum_{\substack{\ell \in B \\ \ell \neq i}}\exp{\left(\h_i^\top\h_\ell - \h_i^\top\h_j\right)}\bigg),
 \end{align}
 where recall $n_{B,c} = |\{i:i\in B,y_i=c\}|$. Thm.~\ref{thm:scl_mini} is an extension of Thm.~\ref{thm:scl_full} for the mini-batch SCL \eqref{eq:scl_batch}. The proof proceeds similarly to that of Thm.~\ref{thm:scl_full}, where the loss over each batch can be independently bounded from below. Interestingly, due to the orthogonality of the optimal embeddings in every batch, the lower bound for each batch can be achieved by the common minimizer. The detailed proof is deferred to Sec.~\ref{app:proof_thm2} in the SM.
 % \tina{probably a one-line explanation that the proof is similar?}
 % 
\begin{theorem}[Mini-batch SCL minimizers]\label{thm:scl_mini}
    Let $d\geq k$ and $\mathcal{B}$ be an arbitrary set of batches of examples. For any feasible $\Hb$ in \ref{eq:SCL_UFM_full}, the following lower bound holds,    
      \begin{align}\label{eq:scl_mini_lb}
      \Lc_\text{\emph{batch}}(\Hb) \geq \sum_{B \in \mathcal{B}}\sum_{c \in [k]}n_{B,c}\log\left(n_{B,c}-1+(n_{B}-n_{B,c})e^{-1}\right).
  \end{align}
  Equality holds if and only if for every $B\in\mathcal{B}$ and every pair of samples $i,j\in B$, $\h_i^\top\h_j=0$ if $y_i\neq y_j$ and $\h_i=\h_j$ if $y_i=y_j$.
\end{theorem}


We remark that the only previous study of SCL geometry with batches by \cite{graf2021dissecting} requires significantly more restrictive conditions on the batch set $\Bc$ to guarantee a common geometry among all batches $B\in\Bc$. Specifically, \cite{graf2021dissecting} assumes a batch set that includes all possible combinations of examples. Instead, thanks to the addition of ReLU, our requirements are significantly relaxed. This is detailed in the following remark. See also Sec.~\ref{rem:compare_graf} in SM.


% \ct{I rephrased this paragraph (See above). if you like keep and delete this:}{ We note that, in the mini-batch analysis of \cite{graf2021dissecting} for SCL without ReLU, it is assumed that for a given batch-size, all possible combinations of examples are taken as the set of mini-batches. The following discussion reveals that the necessary and sufficient conditions on batching for achieving unique OF geometry of SCL with ReLU are far less restrictive. See also Sec.~\ref{rem:compare_graf} in SM.} 
% \ct{do you still need this paragraph that you brought the remark?}

\begin{remark}[Comparison to analysis of \citet{graf2021dissecting}]\label{rem:compare_graf_app} {We elaborate on the comparison to \citet{graf2021dissecting} with an illustrative example below. When optimizing the loss decomposed over a set of mini-batches, it is crucial to consider whether the individual batch minimizers are also overall optimal solutions. }
Consider the following setting: $k= d = 3, y_1 = 1, y_2 = 2, y_3 = 3, B_1 = \{1,2\}, B_2 = \{1,3\}, B_3 = \{2,3\}, \mathcal{B} = \{B_1, B_2, B_3\}$. Let us identify the optimal embeddings for the two scenarios: (i) with and (ii) without non-negativity constraints on the embedding coordinates.
% \ct{don't use enumerate or if use reduce the space. too much white space. otherwise use $\noindent$}
% \begin{enumerate}
\\
    \noindent\textbf{(i)~Without non-negativity (UFM)}, the optimal embedding configurations can be shown to be ETF with $2$ vectors for every batch, which is simply an antipodal structure. In other words, the batch-wise optimal solutions are $\h_1 = -\h_2, \h_1 = -\h_3$ and $\h_2 = -\h_3$, for the batches $B_1, B_2$ and $B_3$, respectively. However, the batch-wise optimal solutions are infeasible due to their contradictory nature. From \cite{graf2021dissecting}, it can be deduced that the overall optimal configuration is instead an ETF with $3$ vectors. This example underscores the difficulty in optimizing the loss over every batch separately in case of SCL without non-negativity. See (a) in Fig.~\ref{fig:remark} in SM.
\\    
    \noindent\textbf{(ii) With non-negativity \eqref{eq:SCL_UFM_full}}, our results imply that the optimal embeddings form a $2$-OF for every batch, i.e., $\h_1 \perp \h_2, \h_1 \perp\h_3$ and $\h_2 \perp\h_3$, for the batches $B_1, B_2$ and $B_3$, respectively. The three conditions are compatible with each other and the fact that the overall optimal solution is a $3$-OF in $\R^3$. Therefore, we were able to break down the overall optimization into individual batches. See (b) in Fig.~\ref{fig:remark} in SM.
% \end{enumerate}
\end{remark} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In Theorem \ref{thm:scl_full} we proved that the global minimizers of the SCL form a $k$-OF in the feature space, regardless of the label distribution of the training data, whenever the optimization is performed over all examples considered as one single batch. In practice, SCL optimization is performed on mini-batches. The natural question is whether the geometry is affected when the objective function is a sum of the losses incurred over a set of mini-batches. Does the method of mini-batch construction matter? In the theorem below, we prove that under UFM with ReLU model, the overall global minimizers continues to remain a $k$-OF, provided the construction of mini-batches satisfies certain properties. We consider the problem stated below:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}\label{thm:scl_relu_batch}
%  The following lower bound holds for the objective function of \eqref{eq:scl_batch} with $d\geq k$:
%   \begin{align}
%       \Lc(\Hb) \geq \sum_{B \in \mathcal{B}}\sum_{c \in [k]}n_{B,c}\log\left(n_{B,c}-1+(n_{B}-n_{B,c})e^{-1}\right),
%   \end{align}
%   and the equality is achieved if and only if
%   in every batch $B:\h_i^T\h_j = 0, \ \forall y_i\neq y_j$ and $\h_i = \h_j, \forall y_j = y_i, \forall i,j \in B$.\\
%   % \gk{key todo: find sufficient if not necessary condition on the batch construction- current thoughts as below. need to look for any corner cases}\\
   
%  \end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \tina{add a sentence after the theorem to highlight uniqueness in the full-batch case more}
\begin{wrapfigure}[16]{h}{0.28\textwidth}
    \centering \includegraphics[width=0.28\textwidth]{Figs/CounterExamples_BatchOF/SCLBatchExample4.pdf} 
    \captionsetup{width=\linewidth}
    \caption{A non-OF geometry minimizing mini-batch SCL with $\mathcal{B}=\{B_1,B_2\}$. Samples with different labels are marked with different colors. %\vala{use image for 1,0,0.}
    }
    \label{fig:counter_example}
\end{wrapfigure}
\noindent\textbf{Global minimizer geometry may not be unique.} It is easy to verify that any $\Hb$ following the OF geometry achieves the lower-bound of Thm.~\ref{thm:scl_mini} and it is also a global optimizer of the mini-batch SCL. However, depending on the choice of $\mathcal{B}$, the lower bound can possibly be attained by other optimal embeddings that do not necessarily satisfy NC or orthogonality. Hence the global optimizer may not have a unique geometry.

To highlight the importance of $\mathcal{B}$ in the characterization of the optimal geometry of \ref{eq:SCL_UFM_full} when using the batch-loss, consider the toy example in Fig.~\ref{fig:counter_example}. Suppose we have $k=3$ classes and we want to find the optimal normalized and non-negative features in $\R^3$ by minimizing \eqref{eq:scl_batch} for $\mathcal{B}=\{B_1, B_2\}$. Although the OF satisfies the global optimality condition in Thm.~\ref{thm:scl_mini}, the theorem requires milder conditions for the optimal $\widehat{\Hb}$: $\widehat{\h}_i$ and $\widehat{\h}_j$ need to be aligned ($y_i=y_j$) or orthogonal ($y_i\neq y_j$) only if they interact within one of the selected batches. Fig.~\ref{fig:counter_example} shows one such optimal geometry that does not satisfy either of NC or orthogonality conditions: Firstly, the samples $i=1$ and $i=3$ have significantly different features despite belonging to the same class. Second, ${\widehat{\h}}_{3}, \widehat{\h}_{4}$ align with $\widehat{\h}_{5}, \widehat{\h}_{6}$ although they have different labels, and  $\widehat{\h}_7, \widehat{\h}_8$ are not orthogonal to samples $\widehat{\h}_1, \widehat{\h}_2$. With this example, we are now ready to discuss the role of batching more formally in the next section.

% 
% \begin{wrapfigure}[19]{r}{0.38\textwidth}
%     \centering \includegraphics[width=0.38\textwidth]{Figs/CounterExamples_BatchOF/SCLBatchExample4.pdf} 
%     \captionsetup{width=0.95\linewidth}
%     \caption{A non-OF optimal feature geometry minimizing the mini-batch SCL \eqref{eq:scl_batch} with $\mathcal{B}=\{B_1,B_2\}$. Samples with different labels are marked with different colors. See text for details. %\vala{use image for 1,0,0.}
%     }
%     \label{fig:counter_example}
% \end{wrapfigure}
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % \noindent\textbf{Non-uniqueness of global minimizers:}\\ Unlike in the case of CE, where mini-batch construction does not impact the global minimizers of the loss function, it plays a critical role in characterizing the solutions of the SCL. As seen from Theorem \ref{thm:scl_full}, the optimal features in the full-batch SCL form an OF. However, in the mini-batch SCL, OF is not guaranteed. In fact, from the equality conditions stated in Theorem \ref{thm:scl_relu_batch}, even NC is not necessary for the minimizer. On the other hand, if the different classes are not \textit{contrasted} against each other due to the nature of mini-batches, the requirement for every class to be orthogonal with every other class does not arise. The following examples convey this message: \todo{Compare with above paragraph and remove if redundant.}\\
  % Counterexamples that do not form OF- no NC and no orthogonality\\
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  % \noindent\textbf{Example}:\\
  % Suppose $k=2, n_1 = n_2 = 4, \mathcal{B} = \{\{1,2,5,6\},\{3,4,7,8\}\}$, with labels $y_1 = y_2 = y_3 = y_4 = 1, y_5 = y_6 = y_7 = y_8 = 2$. With this mini-batch construction, the minimizing conditions are given by: $\h_1 = \h_2 \perp \h_5 = \h_6$ and $\h_3 = \h_4 \perp \h_7 = \h_8$. Now, suppose $d = 4$, then the following is a valid minimizing feature configuration: $\h_1 = \h_2 = [1 \ 0 \ 0 \ 0]^T, \h_3 = \h_4 = [0 \ 1 \ 0 \ 0]^T, \h_5 = \h_6 = [0 \ 0 \ 1 \ 0]^T, \h_7 = \h_8 = [0 \ 0 \ 0 \ 1]^T$. 
  % Therefore, although this is a loss minimizing feature configuration, NC is not satisfied, with examples from the same class being arbitrarily separated from each other, and the features do not form a $2$-OF. On the other hand, another minimizing feature configuration given by $\h_1 = \h_2 =  \h_3 = \h_4 = [1 \ 0 \ 0 \ 0]^T, \h_5 = \h_6 = \h_7 = \h_8 = [0 \ 1 \ 0 \ 0]^T$ satisfies NC and forms a $2$-OF.\\

  % \noindent\textbf{Example}:\\
  % Suppose $k=4, n_1 = n_2 = n_3 = n_4 = 2, \mathcal{B} = \{\{1,2,3,4\},\{5,6,7,8\}\}$, with labels $y_1 = y_2 = 1, y_3 = y_4 = 2, y_5 = y_6 = 3, y_7 = y_8 = 4$. With this mini-batch construction, the minimizing conditions are given by: $\h_1 = \h_2 \perp \h_3 = \h_4$ and $\h_5 = \h_6 \perp \h_7 = \h_8$. Now, suppose $d = 4$, then the following is a valid minimizing feature configuration: $\h_1 = \h_2 = [1 \ 0 \ 0 \ 0]^T, \h_3 = \h_4 = [0 \ 1 \ 0 \ 0]^T, \h_5 = \h_6 = [\nicefrac{1}{\sqrt{2}} \ \nicefrac{1}{\sqrt{2}} \ 0 \ 0]^T, \h_7 = \h_8 = [0 \ 0 \ \nicefrac{1}{\sqrt{2}} \ \nicefrac{1}{\sqrt{2}}]^T$. Therefore, although this is a loss minimizing feature configuration and NC is satisfied, every class is not contrasted against every other class. Therefore, the features do not form a $4$-OF.\\

  % \begin{figure}%
%     \centering
%     \subfloat[ Given the following mini-batch construction, $\h_1 = \h_2 \perp \h_5 = \h_6$ and $\h_3 = \h_4 \perp \h_7 = \h_8$ is a valid minimizing feature configuration. Assuming $d = 4$, the above configuration can ]{{\includegraphics[width=0.45\linewidth]{Figs/CounterExamples_BatchOF/CounterExample_OFBatch_NC.pdf} }}%
%     \qquad
%     \subfloat[ ]{{\includegraphics[width=0.45\linewidth]{Figs/CounterExamples_BatchOF/CounterExample_OFBatch_OFGeom.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
% \end{figure}


% \begin{figure}
%     \begin{subfigure}{0.45\textwidth}
%     \centering
%         \includegraphics[width=\linewidth,
%         height=5cm]{Figs/CounterExamples_BatchOF/CounterExample_OFBatch_NC.pdf} 
%         \caption{}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.45\textwidth}
%     \centering
%         \includegraphics[width=\linewidth,
%         height=5cm]{Figs/CounterExamples_BatchOF/CounterExample_OFBatch_OFGeom.pdf}
%         \caption{}
%     \end{subfigure}
%     \caption{Above scenarios provide counter examples for non-uniqueness of the SCL's global minimizer under mini-batch training. Assume features of the same color belong to the same class and take feature dimension $d = 4$. \textbf{(a)} Gives the mini-batch construction \vala{which breaks the first condition for uniqueness}. The above feature configuration is valid and minimizes the SCL loss; however, it does not satisfy the NC requirements. \textbf{(b)} Provides a mini-batch construction \vala{which breaks the second condition for uniqueness}. The above feature configuration is valid and minimizes the SCL loss; however, it does not form a $4$-OF geometry.}
% \end{figure}


  % \noindent\textbf{Or this Example \todo{choose one of this or previous}}:\\
  % Suppose $k=3, n_1 = n_2 = n_3 = 4, \mathcal{B} = \{\{1,2,3,4,5,6\},\{7,8,9,10,11,12\}\}$, with labels $y_1 = y_2 = y_3 = y_4 = 1, y_5 = y_6 = y_7 = y_8 = 2, y_9 = y_{10} = y_{11} = y_{12} = 3$. With this mini-batch construction, the minimizing conditions are given by: $\h_1 = \h_2 = \h_3 = \h_4 \perp \h_5 = \h_6$ and $\h_7 = \h_8 \perp \h_9 = \h_{10} = \h_{11} = \h_{12}$. Now, suppose $d = 3$, then the following is a valid minimizing feature configuration: $\h_1 = \h_2 = \h_3 = \h_4 = [1 \ 0 \ 0]^T, \h_5 = \h_6 = \h_7 = \h_8 [0 \ 1 \ 0]^T, \h_9 = \h_{10} = \h_{11} = \h_{12} = [1 \ 0 \ 0]^T$. Therefore, although this is a loss minimizing feature configuration and NC is satisfied, every class is not contrasted against every other class. Therefore, the features do not form a $3$-OF.\\
      

  
  % \noindent\textbf{Conditions for unique minimizer.}
    % With the above two examples as our motivation, we now state the necessary and sufficient conditions for the loss minimizing feature configuration to form a $k$-OF whenever $d\geq k$ as follows: 



  
%\subsection{\textit{Binding examples}: Fast convergence to OF}  
\section{Batching matters} \label{sec:batching}
%\ct{Consider bringing some more plots here? Eg. Fig 16?}



% The example given in Fig.~\ref{fig:counter_example} emphasizes the important role of choosing mini-batches while optimizing SCL in order to  avoid ambiguous solutions with different geometries; we study the problem of batching in more detail. 
% \red{Motivated by Fig.~\ref{fig:counter_example} \ct{rather than motivated by a figure, say better something like "by the fact that OF geometry may not be the unique solution"}}
{Since the OF may not be the only solution for the \ref{eq:SCL_UFM_full} with mini-batch SCL \eqref{eq:scl_batch}}, here we study the role of mini-batches to avoid ambiguous solutions with different geometries. In Sec.~\ref{Sec:unique}, 
%Below 
we identify necessary and sufficient conditions for a batching strategy to yield a unique global solution geometry. By this result, in Sec.~\ref{Sec:Binding_examples}, we propose a simple yet effective scheme that provably succeeds in improving the convergence to an OF.
\subsection{When is OF geometry the unique minimizer?}  \label{Sec:unique}
% \ct{I think it is important to emphasize that OF is always a minimizer. So to me the question (thus the title) then becomes, when is OF geometry the unique minimizer}
As discussed in Sec.~\ref{sec:mini_batch_theory} the uniqueness of the global minimizer's geometry when considering mini-batches depends on the interaction of samples in the loss function, {or, in other words, the choice of $\mathcal{B}$.}
%The above example, emphasizes the importance of pairwise interactions between samples in the loss function. 
Before specifying for which $\mathcal{B}$ the minimizer is unique, we need to define the Batch Interaction Graph{, a graph that captures the pairwise interactions of samples within the batches.}
    % \todo{Fix and elaborate on motivations for uniqueness conditions of bathces}


    \begin{definition}[Batch Interaction Graph]\label{def:big}
        Consider an undirected graph $G = (V, E)$ where $V := [n]$. We define the {Batch Interaction Graph} for a given set of batches $\mathcal{B}$ as follows: vertices $u,v\in V$ are connected if and only if there exists a batch $B\in\mathcal{B}$ such that $u,v \in B$. Moreover, $G_c$ denotes the induced subgraph of $G$ with vertices $V_c=\{u:y_u=c\}$. %\tina{check this guys and remove the next def if ok}
    \end{definition}
% 
  % With this definition, we can now state the necessary and sufficient conditions on $\mathcal{B}$ for the minimizer of the mini-batch SCL to be uniquely OF.
    We state necessary and sufficient conditions on $\mathcal{B}$ for the minimizer of mini-batch SCL to be unique:
\begin{corollary}\label{cor:batch}
      Consider the Batch Interaction Graph $G$ corresponding to $\mathcal{B}$. The global optimizer geometry of \ref{eq:SCL_UFM_full} with mini-batch SCL \eqref{eq:scl_batch} is unique and forms an OF if and only if $G$ satisfies the following conditions: (1) For every class $c \in [k]$, $G_c$ is a connected graph. (2) For every pair $c_1,c_2\in[k]$, there exists at least one edge between $G_{c_1}$ and $G_{c_2}$.
  \end{corollary}
Corollary~\ref{cor:batch} serves as a check for whether a given batching scheme yields a unique global minimizer geometry or not. It also provides guidance for designing mini-batches. We elaborate on this below.
\vspace{-0.35cm}
\subsection{\textit{Batch-binding} ensures unique OF minimizer and improves convergence}  \label{Sec:Binding_examples}
%\ct{Prefer active tense: is more direct and shorter. Cor XX shows that an a...}
Corollary~\ref{cor:batch} shows that an arbitrary set of mini-batches is not guaranteed to have OF geometry as its minimizing configuration in the embedding space. To enforce the OF geometry as the unique minimizer, we introduce a simple scheme with low computational overhead as follows. We define \textbf{binding examples} as \emph{a set of examples including exactly one example from every class}. This set has, thus, $k$ elements. The process of \textbf{batch-binding} is simply adding the above set of binding examples to every mini-batch in the given original set. See Sec.~\ref{sec:discussion} of SM for an algorithm and Fig.~\ref{fig:Binding_Examples_Visuals} in SM for a visual example.
 % {First, we need the following definition of a set of \emph{binding examples} of the training set.}

% \begin{wrapfigure}[15]{t}{0.38\textwidth} 
%      \centering
%             \vspace{-0.25in}\begin{tikzpicture}
%                 \node at (0.0,0.0) 
%                 {\includegraphics[width=0.3\textwidth]{Figs/Deepnet_Geometry_Batch_Exp/GMu_Convergence_plots_BindingBatches_vert.pd}};
%                  \node at (0.1,-1.8) [scale=0.7]{Epoch};
%     			\node at (0.0,1.7) [scale=0.9]{\textbf{Loss}};
%                 %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%     \captionsetup{width=0.95\linewidth}
%     \caption{A non-OF optimal feature geometry minimizing the mini-batch SCL \eqref{eq:scl_batch} with $\mathcal{B}=\{B_1,B_2\}$. Samples with different labels are marked with different colors. See text for details.}
%     \label{fig:loss_convergence}
% \end{wrapfigure}

% \begin{wrapfigure}[25]{t}{0.5\textwidth} 
%      \centering
%             \vspace{-0.2in}\begin{tikzpicture}
%                 \node at (0.0,0.0) 
%                 {\includegraphics[width=0.48\textwidth]{Figs/Deepnet_Geometry_Batch_Exp/GMu_Convergence_plots_BindingBatches_vert.pdf}};
%                  \node at (0.1,-3.8) [scale=0.9]{Epoch};
%     			\node at (1.7,3.9) [scale=0.9]{\textbf{Long-tailed}};
%                 \node at (-1.3,3.9) [scale=0.9]{\textbf{STEP}};
%                 \node at (4.0,-2.3) [scale=0.7, rotate=-90]{\textbf{No Batch Shuffling}};
%                 \node at (3.6,-2.3) [scale=0.7, rotate=-90]{\textbf{+ Binding Examples}};
%                 \node at (3.4,0.0) [scale=0.7, rotate=-90]{\textbf{No Batch Shuffling}};
%                 % \node at (3.2,2.1) [scale=0.7]{\textbf{+ Binding Examples}};
%                 % \node at (-4.8,1)  [scale=0.7, rotate=90]{\textbf{Step}};
%                 %\node at (0.0,-1.85)  [scale=0.9]{Epoch};
%                 % \node at (-3.7,-1.5)  [scale=0.9, rotate=90]{\textbf{Resnet-18}};
%             \end{tikzpicture}
%     \captionsetup{width=0.95\linewidth}
%     \caption{Convergence to OF geometry for various batching scenarios. See text for details. Experiments conducted with CIFAR-10 and ResNet-18 with a batch size of 128.
%     }
%     \label{Fig:Deepnet_SCL_Geom_NC_BindingBatch}
% \end{wrapfigure}

% \begin{definition}[Binding Examples]\label{def:binding}
%   % A set of examples of length $k$ including exactly one example from each class.
%   A set of examples represents a set of binding examples if it includes exactly one example from every class. This set has, thus, $k$ elements.
% \end{definition}
% \ct{Shall we make this a 2 line algorithm? So that is more visible?} {Now, we are ready to describe the proposed batching scheme: }Consider a set of mini-batches $\mathcal{B}$ and a set of binding examples. To every batch $B\in\mathcal{B}$ add the chosen set of examples to create a new batch configuration $\mathcal{B}^\prime$. This increases the size of every mini-batch by a constant value $k$. \new{This value is typically smaller than the batch sizes used to train SCL which could range from $2048$ to $6144$ \cite{khosla2020supervised}. While adding small computational overhead, this method guarantees that $\mathcal{B}^\prime$ satisfies the conditions of Cor.~\ref{cor:batch} and SCL learns an OF geometry.}
% \todo{move alg to sm, say in words, bring figure one row}
%  \begin{algorithm}
%   \caption{Batch-binding}\label{alg:binding}
%   \begin{algorithmic}[1]
%     \Procedure{Batch-binding}{a set of mini-batches $\mathcal{B}$, number of classes $k$}
%     \State \textbf{Binding examples}: A set of examples represents a set of binding examples if it includes exactly one example from every class. This set has, thus, $k$ elements. \label{def:binding}
% \State To every batch $B\in\mathcal{B}$ add the chosen set of binding examples to create a new batch configuration $\mathcal{B}^\prime$
%     \EndProcedure
%   \end{algorithmic}
% \end{algorithm}
Batch-binding adds a constant $k$ to the size of every mini-batch. $k$ is typically smaller than the batch sizes used to train SCL which could range from $2048$ to $6144$ \citep{khosla2020supervised}. While adding small computational overhead, this method guarantees that $\mathcal{B}^\prime$ satisfies the conditions of Cor.~\ref{cor:batch} and SCL learns an OF geometry. We conduct a series of experiments to illustrate the impact of batch binding on convergence to OF. 
% \tina{needs refernce to the figure and appendix. also a short conclusion}

To verify the role of batch selection on the learned features, we train ResNet-18 on CIFAR-10 under three batching scenarios: 1) \textbf{No batch-shuffling}: a mini-batch set $\mathcal{B}$ that partitions the training examples once at initialization and is held constant across training epochs. 2) \textbf{Batch-shuffling}: the examples are divided into mini-batch partition, with a random reshuffle of the examples at \textit{every} epoch. 3) \textbf{No batch-shuffling + batch-binding}: we construct a fixed partition of examples into mini-batches; then, we perform batch-binding. In order to focus on the impact of batch selection strategies, we consider a relatively small batch-size of $128$.

% Fig.~\ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} shows the distance of learned embeddings to OF geometry for the three batching scenarios mentioned above. With detailed discussions deferred to Sec.~\ref{app:comp_results} in SM, we remark that our Thm.~\ref{thm:scl_mini} and Cor.~\ref{cor:batch} can explain the behaviors of all three schemes. Moreover, the batch-binding strategy guided by our analytical results is effective at ensuring fast and predictable convergence of deep-nets to a unique OF geometry.

We remark that Thm.~\ref{thm:scl_mini} and Cor.~\ref{cor:batch} can explain the behaviors of all three schemes. Moreover, the batch-binding strategy guided by our analytical results is effective at ensuring fast and predictable convergence of deep-nets to a unique OF geometry. Fig.~\ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch_main} shows the distance of learned embeddings to the OF geometry for the three batching scenarios mentioned above. In case of the fixed partition batching (left), the features do not converge to OF, especially with large imbalance ratios. This behavior is consistent with the conditions identified by Thm.~\ref{thm:scl_mini}, because in a typical random partition, the corresponding induced subgraphs are not necessarily connected. On the other hand, when the batching is performed with a randomly reshuffled data ordering (center), the geometry converges more closely to the OF, albeit with certain epochs deviating significantly from the convergence direction. We hypothesize that random reshuffling creates an opportunity for different examples to interact sufficiently, thus, when trained long enough, to converge close to an OF geometry. 
% 
Finally, with the third batching strategy of batch-binding (right), even without shuffling the samples at every epoch, we observe a consistently fast convergence to the global optimizer, OF. These observations provide strong evidence supporting our analysis of batching predicting the behavior of SCL trained deep-nets. 

While the above studies the impact of batching itself, we perform a number of additional experiments in order to illustrate the impact of binding examples. In particular, we observe that batch binding helps improve convergence to OF geometry when training with less powerful models (see Fig.~\ref{Fig:DenseNet_BindingsComparison} for DenseNet experiments in SM), more complex dataset (see Fig.~\ref{Fig:Deepnet_SCL_CIFAR100_GMu} in SM and Fig.~\ref{Fig:Deepnet_SCL_Geom_GMu}  for CIFAR100 and TinyImageNet results) and even convergence to ETF in the absence of ReLU under balanced training (See Fig.~\ref{fig:binding_ETF} in SM). Such results emphasize the importance of batch binding and encourage further analysis of batching under contrastive learning. 

% \ct{I was expecting you would add sentences here about batch binding impacts when datasets get harder, architectures smaller etc :( now it reads as if there is one experiment in Fig 5}
% Fig.~\ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} shows the distance of learned embeddings to the OF geometry for the three batching scenarios mentioned above. In case of the fixed partition batching (left), the features do not converge to OF, especially with large imbalance ratios. This behavior is consistent with the conditions identified by Thm.~\ref{thm:scl_mini}, because in a typical random partition, the corresponding induced subgraphs are not necessarily connected. On the other hand, when the batching is performed with a randomly reshuffled data ordering (center), the geometry converges more closely to the OF, albeit with certain epochs deviating significantly from the convergence direction. We hypothesize that random reshuffling creates an opportunity for different examples to interact sufficiently, thus, when trained long enough, to converge close to an OF geometry. 
 
% Finally, with the third batching strategy (right), by adding the binding examples to the batches, even without shuffling the samples at every epoch, we observe a consistently fast convergence to the global optimizer, OF. These observations provide strong evidence supporting our analysis of batching predicting the behavior of SCL trained deep-nets.

% Fig.~\ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} demonstrates this effect, where we compare three ways of performing mini-batch optimization of SCL. \textbf{No batch shuffling:} for a given batch-size, a partition of all examples is chosen arbitrarily to give mini-batches, and is held constant across training epochs. \textbf{Batch shuffling:} in every epoch, the example indices are randomly shuffled and then a partition gives the mini-batches used in that particular epoch. \textbf{}


\begin{figure}[t]
    % \centering
    \hspace*{-20pt}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \begin{tikzpicture}
            \node at (0.0,0) 
            {\includegraphics[width=0.75\textwidth]{Figs/Deepnet_Geometry_Batch_Exp/GMu_Convergence_plots_BindingBatches_onlyStep.pdf}};
            \node at (-3.3,1.5) [scale=0.9]{\textbf{No Batch Shuffling}};
            \node at (0.1,1.6) [scale=0.9]{\textbf{Batch Shuffling}};
            \node at (3.8,1.9) [scale=0.9]{\textbf{No Batch Shuffling}};
            \node at (3.7,1.5) [scale=0.9]{\textbf{+ Batch-Binding}};
            \node at (0.1,-1.4) [scale=0.9]{\textbf{Epoch}};
        \end{tikzpicture}
    \end{subfigure}
    \hspace*{-20pt}
    \captionsetup{width=0.95\linewidth}
    \caption
    {{Convergence to the OF geometry for various batching schemes {including the analysis-inspired scheme ``No Batch Shuffling + Batch-Binding''}. ResNet-18 trained on CIFAR-10 with a small batch size of 128, see text. See also Fig.~\ref{Fig:Deepnet_SCL_Geom_NC_BindingBatch} in SM}} 
    \vspace{-15pt}
    \label{Fig:Deepnet_SCL_Geom_NC_BindingBatch_main}
\end{figure}




% \begin{figure}[t]
%     % \centering
%     % \hspace*{-25pt}
%     \begin{minipage}{0.70\textwidth}
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \begin{tikzpicture}
%             \node at (0.0,0) 
%             {\includegraphics[width=\textwidth]{Figs/Deepnet_Geometry_Batch_Exp/GMu_Convergence_plots_BindingBatches_onlyStep.pdf}};
%             \node at (-3.5,1.5) [scale=0.9]{\textbf{No Batch Shuffling}};
%             \node at (0.1,1.5) [scale=0.9]{\textbf{Batch Shuffling}};
%             \node at (3.8,1.9) [scale=0.9]{\textbf{No Batch Shuffling}};
%             \node at (3.7,1.5) [scale=0.9]{\textbf{+ Batch-Binding}};
%             \node at (0.1,-1.4) [scale=0.9]{\textbf{Epoch}};
%         \end{tikzpicture}
%     \end{subfigure}
%     \hspace*{-20pt}
%     \captionsetup{width=0.95\linewidth}
%     \caption
%     {{Convergence to the OF geometry for various batching schemes {including the analysis-inspired scheme ``No Batch Shuffling + Batch-Binding''}. ResNet-18 with ReLU trained on CIFAR-10 with a small batch size of 128, see text.}} 
%     \vspace{-15pt}
%     \label{Fig:Deepnet_SCL_Geom_NC_BindingBatch}
%     \end{minipage}%
% \end{figure}




